Active World Model Learning with Progress Curiosity

World models are self-supervised predictive models of how the world evolves. Humans learn world models by curiously exploring their environment, in the process acquiring compact abstractions of high bandwidth sensory inputs, the ability to plan across long temporal horizons, and an understanding of the behavioral patterns of other agents. In this work, we study how to design such a curiosity-driven Active World Model Learning (AWML) system. To do so, we construct a curious agent building world models while visually exploring a 3D physical environment rich with distillations of representative real-world agents. We propose an AWML system driven by $\gamma$-Progress: a scalable and effective learning progress-based curiosity signal. We show that $\gamma$-Progress naturally gives rise to an exploration policy that directs attention to complex but learnable dynamics in a balanced manner, thus overcoming the "white noise problem". As a result, our $\gamma$-Progress-driven controller achieves significantly higher AWML performance than baseline controllers equipped with state-of-the-art exploration strategies such as Random Network Distillation and Model Disagreement.

==> blue_sky_sections/abstract.tex <==
\begin{abstract}
Children exhibit extraordinary exploratory behaviors hypothesized to contribute to the building of models of their world. Harnessing this capacity in artificial systems promises not only more flexible technology but also cognitive models of the developmental processes we seek to mimic. Yet not all children learn the same way, and for instance children with autism exhibit characteristically different exploratory strategies early in life. What if we could, by developing artificial systems that learn through exploration, model not only typically development, but all its variations? In this work, we present a preliminary analysis of curiosity-driven agents in social environments that establishes links between early behavior and later acuity, with implications for the future of both diagnostics and personalized learning.
\end{abstract}

==> blue_sky_sections/dev_variability.tex <==
\vspace{-10pt}
\section{Sources of variability}
\vspace{-10pt}
\begin{figure}
    \vspace{-5pt}
    \centering
    \includegraphics[width=\textwidth]{figures/blue_sky_figures/fig3.pdf}
    \vspace{-20pt}
    \caption{\textbf{Computational Models of ``developmental variability.''} By varying (a) world model architecture, we see differences in end-state external-agent prediction performance. By varying curiosity signal, we see (b) difference in sample complexity and end-state performance, as well as in (c) behavior timecourses, specifically on an animate-inanimate attention differential. (d) Aggregated differences in animate attention.
    }
    \label{fig3}
    \vspace{-10pt}
\end{figure}

What happens to external agent prediction performance and animate attention when we vary components in the model?
To evaluate the effect of varying the structure of the agent-interaction-centric architecture, independently of controller choice, we produce datasets for offline training for each task and train the world model to convergence. 
We compare the performance of the agent-interaction-centric world model to a parameter-matched \textit{joint} LSTM architecture that takes as input and predicts all external agents together, with no agent-centric disentangling.
As seen in Figure~\ref{fig3}a, the agent-interaction-centric (disentangled) architecture significantly outperforms the entangled model on final external-agent prediction.

To evaluate dependence on curiosity signal, we measure both end-state prediction performance and sample complexity (rate of reduction in loss with respect to the number of environment interactions). We compare performance of \textbf{$\gamma$-Progress} to a range of potential variants, including: \textbf{$\delta$-Progress} \citep{achiam2017surprise}, \textbf{RND} \citep{burda2018exploration}, \textbf{Disagreement} \citep{pathak2019disagreement}, \textbf{Adversarial} \citep{stadie2015predictive}, and a simple \textbf{Random} policy.
Fig.~\ref{fig3}b shows end performance (first row) and sample complexity (second row). $\gamma$-Progress has higher end performance on all baselines and all tasks. $\gamma$-Progress has lower sample complexity than Disagreement, Adversarial, and Random baselines on all behaviors, and RND and $\delta$-Progress on all but one behavior, tying on stochastic chasing. 

Baselines display two distinct modes in failing to exhibit animate attention (Fig \ref{fig3}c). The first is \textit{attentional indifference}, in which it finds no particular external agent interesting. The second failure mode is \textit{white noise fixation}, where the observer is captivated by the noise external agents. Non-progress-based curiosity signals exhibited both kinds of failure mode but were more dominated by white noise. RND, a novelty measure, exhibited both types of failure at a lower rate. $\delta$-Progress, a direct information gain measure, had no white noise failure but frequently led to attentional indifference as the new and old world model, separated by a fixed time difference, were often too similar to generate a useful curiosity signal.
We also found (data not shown) that $\gamma$-Progress exhibited indifference when $\gamma$ was too small, but robustly succeeded across all behaviors for sufficiently large $\gamma$.
Overall, emergence of animate attention is highly correlated with prediction performance, suggesting that $\gamma$-Progress succeeds because its improved ability to flexibly estimate information gain allows it to focus on more informative interactions.

Obviously this is a very preliminary investigation of sources of variability in social prediction performance and attentional allocation.   
Our hypothesis is that variability in a computational model, whether this one or some future better model, will describe the underlying mechanisms behind social behavior variability.

==> blue_sky_sections/diagnostics.tex <==
\vspace{-10pt}
\section{Towards model-based diagnostics.}
\vspace{-10pt}
As mentioned above, Autism Spectrum Disorder is characterized by both differences in low-level attention~\citep{jones2013attention, twinstudy} and high-level social acuity~\citep{hus2014ados}. Yet currently, ASD diagnosis is done by expert clinicians, using only observations of high-level behaviors~\citep{hus2014ados}. 
This method is subjective, expensive, and too late --- the average diagnosis comes after 4 years of age, often preventing interventions during a critical period of development.


% \begin{wrapfigure}{L}{0.7\textwidth}
% \vspace{-10pt}
% \begin{center}
%     \includegraphics[width=.7    \textwidth]{figures/blue_sky_figures/fig4_v2.pdf}
% \end{center}
% \vspace{-10pt}
%     \caption{\textbf{Early diagnostic analysis} (a) Accuracy of early indicators of final performance, as a function of time, and (b) factor analysis hypothesis: curiosity signal determines attention, which determines final performance. (c) Potential lightweight wearable suitable for measuring diagnostic stimuli.}
%     \label{fig:offline_asymptotic_performance}
% \vspace{-10pt}
% \end{wrapfigure}

\begin{figure}
    \vspace{-5pt}
    \centering
    \includegraphics[width=\textwidth]{figures/blue_sky_figures/fig4_v2.pdf}
    \vspace{-20pt}
    \caption{\textbf{Early diagnostic analysis} (a)  Attention-differential diagnostic achieves better diagnostic accuracy than direct social performance measurement in critical early phase — in computational modeling experiment. (b) Factor analysis hypothesis: curiosity signal determines attention, which determines final performance. (c) Lightweight wearable suitable for measuring response to diagnostic stimuli.}
    \label{fig4}
    \vspace{-10pt}
\end{figure}

Motivated by these observations, we sought to determine, using computational models whether the easily-measurable low-level attention could be used as an early indicator of high-level social prediction performance. 
In this interpretation, the attention a readily observable behavioral metric, and performance represents some more difficult-to-obtain measure of social acuity. 
Variation in curiosity signal would, in this account, be a latent correlate of developmental variability. 
To perform an early indicator analysis, we thus train two statistical regression models to predict the final end-state social performance of each variant of our computational agents:
(1) PERF$_{\leq T}$, which takes performance before time $T$ as input, and (2) ATT$_{\leq T}$, which takes attention before time $T$ as input.
As seen in Figure~\ref{fig4}a, ATT$_{\leq T}$ is an effective predictor of late social performance, and in fact, throughout most of the timecourse, a more accurate indicator than direct measurement of early-stage model performance itself. The overall situation is conveyed by the factor diagram Figure~\ref{fig4}b.

This analysis, which establishes a link between early behaviors and downstream social acuity differences via latent factors, is obviously just a toy model. 
Its translation into higher-fidelity simulations of early childhood learning, however, holds exciting possibilities in diagnostics, therapeutics, and personalized learning. 
If variations in simulated agents can represent the learning process of diverse human populations, then such a link enables us to search, entirely in simulation, for stimuli that elicit easily measurable behavioral responses that differentiate between underlying factors of variation which in turn predict differences later in life. Such diagnostics could be performed cheaply using lightweight AR/VR devices (such as those shown in Figure~\ref{fig4}c) that will soon emerge.
In the long run, if computational modeling approaches to developmental variability are able to correctly describe patterns of behavior across the population and produce effective diagnostics, a natural extension will be the development of model-based therapeutics tested in simulation. 




==> blue_sky_sections/intro.tex <==
\section{Introduction}

Human infants exhibit a wide range of interesting, apparently spontaneous, visuo-motor behaviors --- including navigating their environment, seeking out and attending to novel objects, and engaging physically with these objects in novel and surprising ways \citep{fantz_visualexperienceininfants, twomey_curiositybasedlearning, hurley2010_influenceofpets, hurley2015_petexposure, goupil_infantsask, begus_infantslearnwhattheywant, gopnik_scientistincrib}.
In short, young children are excellent at playing --- ``scientists in the crib'' \citep{gopnik_scientistincrib} who intentionally create events that are both fun and greatly informative for driving the self-supervised learning of sensorimotor and social planning capacities~\citep{fantz_visualexperienceininfants, sokolov1963perception, goupil_infantsask,begus_infantslearnwhattheywant, kidd2012_goldilocks}.
Harnessing this sort of capacity in artificial systems promises not only more flexible learning technologies but also cognitive models that will further elucidate early childhood learning.

Evidence suggests that Autism Spectrum Disorder (ASD) children exhibit characteristically {\em different} exploratory learning behaviors.
Children with autism exhibit atypical, uncreative object play, \citep{beyer2000autism_play,rettig1994play}, impaired predictive capacity \citep{sinha2014autism}, lower facial gaze and mutual attention \citep{shic_autism6months,jones2013attention,moriuchi2016mechanisms}, and abnormalities of sensory perception \citep{robertson2017sensory,binocularrivalry}. What if we could model not only typical development, but the full diversity of human developmental variability (Fig. \ref{fig1})?

In this work, we analyze a ``population'' of agents put in an environment meant to loosely represent early childhood learning in social environments: stimuli look either animate or inanimate, and inanimate stimuli vary wildly (from static ones, to dynamic but predictable ones, to dynamic and unpredictable ones), and the agent simply looks about. To decide what to look at, the agent is curious \citep{schmidhuber_formaltheoryoffun, oudeyer2007intrinsic} --- intrinsically motivated to take action as it tries to build a world model of its environment. Within this population, we take implementation differences (specifically, in choice of the agent's intrinsic motivation) to represent latent factors that drive developmental differences. By observing both the agent's behavior and downstream world modeling capacity, we establish a predictive model that, if translated to simulations that have the fidelity to capture early childhood learning, holds exciting implications for diagnostics, therapeutics, and personalized learning.


\begin{figure}
    \vspace{-5pt}
    \centering
    \includegraphics[width=\textwidth]{figures/blue_sky_figures/fig1.pdf}
    \vspace{-20pt}
    \caption{\textbf{Modeling human development.} (a) Our overall goal is to build a computationally quantitative model of the learning principles of early childhood, both for cases of typical and variable developmental trajectories. (b) We develop the learning principles by which they operate within virual environments.} % still need to change objects to be something less awkward 
    \label{fig1}
    \vspace{-10pt}
\end{figure}


==> blue_sky_sections/modeling_social_attention.tex <==
\section{Modeling social attention}

\textbf{Environment}
To simplify but faithfully capture key aspects of the algorithmic challenges children face, we work with a 3D virtual environment (Fig. \ref{fig2}d). 
Within the environment there are two main agent types: a single ``infant-agent'', and various \textit{external agents}. 
Just as very young human babies are not self-mobile but can control their gaze to visually explore their surroundings, our infant-agent is represented by an avatar fixed at the center of the room but with the ability swivel around, obtaining partial observations of whatever is in view at the given moment. 
The \textbf{external agents} are spherical avatars that each act under various hard-coded policies embodying abstract versions of the behaviors of real-world stimuli, both inanimate and animate. 
We experiment with external agent behaviors of increasing complexity and animacy, including static (no motion), periodic, noise, object-reaching, chasing, playing ``peekaboo'', and mimicry. 
See \textcolor{blue}{\url{https://bit.ly/2uf7lEY}} for video descriptions of the environment and external agent behaviors. 
The task of the infant-agent is to learn to predict the behaviors of the external agents.
Since external agents are devoid of surface features, the curious agent must understand behaviors based on spatiotemporal kinematics alone. 

\begin{figure}[b]
    \vspace{-5pt}
    \centering
    \includegraphics[width=\textwidth]{figures/blue_sky_figures/fig2.pdf}
    \vspace{-20pt}
    \caption{\textbf{Modeling social attention.} Proposed (a) agent-interaction-centric world model and (b) curiosity signal to facilitate learning in social environments. In a pilot study, we compared (c) simulation of our artificial agents with (d) data from a human experiment and observed similar attention patterns.} % still need to change objects to be something less awkward 
    \label{fig2}
    \vspace{-10pt}
\end{figure}


\textbf{Learning predictive models of other agents.}
The infant-agent's neural network consists of two components: an {\em agent-interaction-centric world model}, which seeks to learns to predict dynamics of external agents, and a {\em curiosity-driven controller} which uses a novel variant of progress curiosity~\cite{schmidhuber_formaltheoryoffun} to choose swivel actions (e.g. allocate attentional resources) that make world-model learning more effective. \textit{Agent-centric World Model:} (Figure~\ref{fig2}a) 
Our infant-agent learns to predict the dynamics of its environment via an agent-interaction-centric world model $\omega_{\theta}$. $\omega_{\theta}$ consists of an ensemble of component networks $\{\omega_{\theta^{k}}\}_{k = 1}^{N_{\mathrm{cc}}}$ where each $\omega_{\theta^{k}}$ independently predicts the forward dynamics separately, for each minimal group of interacting external agent(s).  
This agent-interaction-centric world model differs from a standard ``joint'' (non-agent-centric) model in that it allocates the parameters and learning gradients in a causally disentangled fashion. 
For example, one external agent reaching toward and pushing around static objects is allocated a separate world-model component than another external agent playing peekaboo with the infant-agent.
If multiple external agents are causally interacting with each other (e.g. one agent chasing or mimicking another), they are allocated a single joint component of the world model. 
In this work, we manually feed the infant-agent knowledge of the causal graph of external agents; in future work estimating this from observations is a key goal. 
\textit{Progress-driven Controller:} (Figure~\ref{fig2}b) We propose \textbf{$\gamma$-Progress}, a scalable progress-based curiosity signal which approximates learning progress by the difference in the losses of an old model and a new model. The old model weights, $\theta_{old}$, lag behind those of the new model, $\theta_{new}$, with a simple update rule: $\theta_{old} \leftarrow \gamma \theta_{old} + (1 - \gamma) \theta_{new}$, where $\gamma$ is scalar mixing constant. The curiosity reward is:
\begin{equation}
R = \LL(\theta_{old}) - \LL(\theta_{new}) 
\label{eq:reward}
\end{equation} 
Our controller $\pi_{\phi}$ follows an $\epsilon\text{-}greedy$ sampling scheme with respect to a Q-function $Q_{\phi}$ trained with the curiosity reward in Eq. \ref{eq:reward} and updated with the DQN \cite{mnih2013playing} learning algorithm.

\textbf{Model Evaluation.} We trained our proposed model on variety of situations with different compositions of external agent behaviors.
Looking at the trained model's behavior, we find that it appears to be able to learn to predict the behavior of a wide array of external agents, across the spectrum of animacy.  
See \textcolor{blue}{\url{https://bit.ly/31vg7v1}} for visualizations of our model's predictions. 

We believe that the key reason that the infant-agent equipped with this two-component active-learning world model was able to capture a wide range of external agent behaviors is that it learned to properly allocate its attention, e.g. spending more time focusing on complex animate external agents, as seen in Figure~\ref{fig2}c.
This increased animate-inanimate attention differential corresponds to a characteristic attentional ``bump'' that occurs early as the $\gamma$-Progress curious agent focuses on animate external agents quickly before eventually ``losing interest'' as prediction accuracy is achieved.

\textbf{Comparisons to human attentional allocation.} 
Our model is a very rudimentary hypothesis for how babies allocate attention in social settings. 
To begin to examine the extent to which this hypothesis is accurate, we ran a simple pilot human subject experiment (Figure~\ref{fig2}d) in which we conveyed static, periodic, animate, and noise stimuli to twelve human participants via spherical robots moving along a mat, while measuring patterns of attention via a mobile eye tracker. 
We find average fixation proportions favoring the animate stimuli, just as in the computational model.
We also find a similar ordering of aggregate attentional fixation across multiple kinds of stimuli. 
In follow-up work, we aim to make a finer model comparison to the behavior of humans shown a diverse array of stimuli.

==> iclr_format_workshop/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> iclr_sections/abstract.tex <==
\begin{abstract}
\vspace{-10pt}
Infants appear to actively build models of their environment by attending to stimuli in a highly non-random manner. In this work, we study how to design such a curiosity-driven Active World Model Learning (AWML) system. To do so, we construct a curious agent building world models while visually exploring a 3D physical environment rich with distillations of representative real-world agents. We propose an AWML system driven by $\gamma$-Progress: a scalable and effective learning progress-based curiosity signal. We show that $\gamma$-Progress naturally gives rise to an exploration policy that directs attention to complex but learnable dynamics in a balanced manner, as a result overcoming the ``white noise problem''. As a result, our $\gamma$-Progress-driven controller achieves significantly higher AWML performance than state-of-the-art baselines. 

\end{abstract}

==> iclr_sections/asymptotic.tex <==
\subsection{Asymptotic Model Performance in Supervised Learning}
\label{sec:offline}

Here we evaluate the capacity for the world model to learn each of the animate external agent behaviors, isolating this measurement from any choice of policy. We gather 400k environment steps of data using a reduced action space random policy: for each action choice, the agent chooses randomly between 0- and 12-degree rotation in either direction. These data collection choices represent ``ideal'' data by ensuring plentiful exposure to each stimulus for long stretches of time. For this metric, we exclude the peekaboo animate external agent behavior, as due to the curious agent-contingent behavior of the peekaboo agent, one cannot expect ``ideal data'' to be gathered without a learned policy. We then train the world model to convergence and aggregate validation performance across five validation cases for each external agent behavior. 

We compare the performance of our causal world model to two acausal ablations: one {\em joined} that instead takes as input and predicts all external agents together, and one {\em split} that treats each agent separately, as opposed to behavior (so e.g. in the case of the chasing behavior, our causal world model takes as input both chaser and runner agent in order to predict the runner, whereas this predicts runner from runner alone). They employs the same architecture as a single behavior network in the causal world model (Section~\ref{sec:methods:worldmodel}), except with the number units for each hidden layer chosen so as to match roughly the total number of weights.

As seen in Figure~\ref{fig:offline_asymptotic_performance}, across all experiments, the causal world model significantly outperforms the ablation, with the acausal ablation obtaining $9.8\times$ the validation loss, on average across seeds and behaviors. Justifying the interpretation of ``ideal data'', for the causal world model, performance is comparable to the best achieved under online learning under the best policy found. Upon visual inspection of predictions, the causal world model appeared to ``get'' each animate external agent behavior, at least up to what the stochasticity of the external agent behaviors allow. To contrast, the acausal ablation exhibits not only poorer performance but considerable variance in performance, and visual inspection found that these models captured essential low order statistics across the first several timesteps of behavior, but that prediction rollouts quickly deteriorated. \nh{We should really add videos!} \ms{add agent-wise causal ablation}



==> iclr_sections/attention_determinants.tex <==
\subsection{Determinants of attention pattern}
\label{sec:app:attention_determinants}
To gain a finer-grained understanding of what, of the factors we vary (curiosity signal, world model architecture, and stimulus type) drives the attentional behavior of these active learning systems, we perform a linear regression. Specifically, we regress
\begin{equation} \label{eq:regression}
R_{\mathrm{animate}/\mathrm{noisy}} = a + b \cdot \chi_{\mathrm{CS}} + c \chi_{\mathrm{causal}} + d \cdot \chi_{\mathrm{BHR}} + \chi_{\mathrm{causal}} * e \cdot \chi_{\mathrm{IM}} + \epsilon
\end{equation}
Here $R_{\mathrm{animate}/\mathrm{noisy}}$ is the ratio of animate to noisy attention, $\chi_{\mathrm{CS}}$ is a one-hot encoding of curiosity signal (all zeros if random policy), $\chi_{\mathrm{causal}}$ is an indicator set to $1$ if the architecture is causal, $\chi_{\mathrm{BHR}}$ is a one-hot encoding of animate external agent behavior shown (all zeros if deterministic reaching), and $a,  b, c, d, e$ are fixed effects ($e$ measures an interaction effect).

Over $371$ individual active learning runs, an ordinary least squares regression achieves an adjusted $R^2$ of $.44$. Please see Table~\ref{table:regression} for details. We found that $\gamma$-Progress receives significant positive weight, while Disagreement and Adversarial receive significant negative weight, with the other curiosity signals having an effect close to that of random policy. In addition, we fail to find a significant effect due to architecture and most external agent behaviors, with two external agent behavior exceptions. In sum, we find that, of the architectural and curiosity signal variations we tested, curiosity signal strongly drives behavior whereas architecture plays an insignificant role.

\begin{table*}
\caption{
\textbf{Attention regression.} Regression model of animate/noisy attention, according to Equation~\ref{eq:regression}. Coefficient values found, and uncorrected p-value for 2-sided t-tests, with significance at the $.05$ level in bold.}
\vspace{-0.1cm}
\label{table:regression}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcc}
\toprule
Coefficient & value & P > |t| \\
\midrule
constant & .80 & .001 \\
$\gamma$-Progress & \textbf{2.24} & .000 \\
$\delta$-Progress & .08 & .788 \\
RND & -.53 & .064 \\
Disagreement & \textbf{-.70} & .014 \\
Adversarial & \textbf{-.79} & .006 \\
\midrule
Causal architecture & .014 & .959 \\
\midrule
stochastic reaching & .14 & .493\\
deterministic chasing & .25 & .222 \\
stochastic chasing & \textbf{.45} & .029 \\
deterministic peekaboo & -.08 & .682\\
stochastic peekaboo & .02 & .920\\
mimicry & \textbf{.56} & .006\\
\midrule
causal $\times \gamma$-Progress & -.32 & .408 \\
causal, $\times \delta$-Progress & .06 & .868 \\
causal $\times$ RND & .03 & .935 \\
causal $\times$ Disagreement & .23 & .555 \\
causal $\times$ Adversarial & -.09 & .813 \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\end{table*} 


==> iclr_sections/causal_confusion.tex <==
\subsection{Causal Confusion in World Models}
\label{sec:causal_conf}

\begin{comment}
Paragraph outline
1. world model framework, introducing and justifying an object-centric representation
2. illustrate by example the causal confusion problem. What is the ground truth function for these coordinates.
3. effect of causal misidentification in the case of partial observability. show this formalization with symbols.
4. our solution. defines a causal graph, and describes the basic point of the solution. maybe a formula for the causal case and the acausal case.
\end{comment}

In this section, we first formalize the disentanglement problem, reason about its propensity to occur in the interactive learning setting, and motivate our causal world model architecture. Consider the (deterministic) dynamics function $P: \X \rightarrow \Y$. We consider deterministic dynamics for compactness of notation in what follows, but the presented analyses may be extended to stochastic dynamics. Henceforth we use the vector slicing notations $\rvx_{I} := [\rvx_{i}]_{i \in I}$, and $\X_{I} := \{\rvx_{I} | \rvx \in \X\}$. We start by defining a causal graph.

\begin{definition}
\label{def:disentanglement_graph}
Let $P : \X = \sR^n \rightarrow \Y = \sR^m$. For each $j \in \{1 \ldots m\}$, let its preimage $j_P^{-1} \subseteq \{1 \ldots n\}$ satisfy the following:
\begin{enumerate}
    \item (modularity) There exists $\tilde P$ such that $P(x) = \tilde P(x_{j_P^{-1}})$, where $x_{j_P^{-1}}$ is the projection of $x \in \sR^n$ onto dimensions $j_P^{-1}$, and
    \item (minimality) There does not exist $I$ strictly contained in $j_P^{-1}$ such that property (1) holds for $I$.
\end{enumerate}
Then the {\em disentanglement graph} is $G_{P} = (V, E)$ where $V$ has one vertex $i_X$ for $i \in \{1 \ldots n\}$ and one vertex $j_Y$ for $j \in \{1 \ldots m\}$, and $E = \{(i_X, j_Y) \ | \ i_X \in j_P^{-1}, j \in \{1 \ldots m\} \}$.
\end{definition}

Implicit in this definition is the fact that $j_P^{-1}$ exists and is unique, and hence there is exactly one disentanglement graph for a given function. Note that this definition heavily depends on a specification of a coordinate system for both the domain and range of the function. We are now ready to formalize a failure mode of models supervised on $P$.

\begin{definition}
\label{def:causal_confusion}
A model $P_{\theta}: \X \rightarrow \Y$ is not disentangled w.r.t $P: \X \rightarrow \Y$ if the identity map on vertices does not induce an embedding of $G_{P_\theta}$ into $G_P$.
\end{definition}

\noindent{\textbf{Observation}}
\textit{
Let $P_{\theta}: \X \rightarrow \Y$ be not disentangled w.r.t $P$. Then there exists $j_Y$ and $x, x' \in X$ with $x_i = x'_i$ for all $i \in j_P^{-1}$ and
\begin{equation*}
    P(x) = P(x')
\end{equation*}
but
\begin{equation*}
    P_\theta(x) \neq P_\theta(x').
\end{equation*}
}

In words, $P_{\theta}$ is non-robust to perturbations of the inputs along the nuisance dimensions $\setminus I_{\Y}^{-1}$. Hence, a causally confused model that has overfit to spurious statistical dependencies $p_{\text{train}}(\rvy_{I_{\Y}} | \rvx_{\setminus I_{\Y}^{-1}})$ in the training set will have poor generalization performance on a validation set when $d(p_{\text{val}}(\rvy_{I_{\Y}} | \rvx_{\setminus I_{\Y}^{-1}}),  p_{\text{train}}(\rvy_{I_{\Y}} | \rvx_{\setminus I_{\Y}^{-1}})) \neq 0$ where $d$ is some distance metric between distributions.\footnote{Note than in the limit of infinite training data with full coverage over $\X$, a model will not be causally confused since the proper disentanglement can be learned by just memorizing the training data}

%% So why does the conditional distribution change? 
%% Need to also explain that true models are likely causally disentangled 
Causal confusion is more likely to occur and more detrimental to generalization performance when learning world models of partially observable environments by interactive learning. To see this, consider a world model $P_{\theta}$ of a partially observable environment with dynamics $P: \X \rightarrow \Y$ that have a non-trivial causal graph. Due to partial observability, the world model must solve two types of predictions problems: supervised prediction and permanence prediction. Supervised prediction involves predicting the dynamics of stimuli that are currently observable and permanence prediction involves predicting the dynamics of non-observable stimuli. For the world model to solve both prediction tasks, the inputs $\rvx \in \X$ should encode both current observations - e.g images, coordinates of stimuli that are in view - when available and permanence information - e.g mental estimates of how the non-visible stimuli are moving. \footnote{Any memory efficient model should minimize the number of observations, which are typically high-bandwith, and maintain a compact encoding of permanence information instead of taking as input an arbitrary sequence of high-bandwith observations} 

Thus, the nuisance factors $\rvx_{\setminus I_{\Y}^{-1}}$ for any output $\rvy_{I_{\Y}}$ must encode permanence information impertinent to predicting $\rvy_{I_{\Y}}$. For example, $\rvx_{I_{\Y}^{-1}}$ could correspond to the position inputs of the currently visible external agent while $\rvx_{\setminus I_{\Y}^{-1}}$ could correspond to a mental estimate of where the non-visible external agents are or a counter that tracks the number timesteps since the last encounter with them. Such permanence information can be explicitly identified when the world model has a structured input ($\X$), output ($\Y$) space that allocates separate space for permanence information and implicitly identified in the hidden states of memory augmented function approximators such as Long Short-Term Memory (LSTM) networks. 

There may exist a drastic distributional shift of the permanence variables between training and validation, i.e $d(p_{\text{val}}(\rvy_{c(I_{\X})} | \rvx_{\setminus I_{\X}}),  p_{\text{train}}(\rvy_{c(I_{\X})} | \rvx_{\setminus I_{\X}})) \gg 0$, due to two factors. First, changes in the data collection policy with interactive learning leads to changes in the visitation frequencies for each stimuli which changes the distribution of permanence variables such as the visitation counters. In the interactive learning setting there indeed may be policy differences between training and validation time and we desire the world model to be robust to changes in policy. 

Second, updates to the world model parameters can change the permanence variable distribution. In the interactive learning setting we interlace data collection and world model update, and will indeed experience constant changes to the world model parameters. Furthermore, permanence predictions, such as predicting the position of an external agent after a long look-away, are typically significantly harder than supervised predictions and thus the permanence representations will take much longer to stabilize in distribution due to large gradients.  

% \begin{wrapfigure}{R}{0.45\textwidth}
% \vspace{-10pt}
% \begin{center}
%     \includegraphics[width=.43\textwidth]{figures/causal_graph.pdf}
% \end{center}
% \vspace{-15pt}
% \caption{\textbf{A causal graph.} Vertices represent external agents at times $t$ and $t+1$, edges represent causal relationships. Dashed boxes denote the connected component {\em external agent behaviors}.}
% \label{fig:causal_graph}
% \vspace{-10pt}
% \end{wrapfigure}

To ameliorate this, we propose to inject a causal prior into the world model, specified by a causal graph $G_{P}$. The causal graph has one vertex $v_{i, t}$ for each external agent $i$ for each timestep $t$, and a (directed) edge from $v_{i, t}$ to $v_{j, t'}$ if the position of external agent $j$ at timestep $t'$ depends on the position of external agent $i$ at timestep $t$. The causal graph thus represents which external agents a given external agent's future trajectory depends on. We identify each connected component of this graph, restricted to the input and output timesteps in question, with an {\em external agent behavior}. For example, the object interaction agent consists of its own behavior, whereas the chaser and runner agents together make a behavior. As noted in Section~\ref{sec:environment} these connected components do not vary across time in our environment. Our causal world model allocates a separate neural network for each external agent behavior, i.e each network has access to only the causally-appropriate inputs, thereby reducing causal confusion across agent behaviors. We assume access to the appropriate causal graph for each instantiation of behaviors. See Section~\ref{sec:methods} for details.






==> iclr_sections/causal_confusion_scrap.tex <==
\subsection{Causal Confusion in World Models}
\label{sec:causal_conf}

\begin{comment}
Paragraph outline
1. world model framework, introducing and justifying an object-centric representation
2. illustrate by example the causal confusion problem. What is the ground truth function for these coordinates.
3. effect of causal misidentification in the case of partial observability. show this formalization with symbols.
4. our solution. defines a causal graph, and describes the basic point of the solution. maybe a formula for the causal case and the acausal case.
\end{comment}

In this section, we first formalize the causal confusion problem, reason about its propensity to occur in the interactive learning setting, and motivate our causal world model architecture. Consider the (deterministic) dynamics function $P: \X \rightarrow \Y$. \kh{include thing about encoding space} We consider deterministic dynamics for compactness of notation in what follows, but the presented analyses may be extended to stochastic dynamics. Henceforth we use the vector slicing notations $\rvx_{I} := [\rvx_{i}]_{i \in I}$, and $\X_{I} := \{\rvx_{I} | \rvx \in \X\}$. We start by defining a causal graph. 

\begin{definition}
\label{def:causal_disentanglement}
Let $P: \X \rightarrow \Y$ be a function. For each $I_{\Y} = 1, ..., \emph{dim}(\Y)$, let its preimage $I_{\Y}^{-1} = \{I_{\X} | I_{\X} \subseteq \{1, ..., \emph{dim}(\X)\}\}$ be a set satisfying the following: 
\vspace{-5pt}
\begin{enumerate}
    \item (modularity) $\forall I_{\X} \in I_{\Y}^{-1}, \exists \tilde{P}: \X_{I_{\X}} \rightarrow \Y_{I_{\Y}}$ such that $P(\rvx)_{I_{\Y}} = \tilde{P}(\rvx_{I_{\X}})~\forall \rvx \in \X$
    \vspace{-5pt}
    \item (minimality) $\forall I_{\X} \in I_{\Y}^{-1}, \nexists i \in I_{\X}$ such that property $1$ holds for $I_{\X} \setminus \{i\}$
\end{enumerate}
\vspace{-5pt}
Then, a \textbf{causal graph} is $G_{P} = (V, E)$ where $V = \{\rvx_{1}, ..., \rvx_{\emph{dim}(\X)}, \rvy_{1}, ..., \rvy_{\emph{dim}(\Y)}\}$ is a set of vertices and $E = \{(\rvx_{i}, \rvy_{I_{\Y})}| i \in I_{\X}, I_{\Y} = 1, ..., \emph{dim}(\Y)\}$ are the directed edges for any $I_{\X} \in I_{\Y}^{-1}$. 

Restatement (see comment): We define a \textbf{causal graph} to be a 
\end{definition}

\nh{I like this definition better, but I think a few things need to be changed:
(1) $I_X$ and $I_Y$ should look more different. One is an integer and the other is a set of integers, whereas the notation suggests that they're analogous for $X$ and $Y$.
(2) Definitions of $V$ and $E$ should not have $x$ and $y$s in them, because then it seems like there are different vertices for the same indices but different points for each $(x, P(x))$ as we vary $x$. Let me try to establish notation in the below lemma, see if you like it.
(3) (And maybe I am misunderstanding the definition, but...) it needs to be clear that for a given causal graph, one makes a unique choice of $I_X \in I_Y$
}

Notice that every dynamics $P$ has a causal graph, since the fully connected bipartite graph from vertices for $\rvx$ to vertices for $\rvy$ can make up a trivial causal graph. However, the causal graph need not be unique (see Appendix \ref{sec:app:causal}). We henceforth use $\Gamma_{P}$ to refer to the family of causal graphs of $P$. We are now ready to formalize causal confusion. 

\begin{definition}
\label{def:causal_confusion}
A world model $P_{\theta}: \X \rightarrow \Y$ is causally confused w.r.t $P: \X \rightarrow \Y$ if $\Gamma_{P_{\theta}} \nsubseteq \Gamma_{P}$ 
\end{definition}

%% Why is causal confusion harmful for prediction?
In words, causal confusion is the failure of a world model to embody the correct disentanglement structure present in the target dynamics. This phenomenon can also be understood as overfitting to spurious correlations in the training data. Thus, causally confused models have poor generalization performance: 

\begin{comment}
Old version:
\begin{corollary}
Let $P_{\theta}: \X \rightarrow \Y$ be causally confused w.r.t $P$. Then for all $\I_{\X}, \I_{\Y}, c$ comprising a causal graph of $P$, there exists an input $\rvx \in \X$, a perturbed input $\rvx + \rvepsilon \in \X$, and $I_{\Y} \in \I_{\Y}$ such that,
\begin{equation*}
P(\rvx)_{I_{\Y}} = P(\rvx + \rvepsilon)_{I_{\Y}} = P_{\theta}(\rvx)_{I_{\Y}} \neq P_{\theta}(\rvx + \rvepsilon)_{I_{\Y}}
\end{equation*}
where $\rvepsilon_{I_{\Y}^{-1}} = \textbf{\emph{0}}^{|I_{\Y}^{-1}|}, \rvepsilon_{\setminus I_{\Y}^{-1}} \neq \textbf{\emph{0}}^{|\setminus I_{\Y}^{-1}|}$ for $I_{\Y}^{-1} = \bigcup_{\{I_{\X} | c(I_{\X}) = I_{\Y}\}} I_{\X}$ and $\textbf{\emph{0}}^{L}$ is an $L$-dim zero vector.
\end{corollary} 
\end{comment}

\nh{I made this a lemma, not a corollary, as stylistically you aren't supposed to have corollaries of definitions, but of other results. I'm not even really sure whether to call this a lemma, as it's basically a restatement of the definition, as is. (Maybe some previous version was more nontrivial? Could be that I just dumbed it down...) Usually in a case like this, I would say something like ``Observation''.}

\begin{lemma}
Let $P_{\theta}: \X \rightarrow \Y$ be causally confused w.r.t $P$. Then for all $G \in \Gamma_P$ such that $G \notin \Gamma_{P_\theta}$, there exists $I_X, I_Y$ with $\{(i, I_Y) \ | \ i \in I_X\} \subseteq G$ and $x, x' \in X$ with $x_i = x'_i$ for all $i \in I_X$ and
\begin{equation*}
    P(x) = P(x')
\end{equation*}
but
\begin{equation*}
    P_\theta(x) \neq P_\theta(x').
\end{equation*}
\end{lemma}


In words, a causally confused model's prediction $P_{\theta}(\rvx)_{I_{\Y}}$ is non-robust to perturbations of the inputs along the nuisance dimensions $\setminus I_{\Y}^{-1}$. Hence, a causally confused model that has overfit to spurious statistical dependencies $p_{\text{train}}(\rvy_{I_{\Y}} | \rvx_{\setminus I_{\Y}^{-1}})$ in the training set will have poor generalization performance on a validation set when $d(p_{\text{val}}(\rvy_{I_{\Y}} | \rvx_{\setminus I_{\Y}^{-1}}),  p_{\text{train}}(\rvy_{I_{\Y}} | \rvx_{\setminus I_{\Y}^{-1}})) \neq 0$ where $d$ is some distance metric between distributions.\footnote{Note than in the limit of infinite training data with full coverage over $\X$, a model will not be causally confused since the proper disentanglement can be learned by just memorizing the training data}

%% So why does the conditional distribution change? 
%% Need to also explain that true models are likely causally disentangled 
Causal confusion is more likely to occur and more detrimental to generalization performance when learning world models of partially observable environments by interactive learning. To see this, consider a world model $P_{\theta}$ of a partially observable environment with dynamics $P: \X \rightarrow \Y$ that have a non-trivial causal graph. Due to partial observability, the world model must solve two types of predictions problems: supervised prediction and permanence prediction. Supervised prediction involves predicting the dynamics of stimuli that are currently observable and permanence prediction involves predicting the dynamics of non-observable stimuli. For the world model to solve both prediction tasks, the inputs $\rvx \in \X$ should encode both current observations - e.g images, coordinates of stimuli that are in view - when available and permanence information - e.g mental estimates of how the non-visible stimuli are moving. \footnote{Any memory efficient model should minimize the number of observations, which are typically high-bandwith, and maintain a compact encoding of permanence information instead of taking as input an arbitrary sequence of high-bandwith observations} 

Thus, the nuisance factors $\rvx_{\setminus I_{\Y}^{-1}}$ for any output $\rvy_{I_{\Y}}$ must encode permanence information impertinent to predicting $\rvy_{I_{\Y}}$. For example, $\rvx_{I_{\Y}^{-1}}$ could correspond to the position inputs of the currently visible external agent while $\rvx_{\setminus I_{\Y}^{-1}}$ could correspond to a mental estimate of where the non-visible external agents are or a counter that tracks the number timesteps since the last encounter with them. Such permanence information can be explicitly identified when the world model has a structured input ($\X$), output ($\Y$) space that allocates separate space for permanence information and implicitly identified in the hidden states of memory augmented function approximators such as Long Short-Term Memory (LSTM) networks. 

There may exist a drastic distributional shift of the permanence variables between training and validation, i.e $d(p_{\text{val}}(\rvy_{c(I_{\X})} | \rvx_{\setminus I_{\X}}),  p_{\text{train}}(\rvy_{c(I_{\X})} | \rvx_{\setminus I_{\X}})) \gg 0$, due to two factors. First, changes in the data collection policy with interactive learning leads to changes in the visitation frequencies for each stimuli which changes the distribution of permanence variables such as the visitation counters. In the interactive learning setting there indeed may be policy differences between training and validation time and we desire the world model to be robust to changes in policy. 

Second, updates to the world model parameters can change the permanence variable distribution. In the interactive learning setting we interlace data collection and world model update, and will indeed experience constant changes to the world model parameters. Furthermore, permanence predictions, such as predicting the position of an external agent after a long look-away, are typically significantly harder than supervised predictions and thus the permanence representations will take much longer to stabilize in distribution due to large gradients.  

\begin{wrapfigure}{R}{0.45\textwidth}
\vspace{-10pt}
\begin{center}
    \includegraphics[width=.43\textwidth]{figures/causal_graph.pdf}
\end{center}
\vspace{-15pt}
\caption{\textbf{A causal graph.} Vertices represent external agents at times $t$ and $t+1$, edges represent causal relationships. Dashed boxes denote the connected component {\em external agent behaviors}.}
\label{fig:causal_graph}
\vspace{-10pt}
\end{wrapfigure}

To gain intuition about causal confusion in interactive learning, consider an environment with two independent external agents $A, B$ oscillating in sync with the same period. Let $\X = \Y$ $I_{A}, I_{B}$ denote indices for each agent so that e.g $\rvx_{I_{A}}$ is the position coordinate of agent $A$ when it is visible and a bootstrapped model estimate of agent $A$'s position when it is not visible. According to Def. \ref{def:causal_disentanglement}, the true dynamics $P: \X \rightarrow \X$ have a causal graph $G_{P}$ defined by $\I_{\X} = \I_{\Y} = \{I_{A}, I_{B}\}$ and the identity bijective pairing $c(I) = I$. The left graph in Fig. \ref{fig:causal_graph} visualizes $G_{P}$ with two connected components, one for each periodic agent. The right graph of Fig. \ref{fig:causal_graph} shows an example world model $P_{\theta}$ that is causally confused. $P_{\theta}$ predicts the next position of agent $A$ from the current position of agent $B$. Such a model could've been learned on a training set collected with a policy that rapidly shifts between agent $A, B$. Frequent shifts allow the model estimated position to remain accurate since the number of bootstrapping steps are small, and thus the model is able to achieve low training error since the agents are oscillating in sync. However the validation set may test for robustness of the world model with data collected by a less frequently switching policy. In this case, the bootstrapped model estimates for agent $B$ may shift in distribution and degrade the predictions for agent $A$ even when agent $A$ is in view. 

To ameliorate this, we propose to inject a causal prior into the world model, specified by a causal graph $G_{P}$. The causal graph has one vertex $v_{i, t}$ for each external agent $i$ for each timestep $t$, and a (directed) edge from $v_{i, t}$ to $v_{j, t'}$ if the position of external agent $j$ at timestep $t'$ depends on the position of external agent $i$ at timestep $t$. The causal graph thus represents which external agents a given external agent's future trajectory depends on. We identify each connected component of this graph, restricted to the input and output timesteps in question, with an {\em external agent behavior}. For example, the object interaction agent consists of its own behavior, whereas the chaser and runner agents together make a behavior. As noted in Section~\ref{sec:environment} these connected components do not vary across time in our environment. Our causal world model allocates a separate neural network for each external agent behavior, i.e each network has access to only the causally-appropriate inputs, thereby reducing causal confusion across agent behaviors. We assume access to the appropriate causal graph for each instantiation of behaviors. See Section~\ref{sec:methods} for details.





%TODOS: (1). Augment reason 1, reason 2 (2). Figure out where to put in periodic example (3). Rewrite the solution paragraph (4). Revise the figure 


% corrollary explaining that causal confusion makes the supervised world model prediction $P(\rvx)_{c(I_{\X})}$ non-robust to drastic changes in $p(\rvx_{I_{\X}} | \rvx_{\setminus I_{\X}})$. It's true that there are two additional sources of degradation in performance. (1). Causal confusion across time within $I_{\X}$ and unsupervised prediction. We don't argue that the agent causal confusion is "theoretically" a bigger issue, but show that getting rid of it leads to really big prediction gains. Supervised world model prediction here, since if you're doing unsupervised prediction, then even $p(\rvx_{I_{\X}})$. I think we should limit the scope to supervised prediction? 

%% Our solution is to eliminate causal confusion among the agent-dimensions. But note that there can still be other sources of causal confusion present after this removal. Namely confusion across time and confusion during unsupervised prediction. However, this still alleviates the problem to a large degree as we observed empirically 


%% TODOS: we should really show object permanence through experiments. That we can make good predicitons of agent behaviors when not looking at them.



%% Why is causal confusion likely to occur 
%% (1). Lack of data that fully covers the space 
%% 

%% Why is validation distribution likely different from training 
%% => we want to test for generalization. Which means the world model should be robust to changes in interaction policy, 
%% => In some sense we're asking the world model to succeed at out of distribution generalization. 
%% 

%% (1). Policy is different 
%% (2). World model performance is different and only little training data was acquired with the most recent world model  



% \begin{wrapfigure}{R}{0.35\textwidth}
% \vskip -0.2in
% \begin{center}
%     \includegraphics[width=.33\textwidth]{figures/causal_graph.pdf}
% \end{center}
% \vspace{-0.7cm}
% \caption{\textbf{A causal graph.} Vertices represent external agents at times $t$ and $t+1$, edges represent causal relationships. Dashed boxes denote the connected component {\em external agent behaviors}.}
% \label{fig:causal_graph}
% \vskip -0.1in
% \end{wrapfigure}


==> iclr_sections/diagnostic.tex <==
\section{Further attention analyses}
\label{app:further_attention_analysis}

Here we provide details of the early indicator analysis (Section~\ref{sec:future}) and a regression of what factors (curiosity signal, architecture, external agent behavior) best predict animate/inanimate attention ratios.

\subsection{Details of early indicator analysis}
\label{sec:app:attention_diagnostic}

We look to predict final performance $P_{\mathrm{final}}$ of a given agent, which we take to be the average of the final four validation runs. To make the modeling problem simple, we discretize this into a classification task by dividing validation performance into 3 equal-sized classes (``high'', ``medium'', and ``low'', computed separately for each external agent behavior), intuitively chosen to reflect performance around, at, and below that of random policy.

We consider two predictive models of final performance, one that takes as input early attention of the agent, and the other, early performance. Early performance may be quantified simply: given time $T$ (``diagnostic age'') during training, let $P_{\leq T}$ be the vector containing all validation losses measured up to time $T$. Early attention, however, is very high-dimensional, so we must make a dimensionality-reducing choice in order to tractably model with our modest sample size. Hence, we ``bucket'' average. Given choice of integer $B$, let
\begin{equation}
    A_{\leq T, B} = (\mathit{f}^{\mathrm{anim}}_{0 : \frac{T}{B}}, \mathit{f}^{\mathrm{rand}}_{ 0 :  \frac{T}{B}}, \mathit{f}^{\mathrm{anim}}_{\frac{T}{B}: \frac{2T}{B}}, \mathit{f}^{\mathrm{rand}}_{\frac{T}{B} : \frac{2T}{B}}, \ldots \mathit{f}^{\mathrm{anim}}_{\frac{(B - 1)T}{B} : T}, \mathit{f}^{\mathrm{rand}}_{\frac{(B - 1)T}{B} : T}),
\end{equation}
where $\mathit{f}^{\mathrm{anim}}_{a : b}$ and $\mathit{f}^{\mathrm{rand}}_{a : b}$ are the fraction of the time $t = a$ and $t = b$ spent looking at the animate external agent and random external agents respectively (so $A_{\leq T, B}$ is the attentional trajectory up to time $T$ discretized into $B$ buckets).

Finally, both models must have knowledge of the external agent behavior to which the agent is exposed --- we expect this to both have an effect on attention as well as the meaning of early performance and expected final performance as a result. Let $\chi_{\mathrm{BHR}}$ be the one-hot encoding of which external animate agent behavior is shown. 

We then consider models
\begin{enumerate}
    \item PERF$_{\leq T}$, which takes as input $P_{\leq T}$ and $\chi_{\mathrm{BHR}}$, and
    \item ATT$_{\leq T}$, which takes as input $A_{\leq T, B}$ and $\chi_{\mathrm{BHR}}$.
\end{enumerate}

Figure~\ref{fig:human_modeling_combined}b shows the plot of PERF$_{\leq T}$ and ATT$_{\leq T}$ accuracy as $T$ varies. We see that, up to a point, ATT$_{\leq T}$ makes a better predictor of final performance, and then PERF$_{\leq T}$ dominates. This confirms the intuition that attention patterns precede performance improvements. Intuitively, early attention predicts performance by being able to predict the sort of curiosity signal the agent is using, which predicts the full timecourse of attention (see~\ref{sec:app:attention_determinants}), which in turn predicts performance.

\input{icml_sections/attention_determinants.tex}


==> iclr_sections/discussion.tex <==
\section{Future directions}
\label{sec:future}

In this work, we propose and test $\gamma$-Progress, a computationally-scalable progress curiosity signal that enables an agent to efficiently train a world model in agent-rich environments while overcoming the white noise problem. Although in this work we limited the agent's ways of interacting with the world to visual attention, future works may explore larger action spaces. Another exciting avenue of research is investigating how to learn the world model priors used in this work such as the visual encoder and disentanglement prior. Finally, we hope see follow-up works applying $\gamma$-Progress to other domains such as video games. 

We also see several key next steps at the intersection of AI and cognitive science.

\noindent{\textbf{Human behavior}}~How might AWML-optimized agents model human behavior? We have run a pilot human subject experiment (Figure~\ref{fig:human_modeling_combined}a) in which we conveyed static, periodic, animate, and noise stimuli to twelve human participants via spherical robots while we tracked their gaze. In aggregate, gaze is similar to $\gamma$-Progress attention. In follow-up work, we aim to make a finer model comparison to the behavior of humans shown a diverse array of stimuli.



\begin{figure}
    \centering
    \includegraphics[width=.5\textwidth]{figures/humans_v6.pdf}
    \vspace{-20pt}
    \caption{\textbf{Modeling human behavior}. (a) A pilot human behavior study. (b)  Accuracy of early indicators of final performance, as a function of time, and (c) factor analysis: curiosity signal determines attention, which determines final performance.}
    \label{fig:human_modeling_combined}
    \vspace{-15pt}
\end{figure}


\noindent{\textbf{Early indicator analysis}}~Eventually, we would like to use curiosity-driven learning as a model for intrinsic motivation in early childhood. In this interpretation, the attention timecourse is a readily observable behavioral metric, and performance represents some more difficult-to-obtain measure of social acuity. Variation in curiosity signal would, in this account, be a latent correlate of developmental variability. For example, Autism Spectrum Disorder is characterized by both differences in low-level facial attention~\cite{jones2013attention} and high-level social acuity~\cite{hus2014ados}. Motivated by this, we sought to determine whether attention could be used as an early indicator of performance. We thus train two models:
(1) PERF$_{\leq T}$, which takes performance before time $T$ as input, and (2) ATT$_{\leq T}$, which takes attention before time $T$ as input.
As seen in Figure~\ref{fig:human_modeling_combined}b, ATT$_{\leq T}$ is throughout most of the timecourse a more accurate indicator than direct measurement of early-stage model performance itself. The overall situation is conveyed by the factor diagram Figure~\ref{fig:human_modeling_combined}c --- for further details, see Appendix~\ref{sec:app:attention_diagnostic}. As models grow in their capacity to model early childhood learning, translating such an analysis into a real-world experimental population could lead to substantial improvements in diagnostics of developmental variability.


==> iclr_sections/discussion_scrap.tex <==
\section{Future Directions}

%\jdf {Summarize results here}
%\jdf {Critically analyze the fact that we had to use a split model architecture, and what we think a more sophisticated system would look like (stuff Dan said about starting with shared parameters).}

Here we describe three next directions for this work. We first describe ongoing human subject experiments that mirror the computational ones described above. We then describe what preliminary results suggest are key ``theory of mind'' properties of world models that perform well in environments such as ours. Last, we interpret the above experiment as a toy model of early childhood development and provide an analysis of how behavior early in ``life'' predicts downstream social acuity.


Limitations:
other sorts of environments (while we designed environments to present a diverse array of stimuli while being able to maintain an understanding of what sorts of stimuli are being chosen without a wide array of confounds)
more complex embodiments
active learning: what is the validation set?
(based on our heuristic understanding of qhat is interesting, understanding broadly how to make this choice in these embodied active learning contetxts)


\noindent\textbf{Human experiments}

A standard hypothesis is that the human brain has a built-in module that specifically detects animacy from visual input \citep{leslie1989autism, leslie1994tomm}. Yet the current modeling results suggest that animate attention in humans might naturally arise from a more general process of curiosity-driven learning. In ongoing work, we are testing this possibility by running human subject experiments to measure important features of animate attention, then comparing our intrinsically-motivated models to this human behavior. 

These experiments include not only random and animate stimuli, but also other behaviors that span the spectrum of predictability, including \textit{static} objects, and \textit{periodic} ones, inspired by the repetitive dynamics seen in objects like seesaws, fans, and flashing lights. We convey these kinematics to humans via self-propelled, spherical robots moving along a mat, while measuring patterns of attention via a mobile eye tracker. So far, we find average fixation proportions favoring the animate stimuli. Furthermore, a progress network tasked to predict the virtual robot trajectories produces a similar aggregate attentional fixation pattern  \ref{fig:fig2_humans_v2.png}. Crucially, the network achieves this without the requirement for any specific built-in modules favoring animacy. Instead, the pattern arises from the agent’s discovery of the inherent relative “interestingness” of animacy as compared to random, periodic, and static motion. 


\begin{figure}[h]
    \centering
    \includegraphics[width=0.7\textwidth]{figures/fig2_humans_v3-01.png}
    \caption{Ongoing work compares our intrinsically-motivated agents to human observers watching analogous displays in the real-world. Human adults wear a mobile eye tracker while watching displays consisting of four sets of self-propelled, spherical robots travelling along a mat. Using kinematics alone, the robots are made to appear animate, random, periodic, or static. Spontaneous human fixations proportions are similar to the patterns of attention exhibited by our neural agent placed in a similar environment.}
    \jdf{Kun Ho: Can we get a version of the model plot with a more comparable hierarchy?}
    \label{fig:my_label}
\end{figure}

\kh{Error bars in the figure, more seeds with randomized location}

\noindent\textbf{Theory of Mind and social mental states}

In order for a curious agent to learn effectively in a social environment, all components of the system (e.g. world model architecture, intrinsic motivation, and controller architecture) must be suited to the task, and world model architecture choice of Section~\ref{sec:methods:worldmodel} reflect choices made to reach acceptable performance given sufficient data --- see Appendix~\ref{sec:app:causal} \ref{sec:offline} for details. In particular, a {\em Theory of Mind v0} motif, which allocates separate models for separate external agent behaviors, and more generally,  causally linked subsets of the environment, may be a crucial such choice. In future work, we will look to both (1) build a system that can infer this causal prior from data and (2) stress-test its utility in a suitable range of environments.

The choice of term {\em Theory of Mind v0} is deliberate because `theory of mind' is also  used to refer to the more sophisticated ability to predict the behaviors of other agents as a function of inferred mental states, such as beliefs, desires, and goals \citep{astington1990developing, premack1978does, wellman1992child}. Determining whether our models represent such mental states will require more deliberate tests inspired from developmental psychology, perhaps in tandem with specially-tailored learning environments and model architectures. For instance, one possibility is that curiosity models will need to solve an inverse reinforcement learning problem, in which they are specifically tasked with inferring an agent's world model and reward function, given its observed actions \citep{jara2019theory}. Relatedly, human agents do not only represent first-order knowledge about what others believe, but can also represent multiply embedded beliefs (e.g., he knows that I know he knows), as well as common knowledge (we all know that we all know), mental states which are a key to understanding more sophisticated social behaviors, such as coordinating on a goal, or turn taking \cite{de2019common, de2019maimonides, thomas2016recursive}. 

Alternatively, theory of mind-like representations might emerge without the need for such deliberate, social tasks. After all, the scope of things that are interesting and worth attending to is not limited to animate agents, so either way a more general purpose learning algorithm may be needed to detect patterns in the surrounding world. At any rate, learning to predict the full complexity of inanimate and animate stimuli using biologically plausible, unsupervised systems that can operate flexibly in the real-world presents a grand challenge for both AI and cognitive science.

\noindent\textbf{In silico models of human development}

An overarching goal of this research program is to develop in silico models of early childhood development. This is a task-driven modeling approach in which we design an artificial system to accomplish a challenging cognitive task that we as humans do well. If the task is sufficiently difficult that the solution space is small, we expect to see reflections of the artificial solution in behavior and biology. This approach has yielded dramatic success as a neural model of our ventral visual stream \cite{yamins_ventralneural}, using the task of visual object recognition. We posit that attention and interaction early in childhood, with the goal of learning to model one's surroundings, is a similarly difficult task, and by solving it, we can both better understand early childhood development as well as test interventions in simulation before resorting to human subject experiments.

Consider the following interpretation of the experiments of Section~\ref{sec:experiments} as a toy model of attention, interaction, and learning early in childhood. We model the development of a "population" of agents that have differently-implemented curiosity: differing intrinsic motivations represent underlying neural/genotype/phenotype correlates of early learning differences. Attention patterns represent abundant/cheaply obtained behavioral measures related to the sorts of exploratory strategies the agents have early in life (e.g. visual attention to animate stimuli), whereas validation performance represents a more difficult to obtain measure of acuity. An easily obtained behavioral measure that predicts outcomes later in life may provide both a valuable diagnostic criterion and a cue for possible interventions.

Using this model of early development, we ask: to what extent does the emergent attention pattern of the agent predict validation performance? We seek to understand whether attention {\em early} in a run predicts {\em final} validation performance, and in particular whether, sufficiently early in a run, attention is a better predictor than early validation performance of final validation performance. Intuitively, we expect attention patterns that lead to good validation performance to precede good validation performance itself.

We look to predict final performance $P_{\mathrm{final}}$ of a given agent, which we take to be the average of the final four validation runs. To make the modeling problem simple, we discretize this into a classification task by dividing validation performance into 3 equal-sized classes (``high'', ``medium'', and ``low'', computed separately for each external agent behavior), intuitively chosen to reflect performance around, at, and below that of random policy.

We consider two predictive models of final performance, one that takes as input early attention of the agent, and the other, early performance. Early performance may be quantified simply: given time $T$ (``diagnostic age'') during training, let $P_{\leq T}$ be the vector containing all validation losses measured up to time $T$. Early attention, however, is very high-dimensional, so we must make a dimensionality-reducing choice in order to tractably model with our modest sample size. Hence, we ``bucket'' average. Given choice of integer $B$, let
\begin{equation}
    A_{\leq T, B} = (\mathit{f}^{\mathrm{anim}}_{0 : \frac{T}{B}}, \mathit{f}^{\mathrm{rand}}_{ 0 :  \frac{T}{B}}, \mathit{f}^{\mathrm{anim}}_{\frac{T}{B}: \frac{2T}{B}}, \mathit{f}^{\mathrm{rand}}_{\frac{T}{B} : \frac{2T}{B}}, \ldots \mathit{f}^{\mathrm{anim}}_{\frac{(B - 1)T}{B} : T}, \mathit{f}^{\mathrm{rand}}_{\frac{(B - 1)T}{B} : T}),
\end{equation}
where $\mathit{f}^{\mathrm{anim}}_{a : b}$ and $\mathit{f}^{\mathrm{rand}}_{a : b}$ are the fraction of the time $t = a$ and $t = b$ spent looking at the animate external agent and random external agents respectively (so $A_{\leq T, B}$ is the attentional trajectory up to time $T$ discretized into $B$ buckets).

Finally, both models must have knowledge of the external agent behavior to which the agent is exposed --- we expect this to both have an effect on attention as well as the meaning of early performance and expected final performance as a result. Let $\chi_{\mathrm{BHR}}$ be the one-hot encoding of which external animate agent behavior is shown. 

We then consider models
\begin{enumerate}
    \item PERF$_{\leq T}$, which takes as input $P_{\leq T}$ and $\chi_{\mathrm{BHR}}$, and
    \item ATT$_{\leq T}$, which takes as input $A_{\leq T, B}$ and $\chi_{\mathrm{BHR}}$.
\end{enumerate}

\begin{figure}[h]
    \centering
    \includegraphics[width=\textwidth]{figures/early_indicator_analysis_with_attn.pdf}
    \caption{\textbf{Early diagnosis analysis}. Accuracy of PERF$_{\leq T}$ and ATT$_{\leq T}$ predictors of final performance, as a function of $T$. Up until late, attentional patterns make for the more informative predictor of final performance. Below, sample real-time attention trajectories that result in high, medial, and low final performance, from left to right. Intuitively, early attention trajectory predicts attention througout the run, which in turn predicts performance.}
    \label{fig:earlypredictor}
\end{figure}


Figure~\ref{fig:earlypredictor} shows the plot of PERF$_{\leq T}$ and ATT$_{\leq T}$ accuracy as $T$ varies. We see that, up to a point, ATT$_{\leq T}$ makes a better predictor of final performance, and then PERF$_{\leq T}$ dominates. This confirms the intuition that attention patterns precede performance improvements. Intuitively, attention predicts performance by being able to predict the sort of intrinsic motivation the agent is using, which in turn predicts performance. The attention trajectories Figure~\ref{fig:earlypredictor} correspond to agents that achieve different levels of final performance, and each display different attention early that characterizes the overall strategy. For example, the high final performance corresponds to a ``bump'' in attention towards the animate agent.







\begin{comment}
NH: prior to my big edits!

\jdf {Summarize results here}
\jdf {Critically analyze the fact that we had to use a split model architecture, and what we think a more sophisticated system would look like (stuff Dan said about starting with shared parameters).}

\noindent\textbf{Ongoing work: Human experiments}

As noted, a standard hypothesis is that the human brain has a built-in module that specifically detects animacy from visual input \citep{leslie1989autism, leslie1994tomm}. Yet the current modeling results suggest that animate attention in humans might naturally arise from a more general process of curiosity-driven learning. In ongoing work, we are testing this possibility by running human subject experiments to measure important features of animate attention, then comparing our intrinsically-motivated models to this human behavior. 

These experiments include not only random and animate stimuli, but also other behaviors that span the spectrum of predictability, including \textit{static} objects, and \textit{periodic} ones, inspired by the repetitive dynamics seen in objects like seesaws, fans, and flashing lights. We convey these kinematics to humans via self-propelled, spherical robots moving along a mat, while measuring patterns of attention via a mobile eye tracker. So far, we find average fixation proportions favoring the animate stimuli. Furthermore, a progress network tasked to predict the virtual robot trajectories produces a similar aggregate attentional fixation pattern  \ref{fig:fig2_humans_v2.png}. Crucially, the network achieves this without the requirement for any specific built-in modules favoring animacy. Instead, the pattern arises from the agent’s discovery of the inherent relative “interestingness” of animacy as compared to random, periodic, and static motion. 


\begin{figure}[h]
    \centering
    \includegraphics[width=0.7\textwidth]{figures/fig2_humans_v3-01.png}
    \caption{Ongoing work compares our intrinsically-motivated agents to human observers watching analogous displays in the real-world. Human adults wear a mobile eye tracker while watching displays consisting of four sets of self-propelled, spherical robots travelling along a mat. Using kinematics alone, the robots are made to appear animate, random, periodic, or static. Spontaneous human fixations proportions are similar to the patterns of attention exhibited by our neural agent placed in a similar environment.}
    \jdf{Kun Ho: Can we get a version of the model plot with a more comparable hierarchy?}
    \label{fig:my_label}
\end{figure}

\kh{Error bars in the figure, more seeds with randomized location}

\noindent\textbf{Future Work: Theory of Mind V1, and Other Mental States}


As noted, even human infants preferentially attend to the primitive kinds of animate behaviors included in the current experiments, and we have referred to the model innovations needed to replicate these behaviors as theory of mind v0. This naming convention is deliberate because `theory of mind' is also  used to refer to the more sophisticated ability to predict the behaviors of other agents as a function of inferred mental states, such as beliefs, desires, and goals \citep{astington1990developing, premack1978does, wellman1992child}. Determining whether our models represent such mental states will require more deliberate tests inspired from developmental psychology, perhaps in tandem with specially-tailored learning environments and model architectures. For instance, one possibility is that curiosity models will need to solve an inverse reinforcement learning problem, in which they are specifically tasked with inferring an agent's world model and reward function, given its observed actions \citep{jara2019theory}. Relatedly, human agents do not only represent first-order knowledge about what others believe, but can also represent multiply embedded beliefs (e.g., he knows that I know he knows), as well as common knowledge (we all know that we all know), mental states which are a key to understanding more sophisticated social behaviors, such as coordinating on a goal, or turn taking \cite{de2019common, de2019maimonides, thomas2016recursive}. 

Alternatively, theory of mind-like representations might emerge without the need for such deliberate, social tasks. After all, the scope of things that are interesting and worth attending to is not limited to animate agents, so either way a more general purpose learning algorithm may be needed to detect patterns in the surrounding world. At any rate, learning to predict the full complexity of inanimate and animate stimuli using biologically plausible, unsupervised systems that can operate flexibly in the real-world presents a grand challenge for both AI and cognitive science.





\end{comment}




\noindent{\textbf{Early indicator analysis}} To better understand how attention drives performance, we perform an {\em early indicator analysis} of whether attention {\em early} in a run predicts {\em final} validation performance, and in particular whether, sufficiently early in a run, attention is a better predictor than early validation performance. We hence train two models:
\begin{enumerate}
    \item PERF$_{\leq T}$, which takes as input performance before time $T$, and stimulus type, and
    \item ATT$_{\leq T}$, which takes as input a summary of attention before time $T$, and stimulus type.
\end{enumerate}
As seen in Figure~\ref{fig:human_modeling_combined}a, ATT$_{\leq T}$ dominates until late. Intuitively, as captured in the factor analysis diagram, we expect performance to be determined by attention throughout the run. Attention drives intrinsic motivation, and if the intrinsic motivation can be inferred early, this predicts later attention and hence performance. Interpreting this as a toy model of early childhood developmental variability (see Discussion for interpretation details), this tells us that attention patterns is a better {\em diagnostic} of later acuity than an early acuity-based diagnostic.

\begin{figure}
    \centering
    \includegraphics[width=.5\textwidth]{figures/humans.pdf}
    \vspace{-20pt}
    \caption{\textbf{Modeling human behavior}. (a)  Accuracy of early performance and early attention predictors of final performance, as a function of $T$, along with factor analysis hypothesis: intrinsic motivation (IM) determines attention, which determines final performance. (b) Human adults wear a mobile eye tracker while watching displays consisting of four sets of self-propelled, spherical robots travelling along a mat. Human and model fixation proportions are similar.}
    \label{fig:human_modeling_combined}
    % \vspace{-20pt}
\end{figure}


\noindent{\textbf{Human behavior}} To quantify how the emergent behavior matches that of humans, we ran a human subject experiment in which we conveyed static, periodic, animate, and noise stimuli to humans via self-propelled, spherical robots moving along a mat, while measuring patterns of attention via a mobile eye tracker. We find average fixation proportions favoring the animate stimuli. Furthermore, a $\gamma$-Progress network tasked to predict the virtual robot trajectories produces a similar aggregate attentional fixation pattern (Figure~\ref{fig:human_modeling_combined}b).

==> iclr_sections/discussion_scrap_2.tex <==
\section{Discussion and future directions}

In this work, we propose an implementation of curiosity that enables an agent to train efficiently a world model in environments containing other agents. Such environments
often contain static stimuli (easy to model), dynamic but largely deterministic stimuli (still relatively easy to model), noisy stimuli (to a large degree inherently unpredictable), as well as animate stimuli (interesting, complex, and to a considerable degree learnable). In order for the curious agent to be able to attend to the interesting without succumbing to the ``white noise problem,'' it mus be able to distinguish between these different sorts of stimuli. To accomplish this, we  propose $\gamma$-Progress, a computationally-scalable variant of progress-driven curiosity. To test this, we design a custom 3D virtual environment a variety of distillations of these classes of stimuli. We find that $\gamma$-Progress outperforms a variety of baselines in sample complexity. These agents learn better, faster, and they do so by learning to attend to what is interesting. The robustness and scalability of this method in relation to baselines makes it a prime candidate for both (1) embodied curiosity with other agents in increasingly ethologically-reasonable settings and (2) broader active learning and curiosity in a wide range of environments and tasks.

\nh{Rehash theory discussion? Let's settle on how we describe in intro first.}

Key next steps include testing these broad utilities. One limitation of the present work is in our restriction to the custom environment built to support our evaluation. We designed the environment to present a diverse array of stimuli while being able to maintain a level of control in understanding agent behavior, but this introduces its own biases. Further, in order to focus on intrinsic motivation implementation, we limited the embodiment of the agent. Lifting this restriction is an important step towards building embodied curiosity.

We see two important related activities. The first concerns the agent's world model: what makes a good world model for environments with other agents? Initial results suggest an important architectural motif, and it remains to validate this and more broadly develop computational ``theory of mind''. The second concerns how humans navigage a social world: does an implementation such as this reflect human decision making? And can we model child development with models such as these? In what follows, we describe progress towards these as well as important next steps.


\subsection{World models of other agents and theory of mind}

The world model architecture of Section~\ref{sec:methods:worldmodel} reflects choices made to guarantee acceptable prediction performance when trained on suitable data. In particular, a {\em Theory of Mind v0} motif, which allocates separate models for separate external agent behaviors, may be crucial. To test this, we construct an offline ``ideal dataset'' compare performance of this {\em causal} world model against two ablations: a {\em joined} acausal ablation that takes all observations and predicts all agents jointly, and a {\em split} acausal ablation that handles each external agent (as opposed to behavior) separately. For details on the training procedure and ablation implementations, see Appendix~\ref{sec:offline}. As seen in Figure~\ref{fig:offline_asymptotic_performance}, across all experiments, the causal world model significantly outperforms the ablations.

\begin{wrapfigure}{R}{0.4\textwidth}
\vspace{-10pt}
\begin{center}
    \includegraphics[width=.4    \textwidth]{figures/offline_asymptotic_performance_v6.pdf}
\end{center}
\vspace{-10pt}
    \caption{\textbf{Asymptotic Model Performance} The causal world model and the non-causal ablation were trained on data gathered under a reduced action space random policy, aimed at producing "ideal data" for learning each animate external agent behavior excluding peekaboo (See Section~\ref{sec:offline} for details.) \ms{Make taller}}
    \label{fig:offline_asymptotic_performance}
\vspace{-10pt}
\end{wrapfigure}

The reason for this performance difference may be understood in terms of {\em disentanglement}, in which the model finds spurious dependence ``nuisance factors'' --- some external agents are irrelevant to the behavior of others. It may be the case that poor disentanglement is more likely to occur and be detrimental to generalization performance when learning world models of partially observable environments via interactive learning. For a formalization of disentanglement and further discussion regarding the challenge in our setting, see Appendix~\ref{sec:app:causal}.

The choice of term {\em Theory of Mind v0} is deliberate because `theory of mind' is also  used to refer to the more sophisticated ability to predict the behaviors of other agents as a function of inferred mental states, such as beliefs, desires, and goals \citep{astington1990developing, premack1978does, wellman1992child}. The above motif represents a proto-version of this in which an agent, upon detecting agents or other stimuli in its environment, infers a causal structure of the environment and allocates modules of its world model that respects this causal structure. In future work, we will look to both (1) build a system that can infer this causal prior from data and (2) stress-test its utility in a suitable range of environments --- in particular, those with changing causal structure and greater interplay between causal structure and partial observability.

\subsection{Modeling human behavior}

An overarching goal of this research program is to develop models of human behavior. As a first step towards this, we would like to quantify how humans explore a similar environment and compare their behavior to that of models. In ongoing work, we are running human subject experiments in which we convey static, periodic, animate, and noise stimuli to humans via self-propelled, spherical robots moving along a mat, while measuring patterns of attention via a mobile eye tracker. The use of these spherical robots mirrors the virtual environment in order to reduce visual confounds and so as to present relatively novel stimuli to human adults. So far, we find average fixation proportions favoring the animate stimuli. Furthermore, a $\gamma$-Progress network tasked to predict the virtual robot trajectories produces a similar aggregate attentional fixation pattern. See Figure~\ref{fig:human_subject_experiment} for details.

\begin{wrapfigure}{L}{0.6\textwidth}
\vspace{-10pt}
\begin{center}
    \includegraphics[width=0.55\textwidth]{figures/fig2_humans_v3-01.png}
\end{center}
\vspace{-10pt}
    \caption{Ongoing work compares our intrinsically-motivated agents to human observers watching analogous displays in the real-world. Human adults wear a mobile eye tracker while watching displays consisting of four sets of self-propelled, spherical robots travelling along a mat. Using kinematics alone, the robots are made to appear animate, random, periodic, or static. Spontaneous human fixations proportions are similar to the patterns of attention exhibited by our neural agent placed in a similar environment.}
    \jdf{Kun Ho: Can we get a version of the model plot with a more comparable hierarchy?} \kh{Error bars in the figure, more seeds with randomized location}
    \label{fig:human_subject_experiment}
\vspace{-10pt}
\end{wrapfigure}

A standard hypothesis of human cognition is that the brain has a built-in module that specifically detects animacy from visual input \citep{leslie1989autism, leslie1994tomm}. The current modeling results suggest that animate attention in humans might naturally arise from a more general process of curiosity-driven learning.

If we can model adult human behavior, can we go further and model early childhood development? Can we model human developmental variability? One possibility is that, if such models can represent development of the general population, then implementation variations (e.g. in intrinsic motivation signal) can represent variability in development. Consider the following interpretation of the experiments of Section~\ref{sec:experiments} as a toy model of attention, interaction, and learning early in childhood. We model the development of a "population" of agents that have differently-implemented curiosity: differing intrinsic motivations represent underlying neural/genotype/phenotype correlates of early learning differences. Attention patterns represent abundant/cheaply obtained behavioral measures related to the sorts of exploratory strategies the agents have early in life (e.g. visual attention to animate stimuli), whereas validation performance represents a more difficult to obtain measure of acuity. An easily obtained behavioral measure that predicts outcomes later in life may provide both a valuable diagnostic criterion and a cue for possible interventions.

\begin{wrapfigure}{R}{0.6\textwidth}
\vspace{-10pt}
\begin{center}
    \includegraphics[width=.6 \textwidth]{figures/early_indicator_analysis_with_factor_analysis.pdf}
\end{center}
\vspace{-10pt}
    \caption{\textbf{Early diagnosis analysis}. (a) Accuracy of PERF$_{\leq T}$ and ATT$_{\leq T}$ predictors of final performance, as a function of $T$. Up until late, attentional patterns make for the more informative predictor of final performance. (b) Factor analysis hypothesis: intrinsic motivation (IM) determines attention, which determines final performance.}
    \label{fig:earlypredictor}
\vspace{-10pt}
\end{wrapfigure}

Using this model of early development, we seek to understand whether attention {\em early} in a run predicts {\em final} validation performance, and in particular whether, sufficiently early in a run, attention is a better predictor than early validation performance of final validation performance. To test this hypothesis, we train models that predict final performance from early attention (ATT$_{\leq T}$) or early performance (PERF$_{\leq T}$) (see Appendix~\ref{sec:app:attention_diagnostic} for details). As seen in Figure~\ref{fig:earlypredictor}, ATT$_{\leq T}$ dominates until late. Intuitively, as captured in the factor analysis diagram of Figure~\ref{fig:earlypredictor}, we expect performance to be determined by attention throughout the run; however, attention is driven by choice of intrinsic motivation, and if the intrinsic motivation implementation can be inferred early, this can be used to predict later attention and hence performance.








==> iclr_sections/environment.tex <==
\section{Virtual World Environment}
\label{sec:environment}
\vspace{-5pt}

We design our 3D virtual environment to preserve the following key properties of real-world environments: \textit{diverse dynamics}, i.e containing various agent-specific programs, \textit{partial observability}, information limited to what lies within view, and \textit{interactivity}, agent's actions influence the world. Our virtual environment consists of two main components, a \textit{curious neural agent} and various \textit{external agents}.

The \textbf{curious neural agent}, embodied by an avatar, fixed at the center of a room (Figure \ref{fig:environment}). Just as a human toddler can control her gaze to visually explore her surroundings, the agent is able to partially observe the environment based on what lies in its field of view (see top of Figure \ref{fig:environment}). The agent can choose from 9 actions: rotate $12^{\circ}, 24^{\circ}, 48^{\circ}$, or $96^{\circ}$, to the left/right, or stay in its current orientation. The \textbf{external agents} are spherical avatars that each act under a policy inspired by real-world inanimate and animate stimuli. An \textit{external agent behavior} consists of either one external agent, e.g reaching, or two interacting ones, e.g chasing. Since external agents are devoid of surface features, the curious agent must learn to attend to different behaviors based on spatiotemporal kinematics alone. We experiment with external agent behaviors (see Figure \ref{fig:environment}, right) including static, periodic, noise, reaching, chasing, peekaboo, and mimicry. (See Appendix \ref{sec:app:behaviors} for details) The animate behaviors have deterministic and stochastic variants, where the stochastic variant preserves the core dynamics underlying the behavior, albeit with more randomness. See \textcolor{blue}{\url{https://bit.ly/31vg7v1}} for video descriptions of the environment and external agent behaviors. 

We divide the room into four quadrants, each of which contains various auxiliary objects (e.g teddy bear, roller skates, surfboard) and one external agent behavior. The room is designed such that the curious agent can see at most one external agent behavior at any given time. 

    

==> iclr_sections/experiments.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/attention.pdf}
    \vspace{-15pt}
    \caption{\textbf{Attention Patterns}. Bar plots show total animate attention, i.e ratio between the number of time steps an animate external agent was visible to the curious agent, and the time steps a noise external agent was visible. Time series plots (zoom-in box) show the differences between mean attention to the animate external agents and the mean of attention to other agents in a 500 step window, with periods of animate preference highlighted in purple. Results averaged across 5 runs. $\gamma$-Progress displays strong animate attention while baselines are indifferent, e.g $\delta$-Progress, or fixating on white noise, e.g Adversarial.} 
    \label{fig:attention}
    \vspace{-5pt}
\end{figure*}

\section{Results}
\label{sec:experiments}
\vspace{-5pt}
%%%%%%%%%%%% Summary of what we seek to show %%%%%%%%%%%%%%

We evaluate the AWML performance of $\gamma$-Progress on two metrics: \emph{end performance} and \emph{sample complexity}. End performance is the inverse of the the final world loss after a larger number of environment interactions, and intuitively measures the ``consistency'' of the proxy reward with respect to the true reward. Sample complexity measures the rate of reduction in world model loss $\LL_{\mu}(\theta)$ with respect to the number of environment interactions. The samples from the validation distribution $\mu$ correspond to core validation cases we crafted for each behavior. For details, see Appendix \ref{sec:app:validation}.
Experiments are run in the Mixture world where the virtual environment is instantiated external agents spanning four representative types: static, periodic, noise, and animate. This set up is a natural distillation of a real-world environment containing a wide spectrum of behaviors. We run separate experiments in which the animate external agents are varied amongst the deterministic and stochastic versions of reaching, chasing, peekaboo, and mimicry agents (see Section \ref{sec:environment}). We compare the AWML performance of the following methods: 

\textbf{$\gamma$-Progress (Ours)} is our proposed variant of progress curiosity which chooses $\theta_{old}$ to be a geometric mixture of all past models as in Eq. \ref{eq:mix_progress}. 

\textbf{$\delta$-Progress \citep{achiam2017surprise, graves2017automated}} is the $\delta$-step learning progress reward from Eq. \ref{eq:kstep_progress} with $\delta = 1$. We found that any $\delta > 3$ is impractical due to memory constraints.  

\textbf{RND \citep{burda2018exploration}} is a novelty-based method that trains a predictor neural net to match the outputs of a random state encoder. States for which the predictor networks fails to match the random encoder are deemed ``novel'', and thus receive high reward. 

\textbf{Disagreement \citep{pathak2019disagreement}} is the disagreement based method from Eq. \ref{eq:disagreement} with $N = 3$ ensemble models. We found that $N > 3$ is impractical due to memory constraints.  

\textbf{Adversarial \citep{stadie2015predictive, pathak2017inverse}} is the prediction error based method from Eq. \ref{eq:adversarial}. We use the $\ell_{2}$ prediction loss of the world model as the reward. 

\textbf{Random} chooses actions uniformly at random among the 9 possible rotations. 

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\textwidth]{figures/sample_complex.pdf}
%     \caption{\textbf{AWML Performance in White Noise World}. Results shown for eight experiments in mixture worlds with the animate external agent varied according to the column labels. End performance (top row) is measured as the average of the last 4 validation losses. Sample complexity plots (bottom row) show validation losses evaluated every 5000 environment steps. Error bars/regions are computed over 5 seeds. $\gamma$-Progress achieves lower sample complexity than baselines on $8/8$ behaviors. Baselines frequently perform worse than the Random baseline due to white noise fixation.}
%     \label{fig:sample_complexity}
% \end{figure}

Fig.~\ref{fig:sample_complexity}a shows end performance (first row) and sample complexity (second row) in the Mixture world. In the Mixture world, we see that $\gamma$-Progress has lower sample complexity than $\delta$-Progress, Disagreement, Adversarial, and Random baselines on all $8/8$ behaviors and outperforms RND on $7/8$ behaviors while tying on stochastic chasing. See \textcolor{blue}{\url{https://bit.ly/31vg7v1}} for visualizations of model predictions.

Figure~\ref{fig:attention} shows the ratio of attention to animate vs other external agents for each behavior in the Mixture world as well as example animate-inanimate attention differential timeseries. The $\gamma$-Progress agents spend substantially more time attending to animate agents than do alternative policies. This increased animate-inanimate attention differential often corresponds to a characteristic attentional ``bump'' that occurs early as the $\gamma$-Progress curious agent focuses on animate external agents quickly before eventually ``losing interest'' as prediction accuracy is achieved. Strong animate attention emerges for $7/7$ behaviors when using $\gamma$-Progress.
Baselines display two distinct modes that lead to lower performance (Figure \ref{fig:attention}, bottom). The first is \textit{attentional indifference}, in which it finds no particular external agent interesting. $\delta$-Progress frequently had attentional indifference as the new and old world model, separated by a fixed time difference, were often too similar to generate a useful curiosity signal. The second failure mode is \textit{white noise fixation}, where the observer is captivated by the noise external agents. RND suffers from white noise fixation due to the fact that our noise behaviors have the most diffuse visited state distribution. We also observe that for noise behaviors, a world model ensemble does not collectively converge to a single mean prediction, and as a result Disagreement finds the noise behavior highly interesting. Finally, the Adversarial baseline fails since noise behaviors yield the highest prediction errors. The white noise failure mode is particularly detrimental to sample complexity, with RND, Disagreement, and Adversarial, as evidenced by their below-Random performance. 


==> iclr_sections/experiments_scrap.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/attention.pdf}
    \vspace{-15pt}
    \caption{\textbf{Attention Patterns in Mixture World}. The bar plot shows the total animate attention, which is the ratio between the number of time steps an animate external agent was visible and the number of time steps a noise external agent was visible. The plots in the zoom-in box show the real time differences between mean attention to the animate external agents and the mean of attention to the noise agents in a 500 time step window. Results are averaged across 5 runs. $\gamma$-Progress displays strong animate attention while baselines are either indifferent, e.g $\delta$-Progress, or fixating on white noise, e.g Adversarial.} 
    \label{fig:attention}
    \vspace{-10pt}
\end{figure*}

\section{Results}
\label{sec:experiments}
%%%%%%%%%%%% Summary of what we seek to show %%%%%%%%%%%%%%

We evaluate the AWML performance of $\gamma$-Progress on two metrics: \emph{end performance} and \emph{sample complexity}. End performance is the inverse of the the final world loss after a larger number of environment interactions, and intuitively measures the ``consistency'' of the proxy reward with respect to the true reward. Sample complexity measures the rate of reduction in world model loss $\LL(\theta, \mu)$ with respect to the number of environment interactions. The samples from the validation distribution $\mu$ correspond to core validation cases we crafted for each behavior. On the reaching behaviors, for example, we validate the world model loss with objects spawned at new locations. For details on each behavior-specific validation case, we refer readers to Appendix \ref{app:validation}. 

Experiments are run in two virtual worlds: Mixture and White Noise. In the Mixture world, the virtual environment is instantiated external agents spanning four representative types: static, periodic, noise, and animate. This set up is a natural distillation of a real-world environment containing a wide spectrum of behaviors. In the White Noise world, the environment is instantiated with three noise agents and one animate agent. This world strain tests the white noise robustness of $\gamma$-Progress. We compare the AWML performance the following methods: 

\textbf{$\gamma$-Progress (Ours)} is our proposed variant of progress curiosity which chooses $\theta_{old}$ to be a geometric mixture of all past models as in Eq. \ref{eq:mix_progress}. 

\textbf{$\delta$-Progress \citep{achiam2017surprise, graves2017automated}} is the $\delta$-step learning progress reward from Eq. \ref{eq:kstep_progress} with $\delta = 1$. We found that any $\delta > 3$ is impractical due to memory constraints.  

\textbf{RND \citep{burda2018exploration}} is a novelty-based method that trains a predictor neural net to match the outputs of a random state encoder. States for which the predictor networks fails to match the random encoder are deemed ``novel'', and thus receive high reward. 

\textbf{Disagreement \citep{pathak2019disagreement}} is the disagreement based method from Eq. \ref{eq:disagreement} with $N = 3$ ensemble models. We found that $N > 3$ is impractical due to memory constraints.  

\textbf{Adversarial \citep{stadie2015predictive, pathak2017inverse}} is the prediction error based method from Eq. \ref{eq:adversarial}. We use the $\ell_{2}$ prediction loss of the world model as the reward. 

\textbf{Random} chooses actions uniformly at random among the 9 possible rotations. 

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\textwidth]{figures/sample_complex.pdf}
%     \caption{\textbf{AWML Performance in White Noise World}. Results shown for eight experiments in mixture worlds with the animate external agent varied according to the column labels. End performance (top row) is measured as the average of the last 4 validation losses. Sample complexity plots (bottom row) show validation losses evaluated every 5000 environment steps. Error bars/regions are computed over 5 seeds. $\gamma$-Progress achieves lower sample complexity than baselines on $8/8$ behaviors. Baselines frequently perform worse than the Random baseline due to white noise fixation.}
%     \label{fig:sample_complexity}
% \end{figure}

\subsection{AWML Performance}
Fig.~\ref{fig:sample_complexity} shows end performance (first row) and sample complexity (second row) in the Mixture world. The validation loss $\LL(\theta, \mu)$ is averaged across the static, periodic, and animate external agents  The animate external agents are varied amongst the deterministic and stochastic versions of reaching, chasing, peekaboo, and mimicry agents (see Section \ref{sec:environment}). We see that $\gamma$-Progress has lower sample complexity than Disagreement, Adversarial, and Random baselines on all $8/8$ behaviors and outperforms RND and $\delta$-Progress on $7/8$ behaviors while tying on stochastic chasing. We found that \emph{$\gamma$-Progress obtains $3.4\times, 4.7\times, 6.5\times, 7.5\times, 7.8 \times$ lower mean end performance than $\delta$-Progress, RND, Disagreement, Adversarial, and Random baselines} across behaviors. See \textcolor{blue}{\url{https://bit.ly/2uf7lEY}} for visualizations of model predictions. 

We observed the baselines displaying two different failure modes. The first failure mode is attentional indifference, in which the curious agent finds no particular external agent in the environment interesting, and as a result its attentional patterns are similar to a random policy. The resulting AWML performance is similar to that of the Random baseline, e.g $\delta$-Progress and RND on the stochastic peekaboo behavior. The second failure mode is white noise fixation which is more detrimental to performance as the attention is heavily directed towards the noise external agents, e.g Adversarial and Disagreement baselines on the deterministic chasing behavior. We discuss this failure mode in more detail in the White Noise world experiments. \ms{Are we already explaining how attention affects performance here? If so should we refer readers to the attention figure?}  

We observed that Disagreement, Adversarial, RND, and $\delta$-Progress exhibit the indifference failure mode on $1/8, 2/8, 2/8, 6/8$ behaviors respectively, performing similar to the Random baseline, and the white noise failure mode on $4/8, 5/8, 2/8, 0/8$ behaviors, performing worse than the Random baseline. In particular, we observed that $\delta$-Progress frequently led to attentional indifference as the reward was not optimistic enough to anticipate future progress on the animate behaviors, i.e the new and old world model performances were similar. Similarly, we saw that $\gamma$-Progress led to attentional indifference when using a value of $\gamma$ that was too small. We thus found that the tractable memory usage of $\gamma$-Progress is key to achieving high AWML performance, as it enables flexible tuning of the progress horizon parameter.

%%%%%%%%%%%%%%%%%%%%%% Active Learning Metric %%%%%%%%%%%%%%%%%%%%%%%%%
Fig.~\ref{fig:sample_complexity} shows end performance (first row) and sample complexity (second row) in the white noise setup. The animate external agents are varied amongst the deterministic and stochastic versions of reaching, chasing, peekaboo, and mimicry agents. We see that $\gamma$-Progress has lower sample complexity than RND, Disagreement, and Adversarial baselines on all $8/8$ behaviors and outperforms $\delta$-Progress on $6/8$ behaviors while tying on the two peekaboo behaviors. We found that \emph{$\gamma$-Progress obtains $2.3\times, 4.6\times, 4.3\times, 7.2\times, 3.7\times$ lower mean end performance than $\delta$-Progress, RND, Disagreement, Adversarial, and Random baselines} across behaviors. 

We also found that the Random baseline obtains $1.9\times, 2.1\times, 3.4\times$ lower sample complexity than RND, Disagreement, Adversarial. This critical failure of the RND, Disagreement, and Adversarial baselines is due to white-noise fixation, i.e. the curiosity signals worsens AWML performance by driving the attention towards the unlearnable noise behavior which in turn reduces the number of data samples for learnable behaviors. In Fig. \ref{fig:attention}, we see that strong attention to the noise external agent emerges when using RND, Disagreement, and Adversarial methods. In particular, the zoom-in plots show that RND, Disagreement, and Adversarial methods attend to the noise agent significantly more than the Random baseline. RND suffers from white noise due to the fact that our noise behaviors have the most diffuse visited state distribution. We also observe that for complex noise behaviors \ms{do you mean the two-agent noise behavior?} the ensemble models do not collectively converge to a single mean prediction, and as a result finds the noise behavior highly interesting. Finally, the Adversarial baseline fails since noise behaviors yield the highest prediction errors. $\delta$-Progress outperforms the Random baseline by achieving $1.7\times$ lower AUC, but falls behind $\gamma$-Progress for the reasons described in the previous section. 

$\delta$-Progress does not suffer from white noise fixation, but exhibits attentional indifference, as shown by the similarity of its attention patterns to the Random baseline. We similarly attribute this to the inevitable usage of a small value of $\delta$, due to memory constraints. On the other hand, strong animate attention emerges for $7/7$ behaviors when using $\gamma$-Progress. In particular we observe that the animate attention arises accutely early on and eventually decays once the animate behavior is learned by the world model. The strong animate attention enables the curious agent to collect more samples of complex behaviors and thus more quickly reduce world model loss. 




==> iclr_sections/introduction.tex <==
\begin{figure*}[b!]
    \vspace{-5pt}
    \centering
    \includegraphics[width=\textwidth]{figures/environment_reduced_size.pdf}
    \vspace{-20pt}
    \caption{\textbf{Virtual environment.} Our 3D virtual environment is a distillation of key aspects of real-world environments. The \textit{curious agent} (white robot) is centered in a room, surrounded by various \textit{external agents} (colored spheres) contained in different quadrants, each with dynamics that correspond to a realistic inanimate or animate behavior (right box). The curious agent can rotate to attend to different behaviors as shown by the first-person view images at the top. See \textcolor{blue}{\url{https://bit.ly/31vg7v1}} for videos.} % still need to change objects to be something less awkward 
    \label{fig:environment}
    \vspace{-10pt}
\end{figure*}

\section{Introduction} 
\label{sec:introduction}
\vspace{-5pt}
Infants appear to actively build models of their environment by attending to stimuli in a highly non-random manner \citep{smith2019modeling, gergely1995taking, frankenhuis2013infants}. With the aim of building a neural agent that can do the same, we study Active World Model Learning (AWML) -- the problem of determining a directed exploration policy that enables efficient construction of better world models. (see Appendix \ref{sec:theory} for formal definition) To do so, we construct a progress-driven curious neural agent performing AWML in a custom-built 3D virtual world environment. Specifically, our contributions are as follows: 
(1). We construct a 3D virtual environment rich with agents displaying a wide spectrum of realistic stimuli behavior types with varying levels of learnability, such as static, periodic, noise, peekaboo, chasing, and mimicry. 
(2). We propose an AWML system driven by $\gamma$-Progress: a novel and scalable learning progress-based curiosity signal. We show that $\gamma$-Progress gives rise to an exploration policy that overcomes the white noise problem \citep{schmidhuber_formaltheoryoffun} and achieves significantly higher AWML performance than state-of-the-art exploration strategies — including Random Network Distillation (RND) \citep{burda2018exploration} and Model Disagreement \citep{pathak2019disagreement}.


% Our evaluations show that $\gamma$-Progress achieves significantly higher AWML performance than baseline controllers equipped with state-of-the-art exploration strategies — including Random Network Distillation (RND) \citep{burda2018exploration} and Model Disagreement \citep{pathak2019disagreement}.

% \sj{I think what could make the introduction more detailed is some intuition of why the proposed exploration strategy solves the problem you mentioned i.e. find interesting things to learn on. Otherwise, the advertisement of good performance in this paragraph aren't too convincing until people have seen either details of the method, or concrete the experimental results.}
% We begin in Section~\ref{sec:relatedworks}  by drawing connections to related works in cognitive science and artificial intelligence. In Section~\ref{sec:environment}, we describe our virtual environment in detail, including the range of inanimate and animate agents that we embed in it. Section~\ref{sec:theory} provides a novel mathematical formalization of Active World Model Learning  that our curious agent is tasked with and  motivates progress curiosity in the context of previously proposed curiosity signals. Section~\ref{sec:methods} details the implementations for all components of our curious active learning agent. Finally, Section~\ref{sec:experiments} presents experimental evaluations showing that our progress-driven controller achieves significantly higher AWML performance than baseline controllers equipped with state-of-the-art exploration strategies — including Random Network Distillation (RND) \citep{burda2018exploration} and Model Disagreement \citep{pathak2019disagreement}.

% \sj{A general comment is that it probably helps to clarify the contribution into different parts. I was initially confused whether the main contribution was the $\gamma$-progress objective. But it seems that proposing the environment and the learning problem is also major. (That was only obvious to me after seeing section 3). Also I was confused in the introduction about the relationship between the learning problem you propose (AWML) and the solution (agent) you propose. Is the agent the only way to perform optimally, or is it just one way to perform well. If the learning problem (AWML) and the solution are separate contributions, then it probably helps to clearly separate them.
% For example, the intro could have two or more paragraphs, one for each contribution.}

==> iclr_sections/introduction_scrap.tex <==
\section{Introduction} 
\label{sec:introduction}

Imagine yourself as a child at a busy playground. You are surrounded by a cornucopia of potentially interesting stimuli, from the leaves rustling along the ground, to the kickball lying abandoned in the sandbox, to the group of other children playing hide and seek in the far yard.
What would you like to do with your play time?   
After staring at the leaves briefly, you grow bored of watching their random motions. You then consider the kickball a bit more seriously --- dribbling and maneuvering it around by yourself could be pretty fun.  But you keep looking back to the hide-and-seekers, drawn by their dynamic moves and complex interplay.  You'll probably go join these other children, at least if you can succeed in convincing them to let you in on their game. 
Amongst this blooming and buzzing confusion, you have strong intuitions about which activities are the most exciting, about how to allocate your limited attention and time. 
This simple scenario exemplifies how humans continually engage in intrinsically-motivated exploration and interaction, a process whose strong naturally-emergent rules are especially salient for balancing attention between inanimate and animate objects~\citep{premack1990infant, gergely1995taking, frankenhuis2013infants}.
But how does this attentional control process occur?  And equally important, why does it occur --- what functional goals does it subserve? 

A fundamental underlying clue is that in the playground scenario, you are  continually learning \emph{world models} --- self-supervised predictions of what the dynamics of the world will bring, both due to its intrinsic dynamics and in response to your actions. 
Through learning world models, humans may acquire compact abstractions of high bandwidth sensory inputs, the ability to plan across long temporal horizons, and an understanding of the behavioral patterns of other agents. 
It is a natural hypothesis that attentional control is a core active learning mechanism enabling the agent to construct better and more robust world models. 
Conversely, better world models enable more effective attentional allocation.  The hide-and-seek game may perhaps be the most engaging option on the playground precisely because it presents the most sophisticated world-model prediction problems -- not unpredictable like the motions of the leaves in the wind, but involving complex inter-agent contingencies that are not as readily found in solo object-centric play. 

Discovering and formally describing the principles underlying such rich interactive scenarios is a key question in computational cognitive psychology. By the same token, devising algorithms that can learn effective world models in unfamiliar circumstances and use them to generate \emph{de novo} natural interactive behaviors is an important challenge for the next generation of socially-integrated AI and robotic systems.
In this work, we contribute to studying these questions by building neural network models of an agent embedded in a custom-built 3D virtual world environment, rich with external agents displaying a wide spectrum of realistic animate behaviors such as peekaboo, chasing, and mimicry. We show that, with proper choice of intrinsic motivation, an attention policy that distinguishes between animate and inanimate behavior emerges organically, without having to be hard-coded. In turn, by spending time on useful scenarios in a balanced fashion, this naturally ``socially-aware'' agent ends up learning world models more effectively and efficiently than alternatives. 

% meg said: we never really talk about the propensity for animate attention in humans (only mentioning the need to balance attention between inanimate and animate objects) and how that leads to more efficient world modeling - I guess it is implicitly conveyed in the sentence about how hide-and-seek game is the most engaging option, but it's just not as explicit as it should be, I think. - or the explicit explanation comes too late in the intro 

%meg said: I understand that this particular order of the last two sentences mirrors the order of the first two paragraphs. I wonder though whether it makes sense to reverse the order here to emphasize that the primary objective is world models and from it arises attention. Here, we don't have the issue of world models being hard to relate to as a real-world scenario so this order could work.
%dan replies: yes, but what I've described here is the actual "causal" pathway.  plus we want the paragraph to end on the most important thing (rather than have it be an intermediate sentence)
% meg replies: makes sense. 

In building an agent with these capabilities, we found it necessary to address the well-known ``white noise problem'', a potential failure mode of intrinsic motivation that has been acknowledged in many prior works~\citep{schmidhuber_formaltheoryoffun, pathak2017inverse, burda2018exploration, pathak2019disagreement}. An active learner must arbitrate between the combinatorially large number of stimuli exhibiting dynamic behaviors with various levels of learnability. The simplest objects in an environment are static, and easy to learn.  Inanimate objects with some reliable dynamics, e.g., a machine exhibiting periodic rotation, make the situation more complex, pressing on the intrinsic motivation to better distinguish interesting from uninteresting dynamics.  The problem is especially acute, however, for dynamics that are inherently unlearnable or chaotic e.g., falling leaves, wavering trees, and splashing water.  Distinguishing these from those that have interesting and complex yet learnable dynamics, e.g. children playing hide-and-seek turns out to be an especially difficult version of the white noise problem, one which is not effectively handled by recent curiosity approaches.  To solve it, we develop a novel variant of progress-driven curiosity, which we term ``$\gamma$-Progress'', that is able to robustly estimate learning progress in a computationally scalable fashion. 

%dan said: this paragraph, especially the end, needs for that will have to wait til we actually finish getting the results. 
%julian said: Can related works be section 1? It seems awkard to say that we begin in section 2}
%dan replies: it's "typical practice" in the AI literature to numner the sections this way.  but let's worry about this when we actually finalize this paragraph later
We begin in Section~\ref{sec:relatedworks}  by drawing connections between our work and related works in cognitive science and artificial intelligence. In Section~\ref{sec:environment}, we describe our virtual environment in detail, including the range of inanimate and animate agents that we embed in it. Section~\ref{sec:theory} mathematically formalizes the active learning problem that our curious agent is tasked with and  motivates progress curiosity in the context of previously proposed curiosity signals. Section~\ref{sec:methods} details the implementations for all components of our curious active learning agent. Finally, Section~\ref{sec:experiments} presents experimental evaluations showing that our progress-driven controller achieves significantly lower online sample complexity than baseline controllers equipped with state-of-the-art exploration strategies — including Random Network Distillation (RND) (Burda et al., 2018b) and Model Disagreement (Pathak et al., 2019).



\begin{comment}
Old version
Imagine yourself as a child at a busy playground. You are surrounded by a cornucopia of potentially interesting stimuli, from the leaves rustling along the ground, to the kickball lying abandoned in the sandbox, to the group of other children playing hide and seek in the far yard.
What would you like to do with your play time?   
After staring at the leaves briefly, you grow bored of watching their random motions. You then consider the kickball a bit more seriously --- dribbling and maneuvering it around by yourself could be pretty fun.  But you keep looking back to the hide-and-seekers, drawn by their dynamic moves and complex interplay.  You'll probably go join these other children, at least if you can succeed in convincing them to let you in on their game. 
Amongst this blooming and buzzing confusion, you have strong intuitions about which activities are the most exciting, about how to allocate your limited attention and time. 
This simple scenario exemplifies how humans continually engage in intrinsically-motivated exploration and interaction, a process whose strong naturally-emergent rules are especially salient for balancing attention between inanimate and animate objects~\citep{premack1990infant, gergely1995taking, frankenhuis2013infants}.
But how does this attentional control process occur?  And equally important, why does it occur --- what functional goals does it subserve? 

A fundamental underlying clue is that in the playground scenario, you are  continually learning \emph{world models} --- self-supervised predictions of what the dynamics of the world will bring, both due to its intrinsic dynamics and in response to your actions. 
Through learning world models, humans may acquire compact abstractions of high bandwidth sensory inputs, the ability to plan across long temporal horizons, and an understanding of the behavioral patterns of other agents. 
It is a natural hypothesis that attentional control is a core active learning mechanism enabling the agent to construct better and more robust world models. 
Conversely, better world models enable more effective attentional allocation.  The hide-and-seek game may perhaps be the most engaging option on the playground precisely because it presents the most sophisticated world-model prediction problems -- not unpredictable like the motions of the leaves in the wind, but involving complex inter-agent contingencies that are not as readily found in solo object-centric play. 

Discovering and formally describing the principles underlying such rich interactive scenarios is a key question in computational cognitive psychology. By the same token, devising algorithms that can learn effective world models in unfamiliar circumstances and use them to generate \emph{de novo} natural interactive behaviors is an important challenge for the next generation of socially-integrated AI and robotic systems.
In this work, we contribute to studying these questions by building neural network models of an agent embedded in a custom-built 3D virtual world environment, rich with external agents displaying a wide spectrum of realistic animate behaviors such as peekaboo, chasing, and mimicry. We show that, with proper choices of architecture and intrinsic motivation, an attention policy that distinguishes between animate and inanimate behavior emerges organically, without having to be hard-coded. In turn, by spending time on useful scenarios in a balanced fashion, this naturally ``socially-aware'' agent ends up learning world models more effectively and efficiently than alternatives. 

% meg said: we never really talk about the propensity for animate attention in humans (only mentioning the need to balance attention between inanimate and animate objects) and how that leads to more efficient world modeling - I guess it is implicitly conveyed in the sentence about how hide-and-seek game is the most engaging option, but it's just not as explicit as it should be, I think. - or the explicit explanation comes too late in the intro 

%meg said: I understand that this particular order of the last two sentences mirrors the order of the first two paragraphs. I wonder though whether it makes sense to reverse the order here to emphasize that the primary objective is world models and from it arises attention. Here, we don't have the issue of world models being hard to relate to as a real-world scenario so this order could work.
%dan replies: yes, but what I've described here is the actual "causal" pathway.  plus we want the paragraph to end on the most important thing (rather than have it be an intermediate sentence)
% meg replies: makes sense. 

In building an agent with these capabilities, we found it necessary to address two key algorithmic challenges. The first challenge is the well-known ``white noise problem'', a potential failure mode of intrinsic motivation that has been acknowledged in many prior works~\citep{schmidhuber_formaltheoryoffun, pathak2017inverse, burda2018exploration, pathak2019disagreement}. An active learner must arbitrate between the combinatorially large number of stimuli exhibiting dynamic behaviors with various levels of learnability. The simplest objects in an environment are static, and easy to learn.  Inanimate objects with some reliable dynamics, e.g., a machine exhibiting periodic rotation, make the situation more complex, pressing on the intrinsic motivation to better distinguish interesting from uninteresting dynamics.  The problem is especially acute, however, for dynamics that are inherently unlearnable or chaotic e.g., falling leaves, wavering trees, and splashing water.  Distinguishing these from those that have interesting and complex yet learnable dynamics, e.g. children playing hide-and-seek turns out to be an especially difficult version of the white noise problem, one which is not effectively handled by recent curiosity approaches.  To solve it, we develop a novel variant of progress-driven curiosity, which we term ``$\gamma$-progress'', that is able to robustly estimate learning progress in a computationally scalable fashion. 
%julian said: I'm wondering whether we should have a name for this second algorithmic challenge, so that we can refer to it later on, e.g., 'the animate detection problem'
%meg said: I think Dan meant that the first algorithmic challenge is white noise problem and second algorithm challenge is causal confusion (in the next paragraph), and animate detection problem is a consequence of white noise problem
%dan replies: @meg: exactly.  @jdf: why is this the second challenge? it's the first. and it's called the "white noise" problem.

%julian said: The following paragraph needs more work, and I think should refer to an example we raise in the introductory scenario, e.g., You initially think that one of the children is inspecting something on the tree, but then realize that she is using the tree to shield her field of view as the other children run to their chosen hiding spots. Could we make the examples here just a tad more specific, so that people really get it?  I don't think we've  explained what about partial observability contributes to causal confusion, so this may be confusing to readers
The second challenge is that in scenarios with several interacting and independent components (e.g. objects and other agents), world models predicting future dynamics are inherently susceptible to causal confusion --- e.g the mistaking spurious correlations for true causality --- a problem that has recently been recognized in the imitation-learning literature~\cite{}CITE.  
In the playground scenario for example, if two children are initially performing similar calisthenics simultaneously, a causally ill-informed observer might think that the apparent coordination between the two is a sign of an actual underlying causal relationship. %JDF: This example is a bit weird. What about something more ordinary, like you see one kid suddenly run away as another kid crosses over to them, but in fact the kid was running away from another child further a field. Therefore, you might predict that the runner always runs away from the first child, when in fact it was a coincidence. 
Later, if the observer only manages to keep only one of the children in view, they are likely to extrapolate their incorrect causal relationship to make spurious predictions about the unobserved child. %JDF: like what? I don't get it. 
More broadly, causal confusion leads to world models that exhibit poor future generalization performance, which turns out to be especially acute in scenarios like those we investigate, which exhibit only very partial observability from any given view. We endow our curious agent with a \emph{causally-aware world model} that integrates a causal prior into its network architecture to preempt causal confusion, and show that this choice is critical for achieving effective world-model learning.

%dan said: this paragraph, especially the end, needs for that will have to wait til we actually finish getting the results. 
%julian said: Can related works be section 1? It seems awkard to say that we begin in section 2}
%dan replies: it's "typical practice" in the AI literature to numner the sections this way.  but let's worry about this when we actually finalize this paragraph later
We begin in Section~\ref{sec:relatedworks}  by drawing connections between our work and related works in cognitive science and artificial intelligence. In Section~\ref{sec:environment}, we describe our virtual environment in detail, including the range of inanimate and animate agents that we embed in it. Section~\ref{sec:theory} mathematically formalizes the active learning problem that our curious agent is tasked with, motivates progress curiosity in the context of previously proposed curiosity signals, and characterizes the causal confusion problem. Section~\ref{sec:methods} details the implementations for all components of our curious active learning agent. Finally, Section~\ref{sec:experiments} presents experimental evaluations of our curious active learning system on two quantitative metrics: We show that (1) injecting a causal prior is essential to attaining high offline asymptotic model performance, and (2) our progress-driven controller achieves significantly lower online sample complexity than baseline controllers equipped with state-of-the-art exploration strategies — including Random Network Distillation (RND) (Burda et al., 2018b) and Model Disagreement (Pathak et al., 2019). Furthermore, when varying both the intrinsic motivation signal (considering several baselines) and world model architecture (with causal structure prior, and without), we find that the intrinsic motivation signal drives behavior, whereas the difference in world model architecture modulates behavior to a lesser degree.
\end{comment}

==> iclr_sections/methods.tex <==
\section{Methods}
\label{sec:methods}
\vspace{-5pt}
We describe a practical instantiation of the two components of our curious neural agent: a {\em world model} fitting the forward dynamics and a {\em progress-driven controller} which acts to maximize $\gamma$-Progress reward.

\noindent\textbf{World Model.} We assume that the agent has access to an oracle encoder $e: \O \rightarrow \X$ that maps an image observation $\rvo_t \in \O$ to a disentangled object-oriented feature vector $\rvx_t = (\rvx_{t}^{ext}, \rvx_{t}^{aux}, \rvx_t^{ego})$ where $\rvx_{t}^{ext} = (\tilde{\rvc}_{t}, \rvm_{t}) = (\tilde{\rvc}_{t, 1}, \ldots \tilde{\rvc}_{t, n_{ext}}, \rvm_{t, 1}, \ldots ,\rvm_{t, n_{ext}})$ contains information about the external agents; namely the observability masks $\rvm_{t, i}$ ($\rvm_{t, i} = 1$ if external agent $i$ is in curious agent's view at time $t$, else $\rvm_{t, i} = 0$) and masked position coordinates $\tilde{\rvc}_{t, i} = \rvc_{t, i}$ if $\rvm_{t, i} = 1$ and else $\tilde{\rvc}_{t, i} = \hat{\rvc}_{t, i}$. Here, $\rvc_{t, i}$ is the true global coordinate of external agent $i$ and $\hat{\rvc}_{t, i}$ is the model's predicted coordinate of external agent $i$ where $i = 1, \ldots , n_{ext}$. $\rvx_{t}^{aux}$ contains coordinates of auxiliary objects, and $\rvx_t^{ego}$ contains the ego-centric orientation of the curious agent. 
Our world model $\omega_{\theta}$ is an ensemble of component networks $\{\omega_{\theta^{k}}\}_{k = 1}^{N_{\mathrm{cc}}}$ where each $\omega_{\theta^{k}}$ independently predicts the forward dynamics for a subset $I_{k} \subseteq \{1, ..., \text{dim}(\rvx^{ext})\}$ of the input dimensions of $\rvx^{ext}$ corresponding to a minimal interdependent group in the world. For example, $\rvx^{ext}_{t:t+\tau, I_{k}}$ may correspond to the masked coordinates and observability masks of the chaser and runner external agents for times $t, t+1, ..., t+\tau$. We assume $\{I_{k}\}_{k = 1}^{n_{cc}}$ is given as prior knowledge but future work may integrate disentanglement learning into our pipeline. A component network $\omega_{\theta^{k}}$ takes as input $(\rvx^{ext}_{t - \tau_{in} : t, I_{k}}~,~\rvx^{aux}_{t - \tau_{in} : t}~,~\rvx^{ego}_{t - \tau_{in} : t}~,~\rva_{t - \tau_{in} : t + \tau_{out}})$, where $\rva$ denotes the curious agent's actions, and outputs $\hat{\rvx}^{ext}_{t : t + \tau_{out}, I_{k}}$. The outputs of the component network are concatenated to get the final output $\hat{\rvx}^{ext}_{t : t + \tau_{out}} = (\hat{\rvc}_{t:t+\tau_{out}}, \hat{\rvm}_{t:t+\tau_{out}})$. The world model loss is:  
\begin{align}
    \LL(\theta, \rvx_{t-\tau_{in}:t+\tau_{out}}, \rva_{t-\tau_{in}:t+\tau_{out}}) = \sum_{t' = t}^{t + \tau_{out}} \sum_{i = 1}^{N_{ext}} \rvm_{t', i} \cdot \|\hat{\rvc}_{t', i} - \tilde{\rvc}_{t', i}\|_2 + \LL_{ce}(\hat \rvm_{t', i}, \rvm_{t', i})
    \label{eq:loss}
\end{align}
where $\mathcal{L}_{ce}$ is cross-entropy loss. We parameterize each component network $\omega_{\theta^{k}}$ with a two-layer Long Short-Term Memory (LSTM) network followed by two-layer Multi Layer Perceptron (MLP). The number of hidden units are adapted to the number of external agents being modeled. 


% if $|I_{k}| = 1$ i.e., the causal group $k$ contains a single external agent, and 512 if $|I_{k}| \geq 2$ to ensure that the size of the parameter space scales with the input and output size. 
% All networks are train using Adam with a learning rate of 0.0001, $\beta_{1} = 0.9, \beta_{2} = 0.999$.

\noindent\textbf{Progress-driven Controller.} We propose \textbf{$\gamma$-Progress}, a scalable progress-based curiosity signal which approximates learning progress by the difference in the losses of an old model and a new model. The old model weights, $\theta_{old}$, lag behind those of the new model, $\theta_{new}$, with a simple update rule: $\theta_{old} \leftarrow \gamma \theta_{old} + (1 - \gamma) \theta_{new}$, where $\gamma$ is scalar mixing constant. The curiosity reward is:
\begin{align}
R(\rvx_{t}) = \LL(&\theta_{new}, \rvx_{t - \tau_{in} - \tau_{out}:t}, \rva_{t - \tau_{in} - \tau_{out}:t}) - \LL(\theta_{old}, \rvx_{t - \tau_{in} - \tau_{out}:t}, \rva_{t - \tau_{in} - \tau_{out}:t})
\label{eq:reward}
\end{align} 
Our controller $\pi_{\phi}$ follows an $\epsilon\text{-}greedy$ sampling scheme with respect to a Q-function $Q_{\phi}$ trained with the curiosity reward in Eq. \ref{eq:reward}. $Q_{\phi}$ is parametrized by a two-layer MLP with 512 hidden units that takes as input $\rvx_{t-2:t}$ and outputs estimated state-action values for all nine possible actions. $Q_{\phi}$ is updated with the DQN \cite{mnih2013playing} learning algorithm. 

==> iclr_sections/relatedwork_scrap.tex <==
\section{Related Works}
\label{sec:relatedworks}

\jdf{I'm starting to wonder whether it makes sense to have divided cognitive science and AI sections. It seems that the narrative at the end of the current cog sci section could just continue into the current AI sections, especially if there continues to be a string of psychological motivations. Currently the sections feel a bit disjointed. At the least we need an explicit statement that links the sections, e.g., talking about how the AI section starts to suggest how the sophisticated statistical learning we talk about at the end of the cog sci section might be implemented.}. 

We draw on cognitive science and ultimately aim to provide cognitive models. People have studied agents modeling their environments in cognitively-plausible ways. Active learning and curiosity have been studied and we add to the program of bringing the active learning of intuitive physics and psychology to artificial systems. 

\subsection{Cognitive science}
\label{sec:related:cognitive}

\noindent\textbf{Object-based attention and object permanence}

Although traditional models characterize attention as a `spotlight' that shines on areas of space, a wealth of work in cognitive science indicates that in many cases the units of attention in space \citep{scholl2001objects} and time \citep{de2014attentional} are distinct, bounded objects, aka \textbf{object-based attention}. Further, when the objects are dynamic, the human attentional system assigns individuated object tokens to each object, in order to keep track of them over time \citep{sears2000multiple}. The well-known limits on attention, then, often concern the maximum number of objects that can be tracked simultaneously, a limit that is thought to arise as multiple objects compete for representation on space-limited cortical real-estate \citep{alvarez2007many}. 

When tracking dynamic objects, the human brain must also deal with momentary disappearances of the objects it is tracking, as when they leave the field of view or become occluded. In such cases, it must solve a correspondence problem: which of the objects that it later sees is the same as the one that it was tracking a moment ago? The human brain appears to solve this problem by maintaining and updating an internal representation of the object even as it goes out of sight \citep{baillargeon1985object}, a phenomenon known as \textbf{object permanence}. This ability appears to rely on additional systems for visual imagery and working memory, which can also be guided by the oculomotor system \citep{de2016tracking, saiki2002multiple}. Working memory, similar to attentional selection, is limited in the number of objects which it can store simultaneously \citep{luck1997capacity}.

In the current work, our modeling framework includes object-based attention, object permanence, and working memory as inductive biases, i.e., knowledge that is built in as a prior of the model. We provide the model with the center coordinates of objects, and require it to predict their future center coordinates. Further, we use a memory system to maintain an active representation of an object whenever it goes out of sight.

\noindent\textbf {Animate attention, prediction, and theory of mind}

Given the limits on attention and memory, the human brain cannot track all of the objects with which it is confronted, and must therefore decide what subset of objects to either automatically or intentionally select for processing. Efficiently determining what to attend to is necessitated by the fact that not all objects are equally rich in information. Of note, in the majority of cases the most information-rich objects tend to be other animate entities, rather than many of the other kinds of entities that also occupy our fields of view, such as objects that are static (e.g., rocks, walls, and buildings), periodic (e.g., fans, wheels), or random (e.g., brownian motion in leaves, water, and the other elements). Unlike random stimuli, the dynamics of animate stimuli are learnable. And unlike static and periodic stimuli, which are either unchanging or repeatable, the spatiotemporal dynamics of animate stimuli contain more complex structures. 

Already as infants, humans are adept at distinguishing between inanimate and animate agents, preferentially paying attention to animate features like faces \citep{maurer2002many} and human body shapes \citep{slaughter2002development}, aka \textbf{animate attention}. Even in the absence of these surface features, infants will preferentially attend to spatiotemporal kinematics indicative of animate agents, such as self-propelled motion \citep{premack1990infant}, efficient movement towards targets \citep{gergely1995taking}, contingent behavior between observed agents, as when one agent chases another \citep{frankenhuis2013infants}, and contingent behavior between an observed agent and the infant herself, as when a robot beeps in response to the infant's babbling \citep{johnson2003detecting, foster1973visual}. In adults, these kinds of kinematics may give rise to an irresistable sense of animacy and intentionality, even when the objects executing the kinematics are simple shapes \citep{heider1944experimental}. In other words, the visual system has been highly tuned to cues that reliably indicate the presence of agents with internal sources of energy that cause them to move without the need for external forces. 

Beyond the ability of infants to discriminate between animate agents and other objects, a more sophisticated ability that emerges later in development is actively interpreting other agents in terms of their underlying mental states (beliefs, desires, and goals) that cause the agents' behavior, aka \textbf{theory of mind} \citep{astington1990developing, premack1978does, wellman1992child}, rather than in terms of physical forces. A theory of mind is needed in order to \textit{predict} what an agent will do next, since often it is only possible to do so accurately by generating expectations about an agent as a function of underlying intentions that are attributed to it. This ability is crucial to social functioning, and the failure to attribute mental states falls under the umbrella of symptoms that define the autism spectrum mental disorders \citep{baron2000theory}.

In the current work, our environment includes inanimate and animate agents with spatiotemporal kinematics inspired from these human experiments, and the agents are deliberately devoid of surface features, so that our modeling agent must discover which agents are interesting and  worth paying attention based on their spatiotemporal properties alone. We task our neural model with learning to discriminate among the different kinds of inanimate and animate agents, based on its ability to learn to predict what they will do next. 

\noindent\textbf {Diverging developmental theories}

Given that the above abilities arise early in human development, some have argued that infants may be born with an already specialized module devoted to representing the mental states of agents \citep{leslie1989autism, leslie1994tomm}. According to one dominant account, such a “theory of mind mechanism” could consist of a hard-wired, set of primitive propositional attitudes about concepts such as “desire” and “belief”. Note also that it is not a problem for this theory that infants are not immediately born with the ability to detect and predict agents, because an innate system could still be programmed to only come online later in life, perhaps triggered by certain environmental inputs \citep{scholl1999modularity}.

At the same time, infants exhibit an impressive ability to learn the statistical regularities in various tasks involving stimuli spanning all modalities, e.g., audition, vision, words \citep{fiser2002statistical, saffran1996statistical, maye2002infant}. As such, an alternative theory states that the bulk of attentional behavior may be driven by a more general-purpose learning mechanism, which allocates attention to stimuli based on their inherent, information-theoretic properties. Under this account, the particular attentional biases that have been characterized in existing work are an inevitable outcome of a smart learning system coming into contact with the different statistical properties of the  stimuli that happen to surround us.

Providing some support for this second view, previous work also finds that infants appear to gather information from environments in a manner that is quite principled: They selectively explore objects that violate their expectations \citep{stahl2015observing}, and they spend little time examining stimuli that are either too simple or too complex; instead, they preferentially attend to stimuli that are sufficiently complex to be interesting but not so complicated that they cannot be predicted \citep{kidd2012goldilocks}.

In the current work, while we do build in inductive biases concerning object-based attention, object-permanence, and working memory, we do not build in a propensity to detect and predict special classes of stimuli. Instead, we test whether reasonable patterns of attention of the form observed in humans can emerge naturally in our model, provided we endow it with a good, general-purpose learning objective. 

%\subsection{AI modeling of physical and social environments}

%While for this work we do not need sophisticated models capable of human-level intuitive physics, much progress has been made along these lines. Intuitive physics approaches: interaction networks, HRN, recent tenenbaum work \cite{This framing makes it sound like you're going to tell the reader about irrelevant stuff; what about framing it as people have focused on modeling the high-level stuff by assuming it exists, but not so much on modeling how you learn that stuff in the first place, using a biologically-plausible architecture.}

%Less progress has been made towards modeling human-level intuitive psychology. Multi-agent learning (relational forward models for multiagent learning), program induction (Human-level concept learning through probabilistic program induction \nh{Is there something newer}?

%In our model architecture, we have created an explicit read/write memory structure useful in predicting the trajectories of animate and inanimate stimuli over modest timescales. NTM, Merlin might embody more generic versions of this ---  one can imagine our explicit structures arising from training within the sorts of environments we consider over long time scales. In our work, we stick with short timescales. \nh{Our contribution here is not as clear, depends on whether we emphasize memory mechanism, or should keep incremental}


%\subsection{Curiosity, multi-task learning, and curriculum learning}

%In order to increase sample efficiency, it is useful for agents gathering data within their own worlds to make smart decisions about what data to capture. Basics of curiosity and intrinsic motivation. Related is classical active learning \cite{settles2011_active, giladbachrach_qbcreal_active} [lots more], in which an agent seeks to minimize the amount of labeling required in order to learn a supervised task.

%Different ways of defining intrinsic motivation, with subtlety of white noise problem
%Prediction Error: \cite{berkeley_mario, haber2018learning, interaction_cogsci}, Stadie.
%Novelty: Pseudocount, RND, Disagreement
%Progress: Schmidhuber, Oudeyer \cite{oudeyer2013intrinsically, oudeyer2007intrinsic}
%Information gain: Prediction Gain, VIME, Surprisal

%Related to curiosity are contexts in which an agent has many possible tasks or a family of tasks and must judiciously choose what to do, when. Curriculum learning, multi-task learning, and goal generation. [Automated Curriculum Learning for Neural Networks] [Control What You Can: Intrinsically Motivated Task-Planning Agent] [Automatic Goal Generation for Reinforcement Learning Agents] \cite{jaderberg2016reinforcement}.

\subsection{Artificial intelligence}

\jdf{What is the story we want to tell in this section?}
\jdf{How about something like this: 
(i) When do we understand the world around us? One idea is that we understand it when we can predict what will happen next. Briefly mention the alternatives (e.g., compression)
(ii) Talk about some psychological evidence that people do this, while gesturing at predictive coding (because we have to).
(iii)Introduce how this problem has been approached in the AI literature.
(iv) But what's missing from these approaches that we think is important?}
\jdf{Currently the content seems to jump around too much. Also, on a minor note, there's a lot of he said she said; can we just talk about the findings, while citing these people parenthetically? I think this puts the focus on the science.}.

\noindent{\textbf{World models concerned with dynamics}}

\jdf{Not sure if we want to cite some of the older biological work related to these ideas, e.g., Rosen R. (1985) Anticipatory systems: Philosophical, mathematical and methodological
foundations. Pergamon Press.}
\jdf{Originator credit? Maybe Gibson? Gibson J. J. (1979) The ecological approach to visual perception. Routledge.}

\jdf{Cites for the (newer idea of) predictive coding: 
Clark A. (2013) Whatever next? Predictive brains, situated agents, and the future of
cognitive science. Behavioral and Brain Science 36:181–204. 
Friston K. (2010) The free-energy principle: A unified brain theory? Nature Reviews
Neuroscience 11:127–38.; Rao R. P. & Ballard D. H. (1999) Predictive coding in the visual cortex: A functional interpretation of some extra-classical receptive-field effects. Nature Neuroscience 2:79–87.}

\jdf{Note that there are broadly two different kinds of predictive 'world' models that seem to battle it out in biology/psychology: (i) sometimes referred to as subjective physics, is the more Gibsonian view, which says that the models are physics models, which take the relations between observables. (ii) predictive coding, which maps internal variables to the observables (e.g., sensory inputs), and so is a 'generative model'. See Brette (2019) BBS- Is coding a relevant metaphor for the brain}.

A natural choice for what to model about one's environment is that of forward dynamics prediction: given a sequence of observations, perhaps along with the planned actions of the observer, predict some number of future observations. \jdf{Not sure why you're suddenly honing in on video frame prediction being hard here; I thought you were going to argue why predicting forward dynamics makes sense}. Video frame prediction \citep{kalchbrenner2016video, finn2016unsupervised} presents immense challenges in producing predictions that are realistic, let alone accurate, although recent innovations in architecture and loss function \citep{lee2018stochastic, wang2018predrnn++, Wu2019ModelIF} have shown considerable improvements. This self-supervised task draws inspiration from the neuroscience theory of \textbf{predictive coding}, and architectural motifs inspired by the neural theory \citep{lotter2016deep} have been shown to produce visual features that support other visual tasks. \jdf{what is an architectural motif exactly?} When conditioned on the actions of the observer, video prediction has shown utility in planning for robotic control tasks \citep{finn2017deep}. Related, \cite{ha2018world} build generative world models of virtual environments and use these ``dream'' environment simulations to train policies. \cite{chua2018deep} enhance performance in reinforcement learning tasks by incorporating calibrated forward dynamics models.

Some of the difficulty of predicting forward dynamics can be obviated by working not with images but in a given latent feature representation. For example, 3D point clouds data has been amenable to the forward dynamics prediction of rigid bodies \citep{byravan2017se3}. Approaches using object-centric, graphical representations of scenes \citep{battaglia2016interaction, chang2016compositional} have grown to be able to predict particulate representations of rigid and soft bodies \citep{mrowca2018flexible}. Coarse, probabilistic object-centric models have the ability to model human expectation violation of intuitive physics \citep{smith2019modeling}. \cite{ke2019learning} incorporate longer-term forward prediction in a latent space in order to enhance performance at reinforcement learning tasks.

Beyond forward dynamics prediction are self-supervised tasks that usefully model the dynamics of environments. Time reversal, in which a model is given an observation or observations and predicts that which preceded, can be used to plan by working backwards from goal states \citep{nair2018time}. \cite{agrawal2016learning} show inverse dynamics prediction, in which a model is given observations of an agent and must recover what actions the agent took, to be useful in robotic manipulation tasks. Networks can also be trained to predict other quantities from video frames, such as the height of an object in free fall, without being given labels of these quantities but rather by using known properties of the output space such as those derived from physics \citep{stewart2017label}.

In our work, we focus on the forward dynamics prediction problem on an object-centric representation of our environment. This representation simply consists of the positions of each object or agent in the environment, lacking other distinguishing features. We thus {\em assume} the agent has access to an encoding giving it this representation. This avoids the dual difficulties of both obtaining these representations from visual features and predicting the dynamics of complex media.

\noindent{\textbf{Active learning}}

\jdf{I still have to read this}

Independently of what is being modeled, the question of what actions to take in order to improve one's model efficiently has long been an important part of machine learning, statistics, and scientific thinking at large. Classically in \textbf{active learning} \citep{settles2011_active}, an agent seeks to learn a supervised task and tries to minimize the number of unlabeled examples it must label (the choice of what to label is the ``action'' of the agent). In doing so, the agent must make use of some signal by which it decides what action to take, with standard techniques including uncertainty sampling \citep{lewis1994heterogeneous}, query by disagreement \citep{cohn1994improving}, query by committee \citep{seung1992query}, error reduction \citep{roy2001toward}, and variance reduction \citep{geman1992neural}. Many of these techniques have been studied thoroughly within statistics, as, if we think of this ``act'' of labeling as deciding which experiment to perform when trying to fit a model or estimate a parameter, we arrive at \textbf{optimal experimental design} \citep{kahn1951estimation, fedorov2013theory, chaloner1995bayesian}.

Modern work on intrinsic motivation and curiosity can be considered a variant of active learning that concerns a reinforcement learning agent with sparse or no extrinsic reward \citep{schmidhuber_formaltheoryoffun, oudeyer2007intrinsic, oudeyer2013intrinsically}. In this, an agent trains a world model, and in taking action, it receives an intrinsic motivation ``reward'' computed using the world model. This intrinsic motivation signal is usually taken to be some estimate of how useful the action and resulting state are at producing an improved world model. In this way, the intrinsic motivation signal can be thought of as analogous to the signals by which more traditional active learning decisions are made, and indeed, many modern techniques take as inspiration the signals used in active learning and optimal experimental design. A number of approaches \citep{stadie2015predictive, interaction_cogsci, haber2018learning} use the world model's \textbf{prediction error}, though these in some contexts can result in the \textbf{white noise problem} in which agents are motivated to take actions that lead to unpredictable examples for the world model. In order to avoid the white noise problem, one can seek to estimate how actions lead to learning \textbf{progress} or \textbf{information gain}. How this is estimated is a core challenge, and many approaches towards estimating learning progress \citep{schmidhuber_formaltheoryoffun, oudeyer2007intrinsic, oudeyer2013intrinsically} or information gain \citep{houthooft_vime} present serious computational challenges when used at scale in complex environments. \textbf{Surprisal} \citep{achiam2017surprise} presents a computationally-tractable alternative to information gain. Model disagreement \cite{pathak2019disagreement}, in which intrinsic motivation is proportional to an ensemble of independently trained world models, presents another computationally-tractable alternative inspired by classical active learning techniques. For comprehensive reviews of intrinsic motivation signal choices, please see \citep{aubret2019survey, linke2019adapting}.

Related approaches rely on a fixed intrinsic motivation objective that does not take into account a specified world model problem. In the context of learning a world model problem, such intrinsic motivations can be thought of as \textbf{novelty} metrics, measuring how much a particular part of the environment has been explored. Examples include count-based exploration \cite{strehl2008analysis}, useful in tabular settings, and generalizations to continuous spaces such as pseudo-counts \citep{bellemare2016unifying} and Neural Density Models \citep{ostrovski2017count}. Certain variants of prediction error-based intrinsic motivation \citep{pathak2017inverse,pathak18largescale} seek to choose judiciously a learned feature space for a forward dynamics world model problem so that white noise issues do not arise. One recent popular approach, Random Network Distillation \citep{burda2018exploration}, takes as intrinsic motivation the prediction error of one neural network trying to match the output of a randomly initialized and frozen network of identical architecture. Related is \textbf{empowerment} \citep{mohamed2015variational}, in which the agent seeks to maximize the mutual information of action and state. \cite{jaderberg2016reinforcement} provides as intrinsic reward auxiliary tasks in order to better performance in sparse reward settings. \cite{kulkarni_hierarchical} combine intrinsic motivation with hierarchical action-value functions operating at different temporal scales, for goal-driven deep reinforcement learning.

The signals exploited in traditional active learning and curiosity have seen broad modern application outside of these classical and sparse reward contexts. \cite{graves2017automated} explore a number of learning progress estimators in order to build a curriculum in a multi-armed bandit setting. \cite{blaes2019control} use several such signals in order to solve several related tasks, some of which build on others, others of which are effectively impossible, providing a multi-task variant of the white noise problem.

It is worth noting how the intent of this work contrasts with several related themes. First, most studies of curiosity study intrinsic reward as either (1) a way to enhance performance at a reinforcement learning task with sparse but present extrinsic reward or (2) a method of encouraging good exploration, as measured by e.g. the amount of territory the agent has seen. In this work, we study curiosity {\em as active learning}, measuring success by improved performance at the world model problem. 

\nh{I took out a mention of attention mechanisms, as it doesn't fit here and is confusing. Any ideas for how to place?}
\ms{I guess our message is that ``attention'' mechansims are \textbf{not} related to this work, so perhaps we could place it somewhere other than related work where we talk about our attention measures to explicitly state that they were different lines of work?}
%Second, on a high level we look to optimize the agent's {\em visual attention} towards learnable stimuli. This, however, is imposed by the environment's strong partial observability at any given time. To contrast, {\em attention mechanisms}, visual or otherwise, seek to reduce the hypothesis space by for a task by directing model attention to limited subsets of observations. \ms{I see how the two  points in the later part of this paragraph correspond to (1) and (2), but it is a little unclear how attentional mechanisms relates to (2) seeing curiosity as a method of encouraging good exploration and especially to the mention of measuring amount of territory agent has seen}
%\nh{Agreed, I think attention comes a little out of left field here...not sure quite where to put it, as we're essentially saying "hey this thing with a name that might remind you of what we're doing is very different. doesn't quite fit the logic of this section or any other. need to think abhout this}

\noindent{\textbf{Multiagent and social learning}}

\nh{I have a note here for Kun Ho to see if there's some particularly salient robosoccer reference}

Environments with multiple artificial agents have been studied in order to optimize their interactions for a goal, understand or see what leads to their emergent behaviors, and exploit in order to train better models. Broadly, the field of multi-agent learning \citep{nguyen2018deep, zheng2018structured} concerns the coordination and communication of multiple agents within an environment in order to solve a reinforcement learning task. \cite{jaques2019social} explores the use of causal influence of one agent on another as intrinsic motivation to learn policies across agents in a decentralized manner. Of particular salience to our proposed world model architecture, \cite{tacchetti2018relational} learn a shared relational forward model, representing a network of relationships between agents, in order to boost performance at a multi-agent learning task. \cite{rabinowitz2018machine} demonstrate the use of a ``Theory of Mind'' neural network architecture that models behaviors in a gridwork environment.

Multi-agent systems can be studied not only through the lens of coordination in order to solve reinforcement learning tasks, but also through competition. \cite{baker2019emergent} study the emergence of interesting behaviors such as the use of tools in competitive multi-agent environments. \cite{vinyals2019grandmaster} use many agents pitted against each other in order to refine policies in the competitive strategy game setting of Starcraft II.

Robotics has been extended beyond multi-agent artificial environments and into social environments by developing predictive models of human behavior and using those to interact with people accordingly. A series of work on a social robot Jackrobbot \citep{ballan2016knowledge, robicquet2016learning, sadeghian2019sophie} uses human behavioral data in order to navigate real-world environments with both physical constraints and humans. \cite{kleinsurprise} learn predictive models of infant visual attention, aimed at designing robots that manipulate and encourage attention.

In the present work, we study the intrinsic motivations that lead to effective policies for, and the world model architectures that can enable, the learning of animate behaviors. Our work thus contrasts with multi-agent learning in that, in order to focus on these two computational factors, we precisely control all behaviors aside from that of our intrinsically motivated agent, and the agents do not cooperate or compete on any further objective.



====
Standard techniques include uncertainty sampling \citep{lewis1994heterogeneous}, query by disagreement \citep{cohn1994improving}, query by committee \citep{seung1992query}, error reduction \citep{roy2001toward}, and variance reduction \citep{geman1992neural}. Similar ideas have also been studied under the rubric of statistical \emph{optimal experimental design} \citep{kahn1951estimation, fedorov2013theory, chaloner1995bayesian}. 

\cite{jaderberg2016reinforcement} provides as intrinsic reward via auxiliary tasks in order to better performance in sparse reward settings. \cite{kulkarni_hierarchical} combine intrinsic motivation with hierarchical action-value functions operating at different temporal scales, for goal-driven deep reinforcement learning.
s
The signals exploited in traditional active learning and curiosity can also be applied outside of these sparse reward contexts. \cite{graves2017automated} explore a number of learning progress estimators in order to build a curriculum in a multi-armed bandit setting. \cite{blaes2019control} use several such signals in order to solve several related tasks, some of which build on others, others of which are effectively impossible, providing a multi-task variant of the white noise problem.

%It is worth noting how the intent of this work contrasts with several related themes. First, most studies of curiosity study intrinsic reward as either (1) a way to enhance performance at a reinforcement learning task with sparse but present extrinsic reward or (2) a method of encouraging good exploration, as measured by e.g. the amount of territory the agent has seen. In this work, we study curiosity {\em as active learning}, measuring success by improved performance at the world model problem. 

















% cogsci section after dan shortened it: 
\noindent\textbf{Object dynamics prediction, attention, and permanence.} 
Humans are extremely effective at understanding dynamics of objects in their environment, excelling at intuitively predicting both the physical interactions of external objects~\cite{} and the physical consequences of their own actions~\cite{}. 
However, both the visual system and the working memory system that support these abilities have substantial limitations~\cite{}. 
Humans thus selectively allocate attention in an object-centric fashion to enable effective prediction despite these limitations \citep{alvarez2007many, scholl2001objects}, and assign individuated tokens to keep track of objects over time \citep{sears2000multiple}. To deal with momentary disappearances of objects as they become occluded or leave the visual frame, the brain maintains and updates an internal persistent representation of objects, a phenomenon known as \emph{object permanence}~\cite{piaget_originsintelligence}.  Studies in human infants have shown that many of these abilities --- including understanding the dynamical continuity of physical trajectories, the solidity of objects, and their persistence even when out of sight --- appear to be present very early in development~\cite{spelke_objectpermanence, spelke2007core, baillargeon1985object}. 
In this work, we include object-based attention, object permanence, and working memory as architectural biases, i.e. knowledge that is built in as a prior of the model. To enable dynamical prediction, we provide the model with the center coordinates of objects, and require it to predict their future center coordinates. Further, we use a memory system to maintain an active representation of an object whenever it goes out of sight. 

\noindent\textbf{Curiosity and Active Learning.} Attentional control also appears to be of great importance for learning how the world works.  Infants appear to gather information from environments in a manner that is quite principled, selectively looking at objects in highly non-random manner~\cite{smith}, and devoting increased attention to objects that violate their expectations \citep{stahl2015observing}.  Infants also appear to self-generate useful learning curricula, preferentially attending to stimuli that are sufficiently complex to be interesting but not so complicated that they cannot be predicted, a phenomenon known as the \emph{goldilocks effect} \citep{kidd2012goldilocks}.  In this work, a key question that we address is the formalization of the intrinsic motivations underlying active learning in a multi-agent context. 

\noindent\textbf{Animate attention.}
From early infancy, humans are especially adept at distinguishing between inanimate and animate agents, preferentially paying attention to animate features like faces \citep{maurer2002many} and human body shapes \citep{slaughter2002development}, a phenomenon called \emph{animate attention}. Even in the absence of these surface features, infants will preferentially attend to spatiotemporal kinematics indicative of animate agents, such as self-propelled motion \citep{premack1990infant}, efficient movement towards targets \citep{gergely1995taking}, contingent behavior between observed agents, as when one agent chases another \citep{frankenhuis2013infants}, and contingent behavior between an observed agent and the infant herself, as when a robot beeps in response to the infant's babbling \citep{johnson2003detecting, foster1973visual}.  The visual system has been highly tuned to cues that reliably indicate the presence of agents with internal sources of energy and volition that cause them to move without the need for external forces. Such kinematic patterns give rise to an irresistable sense of animacy and intentionality, even when the objects executing the kinematics are simple shapes \citep{heider1944experimental}. 
In this work, our environment includes inanimate and animate agents with spatiotemporal kinematics inspired from these human experiments, and the agents are deliberately devoid of surface features, so that our modeling agent must discover which agents are interesting and worth paying attention to based on their spatiotemporal properties alone. 
While we do build in inductive biases concerning object-permanence and working memory, we do not build in a propensity to detect and predict special classes of stimuli. Instead, we test whether reasonable patterns of attention of the form observed in humans can emerge naturally in our model, provided we endow it with a good, general-purpose learning objective.

\noindent\textbf{Social prediction and theory of mind.}
Beyond animate attention, a more sophisticated ability that emerges later in development is the active interpretation of other agents in terms of their underlying mental states (beliefs, desires, and goals) that cause the agents' behavior, aka \emph{theory of mind} \citep{astington1990developing, premack1978does, wellman1992child}. It is hypothesized that theory of mind is needed in order to \textit{predict} what an agent will do next, since often it is only possible to do so accurately by generating expectations about an agent as a function of underlying intentions that are attributed to it. This ability is crucial to social functioning, and the failure to attribute mental states falls under the umbrella of symptoms that define the autism spectrum mental disorders \citep{baron2000theory}.  
In this work, we task our neural model with learning to predict what the objects and agents in the environment will do next, and seek to determine which features of animate attention and theory of mind are required to achieve improved world-model predictions.

==> iclr_sections/relatedwork_scrap2.tex <==
\section{Related Works}
\label{sec:relatedworks}

Both artificial intelligence and cognitive science have developed substantial literatures around  world-modeling and attentional control.

\subsection{Artificial Intelligence}

\noindent{\textbf{World models and prediction.}}
A natural class of world-models involve forward dynamics prediction. The most direct form involves video frame prediction\citep{kalchbrenner2016video, finn2016unsupervised}, inspired by the long-standing neuroscience concept of \emph{predictive coding}\citep{lotter2016deep}.  Action-conditioned video frame prediction models can be used directly in planning for robotic control tasks~\citep{finn2017deep}, as performance-enhancers for reinforcement learning tasks\citep{chua2018deep,ke2019learning}, or as ``dream'' environment simulations for training policies~\citep{ha2018world}. Video frame prediction enormously challenging to accomplish, despite some progress\citep{lee2018stochastic, wang2018predrnn++, Wu2019ModelIF}. 
Some of the difficulty of predicting forward dynamics can be alleviated by working not with images but in latent feature representations such as 3D point clouds~\citep{byravan2017se3} or object-centric, graphical representations of scenes~\citep{battaglia2016interaction, chang2016compositional, mrowca2018flexible}. Such models have been shown to coarsely model human expectation violation of intuitive physics \citep{smith2019modeling}. 
World-models can also be derived from prediction problems other than forward dynamics, including time reversal \citep{nair2018time} and inverse dynamics~\citep{agrawal2016learning}, approaches that have proven useful in building world models for well-defined robotic manipulation tasks. 
World-models can also be targeted toward specific attributes rather than full state-space prediction --- e.g. the height of an object in free fall --- allowing the known physical constraints of the output space to drive learning~\citep{stewart2017label}. 

In our work, we focus on a forward-dynamics prediction problem in an object-centric representation. This representation simply consists of the positions of each object or agent in the environment, lacking other distinguishing features. We thus {\em assume} the agent has access to an encoding giving it this representation, bypassing the important but complex question of how to extract this representation directly from visual features, so as to focus the present work on identifying good solutions for active learning and multi-agent causal modeling. 

\noindent{\textbf{Active learning.}}
Independently of which task the agent self-supervises its world-model on, a key question the agent is faced with is choosing its actions to efficiently learn the world-model. In the classical \emph{active learning} setting~\citep{settles2011_active}, an agent seeks to learn a supervised task with costly labels, judiciously choosing which examples to obtain labels for so as to maximize learning efficiency. 
More recently, active learning has evolved in the context of self-supervised reinforcement learning agents~\citep{schmidhuber_formaltheoryoffun, oudeyer2013intrinsically, jaderberg2016reinforcement}. In this line of work, agents typically self-supervise a world-model using an intrinsically-generated ``curiosity''.  Many different approaches to this general idea exist, all of which are essentially different approaches to estimating \emph{learning progress} --- e.g. determining which actions lead are likely to lead to the highest world-model accuracy gain in the future.  

One popular approach is the use of \emph{novelty} metrics, which measure how much a particular part of the environment has been explored, and direct agents into under-explored parts of state-space. 
Examples include count-based and psuedo-count-based methods~\citep{strehl2008analysis,bellemare2016unifying, ostrovski2017count}, Random Network Distillation (RND)~\citep{burda2018exploration}, and the \emph{empowerment} metric \citep{mohamed2015variational}. 
Novelty-based approaches avoid the difficult world-model-progress estimation problem entirely by not depending at all on a specific world-model state, and relying on novelty as a (potentially flawed) proxy for learning progress. 

The simplest idea that actually takes into account the world-model problem to be learned is \emph{adversarial} curiosity, which estimates current world-model error and directs agents to actions estimated to maximize this error~\citep{stadie2015predictive, pathak2017inverse, haber2018learning}. However, direct error-driven curiosity can result in the \emph{white noise problem}, in which agents are motivated to waste time fruitlessly trying to solve unsolvable world-modeling problems, e.g. where there is degeneracy in the cause or effect of the action. While the white noise problem can to some degree be avoided by solving the world-modeling problem in a learned latent feature-space in which degeneracies are suppressed~\citep{pathak2017inverse, pathak18largescale}, directly estimating learning progress ~\citep{oudeyer2007intrinsic, oudeyer2013intrinsically} or \emph{information gain}~\citep{houthooft_vime} avoids the white noise problem in a more comprehensive fashion. However, such methods have been limited in scope because they involve calculating quantities that cannot easily be estimated in many-dimensional continuous action spaces.
\emph{Surprisal}~\citep{achiam2017surprise} and model disagreement\citep{pathak2019disagreement} present computationally-tractable alternatives to information gain, at the cost of the accuracy of the estimation. For comprehensive reviews of intrinsic motivation signal choices, see \citep{aubret2019survey, linke2019adapting}.
In this work, we present a novel method for estimating learning progress that takes advantage such metrics have in ensuring the directed learning utility of action choices, while being robust and scalable to high-dimensional continuous action-space settings. 

\noindent{\textbf{Multiagent and social learning.}}
The field of multi-agent learning \citep{nguyen2018deep, zheng2018structured} concerns the coordination and communication of multiple agents within an environment in order to solve a reinforcement learning task. \citep{jaques2019social} explores the use of causal influence of one agent on another as intrinsic motivation to learn policies across agents in a decentralized manner.  \citep{rabinowitz2018machine} demonstrate the use of a ``Theory of Mind'' neural network architecture that models behaviors in a gridworld environment.
\citep{baker2019emergent} study the emergence of interesting behaviors such as the use of tools in competitive multi-agent environments. \citep{vinyals2019grandmaster} use many agents pitted against each other in order to refine policies in the competitive strategy game setting of Starcraft II.
\citep{tacchetti2018relational} learns a shared relational forward model, representing a network of relationships between agents, in order to boost performance at a multi-agent learning task.
Multi-agent learning has also been extended beyond artificial environments and into real social environments by developing predictive models of specific human behaviors and using those to enable robots to better interact with people\citep{ballan2016knowledge, robicquet2016learning, sadeghian2019sophie}.
\citep{kleinsurprise} learn predictive models of infant visual attention, aimed at designing robots that manipulate and encourage attention.

In this work, we address a multi-agent reinforcement problem from the point of view of a single agent that seeks to learn about the actions of other agents it observes and interacts with. Like other works, our goal is to build architectures and policies that enable the learning agent to better understand what other agents will do, but unlike other works we do not hard-code in either the learning objective (e.g. our work is self-supervised) or the behavioral outcomes (e.g. natural attention patterns \emph{emerge} as a solution to better multi-agent prediction). 

\noindent{\textbf{Attention.}} A wide variety of problems have been shown to benefit from neural network architectures that employ what has come to be called ``attention'' in the AI literature, e.g. local multiplicative gating that dynamically learns to highlight portions of the network during inference, so as to focus processing on particularly relevant portions of either the input data or intermediate featural content~\cite{}. This literature is related to our current work in that it shows how selective highlighting of some form can improve learning, but differs significantly from our work in the meaning of the term ``attention'', the importance of the active learning setting, and the technical machinery needed use attention in this setting.  What we call ''attention'' in our work is literally the idea that a physically embodied agent will allocate its observational time differently for different stimuli, rather than the more abstract disembodied concept used in most AI literature. In contrast to attentional multiplication in the typical supervised off-line learning setting, our agents need attentional control to perform effective active learning, creating datapoints that without such control would otherwise occur either very rarely or not at all.  The causal world model architecture and learning progress policy we develop to programmatically generate the right types of such control are thus structurally distinct from the multiplicative gating operations used in typical AI attention work.

\subsection{Cognitive Science}
\label{subsec:related:cognitive}

\noindent\textbf{Object dynamics prediction, attention, and permanence.} 
Humans are extremely effective at understanding object dynamics, excelling at intuitively predicting both the physical interactions of external objects~\citep{} and the physical consequences of their own actions~\citep{}. 
However, both the visual system and the working memory system that support these abilities have substantial limitations~\citep{}. 
Humans thus selectively allocate attention in an object-centric fashion to enable effective prediction despite these limitations~\citep{alvarez2007many, scholl2001objects}, and assign individuated tokens to keep track of objects over time~\citep{sears2000multiple}. To deal with momentary disappearances of objects as they become occluded or leave the visual frame, the brain maintains an internal representation of objects, a phenomenon known as \emph{object permanence}~\citep{piaget_originsintelligence}.  Infant studies show that many of these abilities --- including understanding the dynamical continuity of physical trajectories, object solidity, and their persistence even when out of sight --- appear to be present very early in development~\citep{spelke_objectpermanence, spelke2007core, baillargeon1985object}. 
In this work, we include object-based attention, object permanence, and working memory as architectural biases. We require the model to perform dynamimcs prediction on the center coordinates of objects, and we use a memory system to maintain an active representation of an object whenever it goes out of sight. 

\noindent\textbf{Curiosity and Active Learning.} Attentional control also appears to be of great importance for learning how the world works.  Infants appear to gather information from environments in a manner that is quite principled, selectively looking at objects in highly non-random manner~\citep{smith}, and devoting increased attention to objects that violate their expectations \citep{stahl2015observing}.  Infants also appear to self-generate useful learning curricula, preferentially attending to stimuli that are sufficiently complex to be interesting but not so complicated that they cannot be predicted, a phenomenon known as the \emph{goldilocks effect}~\citep{kidd2012goldilocks}.  In this work, a key question that we address is the formalization of the intrinsic motivations underlying active learning in a multi-agent context. 

\noindent\textbf{Animate attention.}
From early infancy, humans are especially adept at distinguishing between inanimate and animate agents, preferentially paying attention to animate features like faces \citep{maurer2002many} and human body shapes~\citep{slaughter2002development}. Even in the absence of these surface features, infants will preferentially attend to spatiotemporal kinematics indicative of animate agents, such as self-propelled motion~\citep{premack1990infant}, efficient movement towards targets~\citep{gergely1995taking}, contingent behavior between observed agents, as when one agent chases another~\citep{frankenhuis2013infants}, and contingent behavior between an observed agent and the infant herself, as when a robot beeps in response to the infant's babbling~\citep{johnson2003detecting, foster1973visual}.  The visual system is highly tuned to cues that reliably indicate the presence of agents with internal sources of energy that cause them to move without external forces. Such kinematic patterns give rise to an irresistable sense of animacy and intentionality, even when the objects executing the kinematics are simple shapes~\citep{heider1944experimental}. 
In this work, our environment includes agents with spatiotemporal kinematics inspired by these human experiments, and the agents are deliberately devoid of surface features, so that our curious agent must discover which agents are interesting and worth paying attention to based on their dynamics alone. 
While we build in inductive biases concerning object-permanence and working memory, we do not build in a propensity to detect and predict special classes of stimuli. Instead, we test whether reasonable patterns of attention of the form observed in humans emerges naturally in our model, provided we endow it with the right intrinsic motivation.

\noindent\textbf{Social prediction and theory of mind.}
Beyond animate attention, a more sophisticated ability that emerges later in development is the active interpretation of other agents in terms of their underlying mental states (beliefs, desires, and goals) that cause the agents' behavior, aka \emph{theory of mind} \citep{astington1990developing, premack1978does, wellman1992child}. It is hypothesized that theory of mind is needed in order to \textit{predict} what an agent will do next, since often it is only possible to do so accurately by generating expectations about an agent as a function of underlying intentions that are attributed to it. This ability is crucial to social functioning, and the failure to attribute mental states falls under the umbrella of symptoms that define the autism spectrum mental disorders~\citep{baron2000theory}.  
In this work, we task our neural model with learning to predict what the objects and agents in the environment will do next, and seek to determine which features of animate attention and theory of mind are required to achieve improved world-model predictions.










==> iclr_sections/relatedworks.tex <==
\begin{figure*}[t!]
    \centering
    \includegraphics[width=\textwidth]{figures/model.pdf}
    \vspace{-20pt}
    \caption{\textbf{Active World Model Learning with $\gamma$-Progress} The curious agent consists of a \emph{world model} and a \emph{progress-driven controller}. Both the new (black) and old (gray) models take as input object-oriented features $\rvx_{t-\tau_{in}:t}$ and predict $\hat{\rvx}_{t:t+\tau_{out}}$. The old model weights, $\theta_{old}$, are slowly updated to the new model weights $\theta_{new}$. The controller, $\pi_{\phi}$, is optimized to maximize $\gamma$-Progress reward, i.e $\LL(\theta_{old}) - \LL(\theta_{new})$.}
    % dotted lines 
    \label{fig:model}
    \vspace{-5pt}
\end{figure*}

\textbf{Related Works}: 
A natural class of world models involve forward dynamics prediction. Action-conditioned forward models can be used directly in planning for robotic control tasks~\citep{finn2017deep}, as performance-enhancers for reinforcement learning tasks~\citep{ke2019learning}, or as ``dream'' environment simulations for training policies~\citep{ha2018world}. A key question the agent is faced with is how to choose its actions to efficiently learn the world model. One approach is to pursue \emph{novelty}, e.g count-based and pseudo-count-based methods~\citep{strehl2008analysis,bellemare2016unifying, ostrovski2017count}, Random Network Distillation (RND)~\citep{burda2018exploration}, and \emph{empowerment} \citep{mohamed2015variational}. Another fundamental approach is to use \emph{adversarial} curiosity, which take actions estimated to maximize world model prediction error ~\citep{stadie2015predictive, pathak2017inverse, haber2018learning}. However, adversarial curiosity is especially prone to the \emph{white noise problem}, in which agents are motivated to waste time fruitlessly trying to solve unsolvable world model problems. \citep{schmidhuber_formaltheoryoffun} Estimating learning progress ~\citep{oudeyer2007intrinsic, oudeyer2013intrinsically, achiam2017surprise} or \emph{information gain}~\citep{houthooft_vime} avoids the white noise problem in a more comprehensive fashion. However, such methods have been limited in scope because they involve high computational costs. In this work, we present a novel method for estimating learning progress in a computationally scalable fashion.   



==> iclr_sections/scrap.tex <==
============intro.tex

Imagine yourself a parent at a playground. There is a plethora of stimuli, spanning wavering trees, leaves blowing in the wind, and children playing hide and seek. After briefly staring at the shaking trees and rustling leaves, you bore of watching their unpredictable motion and instead direct your attention to the game of hide and seek. Unlike with the random motion of trees and leaves, your understanding of the complex but predictable dynamics of hide-and-seek improves over time and you may eventually become capable of predicting a child's specific next move. This simple scenario suggests that humans continually engage in an intrinsically motivated process of furthering their understanding of the world and that directed attention may emerge naturally whilst seeking out maximally informative observations. In this work we aim to develop an intrinsically motivated active learning system that does the same: sample efficiently build models of the world by learning what to attend to.  

Concretely, world models are a family of predictive models that solve self-supervised prediction problems pertaining to the underlying the temporal structure of the world such as forward and inverse dynamics. Through learning world models, humans may acquire compact abstractions of high bandwidth sensory inputs, the ability to plan across long temporal horizons, and an understanding of the behavioral patterns of other agents. To deploy AI active learners in the real world, it is thus crucial that they can efficiently learn world models in complex environments. \kh{emphasize this process should happen without much external supervision}

To this end, there are mainly two algorithmic challenges: The first algorithmic challenge is that the active learner must arbitrate between the combinatorially large number of stimuli exhibiting inherently unlearnable or chaotic dynamics - e.g., falling leaves, wavering trees, and splashing water - and the few \ms{sparsity still hasn't been justified?} stimuli that have interesting and complex, yet learnable dynamics - e.g children playing hide-and-seek. We refer to the former class of stimuli as displaying \emph{noisy} behavior \ms{The thing about ``noisy'' is it has the connotation of ``having some noise'' which is true for stochastic animate agents.} and the latter as displaying \emph{animate} behavior. The term "animate" is drawn from the field of psychology \citep{premack1990infant, gergely1995taking, frankenhuis2013infants} in which "animate agents" denote a class of entities displaying behaviors with human-like kinematics such as self-propelled motion, goal-directed movements, and motion contigent on other agents. This challenge of identifying animate stimuli amid a sea of noisy ones has been acknowledged in many prior works as the "white noise" problem \citep{schmidhuber_formaltheoryoffun, pathak2017inverse, burda2018exploration, pathak2019disagreement}. The second algorithmic challenge is that the world model is susceptible to causal confusion - e.g the mistaking spurious correlations for true causality - which leads to poor generalization performance.

\kh{separate this challenge} Additionally, there is resource challenge that there is a shortage of simulated environments that faithfully preserve the core properties of real-world environments, while removing confounds that may artificially inflate modeling successes.

We address these three challenges with an intrinsically motivated "curious" active learning agent comprising two key components: (i) a \emph{Progress Curiosity-driven Controller} that learns to attend to stimuli with high expected learning progress thereby overcoming the white noise problem and (ii) a \emph{Causal World Model} that integrates a causal prior into its network architecture to preempt causal confusion. (see Fig. \ref{fig:model}) Our experiments are conducted in a custom-built 3D virtual world environment, rich with external agents displaying a wide spectrum of realistic animate behaviors such as peekaboo, chasing, and mimicry. \kh{should summarize key contributions into a couple sentences here}

In what follows, we begin by drawing connections between our work and related works in psychology and artificial intelligence (Section~\ref{sec:relatedworks}). In Section~\ref{sec:environment}, we describe our virtual environment in detail. Section~\ref{sec:theory} formalizes the active learning problem our curious agent is tasked with, motivates progress curiosity in the context of previously proposed curiosity signals, and characterizes the causal confusion problem. \kh{be a bit more detailed here} Section~\ref{sec:methods} details the implementations for all components of our curious active learning agent. Finally, Section~\ref{sec:experiments} presents experimental evaluations of our curious active learning system on two quantitative metrics: We show that (1) injecting causal prior is essential to attaining high offline asymptotic model performance, and (2) our progress-driven controller achieves significantly lower online sample complexity than baseline controllers equipped with state-of-the-art exploration strategies — including Random Network Distillation (RND) (Burda et al., 2018b) and Model Disagreement (Pathak et al., 2019) — which (perhaps surprisingly) fall prey to the white noise problem. \kh{this last sentence still needs to be rephrased} Furthermore, when varying both the intrinsic motivation signal (considering several baselines) and world model architecture (with causal structure prior, and without), we find that the intrinsic motivation signal drives behavior, whereas the difference in world model architecture modulates behavior to a lesser degree.


%In what follows, we begin by drawing connections between our work and related works in psychology and reinforcement learning (Section 1). In Section 2 \jdf{incomplete}. In Section 3, we describe our virtual environment in detail. Section 4 formalizes the core problems that motivate this project, including causal confusion and the shortcomings of curiosity signals that have been previously proposed to solve the white noise problem, while Section 5 presents the components of our active learning system. Finally, Section 6 presents experimental evaluations of our curious active learning system along three metrics: We show that (1) our causal prior is essential to attaining high offline asymptotic model performance, (2) our choice of a progress-driven controller is crucial to obtaining low online sampling complexity, while state-of-the art exploration methods — including Random Network Distillation (RND) (Burda et al., 2018b) and model disagreement (Pathak et al., 2019) — fall prey to the white noise problem, and (3) independent of world model choice, preferential attention towards animate agents emerges only with progress curiosity (but not other kinds of curiosity), suggesting that our model architecture may approximate the neural learning systems employed by humans. \jdf {I’ll circle back around to this to think about the specific human impliciations of ‘independent of a world model choice}.













% X_{ext, t:t+T_{out}}, \hat X_{ext, t:t+T_{out}}) = \sum_{s = t}^{T + T_{out}}\sum_{i = 1}^{N_ext} \alpha \rvx_{i, s} \|c_{i, s} - \hat c_{i, s} \|_2^2 + \beta \mathcal{L}_{ce}(\rvx_{i, s}, \hat \rvx_{i, s})

% As described in Section~\ref{sec:theory}, the world model seeks to solve the forward dynamics prediction problem of external agent behaviors in this encoding space. Specifically, given an encoded observation sequence $\rvx_{t - T_{in} : t}$ and curious agent actions $a_{t - T_{in} : t + T_{out} - 1}$, the world model predicts  $\rvx_{ext, t : t + T_{out}}$. % \ms{Loss function} 


% \ms{Causal prior} 
% In this work, we propose the \textit{Causal World Model}, a world model architecture that injects a causal graph of external agents (see Section~\ref{sec:theory}) as an architectural prior. Specifically, we impose this prior by instantiating, for each behavior $i$, a separate \textit{behavior network} $\mathcal{B}_i$ with independent weights $\theta_i$, such that one causal world model consists of $\{\mathcal{B}_i\}_{i \in \{1, ..., N_{behavior}\}}$

% Given behavior $i$, let $S_i$ be the set of all agents that belong to the behavior. 
% Given an encoded observation sequence $\rvx_{t - T_{in} : t}$, $\mathcal{B}_i$ takes as input only the part of $\rvx_{ext, t - T_{in} : t}$ corresponding to the agents that belong to the behavior, i.e., $(\rvx_{j, t - T_{in} : t} \cdot c_{j, t - T_{in} : t}, \rvx_{j, t - T_{in} : t})$ for all $j \in S_i$, along with $\rvx_{aux, t - T_in: t}$,  $\phi_{t - T_{in} : t }$, and $a_{t - T_{in} : t}$, and outputs predictions of only the part of $\rvx_{ext, t:t+T_{out}}$ that corresponds to the agents that belong to its behavior, i.e., $(\rvx_{j, t:t+T_{out}} \cdot c_{j, t:t+T_{out}}, \rvx_{j, t:t+T_{out}})$ for all $j \in S_i$. The outputs of all behavior networks  are concatenated to construct the overall prediction of $\rvx_{t:t+T_{out}}$, which is then the output of the causal world model.

% \ms{specific architecture 
% (LSTM, layers, units, optimizer, learning rate), excluding indicator coordinate split }

% To measure the gains of our causal world model, we introduce a \textit{non-causal ablation} that does not have this architectural prior. Concretely, the non-causal world model uses an architecture similar to that of a single behavior network in the causal world model, but with larger layers to have a similarly-sized parameter space. It takes as input $\rvx_{t-T_{in};t}$ and predicts $\rvx_{t:t+T_{out}}$ directly, modeling the dynamics of all external agent behaviors simultaneously. 






%\ms{Our self-supervision problem: forward dynamics prediction}
% First, we assume access to an oracle that maps observations $(O_t)$ to  an intermediate representation $(X_t)$ which contains information about the coordinates of each external agent in the room and indicators of whether an agent is in the curious agent's view.
%\ms{What are the inputs and outputs of the world model?}
%Specifically, given a sequence of past observations and past and present actions $(X_{t-n:t}, a_{t+k-1})$, the world model seeks to predict the next sequence of observations $(X_{t+1:t+k})$.


%\subsubsection{Split architecture}
%\ms{What are the solutions?}
%While in environments with only inanimate objects, the physical dynamics is shared between objects, a key property of our multi-agent environment is that different agents behave under widely varied dynamics. 
%In this work, we propose a split world model architecture, which consists of separate networks that each solve forward dynamics prediction of one external agent behavior, where a behavior may consist of one (e.g. peekaboo) or two interacting external agents (e.g. chasing). We argue that this behavior-wise splitting is equivalent to injecting the agent contingency graph as an architectural prior into the world model... 
%We perform ablations where a single neural network is used to model all external agents in the environment.

% Note that the particular dynamics prediction problem posed for a given external agent behavior does not always need to involve the prediction of all external agents involved in the behavior. In the case of mimicry, the input to the corresponding module contains information about both actor and imitator agents, but the prediction only needs to be done on the imitator. 



In this section we evaluate the active learning performance of our progress-driven curious agent. There are two differences from the supervised learning experiments in Section \ref{sec:offline}. First, instead of collecting data under random policy, the curious agent \emph{learns} to attend by optimizing a surrogate curiosity reward in order to minimize the number of environment interactions. Second, the virtual environment is set up with three noise behaviors and one animate behavior, varied amongst the seven animate behaviors listed in Section \ref{sec:environment}. This configuration directly challenges the curious agent to overcome the white-noise problem. We measure the sample complexity of the curious agent optimizing different curiosity signals while changing the animate behaviors and world model types. Specifically, we compare the five curiosity signals and a random policy baseline

\textbf{$\gamma$-Progress (Ours)} is our proposed variant of progress curiosity which chooses $\theta_{old}$ to be a geometric mixture of all past models as in Eq. \ref{eq:mix_progress}. 

\textbf{$\delta$-Progress \citep{achiam2017surprise, graves2017automated}} is the $\delta$-step learning progress reward from Eq. \ref{eq:kstep_progress} with $\delta = 1$. We found that any $\delta > 3$ is impractical due to memory limitations even with 12GB Titan X GPUs. 

\textbf{RND \citep{burda2018exploration}} is a state-of-the-art novelty-based exploration method shown to be effective in video game domains. In this approach, a predictor neural net is trained to match the outputs of a random state encoder. States for which the predictor networks fails to match the random encoder are deemed "novel", and thus receive high reward. 

\textbf{Disagreement \citep{pathak2019disagreement}} is the disagreement reward from Eq. \ref{eq:disagreement} with $N = 3$ ensemble models. We found that $N > 3$ is impractical due to memory constraints.  

\textbf{Adversarial \citep{stadie2015predictive, pathak2017inverse}} is the prediction error from Eq. \ref{eq:adversarial}. 

\textbf{Random} chooses actions uniformly at random among the 9 possible rotations. 


% Fig.~\ref{fig:attention} shows that, for both the causal and non-causal world models, strong animate attention emerges for $7/7$ behaviors $\gamma$-Progress and weak animate attention arises on $1/7$ behaviors for $\delta$-Progress. For RND, Disagreement, and Adversarial we observe the inverse: strong attention to the random agent emerges, i.e the white noise problem is apparent. \kh{We find that animate attention is strongly correlated with the AUC metric of sample complexity (provide number or figure reference), which supports our hypothesis that animate attention naturally emerges from an underlying process of optimizing for efficient world model learning}. 

% We also evaluate active learning performance using the acausal world model which has lower asymptotic model performance. Regardless we see that $\gamma$-Progress outperforms RND, Disagreement, and Adversarial baselines on all $7/7$ behaviors and outperforms $\delta$-Progress on $5/7$ behaviors while tying on the two peekaboo behaviors. While the world model's asymptotic performance is severely affected by architecture choice (causal v.s. acausal), the relative ranking in performance across intrinsic motivation signals is maintained across world model types. 


%%%%%%%%%%%%%%%%%%%%%% Attention Metric %%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
\subsection{Emergence of Animate Attention}

In this section, we analyze the interplay between choice of intrinsic motivation, world model architecture, validation performance, and the attention patterns that emerge within our environment. Fig.~\ref{fig:attention} shows that, for both the causal and acausal world models, strong animate attention emerges for $7/7$ behaviors $\gamma$-Progress and weak animate attention arises on $1/7$ behaviors for $\delta$-Progress. For RND, Disagreement, and Adversarial we observe the inverse: strong attention to the random agent emerges, i.e the white noise problem is apparent. In what follows, we analyze the factors varied in these models in order to quantify more precisely what drives the emergence of animate attention. We then characterize the extent to which the emergent attentional pattern predicts validation performance. This serves as a toy "developmental model" of how  {\em early attention} better predicts later performance than does {\em early performance}.
\end{comment}

%In this section, we evaluate the attention patterns that emerge from our intrinsically motivated active learning system. Fig.~\ref{fig:attention} shows that, for both the causal and non-causal world models, strong animate attention emerges for $7/7$ behaviors $\gamma$-Progress and weak animate attention arises on $1/7$ behaviors for $\delta$-Progress. For RND, Disagreement, and Adversarial we observe the inverse: strong attention to the random agent emerges, i.e the white noise problem is apparent. \kh{We find that animate attention is strongly correlated with the AUC metric of sample complexity (provide number or figure reference), which supports our hypothesis that animate attention naturally emerges from an underlying process of optimizing for efficient world model learning}. 

==> iclr_sections/theory.tex <==
% \section{Theory}
% \label{sec:theory}
% % In this section, we first formalize \textit{learning with intrinsic motivation} as an active learning problem. Under our formalization, a wide range of curiosity signals presented in prior works can be interpreted as approximations to the same objective. First, we elucidate the assumptions underlying different curiosity signals and assess why they may fail in the presence of white noise.  We then derive our proposed Progress curiosity signal and motivate its algorithmic and computational advantages over previously used progress measures. Next, we characterize the causal confusion problem in world model learning and show how it leads to catastrophic compounding errors. We then present our simple solution that involves injecting the causal graph prior into the world model architecture. % meg says: This paragraph starts with mentioning the active learning problem and curiosity signals, which makes it seem like the theory section is just focused on that, even though (with the current structure of the paper) causal confusion is also explained and it doesn't just fall under "active learning" 
% In this section, we formalize Active World Model Learning (AWML) as a Reinforcement Learning (RL) problem that generalizes conventional Active Learning (AL). We show how a wide range of previously proposed curiosity signals can be interpreted as proxies to a common intractable cost. Finally, we derive $\gamma$-Progress, a scalable progress-based curiosity signal with algorithmic and computational advantages over previous methods. 



\input{sections/universal_curiosity.tex}


==> iclr_sections/theory_dump.tex <==
Causal confusion is likely to occur when the training data distribution $p(\rvx)$ only covers a subset of the entire space $\X$, i.e $supp(p(\rvx))$ is small. The smaller the data coverage, the larger the space of degenerate solutions which do not respect the true causal structure of $P$.Causal confusion is likely to occur when the training data distribution $p_{train}(\rvx) \subset \X$ admits a different causal graph. 

Now consider a learned world model $P_{\theta}: \X \rightarrow \Y$.
\kh{formalize the disentanglement condition}
Any optimal world model should satisfy the following disentanglement condition for any causal graph $G_{P}$:
\begin{equation}
(P(\rvx))_{I_{\Y}} = (P_{\theta}(\rvx_{I_{\Y}^{-1}} \oplus \rvepsilon_{\setminus I_{\Y}^{-1}}))_{I_{\Y}} \quad \forall \rvepsilon \in \X, ~~\forall I_{y} \in A_{y}
\label{eq:causal_confusion}
\end{equation}

where $\rvx_{I_{\Y}^{-1}} \oplus \rvepsilon_{\setminus I_{\Y}^{-1}}$ denotes a concatenation of two vectors according to the indices $I_{\Y}^{-1}, \setminus I_{\Y}^{-1}$. In words, the subslices of model outputs $(P(\rvx))_{I_{\Y}}$ should only depend on the factors of variation that cause it, i.e $\rvx_{I_{\Y}^{-1}}$, and be unaffected by changes to nuisance factors of variation, i.e $\rvepsilon_{\setminus I_{\Y}^{-1}}$.

\begin{wrapfigure}{R}{0.45\textwidth}
\vspace{-10pt}
\begin{center}
    \includegraphics[width=.43\textwidth]{figures/causal_graph.pdf}
\end{center}
\vspace{-15pt}
\caption{\textbf{A causal graph.} Vertices represent external agents at times $t$ and $t+1$, edges represent causal relationships. Dashed boxes denote the connected component {\em external agent behaviors}.}
\label{fig:causal_graph}
\vspace{-10pt}
\end{wrapfigure}

%%%%%% What is causal confusion %%%%%%%
A learned model $P_{\theta}$ suffers from \emph{causal confusion} when it violates the disentanglement condition in Eq. \ref{eq:causal_confusion}, i.e changes in nuisance factors of variation $\rvepsilon_{\setminus I_{\Y^{-1}}}$ lead to changes in $P_{\theta}(\rvx)_{I_{\Y}}$. A causally confused model exhibits poor generalization performance when $p(\rvx) = p(\rvx_{I_{\Y}} | \rvx_{\setminus I_{\Y^{-1}}})p(\rvx_{\setminus I_{\Y^{-1}}})$ are distributed differently during training and validation time since off-distribution inputs can affect model outputs in unpredictable ways \citep{de2019causal}. 

As an intuitive example, consider an environment with two independent agents $A, B$ oscillating in sync with the same period. Let $\X = \Y$ comprise the joint position of the two agents and $I_{A}, I_{B}$ denote indices for each agent so that e.g $\rvx_{I_{A}}$ is the position coordinate of agent $A$. According to Def. \ref{def:causal_disentanglement}, the true world model $P: \X \rightarrow \X$ is causally disentangled since there exist partitions $\I_{\X} = \I_{\Y} = \{I_{A}, I_{B}\}$ and the identity bijective pairing $c(I) = I$ for which Eq. \ref{eq:causal_disentanglement} holds. The left graph in Fig. \ref{fig:causal_graph} shows the causal graph $G_{P}$ with two connected components, one for each periodic agent. \Inlike the true world model $P$, a causally confused learned model $P_{\theta}$ may predict the next position of agent $A$ from the current position of agent $B$ as shown in the right graph of Fig. \ref{fig:causal_graph}. $P_{\theta}$ may perform well on the training data so long the nuisance variables follow a fixed distribution




%%%%%% Why is causal confusion likely to occur? %%%%%%%
Now let us reason about why causal confusion is likely to occur when learning world models in real environments. 

% There's a distinction between an example of causal confusions and an example that illustrates why causal confusion is likely in real environments. The above example only shows the former. Is it indeed true that causal confusion is likely to occur? If so, why? 

% However, a causally confused model may have a causal graph with the dotted edge where the $\rvo_{I_{p1}}^{t+1}$ depends on the nuisance variable $\rvo_{I_{p2}}^{t}$. Since the periodic agents are in lockstep

Due to the partial observability of real-world environments (described in Section \ref{sec:environment}), our curious agent must have object permanence in order to make accurate predictions of when and where stimuli that disappear from view will reappear. This requires allocating dimensions of the world model input space $\X$ to tracking states of stimuli that are not in view. For example, $\rvx \in \X$ could include an object-centric representation with dimensions explicitly allocated for each object state or the hidden states of a recurrent neural network.


Object permanence can be encoded as an architectural prior by structuring the world model input space to be object-centric


There exists subdimensions of your input space that corresponds to "permanence" related representations. This could be explicit with an object-centric representation, or implicitly encoded in the hidden state representations learned by an LSTM.



There are several reasons for why we observe a distributional difference in the nuisance variables. First, due to model bootstrapping, the distribution of $\rvepsilon_{\setminus I_{\Y^{-1}}}$ changes with the number of timesteps having not seen the stimuli corresponding to $I_{\Y}$ which is affected by the curious agent's policy. Thus, policy changes during training and validation, i.e $D_{\text{KL}}(\rho_{\pi} || \mu)$, can lead to distributional mismatch of nuisance variables. Second, the nuisance variable distribution changes as a function of the world model. When interlacing validation and world model updates, it's most likely the training data doesn't contain many samples from the most recent version of the world model.
\kh{equipartition theorem. Put in footnote why bijective and not surjective}
\kh{Emphasize this problems arise especially in the interactive learning setting}
\kh{intuition for bipartite graph}

\kh{present simple example with two periodic agents}

\kh{Now explain our solution}











%%%%%%%%%%%%% New theory dump %%%%%%%%%%%%%%
\begin{definition}
\label{def:causal_disentanglement}
Let $\I_{\X} \in \emph{Part}(\{1, ..., \emph{dim}(\X)\}), \I_{\Y} \in \emph{Part}(\{1, ..., \emph{dim}(\Y)\})$ be maximally large partitions for which there exists a surjective map $c: \I_{\X} \rightarrow \I_{\Y}$ and sub-models $\{P^{I_{\X}}: \X_{I_{\X}} \rightarrow \Y_{c(I_{\X})} | I_{\X} \in \I_{\X}\}$ such that
\begin{equation}
P(\rvx)_{c(I_{\X})} = P^{I_{\X}}(\rvx_{I_{\X}}) \quad \forall I_{\X} \in \I_{\X},~~\forall \rvx \in \X
\label{eq:causal_disentanglement}
\end{equation}
where $\emph{Part}(S)$ is the universe of partitions a set $S$, $\rvx_{I_{\X}} := [x_{i}]_{i \in I_{\X}}$, and $\X_{I_{\X}} := \{\rvx_{I_{\X}} | \rvx \in \X\}$. Then, $G_{P} = (V, E)$ is a \textbf{causal graph} of $P$ where $V = \I_{\X} \cup \I_{\Y}, E = \{(I_{\X}, I_{\Y}) | I_{\X} \in \I_{\X}, I_{\Y} \in \I_{\Y}, I_{\Y} = c(I_{\X})\}$. 
\end{definition}

Let $P: \X \rightarrow \Y$ be a function and $\rvx \in \X, \rvy = P(\rvx)$ be random variables. $G_{P} = (V, E)$ of $P$ if 
\begin{enumerate}
\item $V = \{\rvx_{1}, ..., \rvx_{\emph{dim}(\X)}, \rvy_{1}, ..., \rvy_{\emph{dim}(\Y)}\}$
\item $(v_{\X}, v_{\Y}) \in E$ iff $\exists $
\end{enumerate}



and its occupancy measure is defined as $\rho_{\pi}(\rvx, \rvy) = \sum_{t = 0}^{\infty} \beta^{t} \Pr( | \pi)$ where $\beta$ is a discount factor $0 \leq \beta \leq 1$. A world model $\omega_{\theta}: \X \rightarrow \Omega(\Y)$ is stochastic function that encapsulates a property of the world. For example, $P$ is the forward dynamics kernel when $\X = \S \times \A$ and $\Y = \S$. In general, $\X, \Y \subseteq \S^{*} \times \A^{*}$ where $\S^{*}, \A^{*}$ are sets of all arbitrary length state, action sequences, i.e the Kleene closure of $\S, \A$. Further let $f: (\X \times \Y)^{*} \rightarrow \Theta$ be a learning algorithm for $\omega_{\theta}$. GAL aims to learn a policy $\pi$ to collect samples $(\rvx, \rvy)$ from the world which maximally reduce world model loss $\LL(\theta)$. 
\begin{equation}
\min_{\pi_{k+1}}{\mathop{\E}_{\substack{\rvx, \rvy \sim \\ \rho_{\pi_{k+1}}, P(\cdot | \rvx)}}[\LL(f(\cup_{i = 0}^{k} \mc{D}^{i} \cup \{(\rvx, \rvy)\})) - \LL(f(\cup_{i = 0}^{k} \mc{D}^{i}))] }
\label{eq:active_obj}
\end{equation}


\X \rightarrow \Omega(\Y)$, where $\Omega(\Y)$ is the set of probability measures on $\Y$, is a stochastic function that encapsulates a property of the world. For example, $P$ is the forward dynamics kernel when $\X = \S \times \A$ and $\Y = \S$. In general, $\X, \Y \subseteq \S^{*} \times \A^{*}$ where $\S^{*}, \A^{*}$ are sets of all arbitrary length state, action sequences, i.e the Kleene closure of $\S, \A$. The embodied agent agent interacts with the world according to a policy $\pi: \S \rightarrow \Omega(\A)$, in the process collecting samples $(\rvx, \rvy) \in \X \times \Y$ which are used to update its world model $P_{\theta}: \X \rightarrow \Omega(\Y)$ by minimizing a loss $\LL(\theta)$. Intuitively, $\pi$ distills the agent's strategy for querying useful data from the world, e.g directed attention towards animate external agents. For a policy $\pi$, we also define its occupancy measure $\rho_{\pi}: \S \times \A \rightarrow \RR$ as $\rho_{\pi}(s, a) = \sum_{t = 0}^{\infty} \beta^{t} \Pr(s_{t} = s, a_{t} = a | \pi)$ where $\beta$ is a discount factor $0 \leq \beta \leq 1$. Let $f: (\X \times \Y)^{*} \rightarrow \Theta$ be a learning algorithm. \kh{define input/output space explicitly} In traditional active learning, a single round of optimization comprises a data collection strategy update step (choosing which $\rvx$ to query a label for) and model update step. By analogy we can similarly formalize Learning with Intrinsic Motivation. In round $k + 1$, the data collection strategy update step solve the following policy optimization problem: \kh{end state distribution is the initial state distribution}:


\subsection{Active World Model Learning}
\label{sec:active_learning}
\kh{Add general definition with $z$ instead of specifying the forward problem. No access to querying prior distribution}


\kh{Define the generalization of active learning first.}



Informally, Active World Model Learning (AWML) is the process of learning how to efficiently collect information from the world to minimize world model loss. Concretely, we represent an embodied agent in a generic world (or "environment") as a tuple $(\S, \A, P)$ where $\S, \A$ are state, action spaces of the agent and $P: \X \rightarrow \Omega(\Y)$, where $\Omega(\Y)$ is the set of probability measures on $\Y$, is a stochastic function that encapsulates a property of the world. For example, $P$ is the forward dynamics kernel when $\X = \S \times \A$ and $\Y = \S$. In general, $\X, \Y \subseteq \S^{*} \times \A^{*}$ where $\S^{*}, \A^{*}$ are sets of all arbitrary length state, action sequences, i.e the Kleene closure of $\S, \A$. The embodied agent agent interacts with the world according to a policy $\pi: \S \rightarrow \Omega(\A)$, in the process collecting samples $(\rvx, \rvy) \in \X \times \Y$ which are used to update its world model $P_{\theta}: \X \rightarrow \Omega(\Y)$ by minimizing a loss $\LL(\theta)$. Intuitively, $\pi$ distills the agent's strategy for querying useful data from the world, e.g directed attention towards animate external agents. For a policy $\pi$, we also define its occupancy measure $\rho_{\pi}: \S \times \A \rightarrow \RR$ as $\rho_{\pi}(s, a) = \sum_{t = 0}^{\infty} \beta^{t} \Pr(s_{t} = s, a_{t} = a | \pi)$ where $\beta$ is a discount factor $0 \leq \beta \leq 1$. Let $f: (\X \times \Y)^{*} \rightarrow \Theta$ be a learning algorithm. \kh{define input/output space explicitly} In traditional active learning, a single round of optimization comprises a data collection strategy update step (choosing which $\rvx$ to query a label for) and model update step. By analogy we can similarly formalize Learning with Intrinsic Motivation. In round $k + 1$, the data collection strategy update step solve the following policy optimization problem: \kh{end state distribution is the initial state distribution}:


In this work we choose the forward dynamics problem as the world model problem. Specifically, we aim to learn a forward model $P_{\theta}: \X \rightarrow \Omega(\Y)$ over an input space $\X = \S \times \A$ of state-action pairs and a label space $\Y = \S$ of next states. Collectively, $(\rvx, \rvy)$ forms a transition. 


where $\mu(\rvx)$ is a prior distribution over the importance of correctly predicting the transition for $\rvx$. $\mu$ may also be interpreted as the validation data distribution. \kh{Is there something we can say about how active learning will bring $\rho_{\pi}$ closer to $\mu$?} For instance, if $\mu$ is the uniform distribution then an optimal world model must perfectly match the true environment dynamics for all $|\S|^{2}|A|$ possible transitions. Let $f: (\X \times \Y)^{*} \rightarrow \Theta$ be a learning algorithm. \kh{define input/output space explicitly} In traditional active learning, a single round of optimization comprises a data collection strategy update step (choosing which $\rvx$ to query a label for) and model update step. By analogy we can similarly formalize Learning with Intrinsic Motivation. In round $k + 1$, the data collection strategy update step solve the following policy optimization problem: \kh{end state distribution is the initial state distribution}:
\begin{equation}
\min_{\pi_{k+1}}{\mathop{\E}_{\substack{\rvx, \rvy \sim \\ \rho_{\pi_{k+1}}, P(\cdot | \rvx)}}[\LL(f(\cup_{i = 0}^{k} \mc{D}^{i} \cup \{(\rvx, \rvy)\})) - \LL(f(\cup_{i = 0}^{k} \mc{D}^{i}))] }
\label{eq:active_obj}
\end{equation}
where $\mc{D}_{i} = \{(\rvx, \rvy)_{j}\} \sim \pi_{i}$. In words, we seek a policy $\pi_{k + 1}$ which samples transitions that maximally reduce world model loss in expectation. At each iteration of the active learning loop, we perform two steps. First, optimize $\pi_{k}$ by solving Eq. \ref{eq:active_obj}. Second, update the world model parameters on the aggregate dataset $\cup_{i = 0}^{k} \mc{D}_{i}$. \Inlike the classic active learning with a pool setting, in which the data collection policy chooses $\rvx$ from a given pool of unlabeled data, we don't have access to a pool of unlabeled state-action pairs and label queries for $\rvx$ can only be made by learning a policy that can reach $\rvx$ in the environment. \kh{why can't you use a rollout of all possible trajectories as the unlabeled dataset }




\subsection{Connections between Curiosity Signals}
\label{sec:curiosity_signal}



\begin{comment}
We now formalize our the learning problem of our intrinsically motivated active learner as a batch active learning problem. At a high level, the curious agent seeks to minimize world model loss with as few interactions with the world as possible by adaptively collecting  batches of training samples. Concretely, our aim is to solve the forward dynamics world model problem defined over an input space $\X = \S \times \A$ and a label space $\Y = \S$, where $\S, \A$ are (countable) state, action spaces. Let

% While in the context of RL, world models have been leveraged to derive exploration bonuses that aid learning of a different task, our primary objective is to learn world models themselves.
Our intrinsically motivated agent engages in an active learning loop of collecting maximally informative data for the current world model, performing a world model update, and repeating the cycle. This problem corresponds to interlacing reinforcement learning over $\mc{M}(\theta_{i})$ and world model updates via supervised learning. Each MDP $\mc{M}_{i}$ seeks to learn an optimal data collection policy to maximize learning progress of the current world model. Let $\mc{M}(\theta) = (\S, \A, P, R_{\theta}, T)$ be a finite horizon MDP where $\S, \A$ are (countable) state, action spaces, $P: \S \times \A \rightarrow \mc{P}(\S)$ is the dynamics where $\mc{P}(\S)$ is the set of probability measures on $\S$, $R$ is the reward function, and $T$ is the episode length. A (stationary) policy $\pi: \S \rightarrow \mc{P}(\A)$ maps states to distributions over actions. Our objective is to learn a world model $P_{\theta}$ that matches $P$ with more emphasis on state, action pairs specified by a prior distribution $q(s, a)$.
\begin{equation}
J(\theta) = -\E_{(s, a) \sim q}[D_{KL}(P(\cdot | s, a) || P_{\theta}(\cdot | s, a))] \leq 0
\label{eq:model_performance}
\end{equation}
Intuitively, $q$ has concentrated probability mass on state-action pairs for which predicting the next state distribution correctly is more important. For example, the prior $q$ may capture the inherent inclination of humans to attend more to animate agent like features.
% where $u_{\S \times \A}$ is a uniform distribution over $\S \times \A$. A uniform distribution was chosen for simplicity, but it may be replaced with any distribution fully supported on $\S \times \A$.
Let $f: \Theta \times \mc{D} \rightarrow \Theta$ be the optimizer which updates our world model parameters $\theta$ given data $\mc{D} = \{(s, a, s')_{i}\}$ in the form of transition triplets.


\begin{equation}
\pi^*(\theta) = \argmax_{\pi} \E_{\mc{D} \sim \pi} [J(f(\theta, \mc{D})) - J(\theta)] \quad \text{where} \quad |\mc{D}| \leq K
\label{eq:pi_objective}
\end{equation}
In words, a policy behaves optimally with respect to the current world model $\theta$ and an optimizer $f$ if it samples a trajectories that maximally improve the performance of the model. $K$ captures the memory constraint of an active learning agent. We see that Eq. \ref{eq:pi_objective} cannot be directly optimzied since we cannot predict the value of $J(P_{\theta'})$ before performing an optimization step. Let us assume that the optimizer $f$ satisfies the following additive property:
\begin{align*}
J(f(\theta, \{(s, a, s')_{i}\})) - J(\theta) \approx \sum_{i} J(f(\theta, (s, a, s')_{i}) - J(\theta)
\end{align*}
Then, the policy performance objective can be written as:
\begin{align*}
    \argmax_{\pi} \E_{\mc{D} \sim \pi} [\sum_{(s, a) \in \mc{D}} J(f(\theta, (s, a, s'))) - J(\theta)] \quad \text{where} \quad |\mc{D}| \leq K
\end{align*}
Taking the policy gradient we obtain:
\begin{align*}
    \E_{\pi} [\nabla\log{\pi} \sum_{t} J(f(\theta, (s_{t}, a_{t}, s_{t+1}))) - J(\theta)] \quad \text{where} \quad |\mc{D}| \leq K
\end{align*}

The reward quantity of interest is the future progress on the objective that can be made by having the sample $(s_{t}, a_{t}, s_{t+1})$. However this quantity cannot be calculated without evaluating the our objective $J$ and taking an optimization step $f$. The former is intractable and the later is expensive. Instead we seek to make an approximation to $J(P_{\theta'}) - J(P_{\theta})$ based on information we have obtained about $f$ and $J$ in the past.

\subsubsection{adversarial}
uncertainty sampling
For example, we might assume that future progress is proportional to the current world model loss:
\begin{align*}
    J(\theta') - J(\theta) \approx -\beta J(\theta)
\end{align*}

\subsubsection{Progress}
Active learning sampling technique: estimated error reduction \\
We may instead make the assumption that future progress is proportional to our previous experience updating on the data:
\begin{align*}
    J(\theta'') - J(\theta') \approx -\beta (J(\theta') - J(\theta))
\end{align*}

\subsubsection{disagreement}
Active learning sampling technique: query by committee.
In practice we need a prior over the

Notice that we cannot directly perform RL with the objective in Eq. (2) since we do not have access to the ground truth world model $P$. Hence, we formulate a surrogate objective to (2) based on learning progress:

Note that this is equivalent to optimizing over an MDP with a non-stationary reward function. Your behavior not only changes the distribution of states you encounter, but also the reward function.
\end{comment}


==> iclr_sections/universal_curiosity.tex <==
\subsection{Generalization of Active Learning}

Consider an agent in an environment $\mc{E} = (\S, \A, P, P_{0})$ where $\S, \A$ are state, action spaces, and $P: \S \times \A \rightarrow \Omega(\S)$ is the transition dynamics, and $P_{0}$ is the initial state distribution. The agent's goal is to optimize a sequence of data collection decisions in order to learn a model $\omega_{\theta}$ of a target function $\omega: \X \rightarrow \Omega(\Y)$ with as few data samples as possible. We model this agent's decision making process as an infinite horizon Markov Decision Process (MDP) $\mc{M} = (\bar{\S}, \A, \bar{P}, \bar{P}_{0}, c)$. Specifically, $\bar{\rvs} \in \bar{\S} = \S \times \mc{H} \times \Theta$ is a meta-state that decomposes into $\bar{\rvs} = (\rvs, H, \theta)$ where $\rvs \in \S$ is an environment state, $H = \{\rvs_{0}, \rva_{0}, \rvs_{1}, \rva_{1} ...\} \in \mc{H}$ is the history of visited environment states and actions, and $\theta \in \Theta$ is the current model parameters. Intuitively $H$ is a unstructured form of the data collected so far which can be post-processed to yield a training set for $\omega_{\theta}$. $\rva \in \A$ is a data collection decision and the meta-dynamics $\bar{P}: \bar{\S} \times \A \rightarrow \Omega(\bar{\S})$ is defined as: 
\begin{align*}
(\rvs', H', \theta') \sim \bar{P}(\cdot | \bar{\rvs} = (\rvs, H, \theta), \rva) ~~ \text{where}~\rvs' \sim P(\rvs, \rva),~H' = H \cup \{\rva, \rvs'\},~\theta' \sim P_{\ell}(H', \theta) 
\end{align*}
where $P_{\ell}: H \times \Theta \rightarrow \Omega(\Theta)$ is a (stochastic) learning algorithm which updates the parameters on the history of data. In words, $\bar{P}$ steps the environment state $\rvs$ according to the environment dynamics $P$, appends the history with new data, and updates the model $\omega_{\theta}$ on the augmented history. The meta-initial state distribution is $\bar{P}_{0}(\bar{\rvs} = (\rvs, H, \theta)) = P_{0}(\rvs)\mathbbm{1}(H = \{\})q(\theta)$ where $\mathbbm{1}$ is the indicator function and $q(\theta)$ is a prior distribution over the model parameters. $c: \S^* \times \A^* \rightarrow \RR$ is the cost function which encodes the learning objective of the agent. For example, $c(\bar{\rvs} = (\rvs, H, \theta)) = \LL(\theta, \mu)$ encodes the goal of an agent seeking to minimize a loss function $\LL$ on data $(\rvx, \rvy) \sim \mu$ while training on a minimal number of data samples. A policy $\pi: \S \rightarrow \Omega(\A)$ maps states to action distributions and an optimal policy $\pi^* = \argmax_{\pi} J(\pi)$ achieves the highest performance $J(\pi) = -\E_{\pi}[\sum_{t = 0}^{\infty} \beta^{t} c(\bar{\rvs})]$ where $0 \leq \beta \leq 1$ is a discount factor. Overall, the MDP $\mc{M}$ is constructed from an environment $\mc{E} = (\S, \A, P, P_{0})$, a target function $\omega$, a learning algorithm $P_{\ell}$, and a prior parameter distribution $q(\theta)$. Several variants of conventional active learning can be recovered by appropriately defining the MDP $\mc{M}$ in relation to $\omega, \X, \Y$. 

\textbf{Query Synthesis Active Learning} is obtained by taking $\S = \Y, \A = \X, P(\cdot | \cdot, \rva=\rvx) = \omega(\rvx)$ and $c(\bar{\rvs} = (\rvs, H, \theta), \rva, \bar{\rvs}' = (\rvs', H', \theta')) = \LL_{val}(\theta) - \LL_{val}(\theta')$. In words, the agent proposes a synthetic data query $\rva$ and the oracle $P$ provides a label $\rvs'$. The agent's objective is to reduce validation loss with a minimal number of data queries. Most active learning methods take a greedy approach to maximize the model loss reduction after a single data query which corresponds to setting $\beta = 0$. 

\textbf{Pool-based Active Learning} is the same as Query Synthesis Active Learning with the only difference being $\A = \mc{D}_{pool}$ where $\mc{D}_{pool}$ is the initial pool of unlabelled data. 

\textbf{Stream Active Learning} is obtained by choosing $\S = \X \times \Y, \A = \{0, 1\}, P(\cdot | \rvs=(\rvx, \rvy), \rva) = \omega(\rvx)~\text{if}~\rva = 1~\text{else}~\delta(\rvy_{dum})$, and $c(\bar{\rvs} = (\rvs, H, \theta), \rva, \bar{\rvs}' = (\rvs', H', \theta')) = \LL_{val}(\theta) - \LL_{val}(\theta')$, where $\delta$ is the Dirac-delta function and $\rvy_{dum}$ is a dummy label that denotes the case when no label is returned by the oracle. 

\subsection{Active World Model Learning}

We now formalize the Active World Model Learning (AWML) problem using the RL framework presented in the previous section. Formally, AWML aims to find an optimal policy for the meta MDP $\mc{M}$ with the additional constraint that $\X, \Y \subseteq \S^{*} \times \A^{*}$ where $\S^{*}, \A^{*}$ are sets of all arbitrary length state, action sequences, i.e the Kleene closure of $\S, \A$. In words, the target function $\omega$ is a self supervised predictor on trajectories sampled from the environment. We henceforth refer to $\omega_{\theta}$ as the world model. Consider a simple AWML problem of learning the forward dynamics of the environment, i.e $\X = \S \times \A, \Y = \S, P = \omega$, and 
\begin{align}
c(\bar{\rvs} = (\rvs, H, \theta), \rva, \bar{\rvs}' = (\rvs', H', \theta')) = \LL(\theta', \mu) - \LL(\theta, \mu)
\label{eq:cost}
\end{align}
with a discount factor $\beta < 1$ to encourage minimal interactions with the environment. Recall that $\theta' = P_{\ell}(H \cup \{\rva, \rvs'\}, \theta)$ is the updated model parameters after collecting new data $\{\rva, \rvs'\}$. Thus the negative cost measures the reduction in world model loss as a result of obtaining new data $\{\rva, \rvs'\}$, i.e the \emph{prediction gain}. Unfortunately, evaluating prediction gain at every environment step involves repeatedly computing $L(\theta, \mu)$ which is typically intractable as sampling from $\mu$ often involves interacting with the environment. This bottleneck necessitates an efficiently computable proxy reward to estimate Eq. \ref{eq:cost}. Thus, solving the AWML problem entails solving two sub-problems: Proxy reward design and Reinforcement Learning (RL). A variety of curiosity signals proposed in prior work \citep{stadie2015predictive, burda2018exploration, pathak2019disagreement, achiam2017surprise} aim to solve the former problem.   
% with connections to known sampling methods for active learning. 
% Henceforth, we use the symbol $r_{1} \simeq r_{2}$ to denote reward equivalence, i.e the $r_{1}, r_{2}$ yield the same optimal policy. For example, $r_{1} \simeq r_{2}$ if $r_{2}$ is a monotonic transformation of $r_{1}$.



% At the $k^{th}$ iteration of the active learning loop, Eq. \ref{eq:active_obj} can be optimized by a Reinforcement Learning (RL) procedure with the reward function
% \begin{equation}
% -c(\bar{\rvs}, \rva, \bar{\rvs}') = \LL(\theta, \mu) - \LL(\theta', \mu) \quad \forall t
% \label{eq:cost}
% \end{equation}
% where $\theta' = f(\cup_{i = 0}^{k} \mc{D}^{i} \cup \{(s_{t}, a_{t}, s_{t+1})\})$ and $\theta = f(\cup_{i = 0}^{k} \mc{D}^{i})$. Our reward for transition $(s_{t}, a_{t}, s_{t + 1})$ measures the reduction in world model loss resulting from training on that sample. \Infortunately Eq. \ref{eq:cost} cannot be evaluated without knowing the ground truth dynamics $P$ and querying $\mu$, which necessitates a surrogate reward to estimate the \emph{expected} reduction in world model loss. We now show that curiosity signals used in prior work \citep{stadie2015predictive, burda2018exploration, pathak2019disagreement, achiam2017surprise} can be interpreted as approximations to Eq. \ref{eq:cost} with close connections to known sampling methods for active learning. Henceforth, we use the symbol $r_{1} \simeq r_{2}$ to denote reward equivalence, i.e the rewards $r_{1}, r_{2}$ yield the same optimal policy. For example, $r_{1} \simeq r_{2}$ if $r_{2}$ is a monotonic transformation of $r_{1}$.


%%%%%%%%%%%%%% Information Gain %%%%%%%%%%%%%%%%%%
\textbf{Information Gain} \citep{houthooft_vime, linke2019adapting} based methods seek to minimize uncertainty in the Bayesian posterior distribution over model parameters: 
\begin{equation}
-c(\bar{\rvs}, \rva, \bar{\rvs}') = \LL(\theta, \mu) - \LL(\theta', \mu) \simeq D_{\text{KL}}(p(\theta') || p(\theta))
\end{equation}
where $p(\theta') = p(\theta | H \cup \{\rva, \bar{\rvs}'\})$ and $p(\theta) = p(\theta | H)$. Note that, information gain is a lower bound to the prediction gain under weak assumptions \citep{bellemare2016unifying}. If the posterior has a simple form such as Laplace or Gaussian, information gain can be estimated by weight change $|\theta' - \theta|$ \citep{linke2019adapting}, and otherwise one may resort to learning a variational approximation $q$ to approximate the information gain with $D_{\text{KL}}(q(\theta') || q(\theta))$ \citep{houthooft_vime}. The former weight change methods require a model after every step in the environment and is thus impractical in many settings where world model updates are expensive, e.g backpropagation through deep neural nets. The latter family of variational methods require maintenance of a parameter distribution and an interlaced evidence lower bound optimization and are thus impractical to use with modern deep nets \citep{achiam2017surprise}. 

%%%%%%%%%%%%%% Adversarial %%%%%%%%%%%%%%%%%%
\textbf{Adversarial} \citep{stadie2015predictive, pathak2017inverse, schmidhuber2019minimax} curiosity assumes prediction gain is proportional to the current world model loss.
\begin{equation}
-c(\bar{\rvs}, \rva, \bar{\rvs}') = \LL(\theta, \mu) - \LL(\theta', \mu) \simeq -\log{\omega_{\theta}(\rvs' | \rvs, \rva)}
\label{eq:adversarial}
\end{equation}
This assumption holds when the target function $\omega$ is learnable by the model class $\Theta$ and the learning algorithm $P_{\ell}$ makes monotonic improvement without the need for curriculum learning. However, adversarial reward is perpetually high when the target is unlearnable by the model class, e.g deterministic model $\omega_{\theta}$ cannot match stochastic target function $\omega$ on inputs $\rvx$ for which $\omega(\rvx)$ is not a Dirac-delta distribution. This problem is widely known as the white noise problem \citep{schmidhuber_formaltheoryoffun}. 

% Substituting Eq. \ref{eq:adversarial} into Eq. \ref{eq:active_obj} with the approximation $P \approx P_{\theta}$ we obtain
% \begin{equation}
% \max_{\pi_{k+1}}{\E_{\rvx \sim \rho_{\pi_{k+1}}}[\E_{\rvy \sim P(\cdot | \rvx)}[\log{P_{\theta}(\rvy | \rvx)}]] } \approx \max_{\pi_{k+1}}{\E_{\rvx \sim \rho_{\pi_{k+1}}}[\H[P_{\theta}(\cdot | \rvx)]] }
% \end{equation}
% Where $\mc{H}$ is the entropy. Eq. \ref{eq:adversarial} equivalent to uncertainty sampling \citep{lewis1994heterogeneous} in active learning.

%%%%%%%%%%%%%% Disagreement %%%%%%%%%%%%%%%%%%
\textbf{Disagreement} \citep{pathak2019disagreement} assumes future world model loss reduction is proportional to the prediction variance of an ensemble of $N$ world models $\{P_{\theta_{j}}\}_{j = 1}^{N}$.
\begin{equation}
-c(\bar{\rvs}, \rva, \bar{\rvs}') = \LL(\theta, \mu) - \LL(\theta', \mu) \simeq \text{Var}(\{\omega_{\theta_{j}}(\rvs' | \rvs, \rva)\}_{j = 1}^{N})
\label{eq:disagreement}
\end{equation}
This approximation is reasonable when there exists a unique optimal world model. As we will show, for complex target functions all members of the ensemble do not converge to a single model and as a result the white noise problem persists. A key limitation of this method is that memory usage grow linearly with size of the model ensemble. Disagreement-based curiosity is known as query by committee sampling \citep{seung1992query} in active learning.

%%%%%%%%%%%%%% Novelty %%%%%%%%%%%%%%%%%%
\textbf{Novelty} \citep{bellemare2016unifying, dinh2016density, burda2018exploration} methods reward transitions with a low visitation count $\N(s, a, s')$. The prototypical novelty reward is: 
\begin{equation}
-c(\bar{\rvs}, \rva, \bar{\rvs}') = \LL(\theta, \mu) - \LL(\theta', \mu) \simeq \N(s_{t}, a_{t})^{-1/2}
\end{equation}
\cite{bellemare2016unifying} generalize visitation counts to pseudocounts for use in continuous state, action spaces. Novelty is a good surrogate reward when one seeks to maximize coverage over the transition space regardless of the learnability of the transition. This characteristic makes novelty reward prefer noisy data drawn from a high entropy distribution. Novelty reward is not adapted to the world model and thus has a propensity to be inefficient at reducing world model loss. 

%%%%%%%%%%%%%% Progress %%%%%%%%%%%%%%%%%%
\textbf{$\delta$-Progress} \citep{achiam2017surprise, graves2017automated} curiosity measures how much better the current new model $\theta_{new}$ is compared to an old model $\theta_{old}$.
\begin{equation}
-c(\bar{\rvs}, \rva, \bar{\rvs}') = \LL(\theta, \mu) - \LL(\theta', \mu) \simeq \log{\omega_{\theta_{new}}(\rvs' | \rvs, \rva)} - \log{\omega_{\theta_{old}}(\rvs' | \rvs, \rva)}
\label{eq:progress_curr}
\end{equation}
The choice of $\theta_{new}, \theta_{old}$ is crucial to the efficacy of the progress reward. A popular approach \citep{achiam2017constrained, graves2017automated} is to choose
\begin{equation}
\theta_{new} = \theta_{k}, \quad \theta_{old} = \theta_{k - \delta}, \quad \delta >0
\label{eq:kstep_progress}
\end{equation}
where $\theta_{k}$ is the model parameter after $k$ update steps using $P_{\ell}$. Intuitively, if the progress horizon $\delta$ is too large, we obtain an overly optimistic approximation of future progress. However if $\delta$ is too small, the agent may prematurely give up on learning hard transitions, e.g where the next state distribution is very sharp. In practice, tuning the value $\delta$ presents a major challenge. Furthermore, the widely pointed out \citep{pathak2019disagreement} limitation of $\delta$-Progress is that the memory usage grows $\O(\delta)$, i.e one must store $\delta$ world model parameters $\theta_{k - \delta}, ..., \theta$. As a result of these two limitation it is intractable in practice to use $\delta > 3$ with deep neural net models. 

\textbf{$\gamma$-Progress (Ours)} We propose the following choice of $\theta_{new}, \theta_{old}$ to overcome both hurdles:
\begin{equation}
\theta_{new} = \theta, \quad \theta_{old} = (1 - \gamma) \sum_{i = 1}^{k - 1} \gamma^{k - 1 - i} \theta_{0}
\label{eq:mix_progress}
\end{equation}
In words, the old model is a weighted mixture of past models where the weights are exponentially decayed into the past. $\gamma$-Progress can be interpreted as a noise averaged progress signal. Conveniently, $\gamma$-Progress can be implemented with a simple $\theta_{old}$ update rule:
\begin{equation}
    \theta_{old} \leftarrow \gamma \theta_{old} + (1 - \gamma) \theta_{new}
\label{eq:mix_update_rule}
\end{equation}
Similar to Eq. \ref{eq:kstep_progress}, we may control the level of optimism towards expected future loss reduction by controlling the progress horizon $\gamma$, i.e a higher $\gamma$ corresponds to a more optimistic approximation. $\gamma$-Progress has key practical advantages over $\delta$-Progress: $\gamma$ is far easier to tune than $\delta$, e.g we use a single value of $\gamma$ throughout all experiments, memory usage is constant with respect to $\gamma$, and as a result there is no limitation on choosing the value of $\gamma$. The significance of these practical advantages will become apparent from our experiments. 



==> icml_sections/abstract.tex <==
\begin{abstract}
World models are self-supervised predictive models of how the world evolves. Humans learn world models by curiously exploring their environment, in the process acquiring compact abstractions of high bandwidth sensory inputs, the ability to plan across long temporal horizons, and an understanding of the behavioral patterns of other agents. In this work, we study how to design such a curiosity-driven Active World Model Learning (AWML) system. To do so, we construct a curious agent building world models while visually exploring a 3D physical environment rich with distillations of representative real-world agents. We propose an AWML system driven by $\gamma$-Progress: a scalable and effective learning progress-based curiosity signal. We show that $\gamma$-Progress naturally gives rise to an exploration policy that directs attention to complex but learnable dynamics in a balanced manner, as a result overcoming the ``white noise problem''. As a result, our $\gamma$-Progress-driven controller achieves significantly higher AWML performance than baseline controllers equipped with state-of-the-art exploration strategies such as Random Network Distillation and Model Disagreement. 

\end{abstract}

==> icml_sections/asymptotic.tex <==
\subsection{Asymptotic Model Performance in Supervised Learning}
\label{sec:offline}

Here we evaluate the capacity for the world model to learn each of the animate external agent behaviors, isolating this measurement from any choice of policy. We gather 400k environment steps of data using a reduced action space random policy: for each action choice, the agent chooses randomly between 0- and 12-degree rotation in either direction. These data collection choices represent ``ideal'' data by ensuring plentiful exposure to each stimulus for long stretches of time. For this metric, we exclude the peekaboo animate external agent behavior, as due to the curious agent-contingent behavior of the peekaboo agent, one cannot expect ``ideal data'' to be gathered without a learned policy. We then train the world model to convergence and aggregate validation performance across five validation cases for each external agent behavior. 

We compare the performance of our causal world model to two acausal ablations: one {\em joined} that instead takes as input and predicts all external agents together, and one {\em split} that treats each agent separately, as opposed to behavior (so e.g. in the case of the chasing behavior, our causal world model takes as input both chaser and runner agent in order to predict the runner, whereas this predicts runner from runner alone). They employs the same architecture as a single behavior network in the causal world model (Section~\ref{sec:methods:worldmodel}), except with the number units for each hidden layer chosen so as to match roughly the total number of weights.

As seen in Figure~\ref{fig:offline_asymptotic_performance}, across all experiments, the causal world model significantly outperforms the ablation, with the acausal ablation obtaining $9.8\times$ the validation loss, on average across seeds and behaviors. Justifying the interpretation of ``ideal data'', for the causal world model, performance is comparable to the best achieved under online learning under the best policy found. Upon visual inspection of predictions, the causal world model appeared to ``get'' each animate external agent behavior, at least up to what the stochasticity of the external agent behaviors allow. To contrast, the acausal ablation exhibits not only poorer performance but considerable variance in performance, and visual inspection found that these models captured essential low order statistics across the first several timesteps of behavior, but that prediction rollouts quickly deteriorated. \nh{We should really add videos!} \ms{add agent-wise causal ablation}



==> icml_sections/causal_confusion.tex <==
\subsection{Causal Confusion in World Models}
\label{sec:causal_conf}

\begin{comment}
Paragraph outline
1. world model framework, introducing and justifying an object-centric representation
2. illustrate by example the causal confusion problem. What is the ground truth function for these coordinates.
3. effect of causal misidentification in the case of partial observability. show this formalization with symbols.
4. our solution. defines a causal graph, and describes the basic point of the solution. maybe a formula for the causal case and the acausal case.
\end{comment}

In this section, we first formalize the disentanglement problem, reason about its propensity to occur in the interactive learning setting, and motivate our causal world model architecture. Consider the (deterministic) dynamics function $P: \X \rightarrow \Y$. We consider deterministic dynamics for compactness of notation in what follows, but the presented analyses may be extended to stochastic dynamics. Henceforth we use the vector slicing notations $\rvx_{I} := [\rvx_{i}]_{i \in I}$, and $\X_{I} := \{\rvx_{I} | \rvx \in \X\}$. We start by defining a causal graph.

\begin{definition}
\label{def:disentanglement_graph}
Let $P : \X = \sR^n \rightarrow \Y = \sR^m$. For each $j \in \{1 \ldots m\}$, let its preimage $j_P^{-1} \subseteq \{1 \ldots n\}$ satisfy the following:
\begin{enumerate}
    \item (modularity) There exists $\tilde P$ such that $P(x) = \tilde P(x_{j_P^{-1}})$, where $x_{j_P^{-1}}$ is the projection of $x \in \sR^n$ onto dimensions $j_P^{-1}$, and
    \item (minimality) There does not exist $I$ strictly contained in $j_P^{-1}$ such that property (1) holds for $I$.
\end{enumerate}
Then the {\em disentanglement graph} is $G_{P} = (V, E)$ where $V$ has one vertex $i_X$ for $i \in \{1 \ldots n\}$ and one vertex $j_Y$ for $j \in \{1 \ldots m\}$, and $E = \{(i_X, j_Y) \ | \ i_X \in j_P^{-1}, j \in \{1 \ldots m\} \}$.
\end{definition}

Implicit in this definition is the fact that $j_P^{-1}$ exists and is unique, and hence there is exactly one disentanglement graph for a given function. Note that this definition heavily depends on a specification of a coordinate system for both the domain and range of the function. We are now ready to formalize a failure mode of models supervised on $P$.

\begin{definition}
\label{def:causal_confusion}
A model $P_{\theta}: \X \rightarrow \Y$ is not disentangled w.r.t $P: \X \rightarrow \Y$ if the identity map on vertices does not induce an embedding of $G_{P_\theta}$ into $G_P$.
\end{definition}

\noindent{\textbf{Observation}}
\textit{
Let $P_{\theta}: \X \rightarrow \Y$ be not disentangled w.r.t $P$. Then there exists $j_Y$ and $x, x' \in X$ with $x_i = x'_i$ for all $i \in j_P^{-1}$ and
\begin{equation*}
    P(x) = P(x')
\end{equation*}
but
\begin{equation*}
    P_\theta(x) \neq P_\theta(x').
\end{equation*}
}

In words, $P_{\theta}$ is non-robust to perturbations of the inputs along the nuisance dimensions $\setminus I_{\Y}^{-1}$. Hence, a causally confused model that has overfit to spurious statistical dependencies $p_{\text{train}}(\rvy_{I_{\Y}} | \rvx_{\setminus I_{\Y}^{-1}})$ in the training set will have poor generalization performance on a validation set when $d(p_{\text{val}}(\rvy_{I_{\Y}} | \rvx_{\setminus I_{\Y}^{-1}}),  p_{\text{train}}(\rvy_{I_{\Y}} | \rvx_{\setminus I_{\Y}^{-1}})) \neq 0$ where $d$ is some distance metric between distributions.\footnote{Note than in the limit of infinite training data with full coverage over $\X$, a model will not be causally confused since the proper disentanglement can be learned by just memorizing the training data}

%% So why does the conditional distribution change? 
%% Need to also explain that true models are likely causally disentangled 
Causal confusion is more likely to occur and more detrimental to generalization performance when learning world models of partially observable environments by interactive learning. To see this, consider a world model $P_{\theta}$ of a partially observable environment with dynamics $P: \X \rightarrow \Y$ that have a non-trivial causal graph. Due to partial observability, the world model must solve two types of predictions problems: supervised prediction and permanence prediction. Supervised prediction involves predicting the dynamics of stimuli that are currently observable and permanence prediction involves predicting the dynamics of non-observable stimuli. For the world model to solve both prediction tasks, the inputs $\rvx \in \X$ should encode both current observations - e.g images, coordinates of stimuli that are in view - when available and permanence information - e.g mental estimates of how the non-visible stimuli are moving. \footnote{Any memory efficient model should minimize the number of observations, which are typically high-bandwith, and maintain a compact encoding of permanence information instead of taking as input an arbitrary sequence of high-bandwith observations} 

Thus, the nuisance factors $\rvx_{\setminus I_{\Y}^{-1}}$ for any output $\rvy_{I_{\Y}}$ must encode permanence information impertinent to predicting $\rvy_{I_{\Y}}$. For example, $\rvx_{I_{\Y}^{-1}}$ could correspond to the position inputs of the currently visible external agent while $\rvx_{\setminus I_{\Y}^{-1}}$ could correspond to a mental estimate of where the non-visible external agents are or a counter that tracks the number timesteps since the last encounter with them. Such permanence information can be explicitly identified when the world model has a structured input ($\X$), output ($\Y$) space that allocates separate space for permanence information and implicitly identified in the hidden states of memory augmented function approximators such as Long Short-Term Memory (LSTM) networks. 

There may exist a drastic distributional shift of the permanence variables between training and validation, i.e $d(p_{\text{val}}(\rvy_{c(I_{\X})} | \rvx_{\setminus I_{\X}}),  p_{\text{train}}(\rvy_{c(I_{\X})} | \rvx_{\setminus I_{\X}})) \gg 0$, due to two factors. First, changes in the data collection policy with interactive learning leads to changes in the visitation frequencies for each stimuli which changes the distribution of permanence variables such as the visitation counters. In the interactive learning setting there indeed may be policy differences between training and validation time and we desire the world model to be robust to changes in policy. 

Second, updates to the world model parameters can change the permanence variable distribution. In the interactive learning setting we interlace data collection and world model update, and will indeed experience constant changes to the world model parameters. Furthermore, permanence predictions, such as predicting the position of an external agent after a long look-away, are typically significantly harder than supervised predictions and thus the permanence representations will take much longer to stabilize in distribution due to large gradients.  

% \begin{wrapfigure}{R}{0.45\textwidth}
% \vspace{-10pt}
% \begin{center}
%     \includegraphics[width=.43\textwidth]{figures/causal_graph.pdf}
% \end{center}
% \vspace{-15pt}
% \caption{\textbf{A causal graph.} Vertices represent external agents at times $t$ and $t+1$, edges represent causal relationships. Dashed boxes denote the connected component {\em external agent behaviors}.}
% \label{fig:causal_graph}
% \vspace{-10pt}
% \end{wrapfigure}

To ameliorate this, we propose to inject a causal prior into the world model, specified by a causal graph $G_{P}$. The causal graph has one vertex $v_{i, t}$ for each external agent $i$ for each timestep $t$, and a (directed) edge from $v_{i, t}$ to $v_{j, t'}$ if the position of external agent $j$ at timestep $t'$ depends on the position of external agent $i$ at timestep $t$. The causal graph thus represents which external agents a given external agent's future trajectory depends on. We identify each connected component of this graph, restricted to the input and output timesteps in question, with an {\em external agent behavior}. For example, the object interaction agent consists of its own behavior, whereas the chaser and runner agents together make a behavior. As noted in Section~\ref{sec:environment} these connected components do not vary across time in our environment. Our causal world model allocates a separate neural network for each external agent behavior, i.e each network has access to only the causally-appropriate inputs, thereby reducing causal confusion across agent behaviors. We assume access to the appropriate causal graph for each instantiation of behaviors. See Section~\ref{sec:methods} for details.






==> icml_sections/causal_confusion_scrap.tex <==
\subsection{Causal Confusion in World Models}
\label{sec:causal_conf}

\begin{comment}
Paragraph outline
1. world model framework, introducing and justifying an object-centric representation
2. illustrate by example the causal confusion problem. What is the ground truth function for these coordinates.
3. effect of causal misidentification in the case of partial observability. show this formalization with symbols.
4. our solution. defines a causal graph, and describes the basic point of the solution. maybe a formula for the causal case and the acausal case.
\end{comment}

In this section, we first formalize the causal confusion problem, reason about its propensity to occur in the interactive learning setting, and motivate our causal world model architecture. Consider the (deterministic) dynamics function $P: \X \rightarrow \Y$. \kh{include thing about encoding space} We consider deterministic dynamics for compactness of notation in what follows, but the presented analyses may be extended to stochastic dynamics. Henceforth we use the vector slicing notations $\rvx_{I} := [\rvx_{i}]_{i \in I}$, and $\X_{I} := \{\rvx_{I} | \rvx \in \X\}$. We start by defining a causal graph. 

\begin{definition}
\label{def:causal_disentanglement}
Let $P: \X \rightarrow \Y$ be a function. For each $I_{\Y} = 1, ..., \emph{dim}(\Y)$, let its preimage $I_{\Y}^{-1} = \{I_{\X} | I_{\X} \subseteq \{1, ..., \emph{dim}(\X)\}\}$ be a set satisfying the following: 
\vspace{-5pt}
\begin{enumerate}
    \item (modularity) $\forall I_{\X} \in I_{\Y}^{-1}, \exists \tilde{P}: \X_{I_{\X}} \rightarrow \Y_{I_{\Y}}$ such that $P(\rvx)_{I_{\Y}} = \tilde{P}(\rvx_{I_{\X}})~\forall \rvx \in \X$
    \vspace{-5pt}
    \item (minimality) $\forall I_{\X} \in I_{\Y}^{-1}, \nexists i \in I_{\X}$ such that property $1$ holds for $I_{\X} \setminus \{i\}$
\end{enumerate}
\vspace{-5pt}
Then, a \textbf{causal graph} is $G_{P} = (V, E)$ where $V = \{\rvx_{1}, ..., \rvx_{\emph{dim}(\X)}, \rvy_{1}, ..., \rvy_{\emph{dim}(\Y)}\}$ is a set of vertices and $E = \{(\rvx_{i}, \rvy_{I_{\Y})}| i \in I_{\X}, I_{\Y} = 1, ..., \emph{dim}(\Y)\}$ are the directed edges for any $I_{\X} \in I_{\Y}^{-1}$. 

Restatement (see comment): We define a \textbf{causal graph} to be a 
\end{definition}

\nh{I like this definition better, but I think a few things need to be changed:
(1) $I_X$ and $I_Y$ should look more different. One is an integer and the other is a set of integers, whereas the notation suggests that they're analogous for $X$ and $Y$.
(2) Definitions of $V$ and $E$ should not have $x$ and $y$s in them, because then it seems like there are different vertices for the same indices but different points for each $(x, P(x))$ as we vary $x$. Let me try to establish notation in the below lemma, see if you like it.
(3) (And maybe I am misunderstanding the definition, but...) it needs to be clear that for a given causal graph, one makes a unique choice of $I_X \in I_Y$
}

Notice that every dynamics $P$ has a causal graph, since the fully connected bipartite graph from vertices for $\rvx$ to vertices for $\rvy$ can make up a trivial causal graph. However, the causal graph need not be unique (see Appendix \ref{sec:app:causal}). We henceforth use $\Gamma_{P}$ to refer to the family of causal graphs of $P$. We are now ready to formalize causal confusion. 

\begin{definition}
\label{def:causal_confusion}
A world model $P_{\theta}: \X \rightarrow \Y$ is causally confused w.r.t $P: \X \rightarrow \Y$ if $\Gamma_{P_{\theta}} \nsubseteq \Gamma_{P}$ 
\end{definition}

%% Why is causal confusion harmful for prediction?
In words, causal confusion is the failure of a world model to embody the correct disentanglement structure present in the target dynamics. This phenomenon can also be understood as overfitting to spurious correlations in the training data. Thus, causally confused models have poor generalization performance: 

\begin{comment}
Old version:
\begin{corollary}
Let $P_{\theta}: \X \rightarrow \Y$ be causally confused w.r.t $P$. Then for all $\I_{\X}, \I_{\Y}, c$ comprising a causal graph of $P$, there exists an input $\rvx \in \X$, a perturbed input $\rvx + \rvepsilon \in \X$, and $I_{\Y} \in \I_{\Y}$ such that,
\begin{equation*}
P(\rvx)_{I_{\Y}} = P(\rvx + \rvepsilon)_{I_{\Y}} = P_{\theta}(\rvx)_{I_{\Y}} \neq P_{\theta}(\rvx + \rvepsilon)_{I_{\Y}}
\end{equation*}
where $\rvepsilon_{I_{\Y}^{-1}} = \textbf{\emph{0}}^{|I_{\Y}^{-1}|}, \rvepsilon_{\setminus I_{\Y}^{-1}} \neq \textbf{\emph{0}}^{|\setminus I_{\Y}^{-1}|}$ for $I_{\Y}^{-1} = \bigcup_{\{I_{\X} | c(I_{\X}) = I_{\Y}\}} I_{\X}$ and $\textbf{\emph{0}}^{L}$ is an $L$-dim zero vector.
\end{corollary} 
\end{comment}

\nh{I made this a lemma, not a corollary, as stylistically you aren't supposed to have corollaries of definitions, but of other results. I'm not even really sure whether to call this a lemma, as it's basically a restatement of the definition, as is. (Maybe some previous version was more nontrivial? Could be that I just dumbed it down...) Usually in a case like this, I would say something like ``Observation''.}

\begin{lemma}
Let $P_{\theta}: \X \rightarrow \Y$ be causally confused w.r.t $P$. Then for all $G \in \Gamma_P$ such that $G \notin \Gamma_{P_\theta}$, there exists $I_X, I_Y$ with $\{(i, I_Y) \ | \ i \in I_X\} \subseteq G$ and $x, x' \in X$ with $x_i = x'_i$ for all $i \in I_X$ and
\begin{equation*}
    P(x) = P(x')
\end{equation*}
but
\begin{equation*}
    P_\theta(x) \neq P_\theta(x').
\end{equation*}
\end{lemma}


In words, a causally confused model's prediction $P_{\theta}(\rvx)_{I_{\Y}}$ is non-robust to perturbations of the inputs along the nuisance dimensions $\setminus I_{\Y}^{-1}$. Hence, a causally confused model that has overfit to spurious statistical dependencies $p_{\text{train}}(\rvy_{I_{\Y}} | \rvx_{\setminus I_{\Y}^{-1}})$ in the training set will have poor generalization performance on a validation set when $d(p_{\text{val}}(\rvy_{I_{\Y}} | \rvx_{\setminus I_{\Y}^{-1}}),  p_{\text{train}}(\rvy_{I_{\Y}} | \rvx_{\setminus I_{\Y}^{-1}})) \neq 0$ where $d$ is some distance metric between distributions.\footnote{Note than in the limit of infinite training data with full coverage over $\X$, a model will not be causally confused since the proper disentanglement can be learned by just memorizing the training data}

%% So why does the conditional distribution change? 
%% Need to also explain that true models are likely causally disentangled 
Causal confusion is more likely to occur and more detrimental to generalization performance when learning world models of partially observable environments by interactive learning. To see this, consider a world model $P_{\theta}$ of a partially observable environment with dynamics $P: \X \rightarrow \Y$ that have a non-trivial causal graph. Due to partial observability, the world model must solve two types of predictions problems: supervised prediction and permanence prediction. Supervised prediction involves predicting the dynamics of stimuli that are currently observable and permanence prediction involves predicting the dynamics of non-observable stimuli. For the world model to solve both prediction tasks, the inputs $\rvx \in \X$ should encode both current observations - e.g images, coordinates of stimuli that are in view - when available and permanence information - e.g mental estimates of how the non-visible stimuli are moving. \footnote{Any memory efficient model should minimize the number of observations, which are typically high-bandwith, and maintain a compact encoding of permanence information instead of taking as input an arbitrary sequence of high-bandwith observations} 

Thus, the nuisance factors $\rvx_{\setminus I_{\Y}^{-1}}$ for any output $\rvy_{I_{\Y}}$ must encode permanence information impertinent to predicting $\rvy_{I_{\Y}}$. For example, $\rvx_{I_{\Y}^{-1}}$ could correspond to the position inputs of the currently visible external agent while $\rvx_{\setminus I_{\Y}^{-1}}$ could correspond to a mental estimate of where the non-visible external agents are or a counter that tracks the number timesteps since the last encounter with them. Such permanence information can be explicitly identified when the world model has a structured input ($\X$), output ($\Y$) space that allocates separate space for permanence information and implicitly identified in the hidden states of memory augmented function approximators such as Long Short-Term Memory (LSTM) networks. 

There may exist a drastic distributional shift of the permanence variables between training and validation, i.e $d(p_{\text{val}}(\rvy_{c(I_{\X})} | \rvx_{\setminus I_{\X}}),  p_{\text{train}}(\rvy_{c(I_{\X})} | \rvx_{\setminus I_{\X}})) \gg 0$, due to two factors. First, changes in the data collection policy with interactive learning leads to changes in the visitation frequencies for each stimuli which changes the distribution of permanence variables such as the visitation counters. In the interactive learning setting there indeed may be policy differences between training and validation time and we desire the world model to be robust to changes in policy. 

Second, updates to the world model parameters can change the permanence variable distribution. In the interactive learning setting we interlace data collection and world model update, and will indeed experience constant changes to the world model parameters. Furthermore, permanence predictions, such as predicting the position of an external agent after a long look-away, are typically significantly harder than supervised predictions and thus the permanence representations will take much longer to stabilize in distribution due to large gradients.  

\begin{wrapfigure}{R}{0.45\textwidth}
\vspace{-10pt}
\begin{center}
    \includegraphics[width=.43\textwidth]{figures/causal_graph.pdf}
\end{center}
\vspace{-15pt}
\caption{\textbf{A causal graph.} Vertices represent external agents at times $t$ and $t+1$, edges represent causal relationships. Dashed boxes denote the connected component {\em external agent behaviors}.}
\label{fig:causal_graph}
\vspace{-10pt}
\end{wrapfigure}

To gain intuition about causal confusion in interactive learning, consider an environment with two independent external agents $A, B$ oscillating in sync with the same period. Let $\X = \Y$ $I_{A}, I_{B}$ denote indices for each agent so that e.g $\rvx_{I_{A}}$ is the position coordinate of agent $A$ when it is visible and a bootstrapped model estimate of agent $A$'s position when it is not visible. According to Def. \ref{def:causal_disentanglement}, the true dynamics $P: \X \rightarrow \X$ have a causal graph $G_{P}$ defined by $\I_{\X} = \I_{\Y} = \{I_{A}, I_{B}\}$ and the identity bijective pairing $c(I) = I$. The left graph in Fig. \ref{fig:causal_graph} visualizes $G_{P}$ with two connected components, one for each periodic agent. The right graph of Fig. \ref{fig:causal_graph} shows an example world model $P_{\theta}$ that is causally confused. $P_{\theta}$ predicts the next position of agent $A$ from the current position of agent $B$. Such a model could've been learned on a training set collected with a policy that rapidly shifts between agent $A, B$. Frequent shifts allow the model estimated position to remain accurate since the number of bootstrapping steps are small, and thus the model is able to achieve low training error since the agents are oscillating in sync. However the validation set may test for robustness of the world model with data collected by a less frequently switching policy. In this case, the bootstrapped model estimates for agent $B$ may shift in distribution and degrade the predictions for agent $A$ even when agent $A$ is in view. 

To ameliorate this, we propose to inject a causal prior into the world model, specified by a causal graph $G_{P}$. The causal graph has one vertex $v_{i, t}$ for each external agent $i$ for each timestep $t$, and a (directed) edge from $v_{i, t}$ to $v_{j, t'}$ if the position of external agent $j$ at timestep $t'$ depends on the position of external agent $i$ at timestep $t$. The causal graph thus represents which external agents a given external agent's future trajectory depends on. We identify each connected component of this graph, restricted to the input and output timesteps in question, with an {\em external agent behavior}. For example, the object interaction agent consists of its own behavior, whereas the chaser and runner agents together make a behavior. As noted in Section~\ref{sec:environment} these connected components do not vary across time in our environment. Our causal world model allocates a separate neural network for each external agent behavior, i.e each network has access to only the causally-appropriate inputs, thereby reducing causal confusion across agent behaviors. We assume access to the appropriate causal graph for each instantiation of behaviors. See Section~\ref{sec:methods} for details.





%TODOS: (1). Augment reason 1, reason 2 (2). Figure out where to put in periodic example (3). Rewrite the solution paragraph (4). Revise the figure 


% corrollary explaining that causal confusion makes the supervised world model prediction $P(\rvx)_{c(I_{\X})}$ non-robust to drastic changes in $p(\rvx_{I_{\X}} | \rvx_{\setminus I_{\X}})$. It's true that there are two additional sources of degradation in performance. (1). Causal confusion across time within $I_{\X}$ and unsupervised prediction. We don't argue that the agent causal confusion is "theoretically" a bigger issue, but show that getting rid of it leads to really big prediction gains. Supervised world model prediction here, since if you're doing unsupervised prediction, then even $p(\rvx_{I_{\X}})$. I think we should limit the scope to supervised prediction? 

%% Our solution is to eliminate causal confusion among the agent-dimensions. But note that there can still be other sources of causal confusion present after this removal. Namely confusion across time and confusion during unsupervised prediction. However, this still alleviates the problem to a large degree as we observed empirically 


%% TODOS: we should really show object permanence through experiments. That we can make good predicitons of agent behaviors when not looking at them.



%% Why is causal confusion likely to occur 
%% (1). Lack of data that fully covers the space 
%% 

%% Why is validation distribution likely different from training 
%% => we want to test for generalization. Which means the world model should be robust to changes in interaction policy, 
%% => In some sense we're asking the world model to succeed at out of distribution generalization. 
%% 

%% (1). Policy is different 
%% (2). World model performance is different and only little training data was acquired with the most recent world model  



% \begin{wrapfigure}{R}{0.35\textwidth}
% \vskip -0.2in
% \begin{center}
%     \includegraphics[width=.33\textwidth]{figures/causal_graph.pdf}
% \end{center}
% \vspace{-0.7cm}
% \caption{\textbf{A causal graph.} Vertices represent external agents at times $t$ and $t+1$, edges represent causal relationships. Dashed boxes denote the connected component {\em external agent behaviors}.}
% \label{fig:causal_graph}
% \vskip -0.1in
% \end{wrapfigure}


==> icml_sections/diagnostic.tex <==
\section{Further attention analyses}
\label{app:further_attention_analysis}

Here we provide details of the early indicator analysis (Section~\ref{sec:future}) and a regression of what factors (curiosity signal, architecture, external agent behavior) best predict animate/inanimate attention ratios.

\subsection{Details of early indicator analysis}
\label{sec:app:attention_diagnostic}

We look to predict final performance $P_{\mathrm{final}}$ of a given agent, which we take to be the average of the final four validation runs. To make the modeling problem simple, we discretize this into a classification task by dividing validation performance into 3 equal-sized classes (``high'', ``medium'', and ``low'', computed separately for each external agent behavior), intuitively chosen to reflect performance around, at, and below that of random policy.

We consider two predictive models of final performance, one that takes as input early attention of the agent, and the other, early performance. Early performance may be quantified simply: given time $T$ (``diagnostic age'') during training, let $P_{\leq T}$ be the vector containing all validation losses measured up to time $T$. Early attention, however, is very high-dimensional, so we must make a dimensionality-reducing choice in order to tractably model with our modest sample size. Hence, we ``bucket'' average. Given choice of integer $B$, let
\begin{equation}
    A_{\leq T, B} = (\mathit{f}^{\mathrm{anim}}_{0 : \frac{T}{B}}, \mathit{f}^{\mathrm{rand}}_{ 0 :  \frac{T}{B}}, \mathit{f}^{\mathrm{anim}}_{\frac{T}{B}: \frac{2T}{B}}, \mathit{f}^{\mathrm{rand}}_{\frac{T}{B} : \frac{2T}{B}}, \ldots \mathit{f}^{\mathrm{anim}}_{\frac{(B - 1)T}{B} : T}, \mathit{f}^{\mathrm{rand}}_{\frac{(B - 1)T}{B} : T}),
\end{equation}
where $\mathit{f}^{\mathrm{anim}}_{a : b}$ and $\mathit{f}^{\mathrm{rand}}_{a : b}$ are the fraction of the time $t = a$ and $t = b$ spent looking at the animate external agent and random external agents respectively (so $A_{\leq T, B}$ is the attentional trajectory up to time $T$ discretized into $B$ buckets).

Finally, both models must have knowledge of the external agent behavior to which the agent is exposed --- we expect this to both have an effect on attention as well as the meaning of early performance and expected final performance as a result. Let $\chi_{\mathrm{BHR}}$ be the one-hot encoding of which external animate agent behavior is shown. 

We then consider models
\begin{enumerate}
    \item PERF$_{\leq T}$, which takes as input $P_{\leq T}$ and $\chi_{\mathrm{BHR}}$, and
    \item ATT$_{\leq T}$, which takes as input $A_{\leq T, B}$ and $\chi_{\mathrm{BHR}}$.
\end{enumerate}

Figure~\ref{fig:human_modeling_combined}b shows the plot of PERF$_{\leq T}$ and ATT$_{\leq T}$ accuracy as $T$ varies. We see that, up to a point, ATT$_{\leq T}$ makes a better predictor of final performance, and then PERF$_{\leq T}$ dominates. This confirms the intuition that attention patterns precede performance improvements. Intuitively, early attention predicts performance by being able to predict the sort of curiosity signal the agent is using, which predicts the full timecourse of attention (see~\ref{sec:app:attention_determinants}), which in turn predicts performance.

\input{icml_sections/attention_determinants.tex}


==> icml_sections/discussion.tex <==
\section{Future directions}
\label{sec:future}

In this work, we propose and test $\gamma$-Progress, a computationally-scalable progress curiosity signal that enables an agent to efficiently train a world model in agent-rich environments while overcoming the white noise problem. Although in this work we limited the agent's ways of interacting with the world to visual attention, future works may explore larger action spaces. Another exciting avenue of research is investigating how to learn the world model priors used in this work such as the visual encoder and disentanglement prior. Finally, we hope see follow-up works applying $\gamma$-Progress to other domains such as video games. 

We also see several key next steps at the intersection of AI and cognitive science.

\noindent{\textbf{Human behavior}}~How might AWML-optimized agents model human behavior? We have run a pilot human subject experiment (Figure~\ref{fig:human_modeling_combined}a) in which we conveyed static, periodic, animate, and noise stimuli to twelve human participants via spherical robots while we tracked their gaze. In aggregate, gaze is similar to $\gamma$-Progress attention. In follow-up work, we aim to make a finer model comparison to the behavior of humans shown a diverse array of stimuli.



\begin{figure}
    \centering
    \includegraphics[width=.5\textwidth]{figures/humans_v6.pdf}
    \vspace{-20pt}
    \caption{\textbf{Modeling human behavior}. (a) A pilot human behavior study. (b)  Accuracy of early indicators of final performance, as a function of time, and (c) factor analysis: curiosity signal determines attention, which determines final performance.}
    \label{fig:human_modeling_combined}
    \vspace{-15pt}
\end{figure}


\noindent{\textbf{Early indicator analysis}}~Eventually, we would like to use curiosity-driven learning as a model for intrinsic motivation in early childhood. In this interpretation, the attention timecourse is a readily observable behavioral metric, and performance represents some more difficult-to-obtain measure of social acuity. Variation in curiosity signal would, in this account, be a latent correlate of developmental variability. For example, Autism Spectrum Disorder is characterized by both differences in low-level facial attention~\cite{jones2013attention} and high-level social acuity~\cite{hus2014ados}. Motivated by this, we sought to determine whether attention could be used as an early indicator of performance. We thus train two models:
(1) PERF$_{\leq T}$, which takes performance before time $T$ as input, and (2) ATT$_{\leq T}$, which takes attention before time $T$ as input.
As seen in Figure~\ref{fig:human_modeling_combined}b, ATT$_{\leq T}$ is throughout most of the timecourse a more accurate indicator than direct measurement of early-stage model performance itself. The overall situation is conveyed by the factor diagram Figure~\ref{fig:human_modeling_combined}c --- for further details, see Appendix~\ref{sec:app:attention_diagnostic}. As models grow in their capacity to model early childhood learning, translating such an analysis into a real-world experimental population could lead to substantial improvements in diagnostics of developmental variability.


==> icml_sections/discussion_scrap.tex <==
\section{Future Directions}

%\jdf {Summarize results here}
%\jdf {Critically analyze the fact that we had to use a split model architecture, and what we think a more sophisticated system would look like (stuff Dan said about starting with shared parameters).}

Here we describe three next directions for this work. We first describe ongoing human subject experiments that mirror the computational ones described above. We then describe what preliminary results suggest are key ``theory of mind'' properties of world models that perform well in environments such as ours. Last, we interpret the above experiment as a toy model of early childhood development and provide an analysis of how behavior early in ``life'' predicts downstream social acuity.


Limitations:
other sorts of environments (while we designed environments to present a diverse array of stimuli while being able to maintain an understanding of what sorts of stimuli are being chosen without a wide array of confounds)
more complex embodiments
active learning: what is the validation set?
(based on our heuristic understanding of qhat is interesting, understanding broadly how to make this choice in these embodied active learning contetxts)


\noindent\textbf{Human experiments}

A standard hypothesis is that the human brain has a built-in module that specifically detects animacy from visual input \citep{leslie1989autism, leslie1994tomm}. Yet the current modeling results suggest that animate attention in humans might naturally arise from a more general process of curiosity-driven learning. In ongoing work, we are testing this possibility by running human subject experiments to measure important features of animate attention, then comparing our intrinsically-motivated models to this human behavior. 

These experiments include not only random and animate stimuli, but also other behaviors that span the spectrum of predictability, including \textit{static} objects, and \textit{periodic} ones, inspired by the repetitive dynamics seen in objects like seesaws, fans, and flashing lights. We convey these kinematics to humans via self-propelled, spherical robots moving along a mat, while measuring patterns of attention via a mobile eye tracker. So far, we find average fixation proportions favoring the animate stimuli. Furthermore, a progress network tasked to predict the virtual robot trajectories produces a similar aggregate attentional fixation pattern  \ref{fig:fig2_humans_v2.png}. Crucially, the network achieves this without the requirement for any specific built-in modules favoring animacy. Instead, the pattern arises from the agent’s discovery of the inherent relative “interestingness” of animacy as compared to random, periodic, and static motion. 


\begin{figure}[h]
    \centering
    \includegraphics[width=0.7\textwidth]{figures/fig2_humans_v3-01.png}
    \caption{Ongoing work compares our intrinsically-motivated agents to human observers watching analogous displays in the real-world. Human adults wear a mobile eye tracker while watching displays consisting of four sets of self-propelled, spherical robots travelling along a mat. Using kinematics alone, the robots are made to appear animate, random, periodic, or static. Spontaneous human fixations proportions are similar to the patterns of attention exhibited by our neural agent placed in a similar environment.}
    \jdf{Kun Ho: Can we get a version of the model plot with a more comparable hierarchy?}
    \label{fig:my_label}
\end{figure}

\kh{Error bars in the figure, more seeds with randomized location}

\noindent\textbf{Theory of Mind and social mental states}

In order for a curious agent to learn effectively in a social environment, all components of the system (e.g. world model architecture, intrinsic motivation, and controller architecture) must be suited to the task, and world model architecture choice of Section~\ref{sec:methods:worldmodel} reflect choices made to reach acceptable performance given sufficient data --- see Appendix~\ref{sec:app:causal} \ref{sec:offline} for details. In particular, a {\em Theory of Mind v0} motif, which allocates separate models for separate external agent behaviors, and more generally,  causally linked subsets of the environment, may be a crucial such choice. In future work, we will look to both (1) build a system that can infer this causal prior from data and (2) stress-test its utility in a suitable range of environments.

The choice of term {\em Theory of Mind v0} is deliberate because `theory of mind' is also  used to refer to the more sophisticated ability to predict the behaviors of other agents as a function of inferred mental states, such as beliefs, desires, and goals \citep{astington1990developing, premack1978does, wellman1992child}. Determining whether our models represent such mental states will require more deliberate tests inspired from developmental psychology, perhaps in tandem with specially-tailored learning environments and model architectures. For instance, one possibility is that curiosity models will need to solve an inverse reinforcement learning problem, in which they are specifically tasked with inferring an agent's world model and reward function, given its observed actions \citep{jara2019theory}. Relatedly, human agents do not only represent first-order knowledge about what others believe, but can also represent multiply embedded beliefs (e.g., he knows that I know he knows), as well as common knowledge (we all know that we all know), mental states which are a key to understanding more sophisticated social behaviors, such as coordinating on a goal, or turn taking \cite{de2019common, de2019maimonides, thomas2016recursive}. 

Alternatively, theory of mind-like representations might emerge without the need for such deliberate, social tasks. After all, the scope of things that are interesting and worth attending to is not limited to animate agents, so either way a more general purpose learning algorithm may be needed to detect patterns in the surrounding world. At any rate, learning to predict the full complexity of inanimate and animate stimuli using biologically plausible, unsupervised systems that can operate flexibly in the real-world presents a grand challenge for both AI and cognitive science.

\noindent\textbf{In silico models of human development}

An overarching goal of this research program is to develop in silico models of early childhood development. This is a task-driven modeling approach in which we design an artificial system to accomplish a challenging cognitive task that we as humans do well. If the task is sufficiently difficult that the solution space is small, we expect to see reflections of the artificial solution in behavior and biology. This approach has yielded dramatic success as a neural model of our ventral visual stream \cite{yamins_ventralneural}, using the task of visual object recognition. We posit that attention and interaction early in childhood, with the goal of learning to model one's surroundings, is a similarly difficult task, and by solving it, we can both better understand early childhood development as well as test interventions in simulation before resorting to human subject experiments.

Consider the following interpretation of the experiments of Section~\ref{sec:experiments} as a toy model of attention, interaction, and learning early in childhood. We model the development of a "population" of agents that have differently-implemented curiosity: differing intrinsic motivations represent underlying neural/genotype/phenotype correlates of early learning differences. Attention patterns represent abundant/cheaply obtained behavioral measures related to the sorts of exploratory strategies the agents have early in life (e.g. visual attention to animate stimuli), whereas validation performance represents a more difficult to obtain measure of acuity. An easily obtained behavioral measure that predicts outcomes later in life may provide both a valuable diagnostic criterion and a cue for possible interventions.

Using this model of early development, we ask: to what extent does the emergent attention pattern of the agent predict validation performance? We seek to understand whether attention {\em early} in a run predicts {\em final} validation performance, and in particular whether, sufficiently early in a run, attention is a better predictor than early validation performance of final validation performance. Intuitively, we expect attention patterns that lead to good validation performance to precede good validation performance itself.

We look to predict final performance $P_{\mathrm{final}}$ of a given agent, which we take to be the average of the final four validation runs. To make the modeling problem simple, we discretize this into a classification task by dividing validation performance into 3 equal-sized classes (``high'', ``medium'', and ``low'', computed separately for each external agent behavior), intuitively chosen to reflect performance around, at, and below that of random policy.

We consider two predictive models of final performance, one that takes as input early attention of the agent, and the other, early performance. Early performance may be quantified simply: given time $T$ (``diagnostic age'') during training, let $P_{\leq T}$ be the vector containing all validation losses measured up to time $T$. Early attention, however, is very high-dimensional, so we must make a dimensionality-reducing choice in order to tractably model with our modest sample size. Hence, we ``bucket'' average. Given choice of integer $B$, let
\begin{equation}
    A_{\leq T, B} = (\mathit{f}^{\mathrm{anim}}_{0 : \frac{T}{B}}, \mathit{f}^{\mathrm{rand}}_{ 0 :  \frac{T}{B}}, \mathit{f}^{\mathrm{anim}}_{\frac{T}{B}: \frac{2T}{B}}, \mathit{f}^{\mathrm{rand}}_{\frac{T}{B} : \frac{2T}{B}}, \ldots \mathit{f}^{\mathrm{anim}}_{\frac{(B - 1)T}{B} : T}, \mathit{f}^{\mathrm{rand}}_{\frac{(B - 1)T}{B} : T}),
\end{equation}
where $\mathit{f}^{\mathrm{anim}}_{a : b}$ and $\mathit{f}^{\mathrm{rand}}_{a : b}$ are the fraction of the time $t = a$ and $t = b$ spent looking at the animate external agent and random external agents respectively (so $A_{\leq T, B}$ is the attentional trajectory up to time $T$ discretized into $B$ buckets).

Finally, both models must have knowledge of the external agent behavior to which the agent is exposed --- we expect this to both have an effect on attention as well as the meaning of early performance and expected final performance as a result. Let $\chi_{\mathrm{BHR}}$ be the one-hot encoding of which external animate agent behavior is shown. 

We then consider models
\begin{enumerate}
    \item PERF$_{\leq T}$, which takes as input $P_{\leq T}$ and $\chi_{\mathrm{BHR}}$, and
    \item ATT$_{\leq T}$, which takes as input $A_{\leq T, B}$ and $\chi_{\mathrm{BHR}}$.
\end{enumerate}

\begin{figure}[h]
    \centering
    \includegraphics[width=\textwidth]{figures/early_indicator_analysis_with_attn.pdf}
    \caption{\textbf{Early diagnosis analysis}. Accuracy of PERF$_{\leq T}$ and ATT$_{\leq T}$ predictors of final performance, as a function of $T$. Up until late, attentional patterns make for the more informative predictor of final performance. Below, sample real-time attention trajectories that result in high, medial, and low final performance, from left to right. Intuitively, early attention trajectory predicts attention througout the run, which in turn predicts performance.}
    \label{fig:earlypredictor}
\end{figure}


Figure~\ref{fig:earlypredictor} shows the plot of PERF$_{\leq T}$ and ATT$_{\leq T}$ accuracy as $T$ varies. We see that, up to a point, ATT$_{\leq T}$ makes a better predictor of final performance, and then PERF$_{\leq T}$ dominates. This confirms the intuition that attention patterns precede performance improvements. Intuitively, attention predicts performance by being able to predict the sort of intrinsic motivation the agent is using, which in turn predicts performance. The attention trajectories Figure~\ref{fig:earlypredictor} correspond to agents that achieve different levels of final performance, and each display different attention early that characterizes the overall strategy. For example, the high final performance corresponds to a ``bump'' in attention towards the animate agent.







\begin{comment}
NH: prior to my big edits!

\jdf {Summarize results here}
\jdf {Critically analyze the fact that we had to use a split model architecture, and what we think a more sophisticated system would look like (stuff Dan said about starting with shared parameters).}

\noindent\textbf{Ongoing work: Human experiments}

As noted, a standard hypothesis is that the human brain has a built-in module that specifically detects animacy from visual input \citep{leslie1989autism, leslie1994tomm}. Yet the current modeling results suggest that animate attention in humans might naturally arise from a more general process of curiosity-driven learning. In ongoing work, we are testing this possibility by running human subject experiments to measure important features of animate attention, then comparing our intrinsically-motivated models to this human behavior. 

These experiments include not only random and animate stimuli, but also other behaviors that span the spectrum of predictability, including \textit{static} objects, and \textit{periodic} ones, inspired by the repetitive dynamics seen in objects like seesaws, fans, and flashing lights. We convey these kinematics to humans via self-propelled, spherical robots moving along a mat, while measuring patterns of attention via a mobile eye tracker. So far, we find average fixation proportions favoring the animate stimuli. Furthermore, a progress network tasked to predict the virtual robot trajectories produces a similar aggregate attentional fixation pattern  \ref{fig:fig2_humans_v2.png}. Crucially, the network achieves this without the requirement for any specific built-in modules favoring animacy. Instead, the pattern arises from the agent’s discovery of the inherent relative “interestingness” of animacy as compared to random, periodic, and static motion. 


\begin{figure}[h]
    \centering
    \includegraphics[width=0.7\textwidth]{figures/fig2_humans_v3-01.png}
    \caption{Ongoing work compares our intrinsically-motivated agents to human observers watching analogous displays in the real-world. Human adults wear a mobile eye tracker while watching displays consisting of four sets of self-propelled, spherical robots travelling along a mat. Using kinematics alone, the robots are made to appear animate, random, periodic, or static. Spontaneous human fixations proportions are similar to the patterns of attention exhibited by our neural agent placed in a similar environment.}
    \jdf{Kun Ho: Can we get a version of the model plot with a more comparable hierarchy?}
    \label{fig:my_label}
\end{figure}

\kh{Error bars in the figure, more seeds with randomized location}

\noindent\textbf{Future Work: Theory of Mind V1, and Other Mental States}


As noted, even human infants preferentially attend to the primitive kinds of animate behaviors included in the current experiments, and we have referred to the model innovations needed to replicate these behaviors as theory of mind v0. This naming convention is deliberate because `theory of mind' is also  used to refer to the more sophisticated ability to predict the behaviors of other agents as a function of inferred mental states, such as beliefs, desires, and goals \citep{astington1990developing, premack1978does, wellman1992child}. Determining whether our models represent such mental states will require more deliberate tests inspired from developmental psychology, perhaps in tandem with specially-tailored learning environments and model architectures. For instance, one possibility is that curiosity models will need to solve an inverse reinforcement learning problem, in which they are specifically tasked with inferring an agent's world model and reward function, given its observed actions \citep{jara2019theory}. Relatedly, human agents do not only represent first-order knowledge about what others believe, but can also represent multiply embedded beliefs (e.g., he knows that I know he knows), as well as common knowledge (we all know that we all know), mental states which are a key to understanding more sophisticated social behaviors, such as coordinating on a goal, or turn taking \cite{de2019common, de2019maimonides, thomas2016recursive}. 

Alternatively, theory of mind-like representations might emerge without the need for such deliberate, social tasks. After all, the scope of things that are interesting and worth attending to is not limited to animate agents, so either way a more general purpose learning algorithm may be needed to detect patterns in the surrounding world. At any rate, learning to predict the full complexity of inanimate and animate stimuli using biologically plausible, unsupervised systems that can operate flexibly in the real-world presents a grand challenge for both AI and cognitive science.





\end{comment}




\noindent{\textbf{Early indicator analysis}} To better understand how attention drives performance, we perform an {\em early indicator analysis} of whether attention {\em early} in a run predicts {\em final} validation performance, and in particular whether, sufficiently early in a run, attention is a better predictor than early validation performance. We hence train two models:
\begin{enumerate}
    \item PERF$_{\leq T}$, which takes as input performance before time $T$, and stimulus type, and
    \item ATT$_{\leq T}$, which takes as input a summary of attention before time $T$, and stimulus type.
\end{enumerate}
As seen in Figure~\ref{fig:human_modeling_combined}a, ATT$_{\leq T}$ dominates until late. Intuitively, as captured in the factor analysis diagram, we expect performance to be determined by attention throughout the run. Attention drives intrinsic motivation, and if the intrinsic motivation can be inferred early, this predicts later attention and hence performance. Interpreting this as a toy model of early childhood developmental variability (see Discussion for interpretation details), this tells us that attention patterns is a better {\em diagnostic} of later acuity than an early acuity-based diagnostic.

\begin{figure}
    \centering
    \includegraphics[width=.5\textwidth]{figures/humans.pdf}
    \vspace{-20pt}
    \caption{\textbf{Modeling human behavior}. (a)  Accuracy of early performance and early attention predictors of final performance, as a function of $T$, along with factor analysis hypothesis: intrinsic motivation (IM) determines attention, which determines final performance. (b) Human adults wear a mobile eye tracker while watching displays consisting of four sets of self-propelled, spherical robots travelling along a mat. Human and model fixation proportions are similar.}
    \label{fig:human_modeling_combined}
    % \vspace{-20pt}
\end{figure}


\noindent{\textbf{Human behavior}} To quantify how the emergent behavior matches that of humans, we ran a human subject experiment in which we conveyed static, periodic, animate, and noise stimuli to humans via self-propelled, spherical robots moving along a mat, while measuring patterns of attention via a mobile eye tracker. We find average fixation proportions favoring the animate stimuli. Furthermore, a $\gamma$-Progress network tasked to predict the virtual robot trajectories produces a similar aggregate attentional fixation pattern (Figure~\ref{fig:human_modeling_combined}b).

==> icml_sections/discussion_scrap_2.tex <==
\section{Discussion and future directions}

In this work, we propose an implementation of curiosity that enables an agent to train efficiently a world model in environments containing other agents. Such environments
often contain static stimuli (easy to model), dynamic but largely deterministic stimuli (still relatively easy to model), noisy stimuli (to a large degree inherently unpredictable), as well as animate stimuli (interesting, complex, and to a considerable degree learnable). In order for the curious agent to be able to attend to the interesting without succumbing to the ``white noise problem,'' it mus be able to distinguish between these different sorts of stimuli. To accomplish this, we  propose $\gamma$-Progress, a computationally-scalable variant of progress-driven curiosity. To test this, we design a custom 3D virtual environment a variety of distillations of these classes of stimuli. We find that $\gamma$-Progress outperforms a variety of baselines in sample complexity. These agents learn better, faster, and they do so by learning to attend to what is interesting. The robustness and scalability of this method in relation to baselines makes it a prime candidate for both (1) embodied curiosity with other agents in increasingly ethologically-reasonable settings and (2) broader active learning and curiosity in a wide range of environments and tasks.

\nh{Rehash theory discussion? Let's settle on how we describe in intro first.}

Key next steps include testing these broad utilities. One limitation of the present work is in our restriction to the custom environment built to support our evaluation. We designed the environment to present a diverse array of stimuli while being able to maintain a level of control in understanding agent behavior, but this introduces its own biases. Further, in order to focus on intrinsic motivation implementation, we limited the embodiment of the agent. Lifting this restriction is an important step towards building embodied curiosity.

We see two important related activities. The first concerns the agent's world model: what makes a good world model for environments with other agents? Initial results suggest an important architectural motif, and it remains to validate this and more broadly develop computational ``theory of mind''. The second concerns how humans navigage a social world: does an implementation such as this reflect human decision making? And can we model child development with models such as these? In what follows, we describe progress towards these as well as important next steps.


\subsection{World models of other agents and theory of mind}

The world model architecture of Section~\ref{sec:methods:worldmodel} reflects choices made to guarantee acceptable prediction performance when trained on suitable data. In particular, a {\em Theory of Mind v0} motif, which allocates separate models for separate external agent behaviors, may be crucial. To test this, we construct an offline ``ideal dataset'' compare performance of this {\em causal} world model against two ablations: a {\em joined} acausal ablation that takes all observations and predicts all agents jointly, and a {\em split} acausal ablation that handles each external agent (as opposed to behavior) separately. For details on the training procedure and ablation implementations, see Appendix~\ref{sec:offline}. As seen in Figure~\ref{fig:offline_asymptotic_performance}, across all experiments, the causal world model significantly outperforms the ablations.

\begin{wrapfigure}{R}{0.4\textwidth}
\vspace{-10pt}
\begin{center}
    \includegraphics[width=.4    \textwidth]{figures/offline_asymptotic_performance_v6.pdf}
\end{center}
\vspace{-10pt}
    \caption{\textbf{Asymptotic Model Performance} The causal world model and the non-causal ablation were trained on data gathered under a reduced action space random policy, aimed at producing "ideal data" for learning each animate external agent behavior excluding peekaboo (See Section~\ref{sec:offline} for details.) \ms{Make taller}}
    \label{fig:offline_asymptotic_performance}
\vspace{-10pt}
\end{wrapfigure}

The reason for this performance difference may be understood in terms of {\em disentanglement}, in which the model finds spurious dependence ``nuisance factors'' --- some external agents are irrelevant to the behavior of others. It may be the case that poor disentanglement is more likely to occur and be detrimental to generalization performance when learning world models of partially observable environments via interactive learning. For a formalization of disentanglement and further discussion regarding the challenge in our setting, see Appendix~\ref{sec:app:causal}.

The choice of term {\em Theory of Mind v0} is deliberate because `theory of mind' is also  used to refer to the more sophisticated ability to predict the behaviors of other agents as a function of inferred mental states, such as beliefs, desires, and goals \citep{astington1990developing, premack1978does, wellman1992child}. The above motif represents a proto-version of this in which an agent, upon detecting agents or other stimuli in its environment, infers a causal structure of the environment and allocates modules of its world model that respects this causal structure. In future work, we will look to both (1) build a system that can infer this causal prior from data and (2) stress-test its utility in a suitable range of environments --- in particular, those with changing causal structure and greater interplay between causal structure and partial observability.

\subsection{Modeling human behavior}

An overarching goal of this research program is to develop models of human behavior. As a first step towards this, we would like to quantify how humans explore a similar environment and compare their behavior to that of models. In ongoing work, we are running human subject experiments in which we convey static, periodic, animate, and noise stimuli to humans via self-propelled, spherical robots moving along a mat, while measuring patterns of attention via a mobile eye tracker. The use of these spherical robots mirrors the virtual environment in order to reduce visual confounds and so as to present relatively novel stimuli to human adults. So far, we find average fixation proportions favoring the animate stimuli. Furthermore, a $\gamma$-Progress network tasked to predict the virtual robot trajectories produces a similar aggregate attentional fixation pattern. See Figure~\ref{fig:human_subject_experiment} for details.

\begin{wrapfigure}{L}{0.6\textwidth}
\vspace{-10pt}
\begin{center}
    \includegraphics[width=0.55\textwidth]{figures/fig2_humans_v3-01.png}
\end{center}
\vspace{-10pt}
    \caption{Ongoing work compares our intrinsically-motivated agents to human observers watching analogous displays in the real-world. Human adults wear a mobile eye tracker while watching displays consisting of four sets of self-propelled, spherical robots travelling along a mat. Using kinematics alone, the robots are made to appear animate, random, periodic, or static. Spontaneous human fixations proportions are similar to the patterns of attention exhibited by our neural agent placed in a similar environment.}
    \jdf{Kun Ho: Can we get a version of the model plot with a more comparable hierarchy?} \kh{Error bars in the figure, more seeds with randomized location}
    \label{fig:human_subject_experiment}
\vspace{-10pt}
\end{wrapfigure}

A standard hypothesis of human cognition is that the brain has a built-in module that specifically detects animacy from visual input \citep{leslie1989autism, leslie1994tomm}. The current modeling results suggest that animate attention in humans might naturally arise from a more general process of curiosity-driven learning.

If we can model adult human behavior, can we go further and model early childhood development? Can we model human developmental variability? One possibility is that, if such models can represent development of the general population, then implementation variations (e.g. in intrinsic motivation signal) can represent variability in development. Consider the following interpretation of the experiments of Section~\ref{sec:experiments} as a toy model of attention, interaction, and learning early in childhood. We model the development of a "population" of agents that have differently-implemented curiosity: differing intrinsic motivations represent underlying neural/genotype/phenotype correlates of early learning differences. Attention patterns represent abundant/cheaply obtained behavioral measures related to the sorts of exploratory strategies the agents have early in life (e.g. visual attention to animate stimuli), whereas validation performance represents a more difficult to obtain measure of acuity. An easily obtained behavioral measure that predicts outcomes later in life may provide both a valuable diagnostic criterion and a cue for possible interventions.

\begin{wrapfigure}{R}{0.6\textwidth}
\vspace{-10pt}
\begin{center}
    \includegraphics[width=.6 \textwidth]{figures/early_indicator_analysis_with_factor_analysis.pdf}
\end{center}
\vspace{-10pt}
    \caption{\textbf{Early diagnosis analysis}. (a) Accuracy of PERF$_{\leq T}$ and ATT$_{\leq T}$ predictors of final performance, as a function of $T$. Up until late, attentional patterns make for the more informative predictor of final performance. (b) Factor analysis hypothesis: intrinsic motivation (IM) determines attention, which determines final performance.}
    \label{fig:earlypredictor}
\vspace{-10pt}
\end{wrapfigure}

Using this model of early development, we seek to understand whether attention {\em early} in a run predicts {\em final} validation performance, and in particular whether, sufficiently early in a run, attention is a better predictor than early validation performance of final validation performance. To test this hypothesis, we train models that predict final performance from early attention (ATT$_{\leq T}$) or early performance (PERF$_{\leq T}$) (see Appendix~\ref{sec:app:attention_diagnostic} for details). As seen in Figure~\ref{fig:earlypredictor}, ATT$_{\leq T}$ dominates until late. Intuitively, as captured in the factor analysis diagram of Figure~\ref{fig:earlypredictor}, we expect performance to be determined by attention throughout the run; however, attention is driven by choice of intrinsic motivation, and if the intrinsic motivation implementation can be inferred early, this can be used to predict later attention and hence performance.








==> icml_sections/environment.tex <==
\section{Virtual World Environment}
\label{sec:environment}
To faithfully replicate real-world algorithmic challenges, we design our 3D virtual environment to preserve the following key properties of real-world environments: 
\vspace{-5pt} 
\begin{enumerate} 
    \item \textit{Diverse dynamics.} Agents operate under a diverse set of dynamics specified by agent-specific programs. An agent's actions may depend on those of another agent resulting in complex intedependent relationships.
    
    \item \textit{Partial observability.} At no given time do we have full access to the current state of every agent in the environment. Rather, our learning is limited by what lies within our field of view. 
    
    \item \textit{Contingency.} How much we learn is contingent on how we, as embodied agents, choose to interact with the environment. 
    % Attention is a primitive mechanism for exploration and social interaction, since how we attend may trigger different behaviors in agents. \sj{I didn't get this last sentence}
\end{enumerate} 
% it's fine to not explicitly list confounds 
\vspace{-5pt}
% \sj{Why can't other environments (e.g. the ones from deepmind) satisfy these properties? I think it would at least help to point to some comparisons.} 

Concretely, Our virtual environment consists of two main components, a \textit{curious agent} and various \textit{external agents}.

The \textbf{curious agent}, embodied by an avatar, is fixed at the center of a room (Figure \ref{fig:environment}). Just as a human toddler can control her gaze to visually explore her surroundings, the agent is able to partially observe the environment based on what lies in its field of view (see top of Figure \ref{fig:environment}). The agent can choose from 9 actions: rotate $12^{\circ}, 24^{\circ}, 48^{\circ}$, or $96^{\circ}$, to the left/right, or stay in its current orientation. 

The \textbf{external agents} are spherical avatars that each act under a hard-coded policy inspired by real-world inanimate and animate stimuli. An \textit{external agent behavior} consists of either one external agent, e.g reaching, or two interacting ones, e.g chasing. Since external agents are devoid of surface features, the curious agent must learn to attend to different behaviors based on spatiotemporal kinematics alone. We experiment with external agent behaviors (see Figure \ref{fig:environment}, right) including static, periodic, noise, reaching, chasing, peekaboo, and mimicry. The animate behaviors have deterministic and stochastic variants, where the stochastic variant preserves the core dynamics underlying the behavior, albeit with more randomness. See \textcolor{blue}{\url{https://bit.ly/31vg7v1}} for video descriptions of the environment and external agent behaviors. 

We divide the room into four quadrants, each of which contains various auxiliary objects (e.g teddy bear, roller skates, surfboard) and one external agent behavior. The room is designed such that the curious agent can see at most one external agent behavior at any given time. This design is key in ensuring partial observability, such that the agent is faced with the problem of allocating attention between different external agent behaviors in an efficient manner. 
% \sj{Seems very detailed to appear in the main paper instead of appendix}
    % The \textbf{curious agent} is placed in the center of a $3m \times 3m$ room (in Unity, $1$ unit $ =1m$). Sequences of image observations are captured by a camera on its forehead, containing only what lies in its view at a given time (See top of Figure~\ref{fig:environment}). The curious agent has nine available actions: rotate $12^{\circ}, 24^{\circ}, 48^{\circ}$, or $96^{\circ}$ to the left/right, or stay in its current orientation. Its location is fixed at the room center as to isolate the problem of learning to attend. 

    % \textbf{External agents} are spherical avatars that each act under a hard-coded policy inspired by real-world inanimate and animate behaviors. An \textit{external agent behavior} consists of one external agent or two interacting ones. Two external agents are interacting if there exists a causal relationship between their physical positions. In our environment, we fix interagent relationships, so each external agent belongs to the same behavior over time. The animate behaviors have deterministic and stochastic variants, where the stochastic variant preserves the core dynamics underlying the behavior, albeit with more randomness. See \textcolor{blue}{\url{https://bit.ly/31vg7v1}} for a video of the environment and external agent behaviors, and Appendix \ref{sec:app:behaviors} for a list of behavior descriptions.
    
    % We programmatically generate the environment with custom configurations of these components using ThreeDWorld, a general-purpose virtual world simulation platform, designed to interface with the Unity3D engine \citep{gan-forthcoming}.
    
    % We divide the room into four quadrants, each of which contains three auxiliary objects (teddy bear, roller skates, surfboard) arranged in a fixed triangular formation, and an external agent behavior sampled from the total pool of behaviors. The room is designed such that the curious agent can see at most one external agent behavior at any given time. %Since we already mention this above, we could potentially omit the following sentence:
    % Since external agents are devoid of surface features, the curious agent must learn to attend to different behaviors based on spatiotemporal kinematics alone. 
    
    
    
    




==> icml_sections/experiments.tex <==
\begin{table}[t]
    \vspace{-7pt}
    \caption{Mean ratio of baseline end performance over Random baseline end performance (standard error in parentheses)}
    \label{table:aggregate_end_performance}
    \begin{center}
    \begin{small}
    \begin{sc}
    \begin{tabular}{lcc}
    \toprule
    & Mixture World & Noise World \\
    \midrule
         
    $\gamma$-Progress & \textbf{7.83} (3.57) & \textbf{13.79} (5.29) \\
    $\delta$-Progress & 2.2 (0.51) & 2.46 (0.55) \\
    RND & 1.25 (0.25) & 0.85 (0.10) \\
    Disagreement & 0.62 (0.10) & 0.76 (0.06) \\
    Adversarial & 0.62 (0.09) & 0.59 (0.10) \\
    \bottomrule
    \end{tabular}
    \end{sc}
    \end{small}
    \end{center}
    \vspace{-20pt}
\end{table}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/attention.pdf}
    \vspace{-15pt}
    \caption{\textbf{Attention Patterns}. a) The bar plot shows the total animate attention, which is the ratio between the number of time steps an animate external agent was visible to the curious agent, and the number of time steps a noise external agent was visible. The time series plots in the zoom-in box show the differences between mean attention to the animate external agents and the mean of attention to the other agents in a 500 step window, with periods of animate preference highlighted in purple. Results are averaged across 5 runs. $\gamma$-Progress displays strong animate attention while baselines are either indifferent, e.g $\delta$-Progress, or fixating on white noise, e.g Adversarial. b) Fraction of indifference and white noise failures, out of eight tasks.} 
    \label{fig:attention}
    \vspace{-10pt}
\end{figure*}

\section{Results}
\label{sec:experiments}
%%%%%%%%%%%% Summary of what we seek to show %%%%%%%%%%%%%%

We evaluate the AWML performance of $\gamma$-Progress on two metrics: \emph{end performance} and \emph{sample complexity}. End performance is the inverse of the the final world loss after a larger number of environment interactions, and intuitively measures the ``consistency'' of the proxy reward with respect to the true reward. Sample complexity measures the rate of reduction in world model loss $\LL_{\mu}(\theta)$ with respect to the number of environment interactions. The samples from the validation distribution $\mu$ correspond to core validation cases we crafted for each behavior. On the reaching behaviors, for example, we validate the world model loss with objects spawned at new locations. For details on each behavior-specific validation case and metric computation, we refer readers to Appendix \ref{sec:app:validation}.

Experiments are run in two virtual worlds: Mixture and Noise. In the Mixture world, the virtual environment is instantiated external agents spanning four representative types: static, periodic, noise, and animate. This set up is a natural distillation of a real-world environment containing a wide spectrum of behaviors. In the Noise world, the environment is instantiated with three noise agents and one animate agent. This world strain tests the noise robustness of $\gamma$-Progress. For each world, we run separate experiments in which the animate external agents are varied amongst the deterministic and stochastic versions of reaching, chasing, peekaboo, and mimicry agents (see Section \ref{sec:environment}). We compare the AWML performance of the following methods: 

\textbf{$\gamma$-Progress (Ours)} is our proposed variant of progress curiosity which chooses $\theta_{old}$ to be a geometric mixture of all past models as in Eq. \ref{eq:mix_progress}. 

\textbf{$\delta$-Progress \citep{achiam2017surprise, graves2017automated}} is the $\delta$-step learning progress reward from Eq. \ref{eq:kstep_progress} with $\delta = 1$. We found that any $\delta > 3$ is impractical due to memory constraints.  

\textbf{RND \citep{burda2018exploration}} is a novelty-based method that trains a predictor neural net to match the outputs of a random state encoder. States for which the predictor networks fails to match the random encoder are deemed ``novel'', and thus receive high reward. 

\textbf{Disagreement \citep{pathak2019disagreement}} is the disagreement based method from Eq. \ref{eq:disagreement} with $N = 3$ ensemble models. We found that $N > 3$ is impractical due to memory constraints.  

\textbf{Adversarial \citep{stadie2015predictive, pathak2017inverse}} is the prediction error based method from Eq. \ref{eq:adversarial}. We use the $\ell_{2}$ prediction loss of the world model as the reward. 

\textbf{Random} chooses actions uniformly at random among the 9 possible rotations. 

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\textwidth]{figures/sample_complex.pdf}
%     \caption{\textbf{AWML Performance in White Noise World}. Results shown for eight experiments in mixture worlds with the animate external agent varied according to the column labels. End performance (top row) is measured as the average of the last 4 validation losses. Sample complexity plots (bottom row) show validation losses evaluated every 5000 environment steps. Error bars/regions are computed over 5 seeds. $\gamma$-Progress achieves lower sample complexity than baselines on $8/8$ behaviors. Baselines frequently perform worse than the Random baseline due to white noise fixation.}
%     \label{fig:sample_complexity}
% \end{figure}

\subsection{AWML Performance}

Fig.~\ref{fig:sample_complexity}a shows end performance (first row) and sample complexity (second row) in the Mixture world, and Fig.~\ref{fig:sample_complexity}b shows the same for the Noise World.
In the Mixture world, we see that $\gamma$-Progress has lower sample complexity than $\delta$-Progress, Disagreement, Adversarial, and Random baselines on all $8/8$ behaviors and outperforms RND on $7/8$ behaviors while tying on stochastic chasing. In the Noise world, we see that $\gamma$-Progress has lower sample complexity than all baselines on all $8/8$ behaviors. See Table~\ref{table:aggregate_end_performance} for aggregate end performance, and \textcolor{blue}{\url{https://bit.ly/31vg7v1}} for visualizations of model predictions.

% \begin{table}[]
%     \caption{
%     \textbf{End performance} Mean end performance, normalized to Random policy performance (higher is better) and averaged over external agent behaviors.
%     }
%     \label{table:aggregate_end_performance}
%     \begin{center}
%     \begin{small}
%     \begin{sc}
%     \begin{tabular}{lcc}
%     \toprule
%     & Mixture world & Noise world \\
%     \midrule
%     $\gamma$-Progress & \textbf{12.8} & \textbf{24.4}  \\
%     $\delta$-Progress & 2.6 & 4.2 \\
%     RND & 1.8 & 1.6 \\
%     Disagreement & 0.68 & 0.81 \\
%     Adversarial & 0.80 & 0.69 \\
%     Random & 1. & 1. \\
%     \bottomrule
%     \end{tabular}
    
    
%     \end{sc}
    
%     \end{small}
    
    
%     \end{center}


% \end{table}


% \begin{table}[]
%     \caption{
%     \textbf{End performance} Mean end performance (with standard error), normalized to Random policy performance (higher is better) and averaged over external agent behaviors.
%     }
%     \label{table:aggregate_end_performance}
%     \begin{center}
%     \begin{small}
%     \begin{sc}
%     \begin{tabular}{lcccccc}
%     \toprule
%     & $\gamma$-Progress & $\delta$-Progress & RND & Disagreement & Adversarial & Random\\
%     \midrule
%     Mixture world & \textbf{7.83} (3.57) & 2.2 (0.51) & 1.25 (0.25) & 0.62 (0.10) & 0.62 (0.09) & 1. \\
%     Noise world & \textbf{9.09} (3.85) & 2.40 (0.53) & 0.83 (0.09) & 0.76 (0.06) & 0.62 (0.13) & 1. \\
%     \bottomrule
%     \end{tabular}
    
    
%     \end{sc}
    
%     \end{small}
    
    
%     \end{center}

% \end{table}

\subsection{Attention control analysis}

Figure~\ref{fig:attention} shows the ratio of attention to animate vs other external agents for each behavior in the Mixture world as well as example animate-inanimate attention differential timeseries (for the Noise world, see Appendix~\ref{app:noise_world_plot}). The $\gamma$-Progress agents spend substantially more time attending to animate agents than do alternative policies. This increased animate-inanimate attention differential often corresponds to a characteristic attentional ``bump'' that occurs early as the $\gamma$-Progress curious agent focuses on animate external agents quickly before eventually ``losing interest'' as prediction accuracy is achieved. Strong animate attention emerges for $7/7$ behaviors when using $\gamma$-Progress. Please see appendix~\ref{app:further_attention_analysis} for a more in-depth of analysis of how attention, and particular early attention, predicts performance and how curiosity signal predicts attention. 

\vspace{-10pt}
\begin{table}[h]
    \caption{
    \textbf{Failure modes} Fraction of indifference and white noise failures, out of eight external agent behaviors.
    }
    \label{table:failure_modes}
    \begin{center}
    \begin{small}
    \begin{sc}
    \begin{tabular}{lcc}
    \toprule
    & Indifference & Noise Fixation \\
    \midrule
    $\gamma$-Progress & \textbf{0/8} & \textbf{0/8} \\
    $\delta$-Progress & 7/8 & 0/8 \\
    RND & 2/8 & 4/8 \\
    Disagreement & 0/8 & 7/8 \\
    Adversarial & 0/8 & 8/8 \\
    \bottomrule
    \end{tabular}
    \end{sc}
    \end{small}
    \end{center}
    \vspace{-5pt}
\end{table}

Baselines display two distinct modes that lead to lower performance (Table~\ref{table:failure_modes}). The first is \textit{attentional indifference}, in which it finds no particular external agent interesting --- more precisely, we say that an curiosity signal choice displays attentional indifference if its average animate/inanimate ratio in the Mixture world is within two standard deviations of Random policy's. $\delta$-Progress frequently had attentional indifference as the new and old world model, separated by a fixed time difference, were often too similar to generate a useful curiosity signal.

The second failure mode is \textit{white noise fixation}, where the observer is captivated by the noise external agents --- more precisely, we say that a curiosity signal choice displays white noise fixation if its average animate/inanimate ratio in the Noise world is more than two standard deviations below Random policy's. RND suffers from white noise fixation due to the fact that our noise behaviors have the most diffuse visited state distribution. We also observe that for noise behaviors, a world model ensemble does not collectively converge to a single mean prediction, and as a result Disagreement finds the noise behavior highly interesting. Finally, the Adversarial baseline fails since noise behaviors yield the highest prediction errors. The white noise failure mode is particularly detrimental to sample complexity, with RND, Disagreement, and Adversarial, as evidenced by their below-Random performance in the Noise world.


==> icml_sections/experiments_scrap.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/attention.pdf}
    \vspace{-15pt}
    \caption{\textbf{Attention Patterns in Mixture World}. The bar plot shows the total animate attention, which is the ratio between the number of time steps an animate external agent was visible and the number of time steps a noise external agent was visible. The plots in the zoom-in box show the real time differences between mean attention to the animate external agents and the mean of attention to the noise agents in a 500 time step window. Results are averaged across 5 runs. $\gamma$-Progress displays strong animate attention while baselines are either indifferent, e.g $\delta$-Progress, or fixating on white noise, e.g Adversarial.} 
    \label{fig:attention}
    \vspace{-10pt}
\end{figure*}

\section{Results}
\label{sec:experiments}
%%%%%%%%%%%% Summary of what we seek to show %%%%%%%%%%%%%%

We evaluate the AWML performance of $\gamma$-Progress on two metrics: \emph{end performance} and \emph{sample complexity}. End performance is the inverse of the the final world loss after a larger number of environment interactions, and intuitively measures the ``consistency'' of the proxy reward with respect to the true reward. Sample complexity measures the rate of reduction in world model loss $\LL(\theta, \mu)$ with respect to the number of environment interactions. The samples from the validation distribution $\mu$ correspond to core validation cases we crafted for each behavior. On the reaching behaviors, for example, we validate the world model loss with objects spawned at new locations. For details on each behavior-specific validation case, we refer readers to Appendix \ref{app:validation}. 

Experiments are run in two virtual worlds: Mixture and White Noise. In the Mixture world, the virtual environment is instantiated external agents spanning four representative types: static, periodic, noise, and animate. This set up is a natural distillation of a real-world environment containing a wide spectrum of behaviors. In the White Noise world, the environment is instantiated with three noise agents and one animate agent. This world strain tests the white noise robustness of $\gamma$-Progress. We compare the AWML performance the following methods: 

\textbf{$\gamma$-Progress (Ours)} is our proposed variant of progress curiosity which chooses $\theta_{old}$ to be a geometric mixture of all past models as in Eq. \ref{eq:mix_progress}. 

\textbf{$\delta$-Progress \citep{achiam2017surprise, graves2017automated}} is the $\delta$-step learning progress reward from Eq. \ref{eq:kstep_progress} with $\delta = 1$. We found that any $\delta > 3$ is impractical due to memory constraints.  

\textbf{RND \citep{burda2018exploration}} is a novelty-based method that trains a predictor neural net to match the outputs of a random state encoder. States for which the predictor networks fails to match the random encoder are deemed ``novel'', and thus receive high reward. 

\textbf{Disagreement \citep{pathak2019disagreement}} is the disagreement based method from Eq. \ref{eq:disagreement} with $N = 3$ ensemble models. We found that $N > 3$ is impractical due to memory constraints.  

\textbf{Adversarial \citep{stadie2015predictive, pathak2017inverse}} is the prediction error based method from Eq. \ref{eq:adversarial}. We use the $\ell_{2}$ prediction loss of the world model as the reward. 

\textbf{Random} chooses actions uniformly at random among the 9 possible rotations. 

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\textwidth]{figures/sample_complex.pdf}
%     \caption{\textbf{AWML Performance in White Noise World}. Results shown for eight experiments in mixture worlds with the animate external agent varied according to the column labels. End performance (top row) is measured as the average of the last 4 validation losses. Sample complexity plots (bottom row) show validation losses evaluated every 5000 environment steps. Error bars/regions are computed over 5 seeds. $\gamma$-Progress achieves lower sample complexity than baselines on $8/8$ behaviors. Baselines frequently perform worse than the Random baseline due to white noise fixation.}
%     \label{fig:sample_complexity}
% \end{figure}

\subsection{AWML Performance}
Fig.~\ref{fig:sample_complexity} shows end performance (first row) and sample complexity (second row) in the Mixture world. The validation loss $\LL(\theta, \mu)$ is averaged across the static, periodic, and animate external agents  The animate external agents are varied amongst the deterministic and stochastic versions of reaching, chasing, peekaboo, and mimicry agents (see Section \ref{sec:environment}). We see that $\gamma$-Progress has lower sample complexity than Disagreement, Adversarial, and Random baselines on all $8/8$ behaviors and outperforms RND and $\delta$-Progress on $7/8$ behaviors while tying on stochastic chasing. We found that \emph{$\gamma$-Progress obtains $3.4\times, 4.7\times, 6.5\times, 7.5\times, 7.8 \times$ lower mean end performance than $\delta$-Progress, RND, Disagreement, Adversarial, and Random baselines} across behaviors. See \textcolor{blue}{\url{https://bit.ly/2uf7lEY}} for visualizations of model predictions. 

We observed the baselines displaying two different failure modes. The first failure mode is attentional indifference, in which the curious agent finds no particular external agent in the environment interesting, and as a result its attentional patterns are similar to a random policy. The resulting AWML performance is similar to that of the Random baseline, e.g $\delta$-Progress and RND on the stochastic peekaboo behavior. The second failure mode is white noise fixation which is more detrimental to performance as the attention is heavily directed towards the noise external agents, e.g Adversarial and Disagreement baselines on the deterministic chasing behavior. We discuss this failure mode in more detail in the White Noise world experiments. \ms{Are we already explaining how attention affects performance here? If so should we refer readers to the attention figure?}  

We observed that Disagreement, Adversarial, RND, and $\delta$-Progress exhibit the indifference failure mode on $1/8, 2/8, 2/8, 6/8$ behaviors respectively, performing similar to the Random baseline, and the white noise failure mode on $4/8, 5/8, 2/8, 0/8$ behaviors, performing worse than the Random baseline. In particular, we observed that $\delta$-Progress frequently led to attentional indifference as the reward was not optimistic enough to anticipate future progress on the animate behaviors, i.e the new and old world model performances were similar. Similarly, we saw that $\gamma$-Progress led to attentional indifference when using a value of $\gamma$ that was too small. We thus found that the tractable memory usage of $\gamma$-Progress is key to achieving high AWML performance, as it enables flexible tuning of the progress horizon parameter.

%%%%%%%%%%%%%%%%%%%%%% Active Learning Metric %%%%%%%%%%%%%%%%%%%%%%%%%
Fig.~\ref{fig:sample_complexity} shows end performance (first row) and sample complexity (second row) in the white noise setup. The animate external agents are varied amongst the deterministic and stochastic versions of reaching, chasing, peekaboo, and mimicry agents. We see that $\gamma$-Progress has lower sample complexity than RND, Disagreement, and Adversarial baselines on all $8/8$ behaviors and outperforms $\delta$-Progress on $6/8$ behaviors while tying on the two peekaboo behaviors. We found that \emph{$\gamma$-Progress obtains $2.3\times, 4.6\times, 4.3\times, 7.2\times, 3.7\times$ lower mean end performance than $\delta$-Progress, RND, Disagreement, Adversarial, and Random baselines} across behaviors. 

We also found that the Random baseline obtains $1.9\times, 2.1\times, 3.4\times$ lower sample complexity than RND, Disagreement, Adversarial. This critical failure of the RND, Disagreement, and Adversarial baselines is due to white-noise fixation, i.e. the curiosity signals worsens AWML performance by driving the attention towards the unlearnable noise behavior which in turn reduces the number of data samples for learnable behaviors. In Fig. \ref{fig:attention}, we see that strong attention to the noise external agent emerges when using RND, Disagreement, and Adversarial methods. In particular, the zoom-in plots show that RND, Disagreement, and Adversarial methods attend to the noise agent significantly more than the Random baseline. RND suffers from white noise due to the fact that our noise behaviors have the most diffuse visited state distribution. We also observe that for complex noise behaviors \ms{do you mean the two-agent noise behavior?} the ensemble models do not collectively converge to a single mean prediction, and as a result finds the noise behavior highly interesting. Finally, the Adversarial baseline fails since noise behaviors yield the highest prediction errors. $\delta$-Progress outperforms the Random baseline by achieving $1.7\times$ lower AUC, but falls behind $\gamma$-Progress for the reasons described in the previous section. 

$\delta$-Progress does not suffer from white noise fixation, but exhibits attentional indifference, as shown by the similarity of its attention patterns to the Random baseline. We similarly attribute this to the inevitable usage of a small value of $\delta$, due to memory constraints. On the other hand, strong animate attention emerges for $7/7$ behaviors when using $\gamma$-Progress. In particular we observe that the animate attention arises accutely early on and eventually decays once the animate behavior is learned by the world model. The strong animate attention enables the curious agent to collect more samples of complex behaviors and thus more quickly reduce world model loss. 




==> icml_sections/introduction.tex <==
\section{Introduction} 
\label{sec:introduction}

% - Different example (has to show world models are important, large number of stimuli with diverse dynamics)
% - World models (definition, importance) 
% - Explain different types of stimuli, sparseness 
% - Active World Model Learning 
% - In this work... curious neural agent performing AWML... in 3D world environment (restricting to gaze control?)
% - Gamma Progress (only a problem when you start doing AWML) -- which solves white noise 
% - Explain each section 

% Add section for cognitive science (meg), change links 
% Intro should point out theory (also abstract 
% take out 


Imagine yourself as an infant in your parent's arms, sitting on a playground bench. You are surrounded by a variety  of potentially interesting stimuli, from the constantly whirring merry-go-round, to the wildly rustling leaves, to your parent's smiling and cooing face.
After briefly staring at the motionless ball, you grow bored. 
You consider the merry-go-round a bit more seriously, but its periodic motion is ultimately too predictable to keep your attention long. 
The leaves are quite entertaining, but after watching their random motions for a while, your gaze lands on your parent. Here you find something really interesting: you can anticipate, elicit, and guide your parents' changes in expression as you engage them in a game of peekaboo. 
Though just an infant, you have efficiently explored and interacted with the environment, in the process gaining strong intuitions about how different things in your world will behave. 

% Though you are just an infant, you have gained strong intuitions about how the different things in your world will likely behave, and about how to allocate your precious attention to the truly relevant stimuli. But how have you learned to make sense of this blooming and buzzing confusion? 
% A fundamental hypothesis is that you have learned a powerful \emph{world model} --- a self-supervised predictive model of how the world evolves, both due to its intrinsic dynamics and your actions --- that guides both prediction and attention allocation. 
Here, you have learned a powerful \emph{world model} --- a self-supervised predictive model of how the world evolves, both due to its intrinsic dynamics and your actions.
Through learning world models, humans acquire compact abstractions of high bandwidth sensory inputs, the ability to plan across long temporal horizons, and the capacity to anticipate the behavioral patterns of other agents. 
Devising algorithms that can efficiently construct such world models is an important goal for the next generation of socially-integrated AI and robotic systems.

A key challenge in world model learning is that real-world environments contain a diverse range of dynamics with varying levels of learnability. 
The inanimate ball and periodic merry-go-round display dynamics that are easy to learn. 
On the other end of the spectrum, stimuli such as falling leaves exhibit random noise-like dynamics. 
Lying in a ``sweet spot'' on this spectrum are animate agents that have interesting and complex yet learnable dynamics, e.g. your parent's expressions and play offerings. 
Balancing attention amidst a sea of stimuli with diverse dynamics in a way that maximizes learning progress is a challenging problem. Particularly difficult is the \emph{white noise problem} ~\citep{schmidhuber_formaltheoryoffun, pathak2017inverse, burda2018exploration, pathak2019disagreement}, perseverating on unlearnable stimuli rather than pursuing learnable dynamics.
Thus, it is a natural hypothesis that behind the infant's ability to learn powerful world models must be an equally powerful \emph{active learning} algorithm that directs its attention to maximize learning progress. 

In this work, we formalize and study Active World Model Learning (AWML) -- the problem of determining a directed exploration policy that enables efficient construction of better world models. To do so, we construct a progress-driven curious neural agent performing AWML in a custom-built 3D virtual world environment. Specifically, our contributions are as follows:

\begin{enumerate}
    \item We construct a 3D virtual environment rich with agents displaying a wide spectrum of realistic stimuli behavior types with varying levels of learnability, such as static, periodic, noise, peekaboo, chasing, and mimicry.
    \item We formalize AWML within a general reinforcement learning framework that encompasses curiosity-driven exploration and traditional active learning. 
    \item We propose an AWML system driven by $\gamma$-Progress: a novel and scalable learning progress-based curiosity signal. We show that $\gamma$-Progress gives rise to an exploration policy that 
    overcomes the white noise problem and achieves significantly higher AWML performance than state-of-the-art exploration strategies — including Random Network Distillation (RND) \citep{burda2018exploration} and Model Disagreement \citep{pathak2019disagreement}.
\end{enumerate}

% Our evaluations show that $\gamma$-Progress achieves significantly higher AWML performance than baseline controllers equipped with state-of-the-art exploration strategies — including Random Network Distillation (RND) \citep{burda2018exploration} and Model Disagreement \citep{pathak2019disagreement}.

% \sj{I think what could make the introduction more detailed is some intuition of why the proposed exploration strategy solves the problem you mentioned i.e. find interesting things to learn on. Otherwise, the advertisement of good performance in this paragraph aren't too convincing until people have seen either details of the method, or concrete the experimental results.}
% We begin in Section~\ref{sec:relatedworks}  by drawing connections to related works in cognitive science and artificial intelligence. In Section~\ref{sec:environment}, we describe our virtual environment in detail, including the range of inanimate and animate agents that we embed in it. Section~\ref{sec:theory} provides a novel mathematical formalization of Active World Model Learning  that our curious agent is tasked with and  motivates progress curiosity in the context of previously proposed curiosity signals. Section~\ref{sec:methods} details the implementations for all components of our curious active learning agent. Finally, Section~\ref{sec:experiments} presents experimental evaluations showing that our progress-driven controller achieves significantly higher AWML performance than baseline controllers equipped with state-of-the-art exploration strategies — including Random Network Distillation (RND) \citep{burda2018exploration} and Model Disagreement \citep{pathak2019disagreement}.

% \sj{A general comment is that it probably helps to clarify the contribution into different parts. I was initially confused whether the main contribution was the $\gamma$-progress objective. But it seems that proposing the environment and the learning problem is also major. (That was only obvious to me after seeing section 3). Also I was confused in the introduction about the relationship between the learning problem you propose (AWML) and the solution (agent) you propose. Is the agent the only way to perform optimally, or is it just one way to perform well. If the learning problem (AWML) and the solution are separate contributions, then it probably helps to clearly separate them.
% For example, the intro could have two or more paragraphs, one for each contribution.}

==> icml_sections/introduction_scrap.tex <==
\section{Introduction} 
\label{sec:introduction}

Imagine yourself as a child at a busy playground. You are surrounded by a cornucopia of potentially interesting stimuli, from the leaves rustling along the ground, to the kickball lying abandoned in the sandbox, to the group of other children playing hide and seek in the far yard.
What would you like to do with your play time?   
After staring at the leaves briefly, you grow bored of watching their random motions. You then consider the kickball a bit more seriously --- dribbling and maneuvering it around by yourself could be pretty fun.  But you keep looking back to the hide-and-seekers, drawn by their dynamic moves and complex interplay.  You'll probably go join these other children, at least if you can succeed in convincing them to let you in on their game. 
Amongst this blooming and buzzing confusion, you have strong intuitions about which activities are the most exciting, about how to allocate your limited attention and time. 
This simple scenario exemplifies how humans continually engage in intrinsically-motivated exploration and interaction, a process whose strong naturally-emergent rules are especially salient for balancing attention between inanimate and animate objects~\citep{premack1990infant, gergely1995taking, frankenhuis2013infants}.
But how does this attentional control process occur?  And equally important, why does it occur --- what functional goals does it subserve? 

A fundamental underlying clue is that in the playground scenario, you are  continually learning \emph{world models} --- self-supervised predictions of what the dynamics of the world will bring, both due to its intrinsic dynamics and in response to your actions. 
Through learning world models, humans may acquire compact abstractions of high bandwidth sensory inputs, the ability to plan across long temporal horizons, and an understanding of the behavioral patterns of other agents. 
It is a natural hypothesis that attentional control is a core active learning mechanism enabling the agent to construct better and more robust world models. 
Conversely, better world models enable more effective attentional allocation.  The hide-and-seek game may perhaps be the most engaging option on the playground precisely because it presents the most sophisticated world-model prediction problems -- not unpredictable like the motions of the leaves in the wind, but involving complex inter-agent contingencies that are not as readily found in solo object-centric play. 

Discovering and formally describing the principles underlying such rich interactive scenarios is a key question in computational cognitive psychology. By the same token, devising algorithms that can learn effective world models in unfamiliar circumstances and use them to generate \emph{de novo} natural interactive behaviors is an important challenge for the next generation of socially-integrated AI and robotic systems.
In this work, we contribute to studying these questions by building neural network models of an agent embedded in a custom-built 3D virtual world environment, rich with external agents displaying a wide spectrum of realistic animate behaviors such as peekaboo, chasing, and mimicry. We show that, with proper choice of intrinsic motivation, an attention policy that distinguishes between animate and inanimate behavior emerges organically, without having to be hard-coded. In turn, by spending time on useful scenarios in a balanced fashion, this naturally ``socially-aware'' agent ends up learning world models more effectively and efficiently than alternatives. 

% meg said: we never really talk about the propensity for animate attention in humans (only mentioning the need to balance attention between inanimate and animate objects) and how that leads to more efficient world modeling - I guess it is implicitly conveyed in the sentence about how hide-and-seek game is the most engaging option, but it's just not as explicit as it should be, I think. - or the explicit explanation comes too late in the intro 

%meg said: I understand that this particular order of the last two sentences mirrors the order of the first two paragraphs. I wonder though whether it makes sense to reverse the order here to emphasize that the primary objective is world models and from it arises attention. Here, we don't have the issue of world models being hard to relate to as a real-world scenario so this order could work.
%dan replies: yes, but what I've described here is the actual "causal" pathway.  plus we want the paragraph to end on the most important thing (rather than have it be an intermediate sentence)
% meg replies: makes sense. 

In building an agent with these capabilities, we found it necessary to address the well-known ``white noise problem'', a potential failure mode of intrinsic motivation that has been acknowledged in many prior works~\citep{schmidhuber_formaltheoryoffun, pathak2017inverse, burda2018exploration, pathak2019disagreement}. An active learner must arbitrate between the combinatorially large number of stimuli exhibiting dynamic behaviors with various levels of learnability. The simplest objects in an environment are static, and easy to learn.  Inanimate objects with some reliable dynamics, e.g., a machine exhibiting periodic rotation, make the situation more complex, pressing on the intrinsic motivation to better distinguish interesting from uninteresting dynamics.  The problem is especially acute, however, for dynamics that are inherently unlearnable or chaotic e.g., falling leaves, wavering trees, and splashing water.  Distinguishing these from those that have interesting and complex yet learnable dynamics, e.g. children playing hide-and-seek turns out to be an especially difficult version of the white noise problem, one which is not effectively handled by recent curiosity approaches.  To solve it, we develop a novel variant of progress-driven curiosity, which we term ``$\gamma$-Progress'', that is able to robustly estimate learning progress in a computationally scalable fashion. 

%dan said: this paragraph, especially the end, needs for that will have to wait til we actually finish getting the results. 
%julian said: Can related works be section 1? It seems awkard to say that we begin in section 2}
%dan replies: it's "typical practice" in the AI literature to numner the sections this way.  but let's worry about this when we actually finalize this paragraph later
We begin in Section~\ref{sec:relatedworks}  by drawing connections between our work and related works in cognitive science and artificial intelligence. In Section~\ref{sec:environment}, we describe our virtual environment in detail, including the range of inanimate and animate agents that we embed in it. Section~\ref{sec:theory} mathematically formalizes the active learning problem that our curious agent is tasked with and  motivates progress curiosity in the context of previously proposed curiosity signals. Section~\ref{sec:methods} details the implementations for all components of our curious active learning agent. Finally, Section~\ref{sec:experiments} presents experimental evaluations showing that our progress-driven controller achieves significantly lower online sample complexity than baseline controllers equipped with state-of-the-art exploration strategies — including Random Network Distillation (RND) (Burda et al., 2018b) and Model Disagreement (Pathak et al., 2019).



\begin{comment}
Old version
Imagine yourself as a child at a busy playground. You are surrounded by a cornucopia of potentially interesting stimuli, from the leaves rustling along the ground, to the kickball lying abandoned in the sandbox, to the group of other children playing hide and seek in the far yard.
What would you like to do with your play time?   
After staring at the leaves briefly, you grow bored of watching their random motions. You then consider the kickball a bit more seriously --- dribbling and maneuvering it around by yourself could be pretty fun.  But you keep looking back to the hide-and-seekers, drawn by their dynamic moves and complex interplay.  You'll probably go join these other children, at least if you can succeed in convincing them to let you in on their game. 
Amongst this blooming and buzzing confusion, you have strong intuitions about which activities are the most exciting, about how to allocate your limited attention and time. 
This simple scenario exemplifies how humans continually engage in intrinsically-motivated exploration and interaction, a process whose strong naturally-emergent rules are especially salient for balancing attention between inanimate and animate objects~\citep{premack1990infant, gergely1995taking, frankenhuis2013infants}.
But how does this attentional control process occur?  And equally important, why does it occur --- what functional goals does it subserve? 

A fundamental underlying clue is that in the playground scenario, you are  continually learning \emph{world models} --- self-supervised predictions of what the dynamics of the world will bring, both due to its intrinsic dynamics and in response to your actions. 
Through learning world models, humans may acquire compact abstractions of high bandwidth sensory inputs, the ability to plan across long temporal horizons, and an understanding of the behavioral patterns of other agents. 
It is a natural hypothesis that attentional control is a core active learning mechanism enabling the agent to construct better and more robust world models. 
Conversely, better world models enable more effective attentional allocation.  The hide-and-seek game may perhaps be the most engaging option on the playground precisely because it presents the most sophisticated world-model prediction problems -- not unpredictable like the motions of the leaves in the wind, but involving complex inter-agent contingencies that are not as readily found in solo object-centric play. 

Discovering and formally describing the principles underlying such rich interactive scenarios is a key question in computational cognitive psychology. By the same token, devising algorithms that can learn effective world models in unfamiliar circumstances and use them to generate \emph{de novo} natural interactive behaviors is an important challenge for the next generation of socially-integrated AI and robotic systems.
In this work, we contribute to studying these questions by building neural network models of an agent embedded in a custom-built 3D virtual world environment, rich with external agents displaying a wide spectrum of realistic animate behaviors such as peekaboo, chasing, and mimicry. We show that, with proper choices of architecture and intrinsic motivation, an attention policy that distinguishes between animate and inanimate behavior emerges organically, without having to be hard-coded. In turn, by spending time on useful scenarios in a balanced fashion, this naturally ``socially-aware'' agent ends up learning world models more effectively and efficiently than alternatives. 

% meg said: we never really talk about the propensity for animate attention in humans (only mentioning the need to balance attention between inanimate and animate objects) and how that leads to more efficient world modeling - I guess it is implicitly conveyed in the sentence about how hide-and-seek game is the most engaging option, but it's just not as explicit as it should be, I think. - or the explicit explanation comes too late in the intro 

%meg said: I understand that this particular order of the last two sentences mirrors the order of the first two paragraphs. I wonder though whether it makes sense to reverse the order here to emphasize that the primary objective is world models and from it arises attention. Here, we don't have the issue of world models being hard to relate to as a real-world scenario so this order could work.
%dan replies: yes, but what I've described here is the actual "causal" pathway.  plus we want the paragraph to end on the most important thing (rather than have it be an intermediate sentence)
% meg replies: makes sense. 

In building an agent with these capabilities, we found it necessary to address two key algorithmic challenges. The first challenge is the well-known ``white noise problem'', a potential failure mode of intrinsic motivation that has been acknowledged in many prior works~\citep{schmidhuber_formaltheoryoffun, pathak2017inverse, burda2018exploration, pathak2019disagreement}. An active learner must arbitrate between the combinatorially large number of stimuli exhibiting dynamic behaviors with various levels of learnability. The simplest objects in an environment are static, and easy to learn.  Inanimate objects with some reliable dynamics, e.g., a machine exhibiting periodic rotation, make the situation more complex, pressing on the intrinsic motivation to better distinguish interesting from uninteresting dynamics.  The problem is especially acute, however, for dynamics that are inherently unlearnable or chaotic e.g., falling leaves, wavering trees, and splashing water.  Distinguishing these from those that have interesting and complex yet learnable dynamics, e.g. children playing hide-and-seek turns out to be an especially difficult version of the white noise problem, one which is not effectively handled by recent curiosity approaches.  To solve it, we develop a novel variant of progress-driven curiosity, which we term ``$\gamma$-progress'', that is able to robustly estimate learning progress in a computationally scalable fashion. 
%julian said: I'm wondering whether we should have a name for this second algorithmic challenge, so that we can refer to it later on, e.g., 'the animate detection problem'
%meg said: I think Dan meant that the first algorithmic challenge is white noise problem and second algorithm challenge is causal confusion (in the next paragraph), and animate detection problem is a consequence of white noise problem
%dan replies: @meg: exactly.  @jdf: why is this the second challenge? it's the first. and it's called the "white noise" problem.

%julian said: The following paragraph needs more work, and I think should refer to an example we raise in the introductory scenario, e.g., You initially think that one of the children is inspecting something on the tree, but then realize that she is using the tree to shield her field of view as the other children run to their chosen hiding spots. Could we make the examples here just a tad more specific, so that people really get it?  I don't think we've  explained what about partial observability contributes to causal confusion, so this may be confusing to readers
The second challenge is that in scenarios with several interacting and independent components (e.g. objects and other agents), world models predicting future dynamics are inherently susceptible to causal confusion --- e.g the mistaking spurious correlations for true causality --- a problem that has recently been recognized in the imitation-learning literature~\cite{}CITE.  
In the playground scenario for example, if two children are initially performing similar calisthenics simultaneously, a causally ill-informed observer might think that the apparent coordination between the two is a sign of an actual underlying causal relationship. %JDF: This example is a bit weird. What about something more ordinary, like you see one kid suddenly run away as another kid crosses over to them, but in fact the kid was running away from another child further a field. Therefore, you might predict that the runner always runs away from the first child, when in fact it was a coincidence. 
Later, if the observer only manages to keep only one of the children in view, they are likely to extrapolate their incorrect causal relationship to make spurious predictions about the unobserved child. %JDF: like what? I don't get it. 
More broadly, causal confusion leads to world models that exhibit poor future generalization performance, which turns out to be especially acute in scenarios like those we investigate, which exhibit only very partial observability from any given view. We endow our curious agent with a \emph{causally-aware world model} that integrates a causal prior into its network architecture to preempt causal confusion, and show that this choice is critical for achieving effective world-model learning.

%dan said: this paragraph, especially the end, needs for that will have to wait til we actually finish getting the results. 
%julian said: Can related works be section 1? It seems awkard to say that we begin in section 2}
%dan replies: it's "typical practice" in the AI literature to numner the sections this way.  but let's worry about this when we actually finalize this paragraph later
We begin in Section~\ref{sec:relatedworks}  by drawing connections between our work and related works in cognitive science and artificial intelligence. In Section~\ref{sec:environment}, we describe our virtual environment in detail, including the range of inanimate and animate agents that we embed in it. Section~\ref{sec:theory} mathematically formalizes the active learning problem that our curious agent is tasked with, motivates progress curiosity in the context of previously proposed curiosity signals, and characterizes the causal confusion problem. Section~\ref{sec:methods} details the implementations for all components of our curious active learning agent. Finally, Section~\ref{sec:experiments} presents experimental evaluations of our curious active learning system on two quantitative metrics: We show that (1) injecting a causal prior is essential to attaining high offline asymptotic model performance, and (2) our progress-driven controller achieves significantly lower online sample complexity than baseline controllers equipped with state-of-the-art exploration strategies — including Random Network Distillation (RND) (Burda et al., 2018b) and Model Disagreement (Pathak et al., 2019). Furthermore, when varying both the intrinsic motivation signal (considering several baselines) and world model architecture (with causal structure prior, and without), we find that the intrinsic motivation signal drives behavior, whereas the difference in world model architecture modulates behavior to a lesser degree.
\end{comment}

==> icml_sections/methods.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/sample_complex.pdf}
    \vspace{-15pt}
    \caption{\textbf{AWML Performance}. The animate external agent is varied across experiments according to the column labels. End performance is the mean of the last five validation losses. Sample complexity plots show validation losses every 5000 environment steps. Error bars/regions are standard errors of the best $5$ seeds out of $10$. (a). \emph{Mixture World}: $\gamma$-Progress achieves lower sample complexity than all baselines on $7/8$ behaviors while tying with RND on stochastic chasing. Notably, $\gamma$-Progress also outperforms all baselines in end performance on $6/8$ behaviors. (b). \emph{Noise World}: $\gamma$-Progress is more robust to white noise than baselines and achieves lower sample complexity and higher end performance on $8/8$ behaviors. Baselines frequently perform worse than random due to noise fixation}
    \label{fig:sample_complexity}
    \vspace{-10pt}
\end{figure*}

\section{Methods}
\label{sec:methods}
In this section we describe practical instantiations of the two components in our AWML system: a {\em world model} which fits the forward dynamics and a {\em controller} which chooses actions to maximize $\gamma$-Progress reward. See Appendix \ref{sec:app:training_details} for full details on architectures and training procedures.  

\textbf{World Model} As the focus of this work is not to resolve the difficulty of representation learning from high-dimensional visual inputs, we assume that the agent has access to an oracle encoder $e: \O \rightarrow \X$ that maps an image observation $\rvo_t \in \O$ to a disentangled object-oriented feature vector $\rvx_t = (\rvx_{t}^{ext}, \rvx_{t}^{aux}, \rvx_t^{ego})$ where $\rvx_{t}^{ext} = (\tilde{\rvc}_{t}, \rvm_{t}) = (\tilde{\rvc}_{t, 1}, \ldots \tilde{\rvc}_{t, n_{ext}}, \rvm_{t, 1}, \ldots ,\rvm_{t, n_{ext}})$ contains information about the external agents; namely the observability masks $\rvm_{t, i}$ ($\rvm_{t, i} = 1$ if external agent $i$ is in curious agent's view at time $t$, else $\rvm_{t, i} = 0$) and masked position coordinates $\tilde{\rvc}_{t, i} = \rvc_{t, i}$ if $\rvm_{t, i} = 1$ and else $\tilde{\rvc}_{t, i} = \hat{\rvc}_{t, i}$. Here, $\rvc_{t, i}$ is the true global coordinate of external agent $i$ and $\hat{\rvc}_{t, i}$ is the model's predicted coordinate of external agent $i$ where $i = 1, \ldots , n_{ext}$. Note that the partial observability of the environment is preserved under the oracle encoder since it provides coordinates only for external agents in view. $\rvx_{t}^{aux}$ contains coordinates of auxiliary objects, and $\rvx_t^{ego}$ contains the ego-centric orientation of the curious agent. 

\begin{algorithm}[t]
\caption{AWML with $\gamma$-Progress} \label{prog_cur}
\textbf{Require:} progress horizon $\gamma$, step sizes $\eta_{\omega}, \eta_{Q}$ \\ 
Initialize $\theta_{new}, \phi$\\
\For{$k = 1, 2, ...$}{
    Update policy: $\pi_{\phi} \leftarrow \epsilon\text{-}greedy(Q_{\phi}, \epsilon - 0.0001)$ \\
    Sample $(\rvx, \rva, c) \sim \pi_{\phi}$ and place in Buffer $\mc{B}$ \\
    where $c = \LL(\theta_{new}, \rvx, \rva) - \LL(\theta_{old}, \rvx, \rva)$ \\
    \For{$j = 1, ..., M$}{ 
        Sample batch $b_{j} \sim \mc{B}$ 
        
        Update new world model: \\ 
        $\theta_{new} \leftarrow \theta_{new} - \eta_{\omega} \cdot \nabla_{\theta_{new}}\LL(\theta_{new}, b_{j})$

        Update old world model: \\
        $\theta_{old} \leftarrow \gamma \theta_{old} + (1 - \gamma) \theta_{new}$ 

        Update Q-network with DQN \citep{mnih2015human}: \\
        $\phi \leftarrow \text{DQN}(\phi, b_{j}, \eta_{Q})$
    }
}
\label{alg:awml}
\end{algorithm}
Our world model $\omega_{\theta}$ is an ensemble of component networks $\{\omega_{\theta^{k}}\}_{k = 1}^{N_{\mathrm{cc}}}$ where each $\omega_{\theta^{k}}$ independently predicts the forward dynamics for a subset $I_{k} \subseteq \{1, ..., \text{dim}(\rvx^{ext})\}$ of the input dimensions of $\rvx^{ext}$ corresponding to a minimal behaviorally interdependent group. For example, $\rvx^{ext}_{t:t+\tau, I_{k}}$ may correspond to the masked coordinates and observability masks of the chaser and runner external agents for times $t, t+1, ..., t+\tau$. We found that such a "disentangled" architecture outperforms a simple entangled architecture (see Appendix \ref{sec:app:wm_architecture} for details). We assume $\{I_{k}\}_{k = 1}^{n_{cc}}$ is given as prior knowledge but future work may integrate dependency graph learning into our pipeline. A component network $\omega_{\theta^{k}}$ takes as input $(\rvx^{ext}_{t - \tau_{in} : t, I_{k}}~,~\rvx^{aux}_{t - \tau_{in} : t}~,~\rvx^{ego}_{t - \tau_{in} : t}~,~\rva_{t - \tau_{in} : t + \tau_{out}})$, where $\rva$ denotes the curious agent's actions, and outputs $\hat{\rvx}^{ext}_{t : t + \tau_{out}, I_{k}}$. The outputs of the component network are concatenated to get the final output $\hat{\rvx}^{ext}_{t : t + \tau_{out}} = (\hat{\rvc}_{t:t+\tau_{out}}, \hat{\rvm}_{t:t+\tau_{out}})$. The world model loss is:  
\begin{align*}
    \LL(&\theta, \rvx_{t-\tau_{in}:t+\tau_{out}}, \rva_{t-\tau_{in}:t+\tau_{out}}) = \nonumber \\ &\sum_{t' = t}^{t + \tau_{out}} \sum_{i = 1}^{N_{ext}} \rvm_{t', i} \cdot \|\hat{\rvc}_{t', i} - \tilde{\rvc}_{t', i}\|_2 + \LL_{ce}(\hat \rvm_{t', i}, \rvm_{t', i})
\end{align*}
where $\mathcal{L}_{ce}$ is cross-entropy loss. We parameterize each component network $\omega_{\theta^{k}}$ with a two-layer Long Short-Term Memory (LSTM) network followed by two-layer Multi Layer Perceptron (MLP). The number of hidden units are adapted to the number of external agents being modeled. 

\textbf{The Progress-driven Controller} Our controller $\pi_{\phi}$ is a two-layer fully-connected network with 512 hidden units that takes as input $\rvx_{t-2:t}$ and outputs estimated Q-values for 9 possible actions which rotate the curious agent at different velocities. $\pi_{\phi}$ is updated with the DQN \citep{mnih2013playing} learning algorithm using the cost:
\begin{align}
c(\rvx_{t}) = \LL(\theta&_{new}, \rvx_{t - \tau_{in} - \tau_{out}:t}, \rva_{t - \tau_{in} - \tau_{out}:t}) - \nonumber \\
&\LL(\theta_{old}, \rvx_{t - \tau_{in} - \tau_{out}:t}, \rva_{t - \tau_{in} - \tau_{out}:t})
\end{align}
with $\gamma = 0.9995$ across all experiments. 



% % \ms{Policy architecture}
% Our Q-function architecture is a two-layer fully-connected network with 512 hidden units. At time $t$, it takes as input $\rvx_{t-2:t}$ i.e., external agent data for the most recent 2 time steps, and outputs estimated Q-values for the 9 possible actions. 
% We use () optimizer with a learning rate of () to update the weights. 
% The exploration strategy used was a simple $\epsilon$-greedy strategy with $\epsilon$ decreasing from ... to 0.02 with a decay rate of 0.0002. 

% % \ms{Buffer} 
% The executed trajectories are stored in a replay buffer that can store up to 100000 observations before popping off old transitions in FIFO order. To be able to distinguish between the effects of the different intrinsic motivation signals, world model and policy updates begin after the buffer is filled up with 1000 transitions, while the buffer continues to grow to its capacity of 100000. The policy function is only trained on the most recent 10000 transitions to allow stable Q-function optimization, while the world model is trained on the entire buffer. 




% one buffer - wm trains from entire buffer, q-learning only trained on 1 

% \begin{equation} 
%     r_{\text{progress}}(s_t, a_t, s_{t+1}) = \mathcal{L}(\theta_{old}) - \mathcal{L}(\theta_{new})
% \end{equation} 
% where $\mathcal{L}$ is the $L2$ distance between the observed external agent coordinates and the predicted external agent coordinates (first of the two terms in equation \ref{eq:loss}). 

% At the $k$th iteration of the active learning loop, $\theta_{new}$ is simply equivalent to $\theta_{k}$.
% We initialize $\theta_{old}$ as... \ms{Explain old model start time}
% $
% \theta_{old} = (1 - \beta) \sum_{i=1}^{k-1} \beta^{k-1-i} \theta_0
% $. 

% This is achieved by updating $\theta_{old}$ at every iteration as follows: 
% \begin{equation}
%     \theta_{old} = \beta \theta_{old} + (1-\beta) \theta_{new}
% \end{equation}
% Intuitively, the old model's weights are gradually and continually updated to the new model's weights, such that it always lags behind the new world model's performance but does so in a consistent way. This ``lag'' is controlled by $\beta$; the larger the $\beta$ is, the larger the lag will be. 
% Moreover, observe that because of this lag, the larger the difference between the loss of the old world model and the loss of the new world model is, the more progress the world model has made on the self-supervision problem in recent time steps.

% This intrinsic motivation signal is used directly as the reward of the controller

% We now  describe an instantiation of the ideas previously discussed 
% data collection policy is optimized with this choice 
% We optimize this reward with the Q-learning algorithm (default) and cite 
% Algorithm 
% From theory this is what we wanted to optimize , 




==> icml_sections/relatedwork_scrap.tex <==
\section{Related Works}
\label{sec:relatedworks}

\jdf{I'm starting to wonder whether it makes sense to have divided cognitive science and AI sections. It seems that the narrative at the end of the current cog sci section could just continue into the current AI sections, especially if there continues to be a string of psychological motivations. Currently the sections feel a bit disjointed. At the least we need an explicit statement that links the sections, e.g., talking about how the AI section starts to suggest how the sophisticated statistical learning we talk about at the end of the cog sci section might be implemented.}. 

We draw on cognitive science and ultimately aim to provide cognitive models. People have studied agents modeling their environments in cognitively-plausible ways. Active learning and curiosity have been studied and we add to the program of bringing the active learning of intuitive physics and psychology to artificial systems. 

\subsection{Cognitive science}
\label{sec:related:cognitive}

\noindent\textbf{Object-based attention and object permanence}

Although traditional models characterize attention as a `spotlight' that shines on areas of space, a wealth of work in cognitive science indicates that in many cases the units of attention in space \citep{scholl2001objects} and time \citep{de2014attentional} are distinct, bounded objects, aka \textbf{object-based attention}. Further, when the objects are dynamic, the human attentional system assigns individuated object tokens to each object, in order to keep track of them over time \citep{sears2000multiple}. The well-known limits on attention, then, often concern the maximum number of objects that can be tracked simultaneously, a limit that is thought to arise as multiple objects compete for representation on space-limited cortical real-estate \citep{alvarez2007many}. 

When tracking dynamic objects, the human brain must also deal with momentary disappearances of the objects it is tracking, as when they leave the field of view or become occluded. In such cases, it must solve a correspondence problem: which of the objects that it later sees is the same as the one that it was tracking a moment ago? The human brain appears to solve this problem by maintaining and updating an internal representation of the object even as it goes out of sight \citep{baillargeon1985object}, a phenomenon known as \textbf{object permanence}. This ability appears to rely on additional systems for visual imagery and working memory, which can also be guided by the oculomotor system \citep{de2016tracking, saiki2002multiple}. Working memory, similar to attentional selection, is limited in the number of objects which it can store simultaneously \citep{luck1997capacity}.

In the current work, our modeling framework includes object-based attention, object permanence, and working memory as inductive biases, i.e., knowledge that is built in as a prior of the model. We provide the model with the center coordinates of objects, and require it to predict their future center coordinates. Further, we use a memory system to maintain an active representation of an object whenever it goes out of sight.

\noindent\textbf {Animate attention, prediction, and theory of mind}

Given the limits on attention and memory, the human brain cannot track all of the objects with which it is confronted, and must therefore decide what subset of objects to either automatically or intentionally select for processing. Efficiently determining what to attend to is necessitated by the fact that not all objects are equally rich in information. Of note, in the majority of cases the most information-rich objects tend to be other animate entities, rather than many of the other kinds of entities that also occupy our fields of view, such as objects that are static (e.g., rocks, walls, and buildings), periodic (e.g., fans, wheels), or random (e.g., brownian motion in leaves, water, and the other elements). Unlike random stimuli, the dynamics of animate stimuli are learnable. And unlike static and periodic stimuli, which are either unchanging or repeatable, the spatiotemporal dynamics of animate stimuli contain more complex structures. 

Already as infants, humans are adept at distinguishing between inanimate and animate agents, preferentially paying attention to animate features like faces \citep{maurer2002many} and human body shapes \citep{slaughter2002development}, aka \textbf{animate attention}. Even in the absence of these surface features, infants will preferentially attend to spatiotemporal kinematics indicative of animate agents, such as self-propelled motion \citep{premack1990infant}, efficient movement towards targets \citep{gergely1995taking}, contingent behavior between observed agents, as when one agent chases another \citep{frankenhuis2013infants}, and contingent behavior between an observed agent and the infant herself, as when a robot beeps in response to the infant's babbling \citep{johnson2003detecting, foster1973visual}. In adults, these kinds of kinematics may give rise to an irresistable sense of animacy and intentionality, even when the objects executing the kinematics are simple shapes \citep{heider1944experimental}. In other words, the visual system has been highly tuned to cues that reliably indicate the presence of agents with internal sources of energy that cause them to move without the need for external forces. 

Beyond the ability of infants to discriminate between animate agents and other objects, a more sophisticated ability that emerges later in development is actively interpreting other agents in terms of their underlying mental states (beliefs, desires, and goals) that cause the agents' behavior, aka \textbf{theory of mind} \citep{astington1990developing, premack1978does, wellman1992child}, rather than in terms of physical forces. A theory of mind is needed in order to \textit{predict} what an agent will do next, since often it is only possible to do so accurately by generating expectations about an agent as a function of underlying intentions that are attributed to it. This ability is crucial to social functioning, and the failure to attribute mental states falls under the umbrella of symptoms that define the autism spectrum mental disorders \citep{baron2000theory}.

In the current work, our environment includes inanimate and animate agents with spatiotemporal kinematics inspired from these human experiments, and the agents are deliberately devoid of surface features, so that our modeling agent must discover which agents are interesting and  worth paying attention based on their spatiotemporal properties alone. We task our neural model with learning to discriminate among the different kinds of inanimate and animate agents, based on its ability to learn to predict what they will do next. 

\noindent\textbf {Diverging developmental theories}

Given that the above abilities arise early in human development, some have argued that infants may be born with an already specialized module devoted to representing the mental states of agents \citep{leslie1989autism, leslie1994tomm}. According to one dominant account, such a “theory of mind mechanism” could consist of a hard-wired, set of primitive propositional attitudes about concepts such as “desire” and “belief”. Note also that it is not a problem for this theory that infants are not immediately born with the ability to detect and predict agents, because an innate system could still be programmed to only come online later in life, perhaps triggered by certain environmental inputs \citep{scholl1999modularity}.

At the same time, infants exhibit an impressive ability to learn the statistical regularities in various tasks involving stimuli spanning all modalities, e.g., audition, vision, words \citep{fiser2002statistical, saffran1996statistical, maye2002infant}. As such, an alternative theory states that the bulk of attentional behavior may be driven by a more general-purpose learning mechanism, which allocates attention to stimuli based on their inherent, information-theoretic properties. Under this account, the particular attentional biases that have been characterized in existing work are an inevitable outcome of a smart learning system coming into contact with the different statistical properties of the  stimuli that happen to surround us.

Providing some support for this second view, previous work also finds that infants appear to gather information from environments in a manner that is quite principled: They selectively explore objects that violate their expectations \citep{stahl2015observing}, and they spend little time examining stimuli that are either too simple or too complex; instead, they preferentially attend to stimuli that are sufficiently complex to be interesting but not so complicated that they cannot be predicted \citep{kidd2012goldilocks}.

In the current work, while we do build in inductive biases concerning object-based attention, object-permanence, and working memory, we do not build in a propensity to detect and predict special classes of stimuli. Instead, we test whether reasonable patterns of attention of the form observed in humans can emerge naturally in our model, provided we endow it with a good, general-purpose learning objective. 

%\subsection{AI modeling of physical and social environments}

%While for this work we do not need sophisticated models capable of human-level intuitive physics, much progress has been made along these lines. Intuitive physics approaches: interaction networks, HRN, recent tenenbaum work \cite{This framing makes it sound like you're going to tell the reader about irrelevant stuff; what about framing it as people have focused on modeling the high-level stuff by assuming it exists, but not so much on modeling how you learn that stuff in the first place, using a biologically-plausible architecture.}

%Less progress has been made towards modeling human-level intuitive psychology. Multi-agent learning (relational forward models for multiagent learning), program induction (Human-level concept learning through probabilistic program induction \nh{Is there something newer}?

%In our model architecture, we have created an explicit read/write memory structure useful in predicting the trajectories of animate and inanimate stimuli over modest timescales. NTM, Merlin might embody more generic versions of this ---  one can imagine our explicit structures arising from training within the sorts of environments we consider over long time scales. In our work, we stick with short timescales. \nh{Our contribution here is not as clear, depends on whether we emphasize memory mechanism, or should keep incremental}


%\subsection{Curiosity, multi-task learning, and curriculum learning}

%In order to increase sample efficiency, it is useful for agents gathering data within their own worlds to make smart decisions about what data to capture. Basics of curiosity and intrinsic motivation. Related is classical active learning \cite{settles2011_active, giladbachrach_qbcreal_active} [lots more], in which an agent seeks to minimize the amount of labeling required in order to learn a supervised task.

%Different ways of defining intrinsic motivation, with subtlety of white noise problem
%Prediction Error: \cite{berkeley_mario, haber2018learning, interaction_cogsci}, Stadie.
%Novelty: Pseudocount, RND, Disagreement
%Progress: Schmidhuber, Oudeyer \cite{oudeyer2013intrinsically, oudeyer2007intrinsic}
%Information gain: Prediction Gain, VIME, Surprisal

%Related to curiosity are contexts in which an agent has many possible tasks or a family of tasks and must judiciously choose what to do, when. Curriculum learning, multi-task learning, and goal generation. [Automated Curriculum Learning for Neural Networks] [Control What You Can: Intrinsically Motivated Task-Planning Agent] [Automatic Goal Generation for Reinforcement Learning Agents] \cite{jaderberg2016reinforcement}.

\subsection{Artificial intelligence}

\jdf{What is the story we want to tell in this section?}
\jdf{How about something like this: 
(i) When do we understand the world around us? One idea is that we understand it when we can predict what will happen next. Briefly mention the alternatives (e.g., compression)
(ii) Talk about some psychological evidence that people do this, while gesturing at predictive coding (because we have to).
(iii)Introduce how this problem has been approached in the AI literature.
(iv) But what's missing from these approaches that we think is important?}
\jdf{Currently the content seems to jump around too much. Also, on a minor note, there's a lot of he said she said; can we just talk about the findings, while citing these people parenthetically? I think this puts the focus on the science.}.

\noindent{\textbf{World models concerned with dynamics}}

\jdf{Not sure if we want to cite some of the older biological work related to these ideas, e.g., Rosen R. (1985) Anticipatory systems: Philosophical, mathematical and methodological
foundations. Pergamon Press.}
\jdf{Originator credit? Maybe Gibson? Gibson J. J. (1979) The ecological approach to visual perception. Routledge.}

\jdf{Cites for the (newer idea of) predictive coding: 
Clark A. (2013) Whatever next? Predictive brains, situated agents, and the future of
cognitive science. Behavioral and Brain Science 36:181–204. 
Friston K. (2010) The free-energy principle: A unified brain theory? Nature Reviews
Neuroscience 11:127–38.; Rao R. P. & Ballard D. H. (1999) Predictive coding in the visual cortex: A functional interpretation of some extra-classical receptive-field effects. Nature Neuroscience 2:79–87.}

\jdf{Note that there are broadly two different kinds of predictive 'world' models that seem to battle it out in biology/psychology: (i) sometimes referred to as subjective physics, is the more Gibsonian view, which says that the models are physics models, which take the relations between observables. (ii) predictive coding, which maps internal variables to the observables (e.g., sensory inputs), and so is a 'generative model'. See Brette (2019) BBS- Is coding a relevant metaphor for the brain}.

A natural choice for what to model about one's environment is that of forward dynamics prediction: given a sequence of observations, perhaps along with the planned actions of the observer, predict some number of future observations. \jdf{Not sure why you're suddenly honing in on video frame prediction being hard here; I thought you were going to argue why predicting forward dynamics makes sense}. Video frame prediction \citep{kalchbrenner2016video, finn2016unsupervised} presents immense challenges in producing predictions that are realistic, let alone accurate, although recent innovations in architecture and loss function \citep{lee2018stochastic, wang2018predrnn++, Wu2019ModelIF} have shown considerable improvements. This self-supervised task draws inspiration from the neuroscience theory of \textbf{predictive coding}, and architectural motifs inspired by the neural theory \citep{lotter2016deep} have been shown to produce visual features that support other visual tasks. \jdf{what is an architectural motif exactly?} When conditioned on the actions of the observer, video prediction has shown utility in planning for robotic control tasks \citep{finn2017deep}. Related, \cite{ha2018world} build generative world models of virtual environments and use these ``dream'' environment simulations to train policies. \cite{chua2018deep} enhance performance in reinforcement learning tasks by incorporating calibrated forward dynamics models.

Some of the difficulty of predicting forward dynamics can be obviated by working not with images but in a given latent feature representation. For example, 3D point clouds data has been amenable to the forward dynamics prediction of rigid bodies \citep{byravan2017se3}. Approaches using object-centric, graphical representations of scenes \citep{battaglia2016interaction, chang2016compositional} have grown to be able to predict particulate representations of rigid and soft bodies \citep{mrowca2018flexible}. Coarse, probabilistic object-centric models have the ability to model human expectation violation of intuitive physics \citep{smith2019modeling}. \cite{ke2019learning} incorporate longer-term forward prediction in a latent space in order to enhance performance at reinforcement learning tasks.

Beyond forward dynamics prediction are self-supervised tasks that usefully model the dynamics of environments. Time reversal, in which a model is given an observation or observations and predicts that which preceded, can be used to plan by working backwards from goal states \citep{nair2018time}. \cite{agrawal2016learning} show inverse dynamics prediction, in which a model is given observations of an agent and must recover what actions the agent took, to be useful in robotic manipulation tasks. Networks can also be trained to predict other quantities from video frames, such as the height of an object in free fall, without being given labels of these quantities but rather by using known properties of the output space such as those derived from physics \citep{stewart2017label}.

In our work, we focus on the forward dynamics prediction problem on an object-centric representation of our environment. This representation simply consists of the positions of each object or agent in the environment, lacking other distinguishing features. We thus {\em assume} the agent has access to an encoding giving it this representation. This avoids the dual difficulties of both obtaining these representations from visual features and predicting the dynamics of complex media.

\noindent{\textbf{Active learning}}

\jdf{I still have to read this}

Independently of what is being modeled, the question of what actions to take in order to improve one's model efficiently has long been an important part of machine learning, statistics, and scientific thinking at large. Classically in \textbf{active learning} \citep{settles2011_active}, an agent seeks to learn a supervised task and tries to minimize the number of unlabeled examples it must label (the choice of what to label is the ``action'' of the agent). In doing so, the agent must make use of some signal by which it decides what action to take, with standard techniques including uncertainty sampling \citep{lewis1994heterogeneous}, query by disagreement \citep{cohn1994improving}, query by committee \citep{seung1992query}, error reduction \citep{roy2001toward}, and variance reduction \citep{geman1992neural}. Many of these techniques have been studied thoroughly within statistics, as, if we think of this ``act'' of labeling as deciding which experiment to perform when trying to fit a model or estimate a parameter, we arrive at \textbf{optimal experimental design} \citep{kahn1951estimation, fedorov2013theory, chaloner1995bayesian}.

Modern work on intrinsic motivation and curiosity can be considered a variant of active learning that concerns a reinforcement learning agent with sparse or no extrinsic reward \citep{schmidhuber_formaltheoryoffun, oudeyer2007intrinsic, oudeyer2013intrinsically}. In this, an agent trains a world model, and in taking action, it receives an intrinsic motivation ``reward'' computed using the world model. This intrinsic motivation signal is usually taken to be some estimate of how useful the action and resulting state are at producing an improved world model. In this way, the intrinsic motivation signal can be thought of as analogous to the signals by which more traditional active learning decisions are made, and indeed, many modern techniques take as inspiration the signals used in active learning and optimal experimental design. A number of approaches \citep{stadie2015predictive, interaction_cogsci, haber2018learning} use the world model's \textbf{prediction error}, though these in some contexts can result in the \textbf{white noise problem} in which agents are motivated to take actions that lead to unpredictable examples for the world model. In order to avoid the white noise problem, one can seek to estimate how actions lead to learning \textbf{progress} or \textbf{information gain}. How this is estimated is a core challenge, and many approaches towards estimating learning progress \citep{schmidhuber_formaltheoryoffun, oudeyer2007intrinsic, oudeyer2013intrinsically} or information gain \citep{houthooft_vime} present serious computational challenges when used at scale in complex environments. \textbf{Surprisal} \citep{achiam2017surprise} presents a computationally-tractable alternative to information gain. Model disagreement \cite{pathak2019disagreement}, in which intrinsic motivation is proportional to an ensemble of independently trained world models, presents another computationally-tractable alternative inspired by classical active learning techniques. For comprehensive reviews of intrinsic motivation signal choices, please see \citep{aubret2019survey, linke2019adapting}.

Related approaches rely on a fixed intrinsic motivation objective that does not take into account a specified world model problem. In the context of learning a world model problem, such intrinsic motivations can be thought of as \textbf{novelty} metrics, measuring how much a particular part of the environment has been explored. Examples include count-based exploration \cite{strehl2008analysis}, useful in tabular settings, and generalizations to continuous spaces such as pseudo-counts \citep{bellemare2016unifying} and Neural Density Models \citep{ostrovski2017count}. Certain variants of prediction error-based intrinsic motivation \citep{pathak2017inverse,pathak18largescale} seek to choose judiciously a learned feature space for a forward dynamics world model problem so that white noise issues do not arise. One recent popular approach, Random Network Distillation \citep{burda2018exploration}, takes as intrinsic motivation the prediction error of one neural network trying to match the output of a randomly initialized and frozen network of identical architecture. Related is \textbf{empowerment} \citep{mohamed2015variational}, in which the agent seeks to maximize the mutual information of action and state. \cite{jaderberg2016reinforcement} provides as intrinsic reward auxiliary tasks in order to better performance in sparse reward settings. \cite{kulkarni_hierarchical} combine intrinsic motivation with hierarchical action-value functions operating at different temporal scales, for goal-driven deep reinforcement learning.

The signals exploited in traditional active learning and curiosity have seen broad modern application outside of these classical and sparse reward contexts. \cite{graves2017automated} explore a number of learning progress estimators in order to build a curriculum in a multi-armed bandit setting. \cite{blaes2019control} use several such signals in order to solve several related tasks, some of which build on others, others of which are effectively impossible, providing a multi-task variant of the white noise problem.

It is worth noting how the intent of this work contrasts with several related themes. First, most studies of curiosity study intrinsic reward as either (1) a way to enhance performance at a reinforcement learning task with sparse but present extrinsic reward or (2) a method of encouraging good exploration, as measured by e.g. the amount of territory the agent has seen. In this work, we study curiosity {\em as active learning}, measuring success by improved performance at the world model problem. 

\nh{I took out a mention of attention mechanisms, as it doesn't fit here and is confusing. Any ideas for how to place?}
\ms{I guess our message is that ``attention'' mechansims are \textbf{not} related to this work, so perhaps we could place it somewhere other than related work where we talk about our attention measures to explicitly state that they were different lines of work?}
%Second, on a high level we look to optimize the agent's {\em visual attention} towards learnable stimuli. This, however, is imposed by the environment's strong partial observability at any given time. To contrast, {\em attention mechanisms}, visual or otherwise, seek to reduce the hypothesis space by for a task by directing model attention to limited subsets of observations. \ms{I see how the two  points in the later part of this paragraph correspond to (1) and (2), but it is a little unclear how attentional mechanisms relates to (2) seeing curiosity as a method of encouraging good exploration and especially to the mention of measuring amount of territory agent has seen}
%\nh{Agreed, I think attention comes a little out of left field here...not sure quite where to put it, as we're essentially saying "hey this thing with a name that might remind you of what we're doing is very different. doesn't quite fit the logic of this section or any other. need to think abhout this}

\noindent{\textbf{Multiagent and social learning}}

\nh{I have a note here for Kun Ho to see if there's some particularly salient robosoccer reference}

Environments with multiple artificial agents have been studied in order to optimize their interactions for a goal, understand or see what leads to their emergent behaviors, and exploit in order to train better models. Broadly, the field of multi-agent learning \citep{nguyen2018deep, zheng2018structured} concerns the coordination and communication of multiple agents within an environment in order to solve a reinforcement learning task. \cite{jaques2019social} explores the use of causal influence of one agent on another as intrinsic motivation to learn policies across agents in a decentralized manner. Of particular salience to our proposed world model architecture, \cite{tacchetti2018relational} learn a shared relational forward model, representing a network of relationships between agents, in order to boost performance at a multi-agent learning task. \cite{rabinowitz2018machine} demonstrate the use of a ``Theory of Mind'' neural network architecture that models behaviors in a gridwork environment.

Multi-agent systems can be studied not only through the lens of coordination in order to solve reinforcement learning tasks, but also through competition. \cite{baker2019emergent} study the emergence of interesting behaviors such as the use of tools in competitive multi-agent environments. \cite{vinyals2019grandmaster} use many agents pitted against each other in order to refine policies in the competitive strategy game setting of Starcraft II.

Robotics has been extended beyond multi-agent artificial environments and into social environments by developing predictive models of human behavior and using those to interact with people accordingly. A series of work on a social robot Jackrobbot \citep{ballan2016knowledge, robicquet2016learning, sadeghian2019sophie} uses human behavioral data in order to navigate real-world environments with both physical constraints and humans. \cite{kleinsurprise} learn predictive models of infant visual attention, aimed at designing robots that manipulate and encourage attention.

In the present work, we study the intrinsic motivations that lead to effective policies for, and the world model architectures that can enable, the learning of animate behaviors. Our work thus contrasts with multi-agent learning in that, in order to focus on these two computational factors, we precisely control all behaviors aside from that of our intrinsically motivated agent, and the agents do not cooperate or compete on any further objective.



====
Standard techniques include uncertainty sampling \citep{lewis1994heterogeneous}, query by disagreement \citep{cohn1994improving}, query by committee \citep{seung1992query}, error reduction \citep{roy2001toward}, and variance reduction \citep{geman1992neural}. Similar ideas have also been studied under the rubric of statistical \emph{optimal experimental design} \citep{kahn1951estimation, fedorov2013theory, chaloner1995bayesian}. 

\cite{jaderberg2016reinforcement} provides as intrinsic reward via auxiliary tasks in order to better performance in sparse reward settings. \cite{kulkarni_hierarchical} combine intrinsic motivation with hierarchical action-value functions operating at different temporal scales, for goal-driven deep reinforcement learning.
s
The signals exploited in traditional active learning and curiosity can also be applied outside of these sparse reward contexts. \cite{graves2017automated} explore a number of learning progress estimators in order to build a curriculum in a multi-armed bandit setting. \cite{blaes2019control} use several such signals in order to solve several related tasks, some of which build on others, others of which are effectively impossible, providing a multi-task variant of the white noise problem.

%It is worth noting how the intent of this work contrasts with several related themes. First, most studies of curiosity study intrinsic reward as either (1) a way to enhance performance at a reinforcement learning task with sparse but present extrinsic reward or (2) a method of encouraging good exploration, as measured by e.g. the amount of territory the agent has seen. In this work, we study curiosity {\em as active learning}, measuring success by improved performance at the world model problem. 

















% cogsci section after dan shortened it: 
\noindent\textbf{Object dynamics prediction, attention, and permanence.} 
Humans are extremely effective at understanding dynamics of objects in their environment, excelling at intuitively predicting both the physical interactions of external objects~\cite{} and the physical consequences of their own actions~\cite{}. 
However, both the visual system and the working memory system that support these abilities have substantial limitations~\cite{}. 
Humans thus selectively allocate attention in an object-centric fashion to enable effective prediction despite these limitations \citep{alvarez2007many, scholl2001objects}, and assign individuated tokens to keep track of objects over time \citep{sears2000multiple}. To deal with momentary disappearances of objects as they become occluded or leave the visual frame, the brain maintains and updates an internal persistent representation of objects, a phenomenon known as \emph{object permanence}~\cite{piaget_originsintelligence}.  Studies in human infants have shown that many of these abilities --- including understanding the dynamical continuity of physical trajectories, the solidity of objects, and their persistence even when out of sight --- appear to be present very early in development~\cite{spelke_objectpermanence, spelke2007core, baillargeon1985object}. 
In this work, we include object-based attention, object permanence, and working memory as architectural biases, i.e. knowledge that is built in as a prior of the model. To enable dynamical prediction, we provide the model with the center coordinates of objects, and require it to predict their future center coordinates. Further, we use a memory system to maintain an active representation of an object whenever it goes out of sight. 

\noindent\textbf{Curiosity and Active Learning.} Attentional control also appears to be of great importance for learning how the world works.  Infants appear to gather information from environments in a manner that is quite principled, selectively looking at objects in highly non-random manner~\cite{smith}, and devoting increased attention to objects that violate their expectations \citep{stahl2015observing}.  Infants also appear to self-generate useful learning curricula, preferentially attending to stimuli that are sufficiently complex to be interesting but not so complicated that they cannot be predicted, a phenomenon known as the \emph{goldilocks effect} \citep{kidd2012goldilocks}.  In this work, a key question that we address is the formalization of the intrinsic motivations underlying active learning in a multi-agent context. 

\noindent\textbf{Animate attention.}
From early infancy, humans are especially adept at distinguishing between inanimate and animate agents, preferentially paying attention to animate features like faces \citep{maurer2002many} and human body shapes \citep{slaughter2002development}, a phenomenon called \emph{animate attention}. Even in the absence of these surface features, infants will preferentially attend to spatiotemporal kinematics indicative of animate agents, such as self-propelled motion \citep{premack1990infant}, efficient movement towards targets \citep{gergely1995taking}, contingent behavior between observed agents, as when one agent chases another \citep{frankenhuis2013infants}, and contingent behavior between an observed agent and the infant herself, as when a robot beeps in response to the infant's babbling \citep{johnson2003detecting, foster1973visual}.  The visual system has been highly tuned to cues that reliably indicate the presence of agents with internal sources of energy and volition that cause them to move without the need for external forces. Such kinematic patterns give rise to an irresistable sense of animacy and intentionality, even when the objects executing the kinematics are simple shapes \citep{heider1944experimental}. 
In this work, our environment includes inanimate and animate agents with spatiotemporal kinematics inspired from these human experiments, and the agents are deliberately devoid of surface features, so that our modeling agent must discover which agents are interesting and worth paying attention to based on their spatiotemporal properties alone. 
While we do build in inductive biases concerning object-permanence and working memory, we do not build in a propensity to detect and predict special classes of stimuli. Instead, we test whether reasonable patterns of attention of the form observed in humans can emerge naturally in our model, provided we endow it with a good, general-purpose learning objective.

\noindent\textbf{Social prediction and theory of mind.}
Beyond animate attention, a more sophisticated ability that emerges later in development is the active interpretation of other agents in terms of their underlying mental states (beliefs, desires, and goals) that cause the agents' behavior, aka \emph{theory of mind} \citep{astington1990developing, premack1978does, wellman1992child}. It is hypothesized that theory of mind is needed in order to \textit{predict} what an agent will do next, since often it is only possible to do so accurately by generating expectations about an agent as a function of underlying intentions that are attributed to it. This ability is crucial to social functioning, and the failure to attribute mental states falls under the umbrella of symptoms that define the autism spectrum mental disorders \citep{baron2000theory}.  
In this work, we task our neural model with learning to predict what the objects and agents in the environment will do next, and seek to determine which features of animate attention and theory of mind are required to achieve improved world-model predictions.

==> icml_sections/relatedwork_scrap2.tex <==
\section{Related Works}
\label{sec:relatedworks}

Both artificial intelligence and cognitive science have developed substantial literatures around  world-modeling and attentional control.

\subsection{Artificial Intelligence}

\noindent{\textbf{World models and prediction.}}
A natural class of world-models involve forward dynamics prediction. The most direct form involves video frame prediction\citep{kalchbrenner2016video, finn2016unsupervised}, inspired by the long-standing neuroscience concept of \emph{predictive coding}\citep{lotter2016deep}.  Action-conditioned video frame prediction models can be used directly in planning for robotic control tasks~\citep{finn2017deep}, as performance-enhancers for reinforcement learning tasks\citep{chua2018deep,ke2019learning}, or as ``dream'' environment simulations for training policies~\citep{ha2018world}. Video frame prediction enormously challenging to accomplish, despite some progress\citep{lee2018stochastic, wang2018predrnn++, Wu2019ModelIF}. 
Some of the difficulty of predicting forward dynamics can be alleviated by working not with images but in latent feature representations such as 3D point clouds~\citep{byravan2017se3} or object-centric, graphical representations of scenes~\citep{battaglia2016interaction, chang2016compositional, mrowca2018flexible}. Such models have been shown to coarsely model human expectation violation of intuitive physics \citep{smith2019modeling}. 
World-models can also be derived from prediction problems other than forward dynamics, including time reversal \citep{nair2018time} and inverse dynamics~\citep{agrawal2016learning}, approaches that have proven useful in building world models for well-defined robotic manipulation tasks. 
World-models can also be targeted toward specific attributes rather than full state-space prediction --- e.g. the height of an object in free fall --- allowing the known physical constraints of the output space to drive learning~\citep{stewart2017label}. 

In our work, we focus on a forward-dynamics prediction problem in an object-centric representation. This representation simply consists of the positions of each object or agent in the environment, lacking other distinguishing features. We thus {\em assume} the agent has access to an encoding giving it this representation, bypassing the important but complex question of how to extract this representation directly from visual features, so as to focus the present work on identifying good solutions for active learning and multi-agent causal modeling. 

\noindent{\textbf{Active learning.}}
Independently of which task the agent self-supervises its world-model on, a key question the agent is faced with is choosing its actions to efficiently learn the world-model. In the classical \emph{active learning} setting~\citep{settles2011_active}, an agent seeks to learn a supervised task with costly labels, judiciously choosing which examples to obtain labels for so as to maximize learning efficiency. 
More recently, active learning has evolved in the context of self-supervised reinforcement learning agents~\citep{schmidhuber_formaltheoryoffun, oudeyer2013intrinsically, jaderberg2016reinforcement}. In this line of work, agents typically self-supervise a world-model using an intrinsically-generated ``curiosity''.  Many different approaches to this general idea exist, all of which are essentially different approaches to estimating \emph{learning progress} --- e.g. determining which actions lead are likely to lead to the highest world-model accuracy gain in the future.  

One popular approach is the use of \emph{novelty} metrics, which measure how much a particular part of the environment has been explored, and direct agents into under-explored parts of state-space. 
Examples include count-based and psuedo-count-based methods~\citep{strehl2008analysis,bellemare2016unifying, ostrovski2017count}, Random Network Distillation (RND)~\citep{burda2018exploration}, and the \emph{empowerment} metric \citep{mohamed2015variational}. 
Novelty-based approaches avoid the difficult world-model-progress estimation problem entirely by not depending at all on a specific world-model state, and relying on novelty as a (potentially flawed) proxy for learning progress. 

The simplest idea that actually takes into account the world-model problem to be learned is \emph{adversarial} curiosity, which estimates current world-model error and directs agents to actions estimated to maximize this error~\citep{stadie2015predictive, pathak2017inverse, haber2018learning}. However, direct error-driven curiosity can result in the \emph{white noise problem}, in which agents are motivated to waste time fruitlessly trying to solve unsolvable world-modeling problems, e.g. where there is degeneracy in the cause or effect of the action. While the white noise problem can to some degree be avoided by solving the world-modeling problem in a learned latent feature-space in which degeneracies are suppressed~\citep{pathak2017inverse, pathak18largescale}, directly estimating learning progress ~\citep{oudeyer2007intrinsic, oudeyer2013intrinsically} or \emph{information gain}~\citep{houthooft_vime} avoids the white noise problem in a more comprehensive fashion. However, such methods have been limited in scope because they involve calculating quantities that cannot easily be estimated in many-dimensional continuous action spaces.
\emph{Surprisal}~\citep{achiam2017surprise} and model disagreement\citep{pathak2019disagreement} present computationally-tractable alternatives to information gain, at the cost of the accuracy of the estimation. For comprehensive reviews of intrinsic motivation signal choices, see \citep{aubret2019survey, linke2019adapting}.
In this work, we present a novel method for estimating learning progress that takes advantage such metrics have in ensuring the directed learning utility of action choices, while being robust and scalable to high-dimensional continuous action-space settings. 

\noindent{\textbf{Multiagent and social learning.}}
The field of multi-agent learning \citep{nguyen2018deep, zheng2018structured} concerns the coordination and communication of multiple agents within an environment in order to solve a reinforcement learning task. \citep{jaques2019social} explores the use of causal influence of one agent on another as intrinsic motivation to learn policies across agents in a decentralized manner.  \citep{rabinowitz2018machine} demonstrate the use of a ``Theory of Mind'' neural network architecture that models behaviors in a gridworld environment.
\citep{baker2019emergent} study the emergence of interesting behaviors such as the use of tools in competitive multi-agent environments. \citep{vinyals2019grandmaster} use many agents pitted against each other in order to refine policies in the competitive strategy game setting of Starcraft II.
\citep{tacchetti2018relational} learns a shared relational forward model, representing a network of relationships between agents, in order to boost performance at a multi-agent learning task.
Multi-agent learning has also been extended beyond artificial environments and into real social environments by developing predictive models of specific human behaviors and using those to enable robots to better interact with people\citep{ballan2016knowledge, robicquet2016learning, sadeghian2019sophie}.
\citep{kleinsurprise} learn predictive models of infant visual attention, aimed at designing robots that manipulate and encourage attention.

In this work, we address a multi-agent reinforcement problem from the point of view of a single agent that seeks to learn about the actions of other agents it observes and interacts with. Like other works, our goal is to build architectures and policies that enable the learning agent to better understand what other agents will do, but unlike other works we do not hard-code in either the learning objective (e.g. our work is self-supervised) or the behavioral outcomes (e.g. natural attention patterns \emph{emerge} as a solution to better multi-agent prediction). 

\noindent{\textbf{Attention.}} A wide variety of problems have been shown to benefit from neural network architectures that employ what has come to be called ``attention'' in the AI literature, e.g. local multiplicative gating that dynamically learns to highlight portions of the network during inference, so as to focus processing on particularly relevant portions of either the input data or intermediate featural content~\cite{}. This literature is related to our current work in that it shows how selective highlighting of some form can improve learning, but differs significantly from our work in the meaning of the term ``attention'', the importance of the active learning setting, and the technical machinery needed use attention in this setting.  What we call ''attention'' in our work is literally the idea that a physically embodied agent will allocate its observational time differently for different stimuli, rather than the more abstract disembodied concept used in most AI literature. In contrast to attentional multiplication in the typical supervised off-line learning setting, our agents need attentional control to perform effective active learning, creating datapoints that without such control would otherwise occur either very rarely or not at all.  The causal world model architecture and learning progress policy we develop to programmatically generate the right types of such control are thus structurally distinct from the multiplicative gating operations used in typical AI attention work.

\subsection{Cognitive Science}
\label{subsec:related:cognitive}

\noindent\textbf{Object dynamics prediction, attention, and permanence.} 
Humans are extremely effective at understanding object dynamics, excelling at intuitively predicting both the physical interactions of external objects~\citep{} and the physical consequences of their own actions~\citep{}. 
However, both the visual system and the working memory system that support these abilities have substantial limitations~\citep{}. 
Humans thus selectively allocate attention in an object-centric fashion to enable effective prediction despite these limitations~\citep{alvarez2007many, scholl2001objects}, and assign individuated tokens to keep track of objects over time~\citep{sears2000multiple}. To deal with momentary disappearances of objects as they become occluded or leave the visual frame, the brain maintains an internal representation of objects, a phenomenon known as \emph{object permanence}~\citep{piaget_originsintelligence}.  Infant studies show that many of these abilities --- including understanding the dynamical continuity of physical trajectories, object solidity, and their persistence even when out of sight --- appear to be present very early in development~\citep{spelke_objectpermanence, spelke2007core, baillargeon1985object}. 
In this work, we include object-based attention, object permanence, and working memory as architectural biases. We require the model to perform dynamimcs prediction on the center coordinates of objects, and we use a memory system to maintain an active representation of an object whenever it goes out of sight. 

\noindent\textbf{Curiosity and Active Learning.} Attentional control also appears to be of great importance for learning how the world works.  Infants appear to gather information from environments in a manner that is quite principled, selectively looking at objects in highly non-random manner~\citep{smith}, and devoting increased attention to objects that violate their expectations \citep{stahl2015observing}.  Infants also appear to self-generate useful learning curricula, preferentially attending to stimuli that are sufficiently complex to be interesting but not so complicated that they cannot be predicted, a phenomenon known as the \emph{goldilocks effect}~\citep{kidd2012goldilocks}.  In this work, a key question that we address is the formalization of the intrinsic motivations underlying active learning in a multi-agent context. 

\noindent\textbf{Animate attention.}
From early infancy, humans are especially adept at distinguishing between inanimate and animate agents, preferentially paying attention to animate features like faces \citep{maurer2002many} and human body shapes~\citep{slaughter2002development}. Even in the absence of these surface features, infants will preferentially attend to spatiotemporal kinematics indicative of animate agents, such as self-propelled motion~\citep{premack1990infant}, efficient movement towards targets~\citep{gergely1995taking}, contingent behavior between observed agents, as when one agent chases another~\citep{frankenhuis2013infants}, and contingent behavior between an observed agent and the infant herself, as when a robot beeps in response to the infant's babbling~\citep{johnson2003detecting, foster1973visual}.  The visual system is highly tuned to cues that reliably indicate the presence of agents with internal sources of energy that cause them to move without external forces. Such kinematic patterns give rise to an irresistable sense of animacy and intentionality, even when the objects executing the kinematics are simple shapes~\citep{heider1944experimental}. 
In this work, our environment includes agents with spatiotemporal kinematics inspired by these human experiments, and the agents are deliberately devoid of surface features, so that our curious agent must discover which agents are interesting and worth paying attention to based on their dynamics alone. 
While we build in inductive biases concerning object-permanence and working memory, we do not build in a propensity to detect and predict special classes of stimuli. Instead, we test whether reasonable patterns of attention of the form observed in humans emerges naturally in our model, provided we endow it with the right intrinsic motivation.

\noindent\textbf{Social prediction and theory of mind.}
Beyond animate attention, a more sophisticated ability that emerges later in development is the active interpretation of other agents in terms of their underlying mental states (beliefs, desires, and goals) that cause the agents' behavior, aka \emph{theory of mind} \citep{astington1990developing, premack1978does, wellman1992child}. It is hypothesized that theory of mind is needed in order to \textit{predict} what an agent will do next, since often it is only possible to do so accurately by generating expectations about an agent as a function of underlying intentions that are attributed to it. This ability is crucial to social functioning, and the failure to attribute mental states falls under the umbrella of symptoms that define the autism spectrum mental disorders~\citep{baron2000theory}.  
In this work, we task our neural model with learning to predict what the objects and agents in the environment will do next, and seek to determine which features of animate attention and theory of mind are required to achieve improved world-model predictions.










==> icml_sections/relatedworks.tex <==
\begin{figure*}[t!]
    \centering
    \includegraphics[width=\textwidth]{figures/environment_reduced_size.pdf}
    \vspace{-15pt}
    \caption{\textbf{Virtual environment.} Our 3D virtual environment is a distillation of key aspects of real-world environments. The \textit{curious agent} (white robot) is centered in a room, surrounded by various \textit{external agents} (colored spheres) contained in different quadrants, each with dynamics that correspond to a realistic inanimate or animate behavior (right box). The curious agent can rotate to attend to different behaviors as shown by the first-person view images at the top. See \textcolor{blue}{\url{https://bit.ly/31vg7v1}} for videos.} % still need to change objects to be something less awkward 
    \label{fig:environment}
    \vspace{-10pt}
\end{figure*}

\section{Related Works}
\label{sec:relatedworks}

% Both artificial intelligence and cognitive science have developed substantial literatures around  world-modeling and attentional control.

\noindent{\textbf{World Models}}
A natural class of world models involve forward dynamics prediction. Such models can directly predict future video frames~\citep{finn2016unsupervised, wang2018predrnn++, Wu2019ModelIF}, or latent feature representations such as 3D point clouds~\citep{byravan2017se3} or object-centric, graphical representations of scenes~\citep{battaglia2016interaction, chang2016compositional, mrowca2018flexible}. 
Action-conditioned forward-prediction models can be used directly in planning for robotic control tasks~\citep{finn2017deep}, as performance-enhancers for reinforcement learning tasks~\citep{ke2019learning}, or as ``dream'' environment simulations for training policies~\citep{ha2018world}. In our work, we focus on forward dynamics prediction with object-oriented representations. 
% World models can also be derived from prediction problems other than forward dynamics, including time reversal \citep{nair2018time} and inverse dynamics~\citep{agrawal2016learning}.
% World-models can also be targeted not at a full state-space prediction but instead toward specific attributes --- e.g. the height of an object in free fall --- allowing known constraints in the output space (e.g. conservation of momentum) to drive learning~\citep{stewart2017label}. 


% This representation simply consists of the positions of each object or agent in the environment, lacking other distinguishing features. We thus {\em assume} the agent has access to an encoding oracle giving it this representation, bypassing the important but complex question of how to extract this representation directly from visual features, so as to focus the present work on identifying good solutions for AWML.   

\noindent{\textbf{Active Learning and Curiosity}} A key question the agent is faced with is how to choose its actions to efficiently learn the world model. In the classical \emph{active learning} setting~\citep{settles2011_active}, an agent seeks to learn a supervised task with costly labels, judiciously choosing which examples to obtain labels for so as to maximize learning efficiency. 
More recently, active learning has been implicitly generalized to self-supervised reinforcement learning agents~\citep{schmidhuber_formaltheoryoffun, oudeyer2013intrinsically, jaderberg2016reinforcement}. In this line of work, agents typically self-supervise a world model with samples obtained by curiosity-driven exploration. Different approaches to this general idea exist, many of which are essentially different approaches to estimating future \emph{learning progress} --- e.g. determining which actions are likely to lead to the highest world model prediction gain in the future. 
One approach is the use of \emph{novelty} metrics, which measure how much a particular part of the environment has been explored, and direct agents into under-explored parts of state-space. 
Examples include count-based and psuedo-count-based methods~\citep{strehl2008analysis,bellemare2016unifying, ostrovski2017count}, Random Network Distillation (RND)~\citep{burda2018exploration}, and \emph{empowerment} \citep{mohamed2015variational}. 
Novelty-based approaches avoid the difficult world model  progress estimation problem entirely by not depending at all on a specific world model state, and relying on novelty as a (potentially inconsistent) proxy for expected learning progress. 

The simplest idea that takes into account the world model is \emph{adversarial} curiosity, which estimates current world model error and directs agents to take actions estimated to maximize this error~\citep{stadie2015predictive, pathak2017inverse, haber2018learning}. However, adversarial curiosity is especially prone to the \emph{white noise problem}, in which agents are motivated to waste time fruitlessly trying to solve unsolvable world model problems, e.g. predicting the dynamics of random noise. The white noise problem can to some degree be avoided by solving the world-modeling problem in a learned latent feature space in which degeneracies are suppressed~\citep{pathak2017inverse, pathak18largescale}. 

Directly estimating learning progress ~\citep{oudeyer2007intrinsic, oudeyer2013intrinsically} or \emph{information gain}~\citep{houthooft_vime} avoids the white noise problem in a more comprehensive fashion. However, such methods have been limited in scope because they involve calculating quantities that cannot easily be estimated in high-dimensional continuous action spaces.
\emph{Surprisal}~\citep{achiam2017surprise} and model disagreement~\citep{pathak2019disagreement} present computationally-tractable alternatives to information gain, at the cost of the accuracy of the estimation. For comprehensive reviews of intrinsic motivation signal choices, see \citep{aubret2019survey, linke2019adapting}.
In this work, we present a novel method for estimating learning progress that is ``consistent'' with the original prediction gain objective while also scaling to high-dimensional continuous action-spaces. 

\noindent{\textbf{Cognitive Science}}
Research in cognitive science suggests that humans are  active world model learners from a young age. Infants appear to actively gather information from their environment by attending to objects in a highly non-random manner \cite{smith2019modeling}, devoting more attention to objects that violate their expectations \cite{stahl2015observing}. They are also able to self-generate learning curricula, with preference to stimuli that are complex enough to be interesting but still predictable~\cite{kidd2012goldilocks}. Interestingly, infants seem to particularly attend to spatiotemporal kinematics indicative of \textit{animacy}, such as efficient movement towards  targets~\cite{gergely1995taking} and contingent behavior between agents~\cite{frankenhuis2013infants}. 
Our work shows that a similar form of animate attention naturally arises as a result of optimizing for learning progress. 

% \noindent{\textbf{Multiagent and social learning.}}
% The field of multi-agent learning \citep{nguyen2018deep, zheng2018structured} concerns the coordination and communication of multiple agents within an environment to solve a reinforcement learning task. \citep{jaques2019social} explores the use of causal influence between agents as intrinsic motivation to learn policies across agents in a decentralized manner.  \citep{rabinowitz2018machine} demonstrate the use of a ``Theory of Mind'' network architecture that models behaviors in a gridworld environment.
% \citep{baker2019emergent} study the emergence of interesting behaviors such as the use of tools in competitive multi-agent environments. \citep{vinyals2019grandmaster} use many agents pitted against each other to refine policies in the competitive strategy game setting of Starcraft II.
% \citep{tacchetti2018relational} learns a shared relational forward model, representing a network of relationships between agents, in order to boost performance at a multi-agent learning task.
% Multi-agent learning has also been extended beyond artificial environments and into real social environments by developing predictive models of specific human behaviors and using those to enable robots to better interact with people~\citep{ballan2016knowledge, robicquet2016learning, sadeghian2019sophie}.
% \citep{kleinsurprise} learn predictive models of infant visual attention, aimed at designing robots that manipulate and encourage attention.

% In this work, we address the problem of learning models of agents, a useful ability in multi-agent reinforcement learning contexts in which agents do not have access to other agents' reward functions or policies. Like other works, our goal is to build architectures and policies that enable the learning agent to model other agents it observes and interacts with, but we do not hard-code in either the learning objective (e.g. our work is self-supervised) or the behavioral outcomes (e.g. attention patterns \emph{emerge} as a solution to multi-agent prediction). 

% \noindent{\textbf{Attention.}} A wide variety of problems have been shown to benefit from neural network architectures that employ what has come to be called ``attention'' in the AI literature, e.g. local multiplicative gating that dynamically learns to highlight portions of the network during inference, so as to focus processing on particularly relevant portions of either the input data or intermediate featural content~\cite{}CITE. This literature is related to our work in that it shows how selective highlighting of some form improves learning, but differs significantly in the meaning of the term ``attention'', the importance of the active learning setting, and the technical machinery needed to use attention in this setting.  What we call ``attention'' is the idea that a physically embodied agent allocates its observational time differently for different stimuli, rather than the abstract disembodied concept used in most literature. In contrast to attentional multiplication in supervised settings, our agents need attentional control to perform effective active learning, creating datapoints that without such control would occur rarely or not at all.  The causal world model architecture and learning progress policy we develop to generate such control are thus structurally distinct from the multiplicative gating operations used in typical attention work.

% \subsection{Cognitive Science}
% \label{subsec:related:cognitive}

% \noindent\textbf{Object dynamics prediction, attention, and permanence.} 
% Humans are extremely effective at understanding object dynamics, excelling at intuitively predicting both the physical interactions of external objects~\citep{battaglia2018relational, proffitt1989understanding} %JDF: Note: I think the literature is more mixed about this, in part because psychologists tried really hard to find cases in which this wasn't true. So more recently, Battaglia and colleagues would agree with this statement, whereas older work Proffitt and colleagues says we're accurate in some cases but not others.
% and the physical consequences of their own actions~\citep{wolpert1995internal, wolpert2001motor, blakemore2003self}. 
% However, both the visual system and the working memory system that support these abilities have substantial limitations~\citep{alvarez2007many, alvarez2004capacity, miller1956magical}. Humans thus selectively allocate attention in an object-centric fashion to enable effective prediction despite these limitations~\citep{de2014attentional, egly1994shifting, scholl2001objects}, and assign individuated tokens to keep track of objects over time~\citep{sears2000multiple}. To deal with momentary disappearances of objects as they become occluded or leave the visual frame, the brain maintains an internal representation of objects, a phenomenon known as \emph{object permanence}~\citep{piaget_originsintelligence}.  Infant studies show that many of these abilities --- including understanding the dynamical continuity of physical trajectories, object solidity, and their persistence even when out of sight --- appear to be present very early in development~\citep{spelke_objectpermanence, spelke2007core, baillargeon1985object}. 
% In this work, we include object-based attention, object permanence, and working memory as architectural biases. We require the model to perform dynamics prediction on the center coordinates of objects, and we use a memory system to maintain an active representation of an object whenever it goes out of sight. 

% \noindent\textbf{Curiosity and Active Learning.} Attentional control also appears to be of great importance for learning how the world works.  Infants appear to gather information from environments in a manner that is quite principled, selectively looking at objects in a highly non-random manner~\citep{smith}, and devoting increased attention to objects that violate their expectations \citep{stahl2015observing}.  Infants also appear to self-generate useful learning curricula, preferentially attending to stimuli that are complex enough to be interesting but not too complicated that they cannot be predicted, a phenomenon termed the \emph{goldilocks effect}~\citep{kidd2012goldilocks}.  In this work, we study active learning in the context of animate and inanimate stimuli. 

% \noindent\textbf{Animate attention.}
% From early infancy, humans are adept at distinguishing between inanimate and animate agents, preferentially paying attention to animate features like faces \citep{maurer2002many} and human body shapes~\citep{slaughter2002development}. Even in the absence of such surface features, infants will preferentially attend to spatiotemporal kinematics indicative of animacy, such as self-propelled motion~\citep{premack1990infant}, efficient movement towards targets~\citep{gergely1995taking}, contingent behavior between observed agents, as when one agent chases another~\citep{frankenhuis2013infants}, and contingent behavior between an observed agent and the infant herself, as when a robot beeps in response to the infant's babbling~\citep{johnson2003detecting, foster1973visual}.  
% % The visual system is highly tuned to cues that reliably indicate the presence of agents with internal sources of energy that cause them to move without external forces. 
% Such kinematic patterns give rise to an irresistable sense of animacy, even when the objects executing the kinematics are simple shapes~\citep{heider1944experimental}. 
% In this work, our environment includes agents with kinematics inspired by the human experiments and deliberately devoid of surface features, so that our curious agent must discover which agents are worth paying attention to based solely on dynamics.
% While we build in inductive biases concerning object-permanence, we do not build in a propensity to detect special classes of stimuli. Instead, we test whether animate attention of the form observed in humans emerges naturally, provided we endow the model with the right intrinsic motivation.

% \noindent\textbf{Social prediction and theory of mind.}
% Beyond animate attention, a more sophisticated ability that emerges later in development is the active interpretation of other agents in terms of their underlying mental states (beliefs, desires, and goals) that cause the agents' behavior, aka \emph{theory of mind} \citep{astington1990developing, premack1978does, wellman1992child}. It is hypothesized that theory of mind is needed in order to \textit{predict} what an agent will do next, since often it is only possible to do so accurately by generating expectations about an agent as a function of their underlying intentions. This ability is crucial to social functioning, and the failure to attribute mental states falls under the umbrella of symptoms that define the autism spectrum disorders~\citep{baron2000theory}.  
% In this work, we task our model with learning to predict what the agents in the environment will do next.
% % , and seek to determine which features of animate attention and theory of mind are required to achieve improved world-model predictions.










==> icml_sections/scrap.tex <==
============intro.tex

Imagine yourself a parent at a playground. There is a plethora of stimuli, spanning wavering trees, leaves blowing in the wind, and children playing hide and seek. After briefly staring at the shaking trees and rustling leaves, you bore of watching their unpredictable motion and instead direct your attention to the game of hide and seek. Unlike with the random motion of trees and leaves, your understanding of the complex but predictable dynamics of hide-and-seek improves over time and you may eventually become capable of predicting a child's specific next move. This simple scenario suggests that humans continually engage in an intrinsically motivated process of furthering their understanding of the world and that directed attention may emerge naturally whilst seeking out maximally informative observations. In this work we aim to develop an intrinsically motivated active learning system that does the same: sample efficiently build models of the world by learning what to attend to.  

Concretely, world models are a family of predictive models that solve self-supervised prediction problems pertaining to the underlying the temporal structure of the world such as forward and inverse dynamics. Through learning world models, humans may acquire compact abstractions of high bandwidth sensory inputs, the ability to plan across long temporal horizons, and an understanding of the behavioral patterns of other agents. To deploy AI active learners in the real world, it is thus crucial that they can efficiently learn world models in complex environments. \kh{emphasize this process should happen without much external supervision}

To this end, there are mainly two algorithmic challenges: The first algorithmic challenge is that the active learner must arbitrate between the combinatorially large number of stimuli exhibiting inherently unlearnable or chaotic dynamics - e.g., falling leaves, wavering trees, and splashing water - and the few \ms{sparsity still hasn't been justified?} stimuli that have interesting and complex, yet learnable dynamics - e.g children playing hide-and-seek. We refer to the former class of stimuli as displaying \emph{noisy} behavior \ms{The thing about ``noisy'' is it has the connotation of ``having some noise'' which is true for stochastic animate agents.} and the latter as displaying \emph{animate} behavior. The term "animate" is drawn from the field of psychology \citep{premack1990infant, gergely1995taking, frankenhuis2013infants} in which "animate agents" denote a class of entities displaying behaviors with human-like kinematics such as self-propelled motion, goal-directed movements, and motion contigent on other agents. This challenge of identifying animate stimuli amid a sea of noisy ones has been acknowledged in many prior works as the "white noise" problem \citep{schmidhuber_formaltheoryoffun, pathak2017inverse, burda2018exploration, pathak2019disagreement}. The second algorithmic challenge is that the world model is susceptible to causal confusion - e.g the mistaking spurious correlations for true causality - which leads to poor generalization performance.

\kh{separate this challenge} Additionally, there is resource challenge that there is a shortage of simulated environments that faithfully preserve the core properties of real-world environments, while removing confounds that may artificially inflate modeling successes.

We address these three challenges with an intrinsically motivated "curious" active learning agent comprising two key components: (i) a \emph{Progress Curiosity-driven Controller} that learns to attend to stimuli with high expected learning progress thereby overcoming the white noise problem and (ii) a \emph{Causal World Model} that integrates a causal prior into its network architecture to preempt causal confusion. (see Fig. \ref{fig:model}) Our experiments are conducted in a custom-built 3D virtual world environment, rich with external agents displaying a wide spectrum of realistic animate behaviors such as peekaboo, chasing, and mimicry. \kh{should summarize key contributions into a couple sentences here}

In what follows, we begin by drawing connections between our work and related works in psychology and artificial intelligence (Section~\ref{sec:relatedworks}). In Section~\ref{sec:environment}, we describe our virtual environment in detail. Section~\ref{sec:theory} formalizes the active learning problem our curious agent is tasked with, motivates progress curiosity in the context of previously proposed curiosity signals, and characterizes the causal confusion problem. \kh{be a bit more detailed here} Section~\ref{sec:methods} details the implementations for all components of our curious active learning agent. Finally, Section~\ref{sec:experiments} presents experimental evaluations of our curious active learning system on two quantitative metrics: We show that (1) injecting causal prior is essential to attaining high offline asymptotic model performance, and (2) our progress-driven controller achieves significantly lower online sample complexity than baseline controllers equipped with state-of-the-art exploration strategies — including Random Network Distillation (RND) (Burda et al., 2018b) and Model Disagreement (Pathak et al., 2019) — which (perhaps surprisingly) fall prey to the white noise problem. \kh{this last sentence still needs to be rephrased} Furthermore, when varying both the intrinsic motivation signal (considering several baselines) and world model architecture (with causal structure prior, and without), we find that the intrinsic motivation signal drives behavior, whereas the difference in world model architecture modulates behavior to a lesser degree.


%In what follows, we begin by drawing connections between our work and related works in psychology and reinforcement learning (Section 1). In Section 2 \jdf{incomplete}. In Section 3, we describe our virtual environment in detail. Section 4 formalizes the core problems that motivate this project, including causal confusion and the shortcomings of curiosity signals that have been previously proposed to solve the white noise problem, while Section 5 presents the components of our active learning system. Finally, Section 6 presents experimental evaluations of our curious active learning system along three metrics: We show that (1) our causal prior is essential to attaining high offline asymptotic model performance, (2) our choice of a progress-driven controller is crucial to obtaining low online sampling complexity, while state-of-the art exploration methods — including Random Network Distillation (RND) (Burda et al., 2018b) and model disagreement (Pathak et al., 2019) — fall prey to the white noise problem, and (3) independent of world model choice, preferential attention towards animate agents emerges only with progress curiosity (but not other kinds of curiosity), suggesting that our model architecture may approximate the neural learning systems employed by humans. \jdf {I’ll circle back around to this to think about the specific human impliciations of ‘independent of a world model choice}.













% X_{ext, t:t+T_{out}}, \hat X_{ext, t:t+T_{out}}) = \sum_{s = t}^{T + T_{out}}\sum_{i = 1}^{N_ext} \alpha \rvx_{i, s} \|c_{i, s} - \hat c_{i, s} \|_2^2 + \beta \mathcal{L}_{ce}(\rvx_{i, s}, \hat \rvx_{i, s})

% As described in Section~\ref{sec:theory}, the world model seeks to solve the forward dynamics prediction problem of external agent behaviors in this encoding space. Specifically, given an encoded observation sequence $\rvx_{t - T_{in} : t}$ and curious agent actions $a_{t - T_{in} : t + T_{out} - 1}$, the world model predicts  $\rvx_{ext, t : t + T_{out}}$. % \ms{Loss function} 


% \ms{Causal prior} 
% In this work, we propose the \textit{Causal World Model}, a world model architecture that injects a causal graph of external agents (see Section~\ref{sec:theory}) as an architectural prior. Specifically, we impose this prior by instantiating, for each behavior $i$, a separate \textit{behavior network} $\mathcal{B}_i$ with independent weights $\theta_i$, such that one causal world model consists of $\{\mathcal{B}_i\}_{i \in \{1, ..., N_{behavior}\}}$

% Given behavior $i$, let $S_i$ be the set of all agents that belong to the behavior. 
% Given an encoded observation sequence $\rvx_{t - T_{in} : t}$, $\mathcal{B}_i$ takes as input only the part of $\rvx_{ext, t - T_{in} : t}$ corresponding to the agents that belong to the behavior, i.e., $(\rvx_{j, t - T_{in} : t} \cdot c_{j, t - T_{in} : t}, \rvx_{j, t - T_{in} : t})$ for all $j \in S_i$, along with $\rvx_{aux, t - T_in: t}$,  $\phi_{t - T_{in} : t }$, and $a_{t - T_{in} : t}$, and outputs predictions of only the part of $\rvx_{ext, t:t+T_{out}}$ that corresponds to the agents that belong to its behavior, i.e., $(\rvx_{j, t:t+T_{out}} \cdot c_{j, t:t+T_{out}}, \rvx_{j, t:t+T_{out}})$ for all $j \in S_i$. The outputs of all behavior networks  are concatenated to construct the overall prediction of $\rvx_{t:t+T_{out}}$, which is then the output of the causal world model.

% \ms{specific architecture 
% (LSTM, layers, units, optimizer, learning rate), excluding indicator coordinate split }

% To measure the gains of our causal world model, we introduce a \textit{non-causal ablation} that does not have this architectural prior. Concretely, the non-causal world model uses an architecture similar to that of a single behavior network in the causal world model, but with larger layers to have a similarly-sized parameter space. It takes as input $\rvx_{t-T_{in};t}$ and predicts $\rvx_{t:t+T_{out}}$ directly, modeling the dynamics of all external agent behaviors simultaneously. 






%\ms{Our self-supervision problem: forward dynamics prediction}
% First, we assume access to an oracle that maps observations $(O_t)$ to  an intermediate representation $(X_t)$ which contains information about the coordinates of each external agent in the room and indicators of whether an agent is in the curious agent's view.
%\ms{What are the inputs and outputs of the world model?}
%Specifically, given a sequence of past observations and past and present actions $(X_{t-n:t}, a_{t+k-1})$, the world model seeks to predict the next sequence of observations $(X_{t+1:t+k})$.


%\subsubsection{Split architecture}
%\ms{What are the solutions?}
%While in environments with only inanimate objects, the physical dynamics is shared between objects, a key property of our multi-agent environment is that different agents behave under widely varied dynamics. 
%In this work, we propose a split world model architecture, which consists of separate networks that each solve forward dynamics prediction of one external agent behavior, where a behavior may consist of one (e.g. peekaboo) or two interacting external agents (e.g. chasing). We argue that this behavior-wise splitting is equivalent to injecting the agent contingency graph as an architectural prior into the world model... 
%We perform ablations where a single neural network is used to model all external agents in the environment.

% Note that the particular dynamics prediction problem posed for a given external agent behavior does not always need to involve the prediction of all external agents involved in the behavior. In the case of mimicry, the input to the corresponding module contains information about both actor and imitator agents, but the prediction only needs to be done on the imitator. 



In this section we evaluate the active learning performance of our progress-driven curious agent. There are two differences from the supervised learning experiments in Section \ref{sec:offline}. First, instead of collecting data under random policy, the curious agent \emph{learns} to attend by optimizing a surrogate curiosity reward in order to minimize the number of environment interactions. Second, the virtual environment is set up with three noise behaviors and one animate behavior, varied amongst the seven animate behaviors listed in Section \ref{sec:environment}. This configuration directly challenges the curious agent to overcome the white-noise problem. We measure the sample complexity of the curious agent optimizing different curiosity signals while changing the animate behaviors and world model types. Specifically, we compare the five curiosity signals and a random policy baseline

\textbf{$\gamma$-Progress (Ours)} is our proposed variant of progress curiosity which chooses $\theta_{old}$ to be a geometric mixture of all past models as in Eq. \ref{eq:mix_progress}. 

\textbf{$\delta$-Progress \citep{achiam2017surprise, graves2017automated}} is the $\delta$-step learning progress reward from Eq. \ref{eq:kstep_progress} with $\delta = 1$. We found that any $\delta > 3$ is impractical due to memory limitations even with 12GB Titan X GPUs. 

\textbf{RND \citep{burda2018exploration}} is a state-of-the-art novelty-based exploration method shown to be effective in video game domains. In this approach, a predictor neural net is trained to match the outputs of a random state encoder. States for which the predictor networks fails to match the random encoder are deemed "novel", and thus receive high reward. 

\textbf{Disagreement \citep{pathak2019disagreement}} is the disagreement reward from Eq. \ref{eq:disagreement} with $N = 3$ ensemble models. We found that $N > 3$ is impractical due to memory constraints.  

\textbf{Adversarial \citep{stadie2015predictive, pathak2017inverse}} is the prediction error from Eq. \ref{eq:adversarial}. 

\textbf{Random} chooses actions uniformly at random among the 9 possible rotations. 


% Fig.~\ref{fig:attention} shows that, for both the causal and non-causal world models, strong animate attention emerges for $7/7$ behaviors $\gamma$-Progress and weak animate attention arises on $1/7$ behaviors for $\delta$-Progress. For RND, Disagreement, and Adversarial we observe the inverse: strong attention to the random agent emerges, i.e the white noise problem is apparent. \kh{We find that animate attention is strongly correlated with the AUC metric of sample complexity (provide number or figure reference), which supports our hypothesis that animate attention naturally emerges from an underlying process of optimizing for efficient world model learning}. 

% We also evaluate active learning performance using the acausal world model which has lower asymptotic model performance. Regardless we see that $\gamma$-Progress outperforms RND, Disagreement, and Adversarial baselines on all $7/7$ behaviors and outperforms $\delta$-Progress on $5/7$ behaviors while tying on the two peekaboo behaviors. While the world model's asymptotic performance is severely affected by architecture choice (causal v.s. acausal), the relative ranking in performance across intrinsic motivation signals is maintained across world model types. 


%%%%%%%%%%%%%%%%%%%%%% Attention Metric %%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
\subsection{Emergence of Animate Attention}

In this section, we analyze the interplay between choice of intrinsic motivation, world model architecture, validation performance, and the attention patterns that emerge within our environment. Fig.~\ref{fig:attention} shows that, for both the causal and acausal world models, strong animate attention emerges for $7/7$ behaviors $\gamma$-Progress and weak animate attention arises on $1/7$ behaviors for $\delta$-Progress. For RND, Disagreement, and Adversarial we observe the inverse: strong attention to the random agent emerges, i.e the white noise problem is apparent. In what follows, we analyze the factors varied in these models in order to quantify more precisely what drives the emergence of animate attention. We then characterize the extent to which the emergent attentional pattern predicts validation performance. This serves as a toy "developmental model" of how  {\em early attention} better predicts later performance than does {\em early performance}.
\end{comment}

%In this section, we evaluate the attention patterns that emerge from our intrinsically motivated active learning system. Fig.~\ref{fig:attention} shows that, for both the causal and non-causal world models, strong animate attention emerges for $7/7$ behaviors $\gamma$-Progress and weak animate attention arises on $1/7$ behaviors for $\delta$-Progress. For RND, Disagreement, and Adversarial we observe the inverse: strong attention to the random agent emerges, i.e the white noise problem is apparent. \kh{We find that animate attention is strongly correlated with the AUC metric of sample complexity (provide number or figure reference), which supports our hypothesis that animate attention naturally emerges from an underlying process of optimizing for efficient world model learning}. 

==> icml_sections/theory.tex <==
% \section{Theory}
% \label{sec:theory}
% % In this section, we first formalize \textit{learning with intrinsic motivation} as an active learning problem. Under our formalization, a wide range of curiosity signals presented in prior works can be interpreted as approximations to the same objective. First, we elucidate the assumptions underlying different curiosity signals and assess why they may fail in the presence of white noise.  We then derive our proposed Progress curiosity signal and motivate its algorithmic and computational advantages over previously used progress measures. Next, we characterize the causal confusion problem in world model learning and show how it leads to catastrophic compounding errors. We then present our simple solution that involves injecting the causal graph prior into the world model architecture. % meg says: This paragraph starts with mentioning the active learning problem and curiosity signals, which makes it seem like the theory section is just focused on that, even though (with the current structure of the paper) causal confusion is also explained and it doesn't just fall under "active learning" 
% In this section, we formalize Active World Model Learning (AWML) as a Reinforcement Learning (RL) problem that generalizes conventional Active Learning (AL). We show how a wide range of previously proposed curiosity signals can be interpreted as proxies to a common intractable cost. Finally, we derive $\gamma$-Progress, a scalable progress-based curiosity signal with algorithmic and computational advantages over previous methods. 



\input{icml_sections/universal_curiosity.tex}


==> icml_sections/theory_dump.tex <==
Causal confusion is likely to occur when the training data distribution $p(\rvx)$ only covers a subset of the entire space $\X$, i.e $supp(p(\rvx))$ is small. The smaller the data coverage, the larger the space of degenerate solutions which do not respect the true causal structure of $P$.Causal confusion is likely to occur when the training data distribution $p_{train}(\rvx) \subset \X$ admits a different causal graph. 

Now consider a learned world model $P_{\theta}: \X \rightarrow \Y$.
\kh{formalize the disentanglement condition}
Any optimal world model should satisfy the following disentanglement condition for any causal graph $G_{P}$:
\begin{equation}
(P(\rvx))_{I_{\Y}} = (P_{\theta}(\rvx_{I_{\Y}^{-1}} \oplus \rvepsilon_{\setminus I_{\Y}^{-1}}))_{I_{\Y}} \quad \forall \rvepsilon \in \X, ~~\forall I_{y} \in A_{y}
\label{eq:causal_confusion}
\end{equation}

where $\rvx_{I_{\Y}^{-1}} \oplus \rvepsilon_{\setminus I_{\Y}^{-1}}$ denotes a concatenation of two vectors according to the indices $I_{\Y}^{-1}, \setminus I_{\Y}^{-1}$. In words, the subslices of model outputs $(P(\rvx))_{I_{\Y}}$ should only depend on the factors of variation that cause it, i.e $\rvx_{I_{\Y}^{-1}}$, and be unaffected by changes to nuisance factors of variation, i.e $\rvepsilon_{\setminus I_{\Y}^{-1}}$.

\begin{wrapfigure}{R}{0.45\textwidth}
\vspace{-10pt}
\begin{center}
    \includegraphics[width=.43\textwidth]{figures/causal_graph.pdf}
\end{center}
\vspace{-15pt}
\caption{\textbf{A causal graph.} Vertices represent external agents at times $t$ and $t+1$, edges represent causal relationships. Dashed boxes denote the connected component {\em external agent behaviors}.}
\label{fig:causal_graph}
\vspace{-10pt}
\end{wrapfigure}

%%%%%% What is causal confusion %%%%%%%
A learned model $P_{\theta}$ suffers from \emph{causal confusion} when it violates the disentanglement condition in Eq. \ref{eq:causal_confusion}, i.e changes in nuisance factors of variation $\rvepsilon_{\setminus I_{\Y^{-1}}}$ lead to changes in $P_{\theta}(\rvx)_{I_{\Y}}$. A causally confused model exhibits poor generalization performance when $p(\rvx) = p(\rvx_{I_{\Y}} | \rvx_{\setminus I_{\Y^{-1}}})p(\rvx_{\setminus I_{\Y^{-1}}})$ are distributed differently during training and validation time since off-distribution inputs can affect model outputs in unpredictable ways \citep{de2019causal}. 

As an intuitive example, consider an environment with two independent agents $A, B$ oscillating in sync with the same period. Let $\X = \Y$ comprise the joint position of the two agents and $I_{A}, I_{B}$ denote indices for each agent so that e.g $\rvx_{I_{A}}$ is the position coordinate of agent $A$. According to Def. \ref{def:causal_disentanglement}, the true world model $P: \X \rightarrow \X$ is causally disentangled since there exist partitions $\I_{\X} = \I_{\Y} = \{I_{A}, I_{B}\}$ and the identity bijective pairing $c(I) = I$ for which Eq. \ref{eq:causal_disentanglement} holds. The left graph in Fig. \ref{fig:causal_graph} shows the causal graph $G_{P}$ with two connected components, one for each periodic agent. \Inlike the true world model $P$, a causally confused learned model $P_{\theta}$ may predict the next position of agent $A$ from the current position of agent $B$ as shown in the right graph of Fig. \ref{fig:causal_graph}. $P_{\theta}$ may perform well on the training data so long the nuisance variables follow a fixed distribution




%%%%%% Why is causal confusion likely to occur? %%%%%%%
Now let us reason about why causal confusion is likely to occur when learning world models in real environments. 

% There's a distinction between an example of causal confusions and an example that illustrates why causal confusion is likely in real environments. The above example only shows the former. Is it indeed true that causal confusion is likely to occur? If so, why? 

% However, a causally confused model may have a causal graph with the dotted edge where the $\rvo_{I_{p1}}^{t+1}$ depends on the nuisance variable $\rvo_{I_{p2}}^{t}$. Since the periodic agents are in lockstep

Due to the partial observability of real-world environments (described in Section \ref{sec:environment}), our curious agent must have object permanence in order to make accurate predictions of when and where stimuli that disappear from view will reappear. This requires allocating dimensions of the world model input space $\X$ to tracking states of stimuli that are not in view. For example, $\rvx \in \X$ could include an object-centric representation with dimensions explicitly allocated for each object state or the hidden states of a recurrent neural network.


Object permanence can be encoded as an architectural prior by structuring the world model input space to be object-centric


There exists subdimensions of your input space that corresponds to "permanence" related representations. This could be explicit with an object-centric representation, or implicitly encoded in the hidden state representations learned by an LSTM.



There are several reasons for why we observe a distributional difference in the nuisance variables. First, due to model bootstrapping, the distribution of $\rvepsilon_{\setminus I_{\Y^{-1}}}$ changes with the number of timesteps having not seen the stimuli corresponding to $I_{\Y}$ which is affected by the curious agent's policy. Thus, policy changes during training and validation, i.e $D_{\text{KL}}(\rho_{\pi} || \mu)$, can lead to distributional mismatch of nuisance variables. Second, the nuisance variable distribution changes as a function of the world model. When interlacing validation and world model updates, it's most likely the training data doesn't contain many samples from the most recent version of the world model.
\kh{equipartition theorem. Put in footnote why bijective and not surjective}
\kh{Emphasize this problems arise especially in the interactive learning setting}
\kh{intuition for bipartite graph}

\kh{present simple example with two periodic agents}

\kh{Now explain our solution}











%%%%%%%%%%%%% New theory dump %%%%%%%%%%%%%%
\begin{definition}
\label{def:causal_disentanglement}
Let $\I_{\X} \in \emph{Part}(\{1, ..., \emph{dim}(\X)\}), \I_{\Y} \in \emph{Part}(\{1, ..., \emph{dim}(\Y)\})$ be maximally large partitions for which there exists a surjective map $c: \I_{\X} \rightarrow \I_{\Y}$ and sub-models $\{P^{I_{\X}}: \X_{I_{\X}} \rightarrow \Y_{c(I_{\X})} | I_{\X} \in \I_{\X}\}$ such that
\begin{equation}
P(\rvx)_{c(I_{\X})} = P^{I_{\X}}(\rvx_{I_{\X}}) \quad \forall I_{\X} \in \I_{\X},~~\forall \rvx \in \X
\label{eq:causal_disentanglement}
\end{equation}
where $\emph{Part}(S)$ is the universe of partitions a set $S$, $\rvx_{I_{\X}} := [x_{i}]_{i \in I_{\X}}$, and $\X_{I_{\X}} := \{\rvx_{I_{\X}} | \rvx \in \X\}$. Then, $G_{P} = (V, E)$ is a \textbf{causal graph} of $P$ where $V = \I_{\X} \cup \I_{\Y}, E = \{(I_{\X}, I_{\Y}) | I_{\X} \in \I_{\X}, I_{\Y} \in \I_{\Y}, I_{\Y} = c(I_{\X})\}$. 
\end{definition}

Let $P: \X \rightarrow \Y$ be a function and $\rvx \in \X, \rvy = P(\rvx)$ be random variables. $G_{P} = (V, E)$ of $P$ if 
\begin{enumerate}
\item $V = \{\rvx_{1}, ..., \rvx_{\emph{dim}(\X)}, \rvy_{1}, ..., \rvy_{\emph{dim}(\Y)}\}$
\item $(v_{\X}, v_{\Y}) \in E$ iff $\exists $
\end{enumerate}



and its occupancy measure is defined as $\rho_{\pi}(\rvx, \rvy) = \sum_{t = 0}^{\infty} \beta^{t} \Pr( | \pi)$ where $\beta$ is a discount factor $0 \leq \beta \leq 1$. A world model $\omega_{\theta}: \X \rightarrow \Omega(\Y)$ is stochastic function that encapsulates a property of the world. For example, $P$ is the forward dynamics kernel when $\X = \S \times \A$ and $\Y = \S$. In general, $\X, \Y \subseteq \S^{*} \times \A^{*}$ where $\S^{*}, \A^{*}$ are sets of all arbitrary length state, action sequences, i.e the Kleene closure of $\S, \A$. Further let $f: (\X \times \Y)^{*} \rightarrow \Theta$ be a learning algorithm for $\omega_{\theta}$. GAL aims to learn a policy $\pi$ to collect samples $(\rvx, \rvy)$ from the world which maximally reduce world model loss $\LL(\theta)$. 
\begin{equation}
\min_{\pi_{k+1}}{\mathop{\E}_{\substack{\rvx, \rvy \sim \\ \rho_{\pi_{k+1}}, P(\cdot | \rvx)}}[\LL(f(\cup_{i = 0}^{k} \mc{D}^{i} \cup \{(\rvx, \rvy)\})) - \LL(f(\cup_{i = 0}^{k} \mc{D}^{i}))] }
\label{eq:active_obj}
\end{equation}


\X \rightarrow \Omega(\Y)$, where $\Omega(\Y)$ is the set of probability measures on $\Y$, is a stochastic function that encapsulates a property of the world. For example, $P$ is the forward dynamics kernel when $\X = \S \times \A$ and $\Y = \S$. In general, $\X, \Y \subseteq \S^{*} \times \A^{*}$ where $\S^{*}, \A^{*}$ are sets of all arbitrary length state, action sequences, i.e the Kleene closure of $\S, \A$. The embodied agent agent interacts with the world according to a policy $\pi: \S \rightarrow \Omega(\A)$, in the process collecting samples $(\rvx, \rvy) \in \X \times \Y$ which are used to update its world model $P_{\theta}: \X \rightarrow \Omega(\Y)$ by minimizing a loss $\LL(\theta)$. Intuitively, $\pi$ distills the agent's strategy for querying useful data from the world, e.g directed attention towards animate external agents. For a policy $\pi$, we also define its occupancy measure $\rho_{\pi}: \S \times \A \rightarrow \RR$ as $\rho_{\pi}(s, a) = \sum_{t = 0}^{\infty} \beta^{t} \Pr(s_{t} = s, a_{t} = a | \pi)$ where $\beta$ is a discount factor $0 \leq \beta \leq 1$. Let $f: (\X \times \Y)^{*} \rightarrow \Theta$ be a learning algorithm. \kh{define input/output space explicitly} In traditional active learning, a single round of optimization comprises a data collection strategy update step (choosing which $\rvx$ to query a label for) and model update step. By analogy we can similarly formalize Learning with Intrinsic Motivation. In round $k + 1$, the data collection strategy update step solve the following policy optimization problem: \kh{end state distribution is the initial state distribution}:


\subsection{Active World Model Learning}
\label{sec:active_learning}
\kh{Add general definition with $z$ instead of specifying the forward problem. No access to querying prior distribution}


\kh{Define the generalization of active learning first.}



Informally, Active World Model Learning (AWML) is the process of learning how to efficiently collect information from the world to minimize world model loss. Concretely, we represent an embodied agent in a generic world (or "environment") as a tuple $(\S, \A, P)$ where $\S, \A$ are state, action spaces of the agent and $P: \X \rightarrow \Omega(\Y)$, where $\Omega(\Y)$ is the set of probability measures on $\Y$, is a stochastic function that encapsulates a property of the world. For example, $P$ is the forward dynamics kernel when $\X = \S \times \A$ and $\Y = \S$. In general, $\X, \Y \subseteq \S^{*} \times \A^{*}$ where $\S^{*}, \A^{*}$ are sets of all arbitrary length state, action sequences, i.e the Kleene closure of $\S, \A$. The embodied agent agent interacts with the world according to a policy $\pi: \S \rightarrow \Omega(\A)$, in the process collecting samples $(\rvx, \rvy) \in \X \times \Y$ which are used to update its world model $P_{\theta}: \X \rightarrow \Omega(\Y)$ by minimizing a loss $\LL(\theta)$. Intuitively, $\pi$ distills the agent's strategy for querying useful data from the world, e.g directed attention towards animate external agents. For a policy $\pi$, we also define its occupancy measure $\rho_{\pi}: \S \times \A \rightarrow \RR$ as $\rho_{\pi}(s, a) = \sum_{t = 0}^{\infty} \beta^{t} \Pr(s_{t} = s, a_{t} = a | \pi)$ where $\beta$ is a discount factor $0 \leq \beta \leq 1$. Let $f: (\X \times \Y)^{*} \rightarrow \Theta$ be a learning algorithm. \kh{define input/output space explicitly} In traditional active learning, a single round of optimization comprises a data collection strategy update step (choosing which $\rvx$ to query a label for) and model update step. By analogy we can similarly formalize Learning with Intrinsic Motivation. In round $k + 1$, the data collection strategy update step solve the following policy optimization problem: \kh{end state distribution is the initial state distribution}:


In this work we choose the forward dynamics problem as the world model problem. Specifically, we aim to learn a forward model $P_{\theta}: \X \rightarrow \Omega(\Y)$ over an input space $\X = \S \times \A$ of state-action pairs and a label space $\Y = \S$ of next states. Collectively, $(\rvx, \rvy)$ forms a transition. 


where $\mu(\rvx)$ is a prior distribution over the importance of correctly predicting the transition for $\rvx$. $\mu$ may also be interpreted as the validation data distribution. \kh{Is there something we can say about how active learning will bring $\rho_{\pi}$ closer to $\mu$?} For instance, if $\mu$ is the uniform distribution then an optimal world model must perfectly match the true environment dynamics for all $|\S|^{2}|A|$ possible transitions. Let $f: (\X \times \Y)^{*} \rightarrow \Theta$ be a learning algorithm. \kh{define input/output space explicitly} In traditional active learning, a single round of optimization comprises a data collection strategy update step (choosing which $\rvx$ to query a label for) and model update step. By analogy we can similarly formalize Learning with Intrinsic Motivation. In round $k + 1$, the data collection strategy update step solve the following policy optimization problem: \kh{end state distribution is the initial state distribution}:
\begin{equation}
\min_{\pi_{k+1}}{\mathop{\E}_{\substack{\rvx, \rvy \sim \\ \rho_{\pi_{k+1}}, P(\cdot | \rvx)}}[\LL(f(\cup_{i = 0}^{k} \mc{D}^{i} \cup \{(\rvx, \rvy)\})) - \LL(f(\cup_{i = 0}^{k} \mc{D}^{i}))] }
\label{eq:active_obj}
\end{equation}
where $\mc{D}_{i} = \{(\rvx, \rvy)_{j}\} \sim \pi_{i}$. In words, we seek a policy $\pi_{k + 1}$ which samples transitions that maximally reduce world model loss in expectation. At each iteration of the active learning loop, we perform two steps. First, optimize $\pi_{k}$ by solving Eq. \ref{eq:active_obj}. Second, update the world model parameters on the aggregate dataset $\cup_{i = 0}^{k} \mc{D}_{i}$. \Inlike the classic active learning with a pool setting, in which the data collection policy chooses $\rvx$ from a given pool of unlabeled data, we don't have access to a pool of unlabeled state-action pairs and label queries for $\rvx$ can only be made by learning a policy that can reach $\rvx$ in the environment. \kh{why can't you use a rollout of all possible trajectories as the unlabeled dataset }




\subsection{Connections between Curiosity Signals}
\label{sec:curiosity_signal}



\begin{comment}
We now formalize our the learning problem of our intrinsically motivated active learner as a batch active learning problem. At a high level, the curious agent seeks to minimize world model loss with as few interactions with the world as possible by adaptively collecting  batches of training samples. Concretely, our aim is to solve the forward dynamics world model problem defined over an input space $\X = \S \times \A$ and a label space $\Y = \S$, where $\S, \A$ are (countable) state, action spaces. Let

% While in the context of RL, world models have been leveraged to derive exploration bonuses that aid learning of a different task, our primary objective is to learn world models themselves.
Our intrinsically motivated agent engages in an active learning loop of collecting maximally informative data for the current world model, performing a world model update, and repeating the cycle. This problem corresponds to interlacing reinforcement learning over $\mc{M}(\theta_{i})$ and world model updates via supervised learning. Each MDP $\mc{M}_{i}$ seeks to learn an optimal data collection policy to maximize learning progress of the current world model. Let $\mc{M}(\theta) = (\S, \A, P, R_{\theta}, T)$ be a finite horizon MDP where $\S, \A$ are (countable) state, action spaces, $P: \S \times \A \rightarrow \mc{P}(\S)$ is the dynamics where $\mc{P}(\S)$ is the set of probability measures on $\S$, $R$ is the reward function, and $T$ is the episode length. A (stationary) policy $\pi: \S \rightarrow \mc{P}(\A)$ maps states to distributions over actions. Our objective is to learn a world model $P_{\theta}$ that matches $P$ with more emphasis on state, action pairs specified by a prior distribution $q(s, a)$.
\begin{equation}
J(\theta) = -\E_{(s, a) \sim q}[D_{KL}(P(\cdot | s, a) || P_{\theta}(\cdot | s, a))] \leq 0
\label{eq:model_performance}
\end{equation}
Intuitively, $q$ has concentrated probability mass on state-action pairs for which predicting the next state distribution correctly is more important. For example, the prior $q$ may capture the inherent inclination of humans to attend more to animate agent like features.
% where $u_{\S \times \A}$ is a uniform distribution over $\S \times \A$. A uniform distribution was chosen for simplicity, but it may be replaced with any distribution fully supported on $\S \times \A$.
Let $f: \Theta \times \mc{D} \rightarrow \Theta$ be the optimizer which updates our world model parameters $\theta$ given data $\mc{D} = \{(s, a, s')_{i}\}$ in the form of transition triplets.


\begin{equation}
\pi^*(\theta) = \argmax_{\pi} \E_{\mc{D} \sim \pi} [J(f(\theta, \mc{D})) - J(\theta)] \quad \text{where} \quad |\mc{D}| \leq K
\label{eq:pi_objective}
\end{equation}
In words, a policy behaves optimally with respect to the current world model $\theta$ and an optimizer $f$ if it samples a trajectories that maximally improve the performance of the model. $K$ captures the memory constraint of an active learning agent. We see that Eq. \ref{eq:pi_objective} cannot be directly optimzied since we cannot predict the value of $J(P_{\theta'})$ before performing an optimization step. Let us assume that the optimizer $f$ satisfies the following additive property:
\begin{align*}
J(f(\theta, \{(s, a, s')_{i}\})) - J(\theta) \approx \sum_{i} J(f(\theta, (s, a, s')_{i}) - J(\theta)
\end{align*}
Then, the policy performance objective can be written as:
\begin{align*}
    \argmax_{\pi} \E_{\mc{D} \sim \pi} [\sum_{(s, a) \in \mc{D}} J(f(\theta, (s, a, s'))) - J(\theta)] \quad \text{where} \quad |\mc{D}| \leq K
\end{align*}
Taking the policy gradient we obtain:
\begin{align*}
    \E_{\pi} [\nabla\log{\pi} \sum_{t} J(f(\theta, (s_{t}, a_{t}, s_{t+1}))) - J(\theta)] \quad \text{where} \quad |\mc{D}| \leq K
\end{align*}

The reward quantity of interest is the future progress on the objective that can be made by having the sample $(s_{t}, a_{t}, s_{t+1})$. However this quantity cannot be calculated without evaluating the our objective $J$ and taking an optimization step $f$. The former is intractable and the later is expensive. Instead we seek to make an approximation to $J(P_{\theta'}) - J(P_{\theta})$ based on information we have obtained about $f$ and $J$ in the past.

\subsubsection{adversarial}
uncertainty sampling
For example, we might assume that future progress is proportional to the current world model loss:
\begin{align*}
    J(\theta') - J(\theta) \approx -\beta J(\theta)
\end{align*}

\subsubsection{Progress}
Active learning sampling technique: estimated error reduction \\
We may instead make the assumption that future progress is proportional to our previous experience updating on the data:
\begin{align*}
    J(\theta'') - J(\theta') \approx -\beta (J(\theta') - J(\theta))
\end{align*}

\subsubsection{disagreement}
Active learning sampling technique: query by committee.
In practice we need a prior over the

Notice that we cannot directly perform RL with the objective in Eq. (2) since we do not have access to the ground truth world model $P$. Hence, we formulate a surrogate objective to (2) based on learning progress:

Note that this is equivalent to optimizing over an MDP with a non-stationary reward function. Your behavior not only changes the distribution of states you encounter, but also the reward function.
\end{comment}


==> icml_sections/universal_curiosity.tex <==
\section{Active World Model Learning}
\label{sec:theory}
In this section, we formalize Active World Model Learning (AWML) as a Reinforcement Learning (RL) problem that generalizes conventional Active Learning (AL). We then derive $\gamma$-Progress, a scalable progress-based curiosity signal with algorithmic and computational advantages over previous progress-based curiosity signals. 

Consider an agent in an environment $\mc{E} = (\S, \A, P, P_{0})$ where $\S, \A$ are state, action spaces, $P: \S \times \A \rightarrow \Omega(\S)$ is the transition dynamics, $\Omega(\S)$ is the set of probability measures on $\S$, and $P_{0}$ is the initial state distribution. The agent's goal is to optimize a sequence of data collection decisions in order to learn a model $\omega_{\theta}$ of a target function $\omega: \X \rightarrow \Omega(\Y)$ with as few data samples as possible. We model this agent's decision making process as an infinite horizon Markov Decision Process (MDP) $\mc{M} = (\bar{\S}, \A, \bar{P}, \bar{P}_{0}, c)$. Intuitively, $\mc{M}$ is a meta-MDP that jointly characterizes the evolution of the environment, collected data history, and the model as the agent makes data collection decisions to optimize the learning objective encoded by the MDP reward. Specifically, $\bar{\rvs} \in \bar{\S} = \S \times \mc{H} \times \Theta$ is a meta-state that decomposes into $\bar{\rvs} = (\rvs, H, \theta)$ where $\rvs \in \S$ is an environment state, $H = \{\rvs_{0}, \rva_{0}, \rvs_{1}, \rva_{1} ...\} \in \mc{H}$ is the history of visited environment state-actions, and $\theta \in \Theta$ is the current model parameters. Intuitively $H$ is a raw form of the data collected so far which can be post-processed to yield a training set for $\omega_{\theta}$. $\rva \in \A$ is a data collection decision, e.g where to move next in the environment, and the meta-dynamics $\bar{P}: \bar{\S} \times \A \rightarrow \Omega(\bar{\S})$ is defined as: 
\begin{align*}
(\rvs', &H', \theta') \sim \bar{P}(\cdot | \bar{\rvs} = (\rvs, H, \theta), \rva) ~~ \text{where}\\
&\rvs' \sim P(\rvs, \rva),~H' = H \cup \{\rva, \rvs'\},~\theta' \sim P_{\ell}(H', \theta) 
\end{align*}
where $P_{\ell}: H \times \Theta \rightarrow \Omega(\Theta)$ is transition function for the model parameters, e.g a (stochastic) learning algorithm which updates the parameters on the history of data. In words, $\bar{P}$ steps the environment state $\rvs$ according to the environment dynamics $P$, appends the history with new data, and updates the model $\omega_{\theta}$ on the augmented history. The meta-initial state distribution is $\bar{P}_{0}(\bar{\rvs} = (\rvs, H, \theta)) = P_{0}(\rvs)\mathbbm{1}(H = \{\})q(\theta)$ where $\mathbbm{1}$ is the indicator function and $q(\theta)$ is a prior distribution over the model parameters. $c: \S^* \times \A^* \rightarrow \RR$ is the cost function which encodes the learning objective of the agent. For example, $c(\bar{\rvs} = (\rvs, H, \theta)) = \LL_{\mu}(\theta) = \E_{\mu}[\LL(\theta, \rvx, \rvy)]$ encodes the goal of an agent seeking to minimize a loss function $\LL$ on data $(\rvx, \rvy) \sim \mu$ while training on a minimal number of data samples. A policy $\pi: \S \rightarrow \Omega(\A)$ maps states to action distributions and an optimal policy $\pi^* = \argmax_{\pi} J(\pi)$ achieves the highest performance $J(\pi) = -\E_{\pi}[\sum_{t = 0}^{\infty} \beta^{t} c(\bar{\rvs})]$ where $0 \leq \beta \leq 1$ is a discount factor. Overall, the MDP $\mc{M}$ is constructed from an environment $\mc{E} = (\S, \A, P, P_{0})$, a target function $\omega$, a learning algorithm $P_{\ell}$, and a prior parameter distribution $q(\theta)$. Appendix \ref{sec:app:gal_cal_connection} shows how several variants of conventional active learning can be recovered by appropriately defining the MDP $\mc{M}$ in relation to $\omega, \X, \Y$. 

\begin{figure*}[t!]
    \centering
    \includegraphics[width=\textwidth]{figures/model.pdf}
    \vspace{-15pt}
    \caption{\textbf{Active World Model Learning with $\gamma$-Progress} The curious agent consists of a \emph{world model} and a \emph{progress-driven controller}. The curious agent's observations $\rvo_t$ are passed through an encoding oracle $e$ that returns an object-oriented representation $\rvx_t$ containing the positions of external agents that are in view, auxiliary object positions, and the curious agent's orientation. Both the new (black) and old (gray) models take as input $\rvx_{t-\tau_{in}:t}$ and predict $\hat{\rvx}_{t:t+\tau_{out}}$. The old model weights, $\theta_{old}$, are slowly updated to the new model weights $\theta_{new}$. The controller, $\pi_{\phi}$, is optimized to maximize $\gamma$-Progress reward: the difference $\LL(\theta_{old}) - \LL(\theta_{new})$.}
    % dotted lines 
    \label{fig:model}
    \vspace{-10pt}
\end{figure*}


We now formalize the Active World Model Learning (AWML) problem using this general active learning framework. Formally, AWML aims to find an optimal policy for the meta MDP $\mc{M}$ with the additional constraint that $\X, \Y$ are arbitrary length sequences of environment states and actions. In words, the target function $\omega$ is constrained to be a self supervised predictor on trajectories sampled from the environment. We henceforth aptly refer to $\omega_{\theta}$ as the world model. Consider a simple AWML problem of learning the forward dynamics, i.e $\X = \S \times \A, \Y = \S, P = \omega$, and 
\begin{align}
c(\bar{\rvs}, \rva, \bar{\rvs}') = \LL_{\mu}(\theta) - \LL_{\mu}(\theta')
\label{eq:cost}
\end{align}
where $\bar{\rvs} = (\rvs, H, \theta), \bar{\rvs}' = (\rvs', H', \theta')$, with a discount factor $\beta < 1$ to encourage minimal interactions with the environment. Recall that $\theta' = P_{\ell}(H \cup \{\rva, \rvs'\}, \theta)$ is the updated model parameters after collecting new data $\{\rva, \rvs'\}$. Thus $-c(\bar{\rvs}, \rva, \bar{\rvs}')$ measures the reduction in world model loss as a result of obtaining new data $\{\rva, \rvs'\}$, i.e the \emph{prediction gain}. Unfortunately, evaluating prediction gain at every environment step involves repeatedly computing $\LL_{\mu}(\theta) - \LL_{\mu}(\theta')$ which is typically intractable as many samples are needed estimate the expectation. This bottleneck necessitates an efficiently computable proxy reward to estimate Eq. \ref{eq:cost}. Thus, solving the AWML problem entails solving two sub-problems: Proxy reward design and Reinforcement Learning (RL). See Appendix \ref{sec:app:curiosity_connection} to see how a variety of curiosity signals proposed in prior work can be interpretted as \citep{stadie2015predictive, burda2018exploration, pathak2019disagreement, achiam2017surprise} solution attempts to the former problem. We now motivate $\gamma$-Progress by first outlining the limitations of a previously proposed progress-based curiosity signal, $\delta$-Progress.  

%%%%%%%%%%%%%% Progress %%%%%%%%%%%%%%%%%%
\textbf{$\delta$-Progress} \citep{achiam2017surprise, graves2017automated} curiosity measures how much better the current new model $\theta_{new}$ is compared to an old model $\theta_{old}$.
\begin{equation}
\LL_{\mu}(\theta) - \LL_{\mu}(\theta') \simeq \log{\frac{\omega_{\theta_{new}}(\rvs' | \rvs, \rva)}{\omega_{\theta_{old}}(\rvs' | \rvs, \rva)}}
\label{eq:progress_curr}
\end{equation}
The choice of $\theta_{new}, \theta_{old}$ is crucial to the efficacy of the progress reward. A popular approach \citep{achiam2017constrained, graves2017automated} is to choose
\begin{equation}
\theta_{new} = \theta_{k}, \quad \theta_{old} = \theta_{k - \delta}, \quad \delta >0
\label{eq:kstep_progress}
\end{equation}
where $\theta_{k}$ is the model parameter after $k$ update steps using $P_{\ell}$. Intuitively, if the progress horizon $\delta$ is too large, we obtain an overly optimistic approximation of future progress. However if $\delta$ is too small, the agent may prematurely give up on learning hard transitions, e.g where the next state distribution is very sharp. In practice, tuning the value $\delta$ presents a major challenge. Furthermore, the widely pointed out \citep{pathak2019disagreement} limitation of $\delta$-Progress is that the memory usage grows $\O(\delta)$, i.e one must store $\delta$ world model parameters $\theta_{k - \delta}, ..., \theta$. As a result it is intractable in practice to use $\delta > 3$ with deep neural net models. 

\textbf{$\gamma$-Progress (Ours)} We propose the following choice of $\theta_{new}, \theta_{old}$ to overcome both hurdles:
\begin{equation}
\theta_{new} = \theta, \quad \theta_{old} = (1 - \gamma) \sum_{i = 1}^{k - 1} \gamma^{k - 1 - i} \theta_{0}
\label{eq:mix_progress}
\end{equation}
In words, the old model is a weighted mixture of past models where the weights are exponentially decayed into the past. $\gamma$-Progress can be interpreted as a noise averaged progress signal. Conveniently, $\gamma$-Progress can be implemented with a simple $\theta_{old}$ update rule:
\begin{equation}
    \theta_{old} \leftarrow \gamma \theta_{old} + (1 - \gamma) \theta_{new}
\label{eq:mix_update_rule}
\end{equation}
Similar to Eq. \ref{eq:kstep_progress}, we may control the level of optimism towards expected future loss reduction by controlling the progress horizon $\gamma$, i.e a higher $\gamma$ corresponds to a more optimistic approximation. $\gamma$-Progress has key practical advantages over $\delta$-Progress: $\gamma$ is far easier to tune than $\delta$, e.g we use a single value of $\gamma$ throughout all experiments, and memory usage is constant with respect to $\gamma$. Crucially, the second advantage enables us to tune the progress horizon so that the model does not prematurely give up on exploring hard transitions. The significance of these practical advantages will become apparent from our experiments. 



==> sections/asymptotic.tex <==
\subsection{Asymptotic Model Performance in Supervised Learning}
\label{sec:offline}

Here we evaluate the capacity for the world model to learn each of the animate external agent behaviors, isolating this measurement from any choice of policy. We gather 400k environment steps of data using a reduced action space random policy: for each action choice, the agent chooses randomly between 0- and 12-degree rotation in either direction. These data collection choices represent ``ideal'' data by ensuring plentiful exposure to each stimulus for long stretches of time. For this metric, we exclude the peekaboo animate external agent behavior, as due to the curious agent-contingent behavior of the peekaboo agent, one cannot expect ``ideal data'' to be gathered without a learned policy. We then train the world model to convergence and aggregate validation performance across five validation cases for each external agent behavior. 

We compare the performance of our causal world model to two acausal ablations: one {\em joined} that instead takes as input and predicts all external agents together, and one {\em split} that treats each agent separately, as opposed to behavior (so e.g. in the case of the chasing behavior, our causal world model takes as input both chaser and runner agent in order to predict the runner, whereas this predicts runner from runner alone). They employs the same architecture as a single behavior network in the causal world model (Section~\ref{sec:methods:worldmodel}), except with the number units for each hidden layer chosen so as to match roughly the total number of weights.

As seen in Figure~\ref{fig:offline_asymptotic_performance}, across all experiments, the causal world model significantly outperforms the ablation, with the acausal ablation obtaining $9.8\times$ the validation loss, on average across seeds and behaviors. Justifying the interpretation of ``ideal data'', for the causal world model, performance is comparable to the best achieved under online learning under the best policy found. Upon visual inspection of predictions, the causal world model appeared to ``get'' each animate external agent behavior, at least up to what the stochasticity of the external agent behaviors allow. To contrast, the acausal ablation exhibits not only poorer performance but considerable variance in performance, and visual inspection found that these models captured essential low order statistics across the first several timesteps of behavior, but that prediction rollouts quickly deteriorated. \nh{We should really add videos!} \ms{add agent-wise causal ablation}

==> sections/attention_determinants.tex <==
\section{Determinants of attention pattern}
\label{sec:app:attention_determinants}
To gain a finer-grained understanding of what, of the factors we vary (intrinsic motivation, world model architecture, and stimulus type) drives the attentional behavior of these active learning systems, we perform a linear regression. Specifically, we regress
\begin{equation} \label{eq:regression}
R_{\mathrm{animate}/\mathrm{noisy}} = a + b \cdot \chi_{\mathrm{IM}} + c \chi_{\mathrm{causal}} + d \cdot \chi_{\mathrm{BHR}} + \chi_{\mathrm{causal}} * e \cdot \chi_{\mathrm{IM}} + \epsilon
\end{equation}
Here $R_{\mathrm{animate}/\mathrm{noisy}}$ is the ratio of animate to noisy attention, $\chi_{\mathrm{IM}}$ is a one-hot encoding of curiosity signal (all zeros if random policy), $\chi_{\mathrm{causal}}$ is an indicator set to $1$ if the architecture is causal, $\chi_{\mathrm{BHR}}$ is a one-hot encoding of animate external agent behavior shown (all zeros if deterministic reaching), and $a,  b, c, d, e$ are fixed effects ($e$ measures an interaction effect).

Over $371$ individual active learning runs, an ordinary least squares regression achieves an adjusted $R^2$ of $.44$. Please see Table~\ref{table:regression} for details. We found that $\gamma$-Progress receives significant positive weight, while Disagreement and Adversarial receive significant negative weight, with the other curiosity signals having an effect close to that of random policy. In addition, we fail to find a significant effect due to architecture and most external agent behaviors, with two external agent behavior exceptions. In sum, we find that, of the architectural and intrinsic motivation variations we tested, intrinsic motivation strongly drives behavior whereas architecture plays an insignificant role. \nh{i can broaden this to a third architecture class!}

\begin{table*}
\caption{
\textbf{Attention regression.} Regression model of animate/noisy attention, according to Equation~\ref{eq:regression}. Coefficient values found, and uncorrected p-value for 2-sided t-tests, with significance at the $.05$ level in bold.}
\vspace{-0.1cm}
\label{table:regression}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcc}
\toprule
Coefficient & value & P > |t| \\
\midrule
constant & .80 & .001 \\
$\gamma$-Progress & \textbf{2.24} & .000 \\
$\delta$-Progress & .08 & .788 \\
RND & -.53 & .064 \\
Disagreement & \textbf{-.70} & .014 \\
Adversarial & \textbf{-.79} & .006 \\
\midrule
Causal architecture & .014 & .959 \\
\midrule
stochastic reaching & .14 & .493\\
deterministic chasing & .25 & .222 \\
stochastic chasing & \textbf{.45} & .029 \\
deterministic peekaboo & -.08 & .682\\
stochastic peekaboo & .02 & .920\\
mimicry & \textbf{.56} & .006\\
\midrule
causal $\times \gamma$-Progress & -.32 & .408 \\
causal, $\times \delta$-Progress & .06 & .868 \\
causal $\times$ RND & .03 & .935 \\
causal $\times$ Disagreement & .23 & .555 \\
causal $\times$ Adversarial & -.09 & .813 \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\end{table*} 


==> sections/causal_confusion.tex <==
\subsection{Causal Confusion in World Models}
\label{sec:causal_conf}

\begin{comment}
Paragraph outline
1. world model framework, introducing and justifying an object-centric representation
2. illustrate by example the causal confusion problem. What is the ground truth function for these coordinates.
3. effect of causal misidentification in the case of partial observability. show this formalization with symbols.
4. our solution. defines a causal graph, and describes the basic point of the solution. maybe a formula for the causal case and the acausal case.
\end{comment}

In this section, we first formalize the causal confusion problem, reason about its propensity to occur in the interactive learning setting, and motivate our causal world model architecture. Consider the (deterministic) dynamics function $P: \X \rightarrow \Y$. \kh{include thing about encoding space} We consider deterministic dynamics for compactness of notation in what follows, but the presented analyses may be extended to stochastic dynamics. Henceforth we use the vector slicing notations $\rvx_{I} := [\rvx_{i}]_{i \in I}$, and $\X_{I} := \{\rvx_{I} | \rvx \in \X\}$. We start by defining a causal graph. 

\begin{definition}
\label{def:causal_disentanglement}
Let $P: \X \rightarrow \Y$ be a function. For each $I_{\Y} = 1, ..., \emph{dim}(\Y)$, let its preimage $I_{\Y}^{-1} = \{I_{\X} | I_{\X} \subseteq \{1, ..., \emph{dim}(\X)\}\}$ be a set satisfying the following: 
\vspace{-5pt}
\begin{enumerate}
    \item (modularity) $\forall I_{\X} \in I_{\Y}^{-1}, \exists \tilde{P}: \X_{I_{\X}} \rightarrow \Y_{I_{\Y}}$ such that $P(\rvx)_{I_{\Y}} = \tilde{P}(\rvx_{I_{\X}})~\forall \rvx \in \X$
    \vspace{-5pt}
    \item (minimality) $\forall I_{\X} \in I_{\Y}^{-1}, \nexists i \in I_{\X}$ such that property $1$ holds for $I_{\X} \setminus \{i\}$
\end{enumerate}
\vspace{-5pt}
Then, a \textbf{causal graph} is $G_{P} = (V, E)$ where $V = \{\rvx_{1}, ..., \rvx_{\emph{dim}(\X)}, \rvy_{1}, ..., \rvy_{\emph{dim}(\Y)}\}$ is a set of vertices and $E = \{(\rvx_{i}, \rvy_{I_{\Y})}| i \in I_{\X}, I_{\Y} = 1, ..., \emph{dim}(\Y)\}$ are the directed edges for any $I_{\X} \in I_{\Y}^{-1}$. 

Restatement (see comment): We define a \textbf{causal graph} to be a 
\end{definition}

\nh{I like this definition better, but I think a few things need to be changed:
(1) $I_X$ and $I_Y$ should look more different. One is an integer and the other is a set of integers, whereas the notation suggests that they're analogous for $X$ and $Y$.
(2) Definitions of $V$ and $E$ should not have $x$ and $y$s in them, because then it seems like there are different vertices for the same indices but different points for each $(x, P(x))$ as we vary $x$. Let me try to establish notation in the below lemma, see if you like it.
(3) (And maybe I am misunderstanding the definition, but...) it needs to be clear that for a given causal graph, one makes a unique choice of $I_X \in I_Y$
}

Notice that every dynamics $P$ has a causal graph, since the fully connected bipartite graph from vertices for $\rvx$ to vertices for $\rvy$ can make up a trivial causal graph. However, the causal graph need not be unique (see Appendix \ref{sec:app:causal}). We henceforth use $\Gamma_{P}$ to refer to the family of causal graphs of $P$. We are now ready to formalize causal confusion. 

\begin{definition}
\label{def:causal_confusion}
A world model $P_{\theta}: \X \rightarrow \Y$ is causally confused w.r.t $P: \X \rightarrow \Y$ if $\Gamma_{P_{\theta}} \nsubseteq \Gamma_{P}$ 
\end{definition}

%% Why is causal confusion harmful for prediction?
In words, causal confusion is the failure of a world model to embody the correct disentanglement structure present in the target dynamics. This phenomenon can also be understood as overfitting to spurious correlations in the training data. Thus, causally confused models have poor generalization performance: 

\begin{comment}
Old version:
\begin{corollary}
Let $P_{\theta}: \X \rightarrow \Y$ be causally confused w.r.t $P$. Then for all $\I_{\X}, \I_{\Y}, c$ comprising a causal graph of $P$, there exists an input $\rvx \in \X$, a perturbed input $\rvx + \rvepsilon \in \X$, and $I_{\Y} \in \I_{\Y}$ such that,
\begin{equation*}
P(\rvx)_{I_{\Y}} = P(\rvx + \rvepsilon)_{I_{\Y}} = P_{\theta}(\rvx)_{I_{\Y}} \neq P_{\theta}(\rvx + \rvepsilon)_{I_{\Y}}
\end{equation*}
where $\rvepsilon_{I_{\Y}^{-1}} = \textbf{\emph{0}}^{|I_{\Y}^{-1}|}, \rvepsilon_{\setminus I_{\Y}^{-1}} \neq \textbf{\emph{0}}^{|\setminus I_{\Y}^{-1}|}$ for $I_{\Y}^{-1} = \bigcup_{\{I_{\X} | c(I_{\X}) = I_{\Y}\}} I_{\X}$ and $\textbf{\emph{0}}^{L}$ is an $L$-dim zero vector.
\end{corollary} 
\end{comment}

\nh{I made this a lemma, not a corollary, as stylistically you aren't supposed to have corollaries of definitions, but of other results. I'm not even really sure whether to call this a lemma, as it's basically a restatement of the definition, as is. (Maybe some previous version was more nontrivial? Could be that I just dumbed it down...) Usually in a case like this, I would say something like ``Observation''.}

\begin{lemma}
Let $P_{\theta}: \X \rightarrow \Y$ be causally confused w.r.t $P$. Then for all $G \in \Gamma_P$ such that $G \notin \Gamma_{P_\theta}$, there exists $I_X, I_Y$ with $\{(i, I_Y) \ | \ i \in I_X\} \subseteq G$ and $x, x' \in X$ with $x_i = x'_i$ for all $i \in I_X$ and
\begin{equation*}
    P(x) = P(x')
\end{equation*}
but
\begin{equation*}
    P_\theta(x) \neq P_\theta(x').
\end{equation*}
\end{lemma}


In words, a causally confused model's prediction $P_{\theta}(\rvx)_{I_{\Y}}$ is non-robust to perturbations of the inputs along the nuisance dimensions $\setminus I_{\Y}^{-1}$. Hence, a causally confused model that has overfit to spurious statistical dependencies $p_{\text{train}}(\rvy_{I_{\Y}} | \rvx_{\setminus I_{\Y}^{-1}})$ in the training set will have poor generalization performance on a validation set when $d(p_{\text{val}}(\rvy_{I_{\Y}} | \rvx_{\setminus I_{\Y}^{-1}}),  p_{\text{train}}(\rvy_{I_{\Y}} | \rvx_{\setminus I_{\Y}^{-1}})) \neq 0$ where $d$ is some distance metric between distributions.\footnote{Note than in the limit of infinite training data with full coverage over $\X$, a model will not be causally confused since the proper disentanglement can be learned by just memorizing the training data}

%% So why does the conditional distribution change? 
%% Need to also explain that true models are likely causally disentangled 
Causal confusion is more likely to occur and more detrimental to generalization performance when learning world models of partially observable environments by interactive learning. To see this, consider a world model $P_{\theta}$ of a partially observable environment with dynamics $P: \X \rightarrow \Y$ that have a non-trivial causal graph. Due to partial observability, the world model must solve two types of predictions problems: supervised prediction and permanence prediction. Supervised prediction involves predicting the dynamics of stimuli that are currently observable and permanence prediction involves predicting the dynamics of non-observable stimuli. For the world model to solve both prediction tasks, the inputs $\rvx \in \X$ should encode both current observations - e.g images, coordinates of stimuli that are in view - when available and permanence information - e.g mental estimates of how the non-visible stimuli are moving. \footnote{Any memory efficient model should minimize the number of observations, which are typically high-bandwith, and maintain a compact encoding of permanence information instead of taking as input an arbitrary sequence of high-bandwith observations} 

Thus, the nuisance factors $\rvx_{\setminus I_{\Y}^{-1}}$ for any output $\rvy_{I_{\Y}}$ must encode permanence information impertinent to predicting $\rvy_{I_{\Y}}$. For example, $\rvx_{I_{\Y}^{-1}}$ could correspond to the position inputs of the currently visible external agent while $\rvx_{\setminus I_{\Y}^{-1}}$ could correspond to a mental estimate of where the non-visible external agents are or a counter that tracks the number timesteps since the last encounter with them. Such permanence information can be explicitly identified when the world model has a structured input ($\X$), output ($\Y$) space that allocates separate space for permanence information and implicitly identified in the hidden states of memory augmented function approximators such as Long Short-Term Memory (LSTM) networks. 

There may exist a drastic distributional shift of the permanence variables between training and validation, i.e $d(p_{\text{val}}(\rvy_{c(I_{\X})} | \rvx_{\setminus I_{\X}}),  p_{\text{train}}(\rvy_{c(I_{\X})} | \rvx_{\setminus I_{\X}})) \gg 0$, due to two factors. First, changes in the data collection policy with interactive learning leads to changes in the visitation frequencies for each stimuli which changes the distribution of permanence variables such as the visitation counters. In the interactive learning setting there indeed may be policy differences between training and validation time and we desire the world model to be robust to changes in policy. 

Second, updates to the world model parameters can change the permanence variable distribution. In the interactive learning setting we interlace data collection and world model update, and will indeed experience constant changes to the world model parameters. Furthermore, permanence predictions, such as predicting the position of an external agent after a long look-away, are typically significantly harder than supervised predictions and thus the permanence representations will take much longer to stabilize in distribution due to large gradients.  

\begin{wrapfigure}{R}{0.45\textwidth}
\vspace{-10pt}
\begin{center}
    \includegraphics[width=.43\textwidth]{figures/causal_graph.pdf}
\end{center}
\vspace{-15pt}
\caption{\textbf{A causal graph.} Vertices represent external agents at times $t$ and $t+1$, edges represent causal relationships. Dashed boxes denote the connected component {\em external agent behaviors}.}
\label{fig:causal_graph}
\vspace{-10pt}
\end{wrapfigure}

To gain intuition about causal confusion in interactive learning, consider an environment with two independent external agents $A, B$ oscillating in sync with the same period. Let $\X = \Y$ $I_{A}, I_{B}$ denote indices for each agent so that e.g $\rvx_{I_{A}}$ is the position coordinate of agent $A$ when it is visible and a bootstrapped model estimate of agent $A$'s position when it is not visible. According to Def. \ref{def:causal_disentanglement}, the true dynamics $P: \X \rightarrow \X$ have a causal graph $G_{P}$ defined by $\I_{\X} = \I_{\Y} = \{I_{A}, I_{B}\}$ and the identity bijective pairing $c(I) = I$. The left graph in Fig. \ref{fig:causal_graph} visualizes $G_{P}$ with two connected components, one for each periodic agent. The right graph of Fig. \ref{fig:causal_graph} shows an example world model $P_{\theta}$ that is causally confused. $P_{\theta}$ predicts the next position of agent $A$ from the current position of agent $B$. Such a model could've been learned on a training set collected with a policy that rapidly shifts between agent $A, B$. Frequent shifts allow the model estimated position to remain accurate since the number of bootstrapping steps are small, and thus the model is able to achieve low training error since the agents are oscillating in sync. However the validation set may test for robustness of the world model with data collected by a less frequently switching policy. In this case, the bootstrapped model estimates for agent $B$ may shift in distribution and degrade the predictions for agent $A$ even when agent $A$ is in view. 

To ameliorate this, we propose to inject a causal prior into the world model, specified by a causal graph $G_{P}$. The causal graph has one vertex $v_{i, t}$ for each external agent $i$ for each timestep $t$, and a (directed) edge from $v_{i, t}$ to $v_{j, t'}$ if the position of external agent $j$ at timestep $t'$ depends on the position of external agent $i$ at timestep $t$. The causal graph thus represents which external agents a given external agent's future trajectory depends on. We identify each connected component of this graph, restricted to the input and output timesteps in question, with an {\em external agent behavior}. For example, the object interaction agent consists of its own behavior, whereas the chaser and runner agents together make a behavior. As noted in Section~\ref{sec:environment} these connected components do not vary across time in our environment. Our causal world model allocates a separate neural network for each external agent behavior, i.e each network has access to only the causally-appropriate inputs, thereby reducing causal confusion across agent behaviors. We assume access to the appropriate causal graph for each instantiation of behaviors. See Section~\ref{sec:methods} for details.





%TODOS: (1). Augment reason 1, reason 2 (2). Figure out where to put in periodic example (3). Rewrite the solution paragraph (4). Revise the figure 


% corrollary explaining that causal confusion makes the supervised world model prediction $P(\rvx)_{c(I_{\X})}$ non-robust to drastic changes in $p(\rvx_{I_{\X}} | \rvx_{\setminus I_{\X}})$. It's true that there are two additional sources of degradation in performance. (1). Causal confusion across time within $I_{\X}$ and unsupervised prediction. We don't argue that the agent causal confusion is "theoretically" a bigger issue, but show that getting rid of it leads to really big prediction gains. Supervised world model prediction here, since if you're doing unsupervised prediction, then even $p(\rvx_{I_{\X}})$. I think we should limit the scope to supervised prediction? 

%% Our solution is to eliminate causal confusion among the agent-dimensions. But note that there can still be other sources of causal confusion present after this removal. Namely confusion across time and confusion during unsupervised prediction. However, this still alleviates the problem to a large degree as we observed empirically 


%% TODOS: we should really show object permanence through experiments. That we can make good predicitons of agent behaviors when not looking at them.



%% Why is causal confusion likely to occur 
%% (1). Lack of data that fully covers the space 
%% 

%% Why is validation distribution likely different from training 
%% => we want to test for generalization. Which means the world model should be robust to changes in interaction policy, 
%% => In some sense we're asking the world model to succeed at out of distribution generalization. 
%% 

%% (1). Policy is different 
%% (2). World model performance is different and only little training data was acquired with the most recent world model  



% \begin{wrapfigure}{R}{0.35\textwidth}
% \vskip -0.2in
% \begin{center}
%     \includegraphics[width=.33\textwidth]{figures/causal_graph.pdf}
% \end{center}
% \vspace{-0.7cm}
% \caption{\textbf{A causal graph.} Vertices represent external agents at times $t$ and $t+1$, edges represent causal relationships. Dashed boxes denote the connected component {\em external agent behaviors}.}
% \label{fig:causal_graph}
% \vskip -0.1in
% \end{wrapfigure}


==> sections/discussion_scrap.tex <==
\section{Future Directions}

%\jdf {Summarize results here}
%\jdf {Critically analyze the fact that we had to use a split model architecture, and what we think a more sophisticated system would look like (stuff Dan said about starting with shared parameters).}

Here we describe three next directions for this work. We first describe ongoing human subject experiments that mirror the computational ones described above. We then describe what preliminary results suggest are key ``theory of mind'' properties of world models that perform well in environments such as ours. Last, we interpret the above experiment as a toy model of early childhood development and provide an analysis of how behavior early in ``life'' predicts downstream social acuity.


Limitations:
other sorts of environments (while we designed environments to present a diverse array of stimuli while being able to maintain an understanding of what sorts of stimuli are being chosen without a wide array of confounds)
more complex embodiments
active learning: what is the validation set?
(based on our heuristic understanding of qhat is interesting, understanding broadly how to make this choice in these embodied active learning contetxts)


\noindent\textbf{Human experiments}

A standard hypothesis is that the human brain has a built-in module that specifically detects animacy from visual input \citep{leslie1989autism, leslie1994tomm}. Yet the current modeling results suggest that animate attention in humans might naturally arise from a more general process of curiosity-driven learning. In ongoing work, we are testing this possibility by running human subject experiments to measure important features of animate attention, then comparing our intrinsically-motivated models to this human behavior. 

These experiments include not only random and animate stimuli, but also other behaviors that span the spectrum of predictability, including \textit{static} objects, and \textit{periodic} ones, inspired by the repetitive dynamics seen in objects like seesaws, fans, and flashing lights. We convey these kinematics to humans via self-propelled, spherical robots moving along a mat, while measuring patterns of attention via a mobile eye tracker. So far, we find average fixation proportions favoring the animate stimuli. Furthermore, a progress network tasked to predict the virtual robot trajectories produces a similar aggregate attentional fixation pattern  \ref{fig:fig2_humans_v2.png}. Crucially, the network achieves this without the requirement for any specific built-in modules favoring animacy. Instead, the pattern arises from the agent’s discovery of the inherent relative “interestingness” of animacy as compared to random, periodic, and static motion. 


\begin{figure}[h]
    \centering
    \includegraphics[width=0.7\textwidth]{figures/fig2_humans_v3-01.png}
    \caption{Ongoing work compares our intrinsically-motivated agents to human observers watching analogous displays in the real-world. Human adults wear a mobile eye tracker while watching displays consisting of four sets of self-propelled, spherical robots travelling along a mat. Using kinematics alone, the robots are made to appear animate, random, periodic, or static. Spontaneous human fixations proportions are similar to the patterns of attention exhibited by our neural agent placed in a similar environment.}
    \jdf{Kun Ho: Can we get a version of the model plot with a more comparable hierarchy?}
    \label{fig:my_label}
\end{figure}

\kh{Error bars in the figure, more seeds with randomized location}

\noindent\textbf{Theory of Mind and social mental states}

In order for a curious agent to learn effectively in a social environment, all components of the system (e.g. world model architecture, intrinsic motivation, and controller architecture) must be suited to the task, and world model architecture choice of Section~\ref{sec:methods:worldmodel} reflect choices made to reach acceptable performance given sufficient data --- see Appendix~\ref{sec:app:causal} \ref{sec:offline} for details. In particular, a {\em Theory of Mind v0} motif, which allocates separate models for separate external agent behaviors, and more generally,  causally linked subsets of the environment, may be a crucial such choice. In future work, we will look to both (1) build a system that can infer this causal prior from data and (2) stress-test its utility in a suitable range of environments.

The choice of term {\em Theory of Mind v0} is deliberate because `theory of mind' is also  used to refer to the more sophisticated ability to predict the behaviors of other agents as a function of inferred mental states, such as beliefs, desires, and goals \citep{astington1990developing, premack1978does, wellman1992child}. Determining whether our models represent such mental states will require more deliberate tests inspired from developmental psychology, perhaps in tandem with specially-tailored learning environments and model architectures. For instance, one possibility is that curiosity models will need to solve an inverse reinforcement learning problem, in which they are specifically tasked with inferring an agent's world model and reward function, given its observed actions \citep{jara2019theory}. Relatedly, human agents do not only represent first-order knowledge about what others believe, but can also represent multiply embedded beliefs (e.g., he knows that I know he knows), as well as common knowledge (we all know that we all know), mental states which are a key to understanding more sophisticated social behaviors, such as coordinating on a goal, or turn taking \cite{de2019common, de2019maimonides, thomas2016recursive}. 

Alternatively, theory of mind-like representations might emerge without the need for such deliberate, social tasks. After all, the scope of things that are interesting and worth attending to is not limited to animate agents, so either way a more general purpose learning algorithm may be needed to detect patterns in the surrounding world. At any rate, learning to predict the full complexity of inanimate and animate stimuli using biologically plausible, unsupervised systems that can operate flexibly in the real-world presents a grand challenge for both AI and cognitive science.

\noindent\textbf{In silico models of human development}

An overarching goal of this research program is to develop in silico models of early childhood development. This is a task-driven modeling approach in which we design an artificial system to accomplish a challenging cognitive task that we as humans do well. If the task is sufficiently difficult that the solution space is small, we expect to see reflections of the artificial solution in behavior and biology. This approach has yielded dramatic success as a neural model of our ventral visual stream \cite{yamins_ventralneural}, using the task of visual object recognition. We posit that attention and interaction early in childhood, with the goal of learning to model one's surroundings, is a similarly difficult task, and by solving it, we can both better understand early childhood development as well as test interventions in simulation before resorting to human subject experiments.

Consider the following interpretation of the experiments of Section~\ref{sec:experiments} as a toy model of attention, interaction, and learning early in childhood. We model the development of a "population" of agents that have differently-implemented curiosity: differing intrinsic motivations represent underlying neural/genotype/phenotype correlates of early learning differences. Attention patterns represent abundant/cheaply obtained behavioral measures related to the sorts of exploratory strategies the agents have early in life (e.g. visual attention to animate stimuli), whereas validation performance represents a more difficult to obtain measure of acuity. An easily obtained behavioral measure that predicts outcomes later in life may provide both a valuable diagnostic criterion and a cue for possible interventions.

Using this model of early development, we ask: to what extent does the emergent attention pattern of the agent predict validation performance? We seek to understand whether attention {\em early} in a run predicts {\em final} validation performance, and in particular whether, sufficiently early in a run, attention is a better predictor than early validation performance of final validation performance. Intuitively, we expect attention patterns that lead to good validation performance to precede good validation performance itself.

We look to predict final performance $P_{\mathrm{final}}$ of a given agent, which we take to be the average of the final four validation runs. To make the modeling problem simple, we discretize this into a classification task by dividing validation performance into 3 equal-sized classes (``high'', ``medium'', and ``low'', computed separately for each external agent behavior), intuitively chosen to reflect performance around, at, and below that of random policy.

We consider two predictive models of final performance, one that takes as input early attention of the agent, and the other, early performance. Early performance may be quantified simply: given time $T$ (``diagnostic age'') during training, let $P_{\leq T}$ be the vector containing all validation losses measured up to time $T$. Early attention, however, is very high-dimensional, so we must make a dimensionality-reducing choice in order to tractably model with our modest sample size. Hence, we ``bucket'' average. Given choice of integer $B$, let
\begin{equation}
    A_{\leq T, B} = (\mathit{f}^{\mathrm{anim}}_{0 : \frac{T}{B}}, \mathit{f}^{\mathrm{rand}}_{ 0 :  \frac{T}{B}}, \mathit{f}^{\mathrm{anim}}_{\frac{T}{B}: \frac{2T}{B}}, \mathit{f}^{\mathrm{rand}}_{\frac{T}{B} : \frac{2T}{B}}, \ldots \mathit{f}^{\mathrm{anim}}_{\frac{(B - 1)T}{B} : T}, \mathit{f}^{\mathrm{rand}}_{\frac{(B - 1)T}{B} : T}),
\end{equation}
where $\mathit{f}^{\mathrm{anim}}_{a : b}$ and $\mathit{f}^{\mathrm{rand}}_{a : b}$ are the fraction of the time $t = a$ and $t = b$ spent looking at the animate external agent and random external agents respectively (so $A_{\leq T, B}$ is the attentional trajectory up to time $T$ discretized into $B$ buckets).

Finally, both models must have knowledge of the external agent behavior to which the agent is exposed --- we expect this to both have an effect on attention as well as the meaning of early performance and expected final performance as a result. Let $\chi_{\mathrm{BHR}}$ be the one-hot encoding of which external animate agent behavior is shown. 

We then consider models
\begin{enumerate}
    \item PERF$_{\leq T}$, which takes as input $P_{\leq T}$ and $\chi_{\mathrm{BHR}}$, and
    \item ATT$_{\leq T}$, which takes as input $A_{\leq T, B}$ and $\chi_{\mathrm{BHR}}$.
\end{enumerate}

\begin{figure}[h]
    \centering
    \includegraphics[width=\textwidth]{figures/early_indicator_analysis_with_attn.pdf}
    \caption{\textbf{Early diagnosis analysis}. Accuracy of PERF$_{\leq T}$ and ATT$_{\leq T}$ predictors of final performance, as a function of $T$. Up until late, attentional patterns make for the more informative predictor of final performance. Below, sample real-time attention trajectories that result in high, medial, and low final performance, from left to right. Intuitively, early attention trajectory predicts attention througout the run, which in turn predicts performance.}
    \label{fig:earlypredictor}
\end{figure}


Figure~\ref{fig:earlypredictor} shows the plot of PERF$_{\leq T}$ and ATT$_{\leq T}$ accuracy as $T$ varies. We see that, up to a point, ATT$_{\leq T}$ makes a better predictor of final performance, and then PERF$_{\leq T}$ dominates. This confirms the intuition that attention patterns precede performance improvements. Intuitively, attention predicts performance by being able to predict the sort of intrinsic motivation the agent is using, which in turn predicts performance. The attention trajectories Figure~\ref{fig:earlypredictor} correspond to agents that achieve different levels of final performance, and each display different attention early that characterizes the overall strategy. For example, the high final performance corresponds to a ``bump'' in attention towards the animate agent.







\begin{comment}
NH: prior to my big edits!

\jdf {Summarize results here}
\jdf {Critically analyze the fact that we had to use a split model architecture, and what we think a more sophisticated system would look like (stuff Dan said about starting with shared parameters).}

\noindent\textbf{Ongoing work: Human experiments}

As noted, a standard hypothesis is that the human brain has a built-in module that specifically detects animacy from visual input \citep{leslie1989autism, leslie1994tomm}. Yet the current modeling results suggest that animate attention in humans might naturally arise from a more general process of curiosity-driven learning. In ongoing work, we are testing this possibility by running human subject experiments to measure important features of animate attention, then comparing our intrinsically-motivated models to this human behavior. 

These experiments include not only random and animate stimuli, but also other behaviors that span the spectrum of predictability, including \textit{static} objects, and \textit{periodic} ones, inspired by the repetitive dynamics seen in objects like seesaws, fans, and flashing lights. We convey these kinematics to humans via self-propelled, spherical robots moving along a mat, while measuring patterns of attention via a mobile eye tracker. So far, we find average fixation proportions favoring the animate stimuli. Furthermore, a progress network tasked to predict the virtual robot trajectories produces a similar aggregate attentional fixation pattern  \ref{fig:fig2_humans_v2.png}. Crucially, the network achieves this without the requirement for any specific built-in modules favoring animacy. Instead, the pattern arises from the agent’s discovery of the inherent relative “interestingness” of animacy as compared to random, periodic, and static motion. 


\begin{figure}[h]
    \centering
    \includegraphics[width=0.7\textwidth]{figures/fig2_humans_v3-01.png}
    \caption{Ongoing work compares our intrinsically-motivated agents to human observers watching analogous displays in the real-world. Human adults wear a mobile eye tracker while watching displays consisting of four sets of self-propelled, spherical robots travelling along a mat. Using kinematics alone, the robots are made to appear animate, random, periodic, or static. Spontaneous human fixations proportions are similar to the patterns of attention exhibited by our neural agent placed in a similar environment.}
    \jdf{Kun Ho: Can we get a version of the model plot with a more comparable hierarchy?}
    \label{fig:my_label}
\end{figure}

\kh{Error bars in the figure, more seeds with randomized location}

\noindent\textbf{Future Work: Theory of Mind V1, and Other Mental States}


As noted, even human infants preferentially attend to the primitive kinds of animate behaviors included in the current experiments, and we have referred to the model innovations needed to replicate these behaviors as theory of mind v0. This naming convention is deliberate because `theory of mind' is also  used to refer to the more sophisticated ability to predict the behaviors of other agents as a function of inferred mental states, such as beliefs, desires, and goals \citep{astington1990developing, premack1978does, wellman1992child}. Determining whether our models represent such mental states will require more deliberate tests inspired from developmental psychology, perhaps in tandem with specially-tailored learning environments and model architectures. For instance, one possibility is that curiosity models will need to solve an inverse reinforcement learning problem, in which they are specifically tasked with inferring an agent's world model and reward function, given its observed actions \citep{jara2019theory}. Relatedly, human agents do not only represent first-order knowledge about what others believe, but can also represent multiply embedded beliefs (e.g., he knows that I know he knows), as well as common knowledge (we all know that we all know), mental states which are a key to understanding more sophisticated social behaviors, such as coordinating on a goal, or turn taking \cite{de2019common, de2019maimonides, thomas2016recursive}. 

Alternatively, theory of mind-like representations might emerge without the need for such deliberate, social tasks. After all, the scope of things that are interesting and worth attending to is not limited to animate agents, so either way a more general purpose learning algorithm may be needed to detect patterns in the surrounding world. At any rate, learning to predict the full complexity of inanimate and animate stimuli using biologically plausible, unsupervised systems that can operate flexibly in the real-world presents a grand challenge for both AI and cognitive science.





\end{comment}


==> sections/discussion_scrap_2.tex <==
\section{Discussion and future directions}

In this work, we propose an implementation of curiosity that enables an agent to train efficiently a world model in environments containing other agents. Such environments
often contain static stimuli (easy to model), dynamic but largely deterministic stimuli (still relatively easy to model), noisy stimuli (to a large degree inherently unpredictable), as well as animate stimuli (interesting, complex, and to a considerable degree learnable). In order for the curious agent to be able to attend to the interesting without succumbing to the ``white noise problem,'' it mus be able to distinguish between these different sorts of stimuli. To accomplish this, we  propose $\gamma$-Progress, a computationally-scalable variant of progress-driven curiosity. To test this, we design a custom 3D virtual environment a variety of distillations of these classes of stimuli. We find that $\gamma$-Progress outperforms a variety of baselines in sample complexity. These agents learn better, faster, and they do so by learning to attend to what is interesting. The robustness and scalability of this method in relation to baselines makes it a prime candidate for both (1) embodied curiosity with other agents in increasingly ethologically-reasonable settings and (2) broader active learning and curiosity in a wide range of environments and tasks.

\nh{Rehash theory discussion? Let's settle on how we describe in intro first.}

Key next steps include testing these broad utilities. One limitation of the present work is in our restriction to the custom environment built to support our evaluation. We designed the environment to present a diverse array of stimuli while being able to maintain a level of control in understanding agent behavior, but this introduces its own biases. Further, in order to focus on intrinsic motivation implementation, we limited the embodiment of the agent. Lifting this restriction is an important step towards building embodied curiosity.

We see two important related activities. The first concerns the agent's world model: what makes a good world model for environments with other agents? Initial results suggest an important architectural motif, and it remains to validate this and more broadly develop computational ``theory of mind''. The second concerns how humans navigage a social world: does an implementation such as this reflect human decision making? And can we model child development with models such as these? In what follows, we describe progress towards these as well as important next steps.


\subsection{World models of other agents and theory of mind}

The world model architecture of Section~\ref{sec:methods:worldmodel} reflects choices made to guarantee acceptable prediction performance when trained on suitable data. In particular, a {\em Theory of Mind v0} motif, which allocates separate models for separate external agent behaviors, may be crucial. To test this, we construct an offline ``ideal dataset'' compare performance of this {\em causal} world model against two ablations: a {\em joined} acausal ablation that takes all observations and predicts all agents jointly, and a {\em split} acausal ablation that handles each external agent (as opposed to behavior) separately. For details on the training procedure and ablation implementations, see Appendix~\ref{sec:offline}. As seen in Figure~\ref{fig:offline_asymptotic_performance}, across all experiments, the causal world model significantly outperforms the ablations.

\begin{wrapfigure}{R}{0.4\textwidth}
\vspace{-10pt}
\begin{center}
    \includegraphics[width=.4    \textwidth]{figures/offline_asymptotic_performance_v6.pdf}
\end{center}
\vspace{-10pt}
    \caption{\textbf{Asymptotic Model Performance} The causal world model and the non-causal ablation were trained on data gathered under a reduced action space random policy, aimed at producing "ideal data" for learning each animate external agent behavior excluding peekaboo (See Section~\ref{sec:offline} for details.) \ms{Make taller}}
    \label{fig:offline_asymptotic_performance}
\vspace{-10pt}
\end{wrapfigure}

The reason for this performance difference may be understood in terms of {\em disentanglement}, in which the model finds spurious dependence ``nuisance factors'' --- some external agents are irrelevant to the behavior of others. It may be the case that poor disentanglement is more likely to occur and be detrimental to generalization performance when learning world models of partially observable environments via interactive learning. For a formalization of disentanglement and further discussion regarding the challenge in our setting, see Appendix~\ref{sec:app:causal}.

The choice of term {\em Theory of Mind v0} is deliberate because `theory of mind' is also  used to refer to the more sophisticated ability to predict the behaviors of other agents as a function of inferred mental states, such as beliefs, desires, and goals \citep{astington1990developing, premack1978does, wellman1992child}. The above motif represents a proto-version of this in which an agent, upon detecting agents or other stimuli in its environment, infers a causal structure of the environment and allocates modules of its world model that respects this causal structure. In future work, we will look to both (1) build a system that can infer this causal prior from data and (2) stress-test its utility in a suitable range of environments --- in particular, those with changing causal structure and greater interplay between causal structure and partial observability.

\subsection{Modeling human behavior}

An overarching goal of this research program is to develop models of human behavior. As a first step towards this, we would like to quantify how humans explore a similar environment and compare their behavior to that of models. In ongoing work, we are running human subject experiments in which we convey static, periodic, animate, and noise stimuli to humans via self-propelled, spherical robots moving along a mat, while measuring patterns of attention via a mobile eye tracker. The use of these spherical robots mirrors the virtual environment in order to reduce visual confounds and so as to present relatively novel stimuli to human adults. So far, we find average fixation proportions favoring the animate stimuli. Furthermore, a $\gamma$-Progress network tasked to predict the virtual robot trajectories produces a similar aggregate attentional fixation pattern. See Figure~\ref{fig:human_subject_experiment} for details.

\begin{wrapfigure}{L}{0.6\textwidth}
\vspace{-10pt}
\begin{center}
    \includegraphics[width=0.55\textwidth]{figures/fig2_humans_v3-01.png}
\end{center}
\vspace{-10pt}
    \caption{Ongoing work compares our intrinsically-motivated agents to human observers watching analogous displays in the real-world. Human adults wear a mobile eye tracker while watching displays consisting of four sets of self-propelled, spherical robots travelling along a mat. Using kinematics alone, the robots are made to appear animate, random, periodic, or static. Spontaneous human fixations proportions are similar to the patterns of attention exhibited by our neural agent placed in a similar environment.}
    \jdf{Kun Ho: Can we get a version of the model plot with a more comparable hierarchy?} \kh{Error bars in the figure, more seeds with randomized location}
    \label{fig:human_subject_experiment}
\vspace{-10pt}
\end{wrapfigure}

A standard hypothesis of human cognition is that the brain has a built-in module that specifically detects animacy from visual input \citep{leslie1989autism, leslie1994tomm}. The current modeling results suggest that animate attention in humans might naturally arise from a more general process of curiosity-driven learning.

If we can model adult human behavior, can we go further and model early childhood development? Can we model human developmental variability? One possibility is that, if such models can represent development of the general population, then implementation variations (e.g. in intrinsic motivation signal) can represent variability in development. Consider the following interpretation of the experiments of Section~\ref{sec:experiments} as a toy model of attention, interaction, and learning early in childhood. We model the development of a "population" of agents that have differently-implemented curiosity: differing intrinsic motivations represent underlying neural/genotype/phenotype correlates of early learning differences. Attention patterns represent abundant/cheaply obtained behavioral measures related to the sorts of exploratory strategies the agents have early in life (e.g. visual attention to animate stimuli), whereas validation performance represents a more difficult to obtain measure of acuity. An easily obtained behavioral measure that predicts outcomes later in life may provide both a valuable diagnostic criterion and a cue for possible interventions.

\begin{wrapfigure}{R}{0.6\textwidth}
\vspace{-10pt}
\begin{center}
    \includegraphics[width=.6 \textwidth]{figures/early_indicator_analysis_with_factor_analysis.pdf}
\end{center}
\vspace{-10pt}
    \caption{\textbf{Early diagnosis analysis}. (a) Accuracy of PERF$_{\leq T}$ and ATT$_{\leq T}$ predictors of final performance, as a function of $T$. Up until late, attentional patterns make for the more informative predictor of final performance. (b) Factor analysis hypothesis: intrinsic motivation (IM) determines attention, which determines final performance.}
    \label{fig:earlypredictor}
\vspace{-10pt}
\end{wrapfigure}

Using this model of early development, we seek to understand whether attention {\em early} in a run predicts {\em final} validation performance, and in particular whether, sufficiently early in a run, attention is a better predictor than early validation performance of final validation performance. To test this hypothesis, we train models that predict final performance from early attention (ATT$_{\leq T}$) or early performance (PERF$_{\leq T}$) (see Appendix~\ref{sec:app:attention_diagnostic} for details). As seen in Figure~\ref{fig:earlypredictor}, ATT$_{\leq T}$ dominates until late. Intuitively, as captured in the factor analysis diagram of Figure~\ref{fig:earlypredictor}, we expect performance to be determined by attention throughout the run; however, attention is driven by choice of intrinsic motivation, and if the intrinsic motivation implementation can be inferred early, this can be used to predict later attention and hence performance.








==> sections/introduction_scrap.tex <==
\section{Introduction} 
\label{sec:introduction}

Imagine yourself as a child at a busy playground. You are surrounded by a cornucopia of potentially interesting stimuli, from the leaves rustling along the ground, to the kickball lying abandoned in the sandbox, to the group of other children playing hide and seek in the far yard.
What would you like to do with your play time?   
After staring at the leaves briefly, you grow bored of watching their random motions. You then consider the kickball a bit more seriously --- dribbling and maneuvering it around by yourself could be pretty fun.  But you keep looking back to the hide-and-seekers, drawn by their dynamic moves and complex interplay.  You'll probably go join these other children, at least if you can succeed in convincing them to let you in on their game. 
Amongst this blooming and buzzing confusion, you have strong intuitions about which activities are the most exciting, about how to allocate your limited attention and time. 
This simple scenario exemplifies how humans continually engage in intrinsically-motivated exploration and interaction, a process whose strong naturally-emergent rules are especially salient for balancing attention between inanimate and animate objects~\citep{premack1990infant, gergely1995taking, frankenhuis2013infants}.
But how does this attentional control process occur?  And equally important, why does it occur --- what functional goals does it subserve? 

A fundamental underlying clue is that in the playground scenario, you are  continually learning \emph{world models} --- self-supervised predictions of what the dynamics of the world will bring, both due to its intrinsic dynamics and in response to your actions. 
Through learning world models, humans may acquire compact abstractions of high bandwidth sensory inputs, the ability to plan across long temporal horizons, and an understanding of the behavioral patterns of other agents. 
It is a natural hypothesis that attentional control is a core active learning mechanism enabling the agent to construct better and more robust world models. 
Conversely, better world models enable more effective attentional allocation.  The hide-and-seek game may perhaps be the most engaging option on the playground precisely because it presents the most sophisticated world-model prediction problems -- not unpredictable like the motions of the leaves in the wind, but involving complex inter-agent contingencies that are not as readily found in solo object-centric play. 

Discovering and formally describing the principles underlying such rich interactive scenarios is a key question in computational cognitive psychology. By the same token, devising algorithms that can learn effective world models in unfamiliar circumstances and use them to generate \emph{de novo} natural interactive behaviors is an important challenge for the next generation of socially-integrated AI and robotic systems.
In this work, we contribute to studying these questions by building neural network models of an agent embedded in a custom-built 3D virtual world environment, rich with external agents displaying a wide spectrum of realistic animate behaviors such as peekaboo, chasing, and mimicry. We show that, with proper choice of intrinsic motivation, an attention policy that distinguishes between animate and inanimate behavior emerges organically, without having to be hard-coded. In turn, by spending time on useful scenarios in a balanced fashion, this naturally ``socially-aware'' agent ends up learning world models more effectively and efficiently than alternatives. 

% meg said: we never really talk about the propensity for animate attention in humans (only mentioning the need to balance attention between inanimate and animate objects) and how that leads to more efficient world modeling - I guess it is implicitly conveyed in the sentence about how hide-and-seek game is the most engaging option, but it's just not as explicit as it should be, I think. - or the explicit explanation comes too late in the intro 

%meg said: I understand that this particular order of the last two sentences mirrors the order of the first two paragraphs. I wonder though whether it makes sense to reverse the order here to emphasize that the primary objective is world models and from it arises attention. Here, we don't have the issue of world models being hard to relate to as a real-world scenario so this order could work.
%dan replies: yes, but what I've described here is the actual "causal" pathway.  plus we want the paragraph to end on the most important thing (rather than have it be an intermediate sentence)
% meg replies: makes sense. 

In building an agent with these capabilities, we found it necessary to address the well-known ``white noise problem'', a potential failure mode of intrinsic motivation that has been acknowledged in many prior works~\citep{schmidhuber_formaltheoryoffun, pathak2017inverse, burda2018exploration, pathak2019disagreement}. An active learner must arbitrate between the combinatorially large number of stimuli exhibiting dynamic behaviors with various levels of learnability. The simplest objects in an environment are static, and easy to learn.  Inanimate objects with some reliable dynamics, e.g., a machine exhibiting periodic rotation, make the situation more complex, pressing on the intrinsic motivation to better distinguish interesting from uninteresting dynamics.  The problem is especially acute, however, for dynamics that are inherently unlearnable or chaotic e.g., falling leaves, wavering trees, and splashing water.  Distinguishing these from those that have interesting and complex yet learnable dynamics, e.g. children playing hide-and-seek turns out to be an especially difficult version of the white noise problem, one which is not effectively handled by recent curiosity approaches.  To solve it, we develop a novel variant of progress-driven curiosity, which we term ``$\gamma$-Progress'', that is able to robustly estimate learning progress in a computationally scalable fashion. 

%dan said: this paragraph, especially the end, needs for that will have to wait til we actually finish getting the results. 
%julian said: Can related works be section 1? It seems awkard to say that we begin in section 2}
%dan replies: it's "typical practice" in the AI literature to numner the sections this way.  but let's worry about this when we actually finalize this paragraph later
We begin in Section~\ref{sec:relatedworks}  by drawing connections between our work and related works in cognitive science and artificial intelligence. In Section~\ref{sec:environment}, we describe our virtual environment in detail, including the range of inanimate and animate agents that we embed in it. Section~\ref{sec:theory} mathematically formalizes the active learning problem that our curious agent is tasked with and  motivates progress curiosity in the context of previously proposed curiosity signals. Section~\ref{sec:methods} details the implementations for all components of our curious active learning agent. Finally, Section~\ref{sec:experiments} presents experimental evaluations showing that our progress-driven controller achieves significantly lower online sample complexity than baseline controllers equipped with state-of-the-art exploration strategies — including Random Network Distillation (RND) (Burda et al., 2018b) and Model Disagreement (Pathak et al., 2019).



\begin{comment}
Old version
Imagine yourself as a child at a busy playground. You are surrounded by a cornucopia of potentially interesting stimuli, from the leaves rustling along the ground, to the kickball lying abandoned in the sandbox, to the group of other children playing hide and seek in the far yard.
What would you like to do with your play time?   
After staring at the leaves briefly, you grow bored of watching their random motions. You then consider the kickball a bit more seriously --- dribbling and maneuvering it around by yourself could be pretty fun.  But you keep looking back to the hide-and-seekers, drawn by their dynamic moves and complex interplay.  You'll probably go join these other children, at least if you can succeed in convincing them to let you in on their game. 
Amongst this blooming and buzzing confusion, you have strong intuitions about which activities are the most exciting, about how to allocate your limited attention and time. 
This simple scenario exemplifies how humans continually engage in intrinsically-motivated exploration and interaction, a process whose strong naturally-emergent rules are especially salient for balancing attention between inanimate and animate objects~\citep{premack1990infant, gergely1995taking, frankenhuis2013infants}.
But how does this attentional control process occur?  And equally important, why does it occur --- what functional goals does it subserve? 

A fundamental underlying clue is that in the playground scenario, you are  continually learning \emph{world models} --- self-supervised predictions of what the dynamics of the world will bring, both due to its intrinsic dynamics and in response to your actions. 
Through learning world models, humans may acquire compact abstractions of high bandwidth sensory inputs, the ability to plan across long temporal horizons, and an understanding of the behavioral patterns of other agents. 
It is a natural hypothesis that attentional control is a core active learning mechanism enabling the agent to construct better and more robust world models. 
Conversely, better world models enable more effective attentional allocation.  The hide-and-seek game may perhaps be the most engaging option on the playground precisely because it presents the most sophisticated world-model prediction problems -- not unpredictable like the motions of the leaves in the wind, but involving complex inter-agent contingencies that are not as readily found in solo object-centric play. 

Discovering and formally describing the principles underlying such rich interactive scenarios is a key question in computational cognitive psychology. By the same token, devising algorithms that can learn effective world models in unfamiliar circumstances and use them to generate \emph{de novo} natural interactive behaviors is an important challenge for the next generation of socially-integrated AI and robotic systems.
In this work, we contribute to studying these questions by building neural network models of an agent embedded in a custom-built 3D virtual world environment, rich with external agents displaying a wide spectrum of realistic animate behaviors such as peekaboo, chasing, and mimicry. We show that, with proper choices of architecture and intrinsic motivation, an attention policy that distinguishes between animate and inanimate behavior emerges organically, without having to be hard-coded. In turn, by spending time on useful scenarios in a balanced fashion, this naturally ``socially-aware'' agent ends up learning world models more effectively and efficiently than alternatives. 

% meg said: we never really talk about the propensity for animate attention in humans (only mentioning the need to balance attention between inanimate and animate objects) and how that leads to more efficient world modeling - I guess it is implicitly conveyed in the sentence about how hide-and-seek game is the most engaging option, but it's just not as explicit as it should be, I think. - or the explicit explanation comes too late in the intro 

%meg said: I understand that this particular order of the last two sentences mirrors the order of the first two paragraphs. I wonder though whether it makes sense to reverse the order here to emphasize that the primary objective is world models and from it arises attention. Here, we don't have the issue of world models being hard to relate to as a real-world scenario so this order could work.
%dan replies: yes, but what I've described here is the actual "causal" pathway.  plus we want the paragraph to end on the most important thing (rather than have it be an intermediate sentence)
% meg replies: makes sense. 

In building an agent with these capabilities, we found it necessary to address two key algorithmic challenges. The first challenge is the well-known ``white noise problem'', a potential failure mode of intrinsic motivation that has been acknowledged in many prior works~\citep{schmidhuber_formaltheoryoffun, pathak2017inverse, burda2018exploration, pathak2019disagreement}. An active learner must arbitrate between the combinatorially large number of stimuli exhibiting dynamic behaviors with various levels of learnability. The simplest objects in an environment are static, and easy to learn.  Inanimate objects with some reliable dynamics, e.g., a machine exhibiting periodic rotation, make the situation more complex, pressing on the intrinsic motivation to better distinguish interesting from uninteresting dynamics.  The problem is especially acute, however, for dynamics that are inherently unlearnable or chaotic e.g., falling leaves, wavering trees, and splashing water.  Distinguishing these from those that have interesting and complex yet learnable dynamics, e.g. children playing hide-and-seek turns out to be an especially difficult version of the white noise problem, one which is not effectively handled by recent curiosity approaches.  To solve it, we develop a novel variant of progress-driven curiosity, which we term ``$\gamma$-progress'', that is able to robustly estimate learning progress in a computationally scalable fashion. 
%julian said: I'm wondering whether we should have a name for this second algorithmic challenge, so that we can refer to it later on, e.g., 'the animate detection problem'
%meg said: I think Dan meant that the first algorithmic challenge is white noise problem and second algorithm challenge is causal confusion (in the next paragraph), and animate detection problem is a consequence of white noise problem
%dan replies: @meg: exactly.  @jdf: why is this the second challenge? it's the first. and it's called the "white noise" problem.

%julian said: The following paragraph needs more work, and I think should refer to an example we raise in the introductory scenario, e.g., You initially think that one of the children is inspecting something on the tree, but then realize that she is using the tree to shield her field of view as the other children run to their chosen hiding spots. Could we make the examples here just a tad more specific, so that people really get it?  I don't think we've  explained what about partial observability contributes to causal confusion, so this may be confusing to readers
The second challenge is that in scenarios with several interacting and independent components (e.g. objects and other agents), world models predicting future dynamics are inherently susceptible to causal confusion --- e.g the mistaking spurious correlations for true causality --- a problem that has recently been recognized in the imitation-learning literature~\cite{}CITE.  
In the playground scenario for example, if two children are initially performing similar calisthenics simultaneously, a causally ill-informed observer might think that the apparent coordination between the two is a sign of an actual underlying causal relationship. %JDF: This example is a bit weird. What about something more ordinary, like you see one kid suddenly run away as another kid crosses over to them, but in fact the kid was running away from another child further a field. Therefore, you might predict that the runner always runs away from the first child, when in fact it was a coincidence. 
Later, if the observer only manages to keep only one of the children in view, they are likely to extrapolate their incorrect causal relationship to make spurious predictions about the unobserved child. %JDF: like what? I don't get it. 
More broadly, causal confusion leads to world models that exhibit poor future generalization performance, which turns out to be especially acute in scenarios like those we investigate, which exhibit only very partial observability from any given view. We endow our curious agent with a \emph{causally-aware world model} that integrates a causal prior into its network architecture to preempt causal confusion, and show that this choice is critical for achieving effective world-model learning.

%dan said: this paragraph, especially the end, needs for that will have to wait til we actually finish getting the results. 
%julian said: Can related works be section 1? It seems awkard to say that we begin in section 2}
%dan replies: it's "typical practice" in the AI literature to numner the sections this way.  but let's worry about this when we actually finalize this paragraph later
We begin in Section~\ref{sec:relatedworks}  by drawing connections between our work and related works in cognitive science and artificial intelligence. In Section~\ref{sec:environment}, we describe our virtual environment in detail, including the range of inanimate and animate agents that we embed in it. Section~\ref{sec:theory} mathematically formalizes the active learning problem that our curious agent is tasked with, motivates progress curiosity in the context of previously proposed curiosity signals, and characterizes the causal confusion problem. Section~\ref{sec:methods} details the implementations for all components of our curious active learning agent. Finally, Section~\ref{sec:experiments} presents experimental evaluations of our curious active learning system on two quantitative metrics: We show that (1) injecting a causal prior is essential to attaining high offline asymptotic model performance, and (2) our progress-driven controller achieves significantly lower online sample complexity than baseline controllers equipped with state-of-the-art exploration strategies — including Random Network Distillation (RND) (Burda et al., 2018b) and Model Disagreement (Pathak et al., 2019). Furthermore, when varying both the intrinsic motivation signal (considering several baselines) and world model architecture (with causal structure prior, and without), we find that the intrinsic motivation signal drives behavior, whereas the difference in world model architecture modulates behavior to a lesser degree.
\end{comment}



% Our evaluations show that $\gamma$-Progress achieves significantly higher AWML performance than baseline controllers equipped with state-of-the-art exploration strategies — including Random Network Distillation (RND) \citep{burda2018exploration} and Model Disagreement \citep{pathak2019disagreement}.

% \sj{I think what could make the introduction more detailed is some intuition of why the proposed exploration strategy solves the problem you mentioned i.e. find interesting things to learn on. Otherwise, the advertisement of good performance in this paragraph aren't too convincing until people have seen either details of the method, or concrete the experimental results.}
% We begin in Section~\ref{sec:relatedworks}  by drawing connections to related works in cognitive science and artificial intelligence. In Section~\ref{sec:environment}, we describe our virtual environment in detail, including the range of inanimate and animate agents that we embed in it. Section~\ref{sec:theory} provides a novel mathematical formalization of Active World Model Learning  that our curious agent is tasked with and  motivates progress curiosity in the context of previously proposed curiosity signals. Section~\ref{sec:methods} details the implementations for all components of our curious active learning agent. Finally, Section~\ref{sec:experiments} presents experimental evaluations showing that our progress-driven controller achieves significantly higher AWML performance than baseline controllers equipped with state-of-the-art exploration strategies — including Random Network Distillation (RND) \citep{burda2018exploration} and Model Disagreement \citep{pathak2019disagreement}.

% \sj{A general comment is that it probably helps to clarify the contribution into different parts. I was initially confused whether the main contribution was the $\gamma$-progress objective. But it seems that proposing the environment and the learning problem is also major. (That was only obvious to me after seeing section 3). Also I was confused in the introduction about the relationship between the learning problem you propose (AWML) and the solution (agent) you propose. Is the agent the only way to perform optimally, or is it just one way to perform well. If the learning problem (AWML) and the solution are separate contributions, then it probably helps to clearly separate them.
% For example, the intro could have two or more paragraphs, one for each contribution.}

==> sections/relatedwork_scrap.tex <==
\section{Related Works}
\label{sec:relatedworks}

\jdf{I'm starting to wonder whether it makes sense to have divided cognitive science and AI sections. It seems that the narrative at the end of the current cog sci section could just continue into the current AI sections, especially if there continues to be a string of psychological motivations. Currently the sections feel a bit disjointed. At the least we need an explicit statement that links the sections, e.g., talking about how the AI section starts to suggest how the sophisticated statistical learning we talk about at the end of the cog sci section might be implemented.}. 

We draw on cognitive science and ultimately aim to provide cognitive models. People have studied agents modeling their environments in cognitively-plausible ways. Active learning and curiosity have been studied and we add to the program of bringing the active learning of intuitive physics and psychology to artificial systems. 

\subsection{Cognitive science}
\label{sec:related:cognitive}

\noindent\textbf{Object-based attention and object permanence}

Although traditional models characterize attention as a `spotlight' that shines on areas of space, a wealth of work in cognitive science indicates that in many cases the units of attention in space \citep{scholl2001objects} and time \citep{de2014attentional} are distinct, bounded objects, aka \textbf{object-based attention}. Further, when the objects are dynamic, the human attentional system assigns individuated object tokens to each object, in order to keep track of them over time \citep{sears2000multiple}. The well-known limits on attention, then, often concern the maximum number of objects that can be tracked simultaneously, a limit that is thought to arise as multiple objects compete for representation on space-limited cortical real-estate \citep{alvarez2007many}. 

When tracking dynamic objects, the human brain must also deal with momentary disappearances of the objects it is tracking, as when they leave the field of view or become occluded. In such cases, it must solve a correspondence problem: which of the objects that it later sees is the same as the one that it was tracking a moment ago? The human brain appears to solve this problem by maintaining and updating an internal representation of the object even as it goes out of sight \citep{baillargeon1985object}, a phenomenon known as \textbf{object permanence}. This ability appears to rely on additional systems for visual imagery and working memory, which can also be guided by the oculomotor system \citep{de2016tracking, saiki2002multiple}. Working memory, similar to attentional selection, is limited in the number of objects which it can store simultaneously \citep{luck1997capacity}.

In the current work, our modeling framework includes object-based attention, object permanence, and working memory as inductive biases, i.e., knowledge that is built in as a prior of the model. We provide the model with the center coordinates of objects, and require it to predict their future center coordinates. Further, we use a memory system to maintain an active representation of an object whenever it goes out of sight.

\noindent\textbf {Animate attention, prediction, and theory of mind}

Given the limits on attention and memory, the human brain cannot track all of the objects with which it is confronted, and must therefore decide what subset of objects to either automatically or intentionally select for processing. Efficiently determining what to attend to is necessitated by the fact that not all objects are equally rich in information. Of note, in the majority of cases the most information-rich objects tend to be other animate entities, rather than many of the other kinds of entities that also occupy our fields of view, such as objects that are static (e.g., rocks, walls, and buildings), periodic (e.g., fans, wheels), or random (e.g., brownian motion in leaves, water, and the other elements). Unlike random stimuli, the dynamics of animate stimuli are learnable. And unlike static and periodic stimuli, which are either unchanging or repeatable, the spatiotemporal dynamics of animate stimuli contain more complex structures. 

Already as infants, humans are adept at distinguishing between inanimate and animate agents, preferentially paying attention to animate features like faces \citep{maurer2002many} and human body shapes \citep{slaughter2002development}, aka \textbf{animate attention}. Even in the absence of these surface features, infants will preferentially attend to spatiotemporal kinematics indicative of animate agents, such as self-propelled motion \citep{premack1990infant}, efficient movement towards targets \citep{gergely1995taking}, contingent behavior between observed agents, as when one agent chases another \citep{frankenhuis2013infants}, and contingent behavior between an observed agent and the infant herself, as when a robot beeps in response to the infant's babbling \citep{johnson2003detecting, foster1973visual}. In adults, these kinds of kinematics may give rise to an irresistable sense of animacy and intentionality, even when the objects executing the kinematics are simple shapes \citep{heider1944experimental}. In other words, the visual system has been highly tuned to cues that reliably indicate the presence of agents with internal sources of energy that cause them to move without the need for external forces. 

Beyond the ability of infants to discriminate between animate agents and other objects, a more sophisticated ability that emerges later in development is actively interpreting other agents in terms of their underlying mental states (beliefs, desires, and goals) that cause the agents' behavior, aka \textbf{theory of mind} \citep{astington1990developing, premack1978does, wellman1992child}, rather than in terms of physical forces. A theory of mind is needed in order to \textit{predict} what an agent will do next, since often it is only possible to do so accurately by generating expectations about an agent as a function of underlying intentions that are attributed to it. This ability is crucial to social functioning, and the failure to attribute mental states falls under the umbrella of symptoms that define the autism spectrum mental disorders \citep{baron2000theory}.

In the current work, our environment includes inanimate and animate agents with spatiotemporal kinematics inspired from these human experiments, and the agents are deliberately devoid of surface features, so that our modeling agent must discover which agents are interesting and  worth paying attention based on their spatiotemporal properties alone. We task our neural model with learning to discriminate among the different kinds of inanimate and animate agents, based on its ability to learn to predict what they will do next. 

\noindent\textbf {Diverging developmental theories}

Given that the above abilities arise early in human development, some have argued that infants may be born with an already specialized module devoted to representing the mental states of agents \citep{leslie1989autism, leslie1994tomm}. According to one dominant account, such a “theory of mind mechanism” could consist of a hard-wired, set of primitive propositional attitudes about concepts such as “desire” and “belief”. Note also that it is not a problem for this theory that infants are not immediately born with the ability to detect and predict agents, because an innate system could still be programmed to only come online later in life, perhaps triggered by certain environmental inputs \citep{scholl1999modularity}.

At the same time, infants exhibit an impressive ability to learn the statistical regularities in various tasks involving stimuli spanning all modalities, e.g., audition, vision, words \citep{fiser2002statistical, saffran1996statistical, maye2002infant}. As such, an alternative theory states that the bulk of attentional behavior may be driven by a more general-purpose learning mechanism, which allocates attention to stimuli based on their inherent, information-theoretic properties. Under this account, the particular attentional biases that have been characterized in existing work are an inevitable outcome of a smart learning system coming into contact with the different statistical properties of the  stimuli that happen to surround us.

Providing some support for this second view, previous work also finds that infants appear to gather information from environments in a manner that is quite principled: They selectively explore objects that violate their expectations \citep{stahl2015observing}, and they spend little time examining stimuli that are either too simple or too complex; instead, they preferentially attend to stimuli that are sufficiently complex to be interesting but not so complicated that they cannot be predicted \citep{kidd2012goldilocks}.

In the current work, while we do build in inductive biases concerning object-based attention, object-permanence, and working memory, we do not build in a propensity to detect and predict special classes of stimuli. Instead, we test whether reasonable patterns of attention of the form observed in humans can emerge naturally in our model, provided we endow it with a good, general-purpose learning objective. 

%\subsection{AI modeling of physical and social environments}

%While for this work we do not need sophisticated models capable of human-level intuitive physics, much progress has been made along these lines. Intuitive physics approaches: interaction networks, HRN, recent tenenbaum work \cite{This framing makes it sound like you're going to tell the reader about irrelevant stuff; what about framing it as people have focused on modeling the high-level stuff by assuming it exists, but not so much on modeling how you learn that stuff in the first place, using a biologically-plausible architecture.}

%Less progress has been made towards modeling human-level intuitive psychology. Multi-agent learning (relational forward models for multiagent learning), program induction (Human-level concept learning through probabilistic program induction \nh{Is there something newer}?

%In our model architecture, we have created an explicit read/write memory structure useful in predicting the trajectories of animate and inanimate stimuli over modest timescales. NTM, Merlin might embody more generic versions of this ---  one can imagine our explicit structures arising from training within the sorts of environments we consider over long time scales. In our work, we stick with short timescales. \nh{Our contribution here is not as clear, depends on whether we emphasize memory mechanism, or should keep incremental}


%\subsection{Curiosity, multi-task learning, and curriculum learning}

%In order to increase sample efficiency, it is useful for agents gathering data within their own worlds to make smart decisions about what data to capture. Basics of curiosity and intrinsic motivation. Related is classical active learning \cite{settles2011_active, giladbachrach_qbcreal_active} [lots more], in which an agent seeks to minimize the amount of labeling required in order to learn a supervised task.

%Different ways of defining intrinsic motivation, with subtlety of white noise problem
%Prediction Error: \cite{berkeley_mario, haber2018learning, interaction_cogsci}, Stadie.
%Novelty: Pseudocount, RND, Disagreement
%Progress: Schmidhuber, Oudeyer \cite{oudeyer2013intrinsically, oudeyer2007intrinsic}
%Information gain: Prediction Gain, VIME, Surprisal

%Related to curiosity are contexts in which an agent has many possible tasks or a family of tasks and must judiciously choose what to do, when. Curriculum learning, multi-task learning, and goal generation. [Automated Curriculum Learning for Neural Networks] [Control What You Can: Intrinsically Motivated Task-Planning Agent] [Automatic Goal Generation for Reinforcement Learning Agents] \cite{jaderberg2016reinforcement}.

\subsection{Artificial intelligence}

\jdf{What is the story we want to tell in this section?}
\jdf{How about something like this: 
(i) When do we understand the world around us? One idea is that we understand it when we can predict what will happen next. Briefly mention the alternatives (e.g., compression)
(ii) Talk about some psychological evidence that people do this, while gesturing at predictive coding (because we have to).
(iii)Introduce how this problem has been approached in the AI literature.
(iv) But what's missing from these approaches that we think is important?}
\jdf{Currently the content seems to jump around too much. Also, on a minor note, there's a lot of he said she said; can we just talk about the findings, while citing these people parenthetically? I think this puts the focus on the science.}.

\noindent{\textbf{World models concerned with dynamics}}

\jdf{Not sure if we want to cite some of the older biological work related to these ideas, e.g., Rosen R. (1985) Anticipatory systems: Philosophical, mathematical and methodological
foundations. Pergamon Press.}
\jdf{Originator credit? Maybe Gibson? Gibson J. J. (1979) The ecological approach to visual perception. Routledge.}

\jdf{Cites for the (newer idea of) predictive coding: 
Clark A. (2013) Whatever next? Predictive brains, situated agents, and the future of
cognitive science. Behavioral and Brain Science 36:181–204. 
Friston K. (2010) The free-energy principle: A unified brain theory? Nature Reviews
Neuroscience 11:127–38.; Rao R. P. & Ballard D. H. (1999) Predictive coding in the visual cortex: A functional interpretation of some extra-classical receptive-field effects. Nature Neuroscience 2:79–87.}

\jdf{Note that there are broadly two different kinds of predictive 'world' models that seem to battle it out in biology/psychology: (i) sometimes referred to as subjective physics, is the more Gibsonian view, which says that the models are physics models, which take the relations between observables. (ii) predictive coding, which maps internal variables to the observables (e.g., sensory inputs), and so is a 'generative model'. See Brette (2019) BBS- Is coding a relevant metaphor for the brain}.

A natural choice for what to model about one's environment is that of forward dynamics prediction: given a sequence of observations, perhaps along with the planned actions of the observer, predict some number of future observations. \jdf{Not sure why you're suddenly honing in on video frame prediction being hard here; I thought you were going to argue why predicting forward dynamics makes sense}. Video frame prediction \citep{kalchbrenner2016video, finn2016unsupervised} presents immense challenges in producing predictions that are realistic, let alone accurate, although recent innovations in architecture and loss function \citep{lee2018stochastic, wang2018predrnn++, Wu2019ModelIF} have shown considerable improvements. This self-supervised task draws inspiration from the neuroscience theory of \textbf{predictive coding}, and architectural motifs inspired by the neural theory \citep{lotter2016deep} have been shown to produce visual features that support other visual tasks. \jdf{what is an architectural motif exactly?} When conditioned on the actions of the observer, video prediction has shown utility in planning for robotic control tasks \citep{finn2017deep}. Related, \cite{ha2018world} build generative world models of virtual environments and use these ``dream'' environment simulations to train policies. \cite{chua2018deep} enhance performance in reinforcement learning tasks by incorporating calibrated forward dynamics models.

Some of the difficulty of predicting forward dynamics can be obviated by working not with images but in a given latent feature representation. For example, 3D point clouds data has been amenable to the forward dynamics prediction of rigid bodies \citep{byravan2017se3}. Approaches using object-centric, graphical representations of scenes \citep{battaglia2016interaction, chang2016compositional} have grown to be able to predict particulate representations of rigid and soft bodies \citep{mrowca2018flexible}. Coarse, probabilistic object-centric models have the ability to model human expectation violation of intuitive physics \citep{smith2019modeling}. \cite{ke2019learning} incorporate longer-term forward prediction in a latent space in order to enhance performance at reinforcement learning tasks.

Beyond forward dynamics prediction are self-supervised tasks that usefully model the dynamics of environments. Time reversal, in which a model is given an observation or observations and predicts that which preceded, can be used to plan by working backwards from goal states \citep{nair2018time}. \cite{agrawal2016learning} show inverse dynamics prediction, in which a model is given observations of an agent and must recover what actions the agent took, to be useful in robotic manipulation tasks. Networks can also be trained to predict other quantities from video frames, such as the height of an object in free fall, without being given labels of these quantities but rather by using known properties of the output space such as those derived from physics \citep{stewart2017label}.

In our work, we focus on the forward dynamics prediction problem on an object-centric representation of our environment. This representation simply consists of the positions of each object or agent in the environment, lacking other distinguishing features. We thus {\em assume} the agent has access to an encoding giving it this representation. This avoids the dual difficulties of both obtaining these representations from visual features and predicting the dynamics of complex media.

\noindent{\textbf{Active learning}}

\jdf{I still have to read this}

Independently of what is being modeled, the question of what actions to take in order to improve one's model efficiently has long been an important part of machine learning, statistics, and scientific thinking at large. Classically in \textbf{active learning} \citep{settles2011_active}, an agent seeks to learn a supervised task and tries to minimize the number of unlabeled examples it must label (the choice of what to label is the ``action'' of the agent). In doing so, the agent must make use of some signal by which it decides what action to take, with standard techniques including uncertainty sampling \citep{lewis1994heterogeneous}, query by disagreement \citep{cohn1994improving}, query by committee \citep{seung1992query}, error reduction \citep{roy2001toward}, and variance reduction \citep{geman1992neural}. Many of these techniques have been studied thoroughly within statistics, as, if we think of this ``act'' of labeling as deciding which experiment to perform when trying to fit a model or estimate a parameter, we arrive at \textbf{optimal experimental design} \citep{kahn1951estimation, fedorov2013theory, chaloner1995bayesian}.

Modern work on intrinsic motivation and curiosity can be considered a variant of active learning that concerns a reinforcement learning agent with sparse or no extrinsic reward \citep{schmidhuber_formaltheoryoffun, oudeyer2007intrinsic, oudeyer2013intrinsically}. In this, an agent trains a world model, and in taking action, it receives an intrinsic motivation ``reward'' computed using the world model. This intrinsic motivation signal is usually taken to be some estimate of how useful the action and resulting state are at producing an improved world model. In this way, the intrinsic motivation signal can be thought of as analogous to the signals by which more traditional active learning decisions are made, and indeed, many modern techniques take as inspiration the signals used in active learning and optimal experimental design. A number of approaches \citep{stadie2015predictive, interaction_cogsci, haber2018learning} use the world model's \textbf{prediction error}, though these in some contexts can result in the \textbf{white noise problem} in which agents are motivated to take actions that lead to unpredictable examples for the world model. In order to avoid the white noise problem, one can seek to estimate how actions lead to learning \textbf{progress} or \textbf{information gain}. How this is estimated is a core challenge, and many approaches towards estimating learning progress \citep{schmidhuber_formaltheoryoffun, oudeyer2007intrinsic, oudeyer2013intrinsically} or information gain \citep{houthooft_vime} present serious computational challenges when used at scale in complex environments. \textbf{Surprisal} \citep{achiam2017surprise} presents a computationally-tractable alternative to information gain. Model disagreement \cite{pathak2019disagreement}, in which intrinsic motivation is proportional to an ensemble of independently trained world models, presents another computationally-tractable alternative inspired by classical active learning techniques. For comprehensive reviews of intrinsic motivation signal choices, please see \citep{aubret2019survey, linke2019adapting}.

Related approaches rely on a fixed intrinsic motivation objective that does not take into account a specified world model problem. In the context of learning a world model problem, such intrinsic motivations can be thought of as \textbf{novelty} metrics, measuring how much a particular part of the environment has been explored. Examples include count-based exploration \cite{strehl2008analysis}, useful in tabular settings, and generalizations to continuous spaces such as pseudo-counts \citep{bellemare2016unifying} and Neural Density Models \citep{ostrovski2017count}. Certain variants of prediction error-based intrinsic motivation \citep{pathak2017inverse,pathak18largescale} seek to choose judiciously a learned feature space for a forward dynamics world model problem so that white noise issues do not arise. One recent popular approach, Random Network Distillation \citep{burda2018exploration}, takes as intrinsic motivation the prediction error of one neural network trying to match the output of a randomly initialized and frozen network of identical architecture. Related is \textbf{empowerment} \citep{mohamed2015variational}, in which the agent seeks to maximize the mutual information of action and state. \cite{jaderberg2016reinforcement} provides as intrinsic reward auxiliary tasks in order to better performance in sparse reward settings. \cite{kulkarni_hierarchical} combine intrinsic motivation with hierarchical action-value functions operating at different temporal scales, for goal-driven deep reinforcement learning.

The signals exploited in traditional active learning and curiosity have seen broad modern application outside of these classical and sparse reward contexts. \cite{graves2017automated} explore a number of learning progress estimators in order to build a curriculum in a multi-armed bandit setting. \cite{blaes2019control} use several such signals in order to solve several related tasks, some of which build on others, others of which are effectively impossible, providing a multi-task variant of the white noise problem.

It is worth noting how the intent of this work contrasts with several related themes. First, most studies of curiosity study intrinsic reward as either (1) a way to enhance performance at a reinforcement learning task with sparse but present extrinsic reward or (2) a method of encouraging good exploration, as measured by e.g. the amount of territory the agent has seen. In this work, we study curiosity {\em as active learning}, measuring success by improved performance at the world model problem. 

\nh{I took out a mention of attention mechanisms, as it doesn't fit here and is confusing. Any ideas for how to place?}
\ms{I guess our message is that ``attention'' mechansims are \textbf{not} related to this work, so perhaps we could place it somewhere other than related work where we talk about our attention measures to explicitly state that they were different lines of work?}
%Second, on a high level we look to optimize the agent's {\em visual attention} towards learnable stimuli. This, however, is imposed by the environment's strong partial observability at any given time. To contrast, {\em attention mechanisms}, visual or otherwise, seek to reduce the hypothesis space by for a task by directing model attention to limited subsets of observations. \ms{I see how the two  points in the later part of this paragraph correspond to (1) and (2), but it is a little unclear how attentional mechanisms relates to (2) seeing curiosity as a method of encouraging good exploration and especially to the mention of measuring amount of territory agent has seen}
%\nh{Agreed, I think attention comes a little out of left field here...not sure quite where to put it, as we're essentially saying "hey this thing with a name that might remind you of what we're doing is very different. doesn't quite fit the logic of this section or any other. need to think abhout this}

\noindent{\textbf{Multiagent and social learning}}

\nh{I have a note here for Kun Ho to see if there's some particularly salient robosoccer reference}

Environments with multiple artificial agents have been studied in order to optimize their interactions for a goal, understand or see what leads to their emergent behaviors, and exploit in order to train better models. Broadly, the field of multi-agent learning \citep{nguyen2018deep, zheng2018structured} concerns the coordination and communication of multiple agents within an environment in order to solve a reinforcement learning task. \cite{jaques2019social} explores the use of causal influence of one agent on another as intrinsic motivation to learn policies across agents in a decentralized manner. Of particular salience to our proposed world model architecture, \cite{tacchetti2018relational} learn a shared relational forward model, representing a network of relationships between agents, in order to boost performance at a multi-agent learning task. \cite{rabinowitz2018machine} demonstrate the use of a ``Theory of Mind'' neural network architecture that models behaviors in a gridwork environment.

Multi-agent systems can be studied not only through the lens of coordination in order to solve reinforcement learning tasks, but also through competition. \cite{baker2019emergent} study the emergence of interesting behaviors such as the use of tools in competitive multi-agent environments. \cite{vinyals2019grandmaster} use many agents pitted against each other in order to refine policies in the competitive strategy game setting of Starcraft II.

Robotics has been extended beyond multi-agent artificial environments and into social environments by developing predictive models of human behavior and using those to interact with people accordingly. A series of work on a social robot Jackrobbot \citep{ballan2016knowledge, robicquet2016learning, sadeghian2019sophie} uses human behavioral data in order to navigate real-world environments with both physical constraints and humans. \cite{kleinsurprise} learn predictive models of infant visual attention, aimed at designing robots that manipulate and encourage attention.

In the present work, we study the intrinsic motivations that lead to effective policies for, and the world model architectures that can enable, the learning of animate behaviors. Our work thus contrasts with multi-agent learning in that, in order to focus on these two computational factors, we precisely control all behaviors aside from that of our intrinsically motivated agent, and the agents do not cooperate or compete on any further objective.



====
Standard techniques include uncertainty sampling \citep{lewis1994heterogeneous}, query by disagreement \citep{cohn1994improving}, query by committee \citep{seung1992query}, error reduction \citep{roy2001toward}, and variance reduction \citep{geman1992neural}. Similar ideas have also been studied under the rubric of statistical \emph{optimal experimental design} \citep{kahn1951estimation, fedorov2013theory, chaloner1995bayesian}. 

\cite{jaderberg2016reinforcement} provides as intrinsic reward via auxiliary tasks in order to better performance in sparse reward settings. \cite{kulkarni_hierarchical} combine intrinsic motivation with hierarchical action-value functions operating at different temporal scales, for goal-driven deep reinforcement learning.
s
The signals exploited in traditional active learning and curiosity can also be applied outside of these sparse reward contexts. \cite{graves2017automated} explore a number of learning progress estimators in order to build a curriculum in a multi-armed bandit setting. \cite{blaes2019control} use several such signals in order to solve several related tasks, some of which build on others, others of which are effectively impossible, providing a multi-task variant of the white noise problem.

%It is worth noting how the intent of this work contrasts with several related themes. First, most studies of curiosity study intrinsic reward as either (1) a way to enhance performance at a reinforcement learning task with sparse but present extrinsic reward or (2) a method of encouraging good exploration, as measured by e.g. the amount of territory the agent has seen. In this work, we study curiosity {\em as active learning}, measuring success by improved performance at the world model problem. 

















% cogsci section after dan shortened it: 
\noindent\textbf{Object dynamics prediction, attention, and permanence.} 
Humans are extremely effective at understanding dynamics of objects in their environment, excelling at intuitively predicting both the physical interactions of external objects~\cite{} and the physical consequences of their own actions~\cite{}. 
However, both the visual system and the working memory system that support these abilities have substantial limitations~\cite{}. 
Humans thus selectively allocate attention in an object-centric fashion to enable effective prediction despite these limitations \citep{alvarez2007many, scholl2001objects}, and assign individuated tokens to keep track of objects over time \citep{sears2000multiple}. To deal with momentary disappearances of objects as they become occluded or leave the visual frame, the brain maintains and updates an internal persistent representation of objects, a phenomenon known as \emph{object permanence}~\cite{piaget_originsintelligence}.  Studies in human infants have shown that many of these abilities --- including understanding the dynamical continuity of physical trajectories, the solidity of objects, and their persistence even when out of sight --- appear to be present very early in development~\cite{spelke_objectpermanence, spelke2007core, baillargeon1985object}. 
In this work, we include object-based attention, object permanence, and working memory as architectural biases, i.e. knowledge that is built in as a prior of the model. To enable dynamical prediction, we provide the model with the center coordinates of objects, and require it to predict their future center coordinates. Further, we use a memory system to maintain an active representation of an object whenever it goes out of sight. 

\noindent\textbf{Curiosity and Active Learning.} Attentional control also appears to be of great importance for learning how the world works.  Infants appear to gather information from environments in a manner that is quite principled, selectively looking at objects in highly non-random manner~\cite{smith}, and devoting increased attention to objects that violate their expectations \citep{stahl2015observing}.  Infants also appear to self-generate useful learning curricula, preferentially attending to stimuli that are sufficiently complex to be interesting but not so complicated that they cannot be predicted, a phenomenon known as the \emph{goldilocks effect} \citep{kidd2012goldilocks}.  In this work, a key question that we address is the formalization of the intrinsic motivations underlying active learning in a multi-agent context. 

\noindent\textbf{Animate attention.}
From early infancy, humans are especially adept at distinguishing between inanimate and animate agents, preferentially paying attention to animate features like faces \citep{maurer2002many} and human body shapes \citep{slaughter2002development}, a phenomenon called \emph{animate attention}. Even in the absence of these surface features, infants will preferentially attend to spatiotemporal kinematics indicative of animate agents, such as self-propelled motion \citep{premack1990infant}, efficient movement towards targets \citep{gergely1995taking}, contingent behavior between observed agents, as when one agent chases another \citep{frankenhuis2013infants}, and contingent behavior between an observed agent and the infant herself, as when a robot beeps in response to the infant's babbling \citep{johnson2003detecting, foster1973visual}.  The visual system has been highly tuned to cues that reliably indicate the presence of agents with internal sources of energy and volition that cause them to move without the need for external forces. Such kinematic patterns give rise to an irresistable sense of animacy and intentionality, even when the objects executing the kinematics are simple shapes \citep{heider1944experimental}. 
In this work, our environment includes inanimate and animate agents with spatiotemporal kinematics inspired from these human experiments, and the agents are deliberately devoid of surface features, so that our modeling agent must discover which agents are interesting and worth paying attention to based on their spatiotemporal properties alone. 
While we do build in inductive biases concerning object-permanence and working memory, we do not build in a propensity to detect and predict special classes of stimuli. Instead, we test whether reasonable patterns of attention of the form observed in humans can emerge naturally in our model, provided we endow it with a good, general-purpose learning objective.

\noindent\textbf{Social prediction and theory of mind.}
Beyond animate attention, a more sophisticated ability that emerges later in development is the active interpretation of other agents in terms of their underlying mental states (beliefs, desires, and goals) that cause the agents' behavior, aka \emph{theory of mind} \citep{astington1990developing, premack1978does, wellman1992child}. It is hypothesized that theory of mind is needed in order to \textit{predict} what an agent will do next, since often it is only possible to do so accurately by generating expectations about an agent as a function of underlying intentions that are attributed to it. This ability is crucial to social functioning, and the failure to attribute mental states falls under the umbrella of symptoms that define the autism spectrum mental disorders \citep{baron2000theory}.  
In this work, we task our neural model with learning to predict what the objects and agents in the environment will do next, and seek to determine which features of animate attention and theory of mind are required to achieve improved world-model predictions.

==> sections/relatedworks.tex <==
\section{Related Works}
\label{sec:relatedworks}

Both artificial intelligence and cognitive science have developed substantial literatures around  world-modeling and attentional control.

\subsection{Artificial Intelligence}

\noindent{\textbf{World models and prediction.}}
A natural class of world-models involve forward dynamics prediction. Such models can directly predict future video frames~\citep{kalchbrenner2016video, finn2016unsupervised, lotter2016deep, lee2018stochastic, wang2018predrnn++, Wu2019ModelIF}, or latent feature representations such as 3D point clouds~\citep{byravan2017se3} or object-centric, graphical representations of scenes~\citep{battaglia2016interaction, chang2016compositional, mrowca2018flexible}. 
Action-conditioned forward-prediction models can be used directly in planning for robotic control tasks~\citep{finn2017deep}, as performance-enhancers for reinforcement learning tasks~\citep{chua2018deep,ke2019learning}, or as ``dream'' environment simulations for training policies~\citep{ha2018world}.
World-models can also be derived from prediction problems other than forward dynamics, including time reversal \citep{nair2018time} and inverse dynamics~\citep{agrawal2016learning}, which have proven useful in building world models for well-defined robotic manipulation tasks. 
World-models can also be targeted not at a full state-space prediction but instead toward specific attributes --- e.g. the height of an object in free fall --- allowing known constraints in the output space (e.g. conservation of momentum) to drive learning~\citep{stewart2017label}. 

In our work, we focus on a forward-dynamics prediction problem in an object-centric representation. This representation simply consists of the positions of each object or agent in the environment, lacking other distinguishing features. We thus {\em assume} the agent has access to an encoding giving it this representation, bypassing the important but complex question of how to extract this representation directly from visual features, so as to focus the present work on identifying good solutions for active learning and multi-agent causal modeling. 

\noindent{\textbf{Active learning.}}
Independently of which task the agent self-supervises its world-model on, a key question the agent is faced with is how to choose its actions to efficiently learn the world-model. In the classical \emph{active learning} setting~\citep{settles2011_active}, an agent seeks to learn a supervised task with costly labels, judiciously choosing which examples to obtain labels for so as to maximize learning efficiency. 
More recently, active learning has evolved in the context of self-supervised reinforcement learning agents~\citep{schmidhuber_formaltheoryoffun, oudeyer2013intrinsically, jaderberg2016reinforcement}. In this line of work, agents typically self-supervise a world-model using an intrinsically-generated ``curiosity''.  Many different approaches to this general idea exist, all of which are essentially different approaches to estimating \emph{learning progress} --- e.g. determining which actions are likely to lead to the highest world-model accuracy gain in the future. % refer readers to theory section   
One popular approach is the use of \emph{novelty} metrics, which measure how much a particular part of the environment has been explored, and direct agents into under-explored parts of state-space. 
Examples include count-based and psuedo-count-based methods~\citep{strehl2008analysis,bellemare2016unifying, ostrovski2017count}, Random Network Distillation (RND)~\citep{burda2018exploration}, and the \emph{empowerment} metric \citep{mohamed2015variational}. 
Novelty-based approaches avoid the difficult world-model-progress estimation problem entirely by not depending at all on a specific world-model state, and relying on novelty as a (potentially flawed) proxy for learning progress. 


The simplest idea that actually takes into account the world-model problem to be learned is \emph{adversarial} curiosity, which estimates current world-model error and directs agents to actions estimated to maximize this error~\citep{stadie2015predictive, pathak2017inverse, haber2018learning}. However, adversarial curiosity can result in the \emph{white noise problem}, in which agents are motivated to waste time fruitlessly trying to solve unsolvable world-modeling problems, e.g. where there is degeneracy in the cause or effect of the action. The white noise problem can to some degree be avoided by solving the world-modeling problem in a learned latent feature-space in which degeneracies are suppressed~\citep{pathak2017inverse, pathak18largescale}. 

Directly estimating learning progress ~\citep{oudeyer2007intrinsic, oudeyer2013intrinsically} or \emph{information gain}~\citep{houthooft_vime} avoids the white noise problem in a more comprehensive fashion. However, such methods have been limited in scope because they involve calculating quantities that cannot easily be estimated in high-dimensional continuous action spaces.
\emph{Surprisal}~\citep{achiam2017surprise} and model disagreement\citep{pathak2019disagreement} present computationally-tractable alternatives to information gain, at the cost of the accuracy of the estimation. For comprehensive reviews of intrinsic motivation signal choices, see \citep{aubret2019survey, linke2019adapting}.
In this work, we present a novel method for estimating learning progress that takes advantage such metrics have in ensuring the directed learning utility of action choices, while being robust and scalable to high-dimensional continuous action-space settings. 

\noindent{\textbf{Multiagent and social learning.}}
The field of multi-agent learning \citep{nguyen2018deep, zheng2018structured} concerns the coordination and communication of multiple agents within an environment to solve a reinforcement learning task. \citep{jaques2019social} explores the use of causal influence between agents as intrinsic motivation to learn policies across agents in a decentralized manner.  \citep{rabinowitz2018machine} demonstrate the use of a ``Theory of Mind'' network architecture that models behaviors in a gridworld environment.
\citep{baker2019emergent} study the emergence of interesting behaviors such as the use of tools in competitive multi-agent environments. \citep{vinyals2019grandmaster} use many agents pitted against each other to refine policies in the competitive strategy game setting of Starcraft II.
\citep{tacchetti2018relational} learns a shared relational forward model, representing a network of relationships between agents, in order to boost performance at a multi-agent learning task.
Multi-agent learning has also been extended beyond artificial environments and into real social environments by developing predictive models of specific human behaviors and using those to enable robots to better interact with people~\citep{ballan2016knowledge, robicquet2016learning, sadeghian2019sophie}.
\citep{kleinsurprise} learn predictive models of infant visual attention, aimed at designing robots that manipulate and encourage attention.

In this work, we address the problem of learning models of agents, a useful ability in multi-agent reinforcement learning contexts in which agents do not have access to other agents' reward functions or policies. Like other works, our goal is to build architectures and policies that enable the learning agent to model other agents it observes and interacts with, but we do not hard-code in either the learning objective (e.g. our work is self-supervised) or the behavioral outcomes (e.g. attention patterns \emph{emerge} as a solution to multi-agent prediction). 

\noindent{\textbf{Attention.}} A wide variety of problems have been shown to benefit from neural network architectures that employ what has come to be called ``attention'' in the AI literature, e.g. local multiplicative gating that dynamically learns to highlight portions of the network during inference, so as to focus processing on particularly relevant portions of either the input data or intermediate featural content~\cite{}CITE. This literature is related to our work in that it shows how selective highlighting of some form improves learning, but differs significantly in the meaning of the term ``attention'', the importance of the active learning setting, and the technical machinery needed to use attention in this setting.  What we call ``attention'' is the idea that a physically embodied agent allocates its observational time differently for different stimuli, rather than the abstract disembodied concept used in most literature. In contrast to attentional multiplication in supervised settings, our agents need attentional control to perform effective active learning, creating datapoints that without such control would occur rarely or not at all.  The causal world model architecture and learning progress policy we develop to generate such control are thus structurally distinct from the multiplicative gating operations used in typical attention work.

\subsection{Cognitive Science}
\label{subsec:related:cognitive}

\noindent\textbf{Object dynamics prediction, attention, and permanence.} 
Humans are extremely effective at understanding object dynamics, excelling at intuitively predicting both the physical interactions of external objects~\citep{battaglia2018relational, proffitt1989understanding} %JDF: Note: I think the literature is more mixed about this, in part because psychologists tried really hard to find cases in which this wasn't true. So more recently, Battaglia and colleagues would agree with this statement, whereas older work Proffitt and colleagues says we're accurate in some cases but not others.
and the physical consequences of their own actions~\citep{wolpert1995internal, wolpert2001motor, blakemore2003self}. 
However, both the visual system and the working memory system that support these abilities have substantial limitations~\citep{alvarez2007many, alvarez2004capacity, miller1956magical}. Humans thus selectively allocate attention in an object-centric fashion to enable effective prediction despite these limitations~\citep{de2014attentional, egly1994shifting, scholl2001objects}, and assign individuated tokens to keep track of objects over time~\citep{sears2000multiple}. To deal with momentary disappearances of objects as they become occluded or leave the visual frame, the brain maintains an internal representation of objects, a phenomenon known as \emph{object permanence}~\citep{piaget_originsintelligence}.  Infant studies show that many of these abilities --- including understanding the dynamical continuity of physical trajectories, object solidity, and their persistence even when out of sight --- appear to be present very early in development~\citep{spelke_objectpermanence, spelke2007core, baillargeon1985object}. 
In this work, we include object-based attention, object permanence, and working memory as architectural biases. We require the model to perform dynamics prediction on the center coordinates of objects, and we use a memory system to maintain an active representation of an object whenever it goes out of sight. 

\noindent\textbf{Curiosity and Active Learning.} Attentional control also appears to be of great importance for learning how the world works.  Infants appear to gather information from environments in a manner that is quite principled, selectively looking at objects in a highly non-random manner~\citep{smith}, and devoting increased attention to objects that violate their expectations \citep{stahl2015observing}.  Infants also appear to self-generate useful learning curricula, preferentially attending to stimuli that are complex enough to be interesting but not too complicated that they cannot be predicted, a phenomenon termed the \emph{goldilocks effect}~\citep{kidd2012goldilocks}.  In this work, we study active learning in the context of animate and inanimate stimuli. 

\noindent\textbf{Animate attention.}
From early infancy, humans are adept at distinguishing between inanimate and animate agents, preferentially paying attention to animate features like faces \citep{maurer2002many} and human body shapes~\citep{slaughter2002development}. Even in the absence of such surface features, infants will preferentially attend to spatiotemporal kinematics indicative of animacy, such as self-propelled motion~\citep{premack1990infant}, efficient movement towards targets~\citep{gergely1995taking}, contingent behavior between observed agents, as when one agent chases another~\citep{frankenhuis2013infants}, and contingent behavior between an observed agent and the infant herself, as when a robot beeps in response to the infant's babbling~\citep{johnson2003detecting, foster1973visual}.  
% The visual system is highly tuned to cues that reliably indicate the presence of agents with internal sources of energy that cause them to move without external forces. 
Such kinematic patterns give rise to an irresistable sense of animacy, even when the objects executing the kinematics are simple shapes~\citep{heider1944experimental}. 
In this work, our environment includes agents with kinematics inspired by the human experiments and deliberately devoid of surface features, so that our curious agent must discover which agents are worth paying attention to based solely on dynamics.
While we build in inductive biases concerning object-permanence, we do not build in a propensity to detect special classes of stimuli. Instead, we test whether animate attention of the form observed in humans emerges naturally, provided we endow the model with the right intrinsic motivation.

\noindent\textbf{Social prediction and theory of mind.}
Beyond animate attention, a more sophisticated ability that emerges later in development is the active interpretation of other agents in terms of their underlying mental states (beliefs, desires, and goals) that cause the agents' behavior, aka \emph{theory of mind} \citep{astington1990developing, premack1978does, wellman1992child}. It is hypothesized that theory of mind is needed in order to \textit{predict} what an agent will do next, since often it is only possible to do so accurately by generating expectations about an agent as a function of their underlying intentions. This ability is crucial to social functioning, and the failure to attribute mental states falls under the umbrella of symptoms that define the autism spectrum disorders~\citep{baron2000theory}.  
In this work, we task our model with learning to predict what the agents in the environment will do next.
% , and seek to determine which features of animate attention and theory of mind are required to achieve improved world-model predictions.










==> sections/scrap.tex <==
============intro.tex

Imagine yourself a parent at a playground. There is a plethora of stimuli, spanning wavering trees, leaves blowing in the wind, and children playing hide and seek. After briefly staring at the shaking trees and rustling leaves, you bore of watching their unpredictable motion and instead direct your attention to the game of hide and seek. Unlike with the random motion of trees and leaves, your understanding of the complex but predictable dynamics of hide-and-seek improves over time and you may eventually become capable of predicting a child's specific next move. This simple scenario suggests that humans continually engage in an intrinsically motivated process of furthering their understanding of the world and that directed attention may emerge naturally whilst seeking out maximally informative observations. In this work we aim to develop an intrinsically motivated active learning system that does the same: sample efficiently build models of the world by learning what to attend to.  

Concretely, world models are a family of predictive models that solve self-supervised prediction problems pertaining to the underlying the temporal structure of the world such as forward and inverse dynamics. Through learning world models, humans may acquire compact abstractions of high bandwidth sensory inputs, the ability to plan across long temporal horizons, and an understanding of the behavioral patterns of other agents. To deploy AI active learners in the real world, it is thus crucial that they can efficiently learn world models in complex environments. \kh{emphasize this process should happen without much external supervision}

To this end, there are mainly two algorithmic challenges: The first algorithmic challenge is that the active learner must arbitrate between the combinatorially large number of stimuli exhibiting inherently unlearnable or chaotic dynamics - e.g., falling leaves, wavering trees, and splashing water - and the few \ms{sparsity still hasn't been justified?} stimuli that have interesting and complex, yet learnable dynamics - e.g children playing hide-and-seek. We refer to the former class of stimuli as displaying \emph{noisy} behavior \ms{The thing about ``noisy'' is it has the connotation of ``having some noise'' which is true for stochastic animate agents.} and the latter as displaying \emph{animate} behavior. The term "animate" is drawn from the field of psychology \citep{premack1990infant, gergely1995taking, frankenhuis2013infants} in which "animate agents" denote a class of entities displaying behaviors with human-like kinematics such as self-propelled motion, goal-directed movements, and motion contigent on other agents. This challenge of identifying animate stimuli amid a sea of noisy ones has been acknowledged in many prior works as the "white noise" problem \citep{schmidhuber_formaltheoryoffun, pathak2017inverse, burda2018exploration, pathak2019disagreement}. The second algorithmic challenge is that the world model is susceptible to causal confusion - e.g the mistaking spurious correlations for true causality - which leads to poor generalization performance.

\kh{separate this challenge} Additionally, there is resource challenge that there is a shortage of simulated environments that faithfully preserve the core properties of real-world environments, while removing confounds that may artificially inflate modeling successes.

We address these three challenges with an intrinsically motivated "curious" active learning agent comprising two key components: (i) a \emph{Progress Curiosity-driven Controller} that learns to attend to stimuli with high expected learning progress thereby overcoming the white noise problem and (ii) a \emph{Causal World Model} that integrates a causal prior into its network architecture to preempt causal confusion. (see Fig. \ref{fig:model}) Our experiments are conducted in a custom-built 3D virtual world environment, rich with external agents displaying a wide spectrum of realistic animate behaviors such as peekaboo, chasing, and mimicry. \kh{should summarize key contributions into a couple sentences here}

In what follows, we begin by drawing connections between our work and related works in psychology and artificial intelligence (Section~\ref{sec:relatedworks}). In Section~\ref{sec:environment}, we describe our virtual environment in detail. Section~\ref{sec:theory} formalizes the active learning problem our curious agent is tasked with, motivates progress curiosity in the context of previously proposed curiosity signals, and characterizes the causal confusion problem. \kh{be a bit more detailed here} Section~\ref{sec:methods} details the implementations for all components of our curious active learning agent. Finally, Section~\ref{sec:experiments} presents experimental evaluations of our curious active learning system on two quantitative metrics: We show that (1) injecting causal prior is essential to attaining high offline asymptotic model performance, and (2) our progress-driven controller achieves significantly lower online sample complexity than baseline controllers equipped with state-of-the-art exploration strategies — including Random Network Distillation (RND) (Burda et al., 2018b) and Model Disagreement (Pathak et al., 2019) — which (perhaps surprisingly) fall prey to the white noise problem. \kh{this last sentence still needs to be rephrased} Furthermore, when varying both the intrinsic motivation signal (considering several baselines) and world model architecture (with causal structure prior, and without), we find that the intrinsic motivation signal drives behavior, whereas the difference in world model architecture modulates behavior to a lesser degree.


%In what follows, we begin by drawing connections between our work and related works in psychology and reinforcement learning (Section 1). In Section 2 \jdf{incomplete}. In Section 3, we describe our virtual environment in detail. Section 4 formalizes the core problems that motivate this project, including causal confusion and the shortcomings of curiosity signals that have been previously proposed to solve the white noise problem, while Section 5 presents the components of our active learning system. Finally, Section 6 presents experimental evaluations of our curious active learning system along three metrics: We show that (1) our causal prior is essential to attaining high offline asymptotic model performance, (2) our choice of a progress-driven controller is crucial to obtaining low online sampling complexity, while state-of-the art exploration methods — including Random Network Distillation (RND) (Burda et al., 2018b) and model disagreement (Pathak et al., 2019) — fall prey to the white noise problem, and (3) independent of world model choice, preferential attention towards animate agents emerges only with progress curiosity (but not other kinds of curiosity), suggesting that our model architecture may approximate the neural learning systems employed by humans. \jdf {I’ll circle back around to this to think about the specific human impliciations of ‘independent of a world model choice}.













% X_{ext, t:t+T_{out}}, \hat X_{ext, t:t+T_{out}}) = \sum_{s = t}^{T + T_{out}}\sum_{i = 1}^{N_ext} \alpha \rvx_{i, s} \|c_{i, s} - \hat c_{i, s} \|_2^2 + \beta \mathcal{L}_{ce}(\rvx_{i, s}, \hat \rvx_{i, s})

% As described in Section~\ref{sec:theory}, the world model seeks to solve the forward dynamics prediction problem of external agent behaviors in this encoding space. Specifically, given an encoded observation sequence $\rvx_{t - T_{in} : t}$ and curious agent actions $a_{t - T_{in} : t + T_{out} - 1}$, the world model predicts  $\rvx_{ext, t : t + T_{out}}$. % \ms{Loss function} 


% \ms{Causal prior} 
% In this work, we propose the \textit{Causal World Model}, a world model architecture that injects a causal graph of external agents (see Section~\ref{sec:theory}) as an architectural prior. Specifically, we impose this prior by instantiating, for each behavior $i$, a separate \textit{behavior network} $\mathcal{B}_i$ with independent weights $\theta_i$, such that one causal world model consists of $\{\mathcal{B}_i\}_{i \in \{1, ..., N_{behavior}\}}$

% Given behavior $i$, let $S_i$ be the set of all agents that belong to the behavior. 
% Given an encoded observation sequence $\rvx_{t - T_{in} : t}$, $\mathcal{B}_i$ takes as input only the part of $\rvx_{ext, t - T_{in} : t}$ corresponding to the agents that belong to the behavior, i.e., $(\rvx_{j, t - T_{in} : t} \cdot c_{j, t - T_{in} : t}, \rvx_{j, t - T_{in} : t})$ for all $j \in S_i$, along with $\rvx_{aux, t - T_in: t}$,  $\phi_{t - T_{in} : t }$, and $a_{t - T_{in} : t}$, and outputs predictions of only the part of $\rvx_{ext, t:t+T_{out}}$ that corresponds to the agents that belong to its behavior, i.e., $(\rvx_{j, t:t+T_{out}} \cdot c_{j, t:t+T_{out}}, \rvx_{j, t:t+T_{out}})$ for all $j \in S_i$. The outputs of all behavior networks  are concatenated to construct the overall prediction of $\rvx_{t:t+T_{out}}$, which is then the output of the causal world model.

% \ms{specific architecture 
% (LSTM, layers, units, optimizer, learning rate), excluding indicator coordinate split }

% To measure the gains of our causal world model, we introduce a \textit{non-causal ablation} that does not have this architectural prior. Concretely, the non-causal world model uses an architecture similar to that of a single behavior network in the causal world model, but with larger layers to have a similarly-sized parameter space. It takes as input $\rvx_{t-T_{in};t}$ and predicts $\rvx_{t:t+T_{out}}$ directly, modeling the dynamics of all external agent behaviors simultaneously. 






%\ms{Our self-supervision problem: forward dynamics prediction}
% First, we assume access to an oracle that maps observations $(O_t)$ to  an intermediate representation $(X_t)$ which contains information about the coordinates of each external agent in the room and indicators of whether an agent is in the curious agent's view.
%\ms{What are the inputs and outputs of the world model?}
%Specifically, given a sequence of past observations and past and present actions $(X_{t-n:t}, a_{t+k-1})$, the world model seeks to predict the next sequence of observations $(X_{t+1:t+k})$.


%\subsubsection{Split architecture}
%\ms{What are the solutions?}
%While in environments with only inanimate objects, the physical dynamics is shared between objects, a key property of our multi-agent environment is that different agents behave under widely varied dynamics. 
%In this work, we propose a split world model architecture, which consists of separate networks that each solve forward dynamics prediction of one external agent behavior, where a behavior may consist of one (e.g. peekaboo) or two interacting external agents (e.g. chasing). We argue that this behavior-wise splitting is equivalent to injecting the agent contingency graph as an architectural prior into the world model... 
%We perform ablations where a single neural network is used to model all external agents in the environment.

% Note that the particular dynamics prediction problem posed for a given external agent behavior does not always need to involve the prediction of all external agents involved in the behavior. In the case of mimicry, the input to the corresponding module contains information about both actor and imitator agents, but the prediction only needs to be done on the imitator. 



In this section we evaluate the active learning performance of our progress-driven curious agent. There are two differences from the supervised learning experiments in Section \ref{sec:offline}. First, instead of collecting data under random policy, the curious agent \emph{learns} to attend by optimizing a surrogate curiosity reward in order to minimize the number of environment interactions. Second, the virtual environment is set up with three noise behaviors and one animate behavior, varied amongst the seven animate behaviors listed in Section \ref{sec:environment}. This configuration directly challenges the curious agent to overcome the white-noise problem. We measure the sample complexity of the curious agent optimizing different curiosity signals while changing the animate behaviors and world model types. Specifically, we compare the five curiosity signals and a random policy baseline

\textbf{$\gamma$-Progress (Ours)} is our proposed variant of progress curiosity which chooses $\theta_{old}$ to be a geometric mixture of all past models as in Eq. \ref{eq:mix_progress}. 

\textbf{$\delta$-Progress \citep{achiam2017surprise, graves2017automated}} is the $\delta$-step learning progress reward from Eq. \ref{eq:kstep_progress} with $\delta = 1$. We found that any $\delta > 3$ is impractical due to memory limitations even with 12GB Titan X GPUs. 

\textbf{RND \citep{burda2018exploration}} is a state-of-the-art novelty-based exploration method shown to be effective in video game domains. In this approach, a predictor neural net is trained to match the outputs of a random state encoder. States for which the predictor networks fails to match the random encoder are deemed "novel", and thus receive high reward. 

\textbf{Disagreement \citep{pathak2019disagreement}} is the disagreement reward from Eq. \ref{eq:disagreement} with $N = 3$ ensemble models. We found that $N > 3$ is impractical due to memory constraints.  

\textbf{Adversarial \citep{stadie2015predictive, pathak2017inverse}} is the prediction error from Eq. \ref{eq:adversarial}. 

\textbf{Random} chooses actions uniformly at random among the 9 possible rotations. 


% Fig.~\ref{fig:attention} shows that, for both the causal and non-causal world models, strong animate attention emerges for $7/7$ behaviors $\gamma$-Progress and weak animate attention arises on $1/7$ behaviors for $\delta$-Progress. For RND, Disagreement, and Adversarial we observe the inverse: strong attention to the random agent emerges, i.e the white noise problem is apparent. \kh{We find that animate attention is strongly correlated with the AUC metric of sample complexity (provide number or figure reference), which supports our hypothesis that animate attention naturally emerges from an underlying process of optimizing for efficient world model learning}. 

% We also evaluate active learning performance using the acausal world model which has lower asymptotic model performance. Regardless we see that $\gamma$-Progress outperforms RND, Disagreement, and Adversarial baselines on all $7/7$ behaviors and outperforms $\delta$-Progress on $5/7$ behaviors while tying on the two peekaboo behaviors. While the world model's asymptotic performance is severely affected by architecture choice (causal v.s. acausal), the relative ranking in performance across intrinsic motivation signals is maintained across world model types. 


%%%%%%%%%%%%%%%%%%%%%% Attention Metric %%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
\subsection{Emergence of Animate Attention}

In this section, we analyze the interplay between choice of intrinsic motivation, world model architecture, validation performance, and the attention patterns that emerge within our environment. Fig.~\ref{fig:attention} shows that, for both the causal and acausal world models, strong animate attention emerges for $7/7$ behaviors $\gamma$-Progress and weak animate attention arises on $1/7$ behaviors for $\delta$-Progress. For RND, Disagreement, and Adversarial we observe the inverse: strong attention to the random agent emerges, i.e the white noise problem is apparent. In what follows, we analyze the factors varied in these models in order to quantify more precisely what drives the emergence of animate attention. We then characterize the extent to which the emergent attentional pattern predicts validation performance. This serves as a toy "developmental model" of how  {\em early attention} better predicts later performance than does {\em early performance}.
\end{comment}

%In this section, we evaluate the attention patterns that emerge from our intrinsically motivated active learning system. Fig.~\ref{fig:attention} shows that, for both the causal and non-causal world models, strong animate attention emerges for $7/7$ behaviors $\gamma$-Progress and weak animate attention arises on $1/7$ behaviors for $\delta$-Progress. For RND, Disagreement, and Adversarial we observe the inverse: strong attention to the random agent emerges, i.e the white noise problem is apparent. \kh{We find that animate attention is strongly correlated with the AUC metric of sample complexity (provide number or figure reference), which supports our hypothesis that animate attention naturally emerges from an underlying process of optimizing for efficient world model learning}. 




% For example, one may choose $c(\bar{\rvs} = (\rvs, H, \theta)) := \LL_{\mu}(\theta) = \E_{\mu}[\LL(\theta, \rvx, \rvy)]$, where $\LL_{\mu}: \Theta \rightarrow \RR$ is the expected loss on data $(\rvx, \rvy) \sim \mu$ where $\mu$ is a distribution. This choice of $c$ with a encodes a learning objective which seeks to minimize validation loss while training on a minimal number of data samples. 


%  Overall, the MDP $\mc{M}$ is constructed from an environment $\mc{E} = (\S, \A, P, P_{0})$, a target function $\omega$, a learning algorithm $P_{\ell}$, and a prior parameter distribution $q(\theta)$. Several variants of conventional active learning can be recovered by appropriately defining the MDP $\mc{M}$ in relation to $\omega, \X, \Y$.

\begin{comment}
\textbf{Query Synthesis Active Learning} is obtained by taking $\S = \Y, \A = \X, P(\cdot |  \cdot, \rva=\rvx) = \omega(\rvx)$ and $r(\bar{\rvs} = (\rvs, H, \theta), \rva, \bar{\rvs}' = (\rvs', H', \theta')) = \LL_{\mu}(\theta') = \E_{\mu}[\LL(\theta', \rvx, \rvy)]$ where $\LL: \Theta \times \X \times \Y \rightarrow \RR$ is a loss function and $\mu: \rvx \times \rvy \rightarrow \RR$ is a validation distribution. In words, the agent proposes a synthetic data query $\rva$ and the oracle $P$ provides a label $\rvs'$. The agent's objective is to reduce model loss on a known validation set sampled from $\mu$ while minimizing the number of data queries. Appendix \ref{sec:app:gal_cal_connection} further shows how to recover Pool-based and Stream Active Learning using our RL framework.

% Most active learning methods take a greedy approach to maximize the model loss reduction after a single data query, which corresponds to setting the discount factor $\beta = 0$

\textbf{Forward AWML} Consider a simple AWML problem of learning the forward dynamics, i.e $\X = \S \times \A, \Y = \S, P = \omega$, and 
\begin{align}
r(\bar{\rvs}, \rva, \bar{\rvs}') = \LL_{\mu}(\theta) - \LL_{\mu}(\theta')
\label{eq:cost}
\end{align}
where $\bar{\rvs} = (\rvs, H, \theta), \bar{\rvs}' = (\rvs', H', \theta')$, with a discount factor $\beta < 1$ to encourage minimal interactions with the environment. Recall that $\theta' = P_{\ell}(H \cup \{\rva, \rvs'\}, \theta)$ is the updated model parameters after collecting new data $\{\rva, \rvs'\}$. Thus $r(\bar{\rvs}, \rva, \bar{\rvs}')$ measures the reduction in world model loss as a result of obtaining new data $\{\rva, \rvs'\}$, i.e the \emph{prediction gain}. The validation distribution $\mu(\rvx, \rvy)$ specifies prior knowledge on which data the world model should \emph{learn} in order for it to be useful for downstream tasks, e.g Imagenet classification or household robotic tasks. In this work, we consider a more general AWML setting where $\mu(\rvx, \rvy)$ is proportional to the \emph{learnability} of $\rvx, \rvy$ with respect to a model class $\Theta$, e.g $\mu(\rvx, \rvy) \propto 1 / \min_{\theta \in \Theta} \LL(\theta, \rvx, \rvy)$. This objective encourages the agent to be maximally exploratory while seeking out learnable data, much like how humans explore the world.

% \nh{could "most general" be too aggressive a claim, given that we've not delineated some version of things for which this is most general? maybe one's stubborn priors could involve totally unlearnable things? And, saying that we consider it in this work seems like a stretch --- some notion like this informs validation choices, but afaik this particular choice isn't mentioned again. Also what happens when the loss is zero? Why is this the right thing to be proportional to? I'm sure we could have good answers to all of this, but one option would be to be a bit more explicit in our inexactness, here.}

Unfortunately, $\mu$ is not known prior to interacting with the environment in AWML (or else one could instead perform supervised learning!). Even with an online estimate of it, $\mu$ is a rather diffuse distribution (assuming a sufficiently expressive model class and a rich environment) which makes it intractable to compute Eq. \ref{eq:cost} at every environment step. These bottlenecks necessitate an efficiently computable proxy reward. Thus, solving the AWML problem can be recast as a proxy reward design problem. Specifically, in AWML one seeks a proxy reward, or ``curiosity'' signal, that is \emph{consistent} with Eq. \ref{eq:cost}, i.e the optimal policy with respect to both rewards are equivalent, and \emph{computationally efficient}. 
\end{comment}

==> sections/theory_dump.tex <==
Causal confusion is likely to occur when the training data distribution $p(\rvx)$ only covers a subset of the entire space $\X$, i.e $supp(p(\rvx))$ is small. The smaller the data coverage, the larger the space of degenerate solutions which do not respect the true causal structure of $P$.Causal confusion is likely to occur when the training data distribution $p_{train}(\rvx) \subset \X$ admits a different causal graph. 

Now consider a learned world model $P_{\theta}: \X \rightarrow \Y$.
\kh{formalize the disentanglement condition}
Any optimal world model should satisfy the following disentanglement condition for any causal graph $G_{P}$:
\begin{equation}
(P(\rvx))_{I_{\Y}} = (P_{\theta}(\rvx_{I_{\Y}^{-1}} \oplus \rvepsilon_{\setminus I_{\Y}^{-1}}))_{I_{\Y}} \quad \forall \rvepsilon \in \X, ~~\forall I_{y} \in A_{y}
\label{eq:causal_confusion}
\end{equation}

where $\rvx_{I_{\Y}^{-1}} \oplus \rvepsilon_{\setminus I_{\Y}^{-1}}$ denotes a concatenation of two vectors according to the indices $I_{\Y}^{-1}, \setminus I_{\Y}^{-1}$. In words, the subslices of model outputs $(P(\rvx))_{I_{\Y}}$ should only depend on the factors of variation that cause it, i.e $\rvx_{I_{\Y}^{-1}}$, and be unaffected by changes to nuisance factors of variation, i.e $\rvepsilon_{\setminus I_{\Y}^{-1}}$.

\begin{wrapfigure}{R}{0.45\textwidth}
\vspace{-10pt}
\begin{center}
    \includegraphics[width=.43\textwidth]{figures/causal_graph.pdf}
\end{center}
\vspace{-15pt}
\caption{\textbf{A causal graph.} Vertices represent external agents at times $t$ and $t+1$, edges represent causal relationships. Dashed boxes denote the connected component {\em external agent behaviors}.}
\label{fig:causal_graph}
\vspace{-10pt}
\end{wrapfigure}

%%%%%% What is causal confusion %%%%%%%
A learned model $P_{\theta}$ suffers from \emph{causal confusion} when it violates the disentanglement condition in Eq. \ref{eq:causal_confusion}, i.e changes in nuisance factors of variation $\rvepsilon_{\setminus I_{\Y^{-1}}}$ lead to changes in $P_{\theta}(\rvx)_{I_{\Y}}$. A causally confused model exhibits poor generalization performance when $p(\rvx) = p(\rvx_{I_{\Y}} | \rvx_{\setminus I_{\Y^{-1}}})p(\rvx_{\setminus I_{\Y^{-1}}})$ are distributed differently during training and validation time since off-distribution inputs can affect model outputs in unpredictable ways \citep{de2019causal}. 

As an intuitive example, consider an environment with two independent agents $A, B$ oscillating in sync with the same period. Let $\X = \Y$ comprise the joint position of the two agents and $I_{A}, I_{B}$ denote indices for each agent so that e.g $\rvx_{I_{A}}$ is the position coordinate of agent $A$. According to Def. \ref{def:causal_disentanglement}, the true world model $P: \X \rightarrow \X$ is causally disentangled since there exist partitions $\I_{\X} = \I_{\Y} = \{I_{A}, I_{B}\}$ and the identity bijective pairing $c(I) = I$ for which Eq. \ref{eq:causal_disentanglement} holds. The left graph in Fig. \ref{fig:causal_graph} shows the causal graph $G_{P}$ with two connected components, one for each periodic agent. \Inlike the true world model $P$, a causally confused learned model $P_{\theta}$ may predict the next position of agent $A$ from the current position of agent $B$ as shown in the right graph of Fig. \ref{fig:causal_graph}. $P_{\theta}$ may perform well on the training data so long the nuisance variables follow a fixed distribution




%%%%%% Why is causal confusion likely to occur? %%%%%%%
Now let us reason about why causal confusion is likely to occur when learning world models in real environments. 

% There's a distinction between an example of causal confusions and an example that illustrates why causal confusion is likely in real environments. The above example only shows the former. Is it indeed true that causal confusion is likely to occur? If so, why? 

% However, a causally confused model may have a causal graph with the dotted edge where the $\rvo_{I_{p1}}^{t+1}$ depends on the nuisance variable $\rvo_{I_{p2}}^{t}$. Since the periodic agents are in lockstep

Due to the partial observability of real-world environments (described in Section \ref{sec:environment}), our curious agent must have object permanence in order to make accurate predictions of when and where stimuli that disappear from view will reappear. This requires allocating dimensions of the world model input space $\X$ to tracking states of stimuli that are not in view. For example, $\rvx \in \X$ could include an object-centric representation with dimensions explicitly allocated for each object state or the hidden states of a recurrent neural network.


Object permanence can be encoded as an architectural prior by structuring the world model input space to be object-centric


There exists subdimensions of your input space that corresponds to "permanence" related representations. This could be explicit with an object-centric representation, or implicitly encoded in the hidden state representations learned by an LSTM.



There are several reasons for why we observe a distributional difference in the nuisance variables. First, due to model bootstrapping, the distribution of $\rvepsilon_{\setminus I_{\Y^{-1}}}$ changes with the number of timesteps having not seen the stimuli corresponding to $I_{\Y}$ which is affected by the curious agent's policy. Thus, policy changes during training and validation, i.e $D_{\text{KL}}(\rho_{\pi} || \mu)$, can lead to distributional mismatch of nuisance variables. Second, the nuisance variable distribution changes as a function of the world model. When interlacing validation and world model updates, it's most likely the training data doesn't contain many samples from the most recent version of the world model.
\kh{equipartition theorem. Put in footnote why bijective and not surjective}
\kh{Emphasize this problems arise especially in the interactive learning setting}
\kh{intuition for bipartite graph}

\kh{present simple example with two periodic agents}

\kh{Now explain our solution}











%%%%%%%%%%%%% New theory dump %%%%%%%%%%%%%%
\begin{definition}
\label{def:causal_disentanglement}
Let $\I_{\X} \in \emph{Part}(\{1, ..., \emph{dim}(\X)\}), \I_{\Y} \in \emph{Part}(\{1, ..., \emph{dim}(\Y)\})$ be maximally large partitions for which there exists a surjective map $c: \I_{\X} \rightarrow \I_{\Y}$ and sub-models $\{P^{I_{\X}}: \X_{I_{\X}} \rightarrow \Y_{c(I_{\X})} | I_{\X} \in \I_{\X}\}$ such that
\begin{equation}
P(\rvx)_{c(I_{\X})} = P^{I_{\X}}(\rvx_{I_{\X}}) \quad \forall I_{\X} \in \I_{\X},~~\forall \rvx \in \X
\label{eq:causal_disentanglement}
\end{equation}
where $\emph{Part}(S)$ is the universe of partitions a set $S$, $\rvx_{I_{\X}} := [x_{i}]_{i \in I_{\X}}$, and $\X_{I_{\X}} := \{\rvx_{I_{\X}} | \rvx \in \X\}$. Then, $G_{P} = (V, E)$ is a \textbf{causal graph} of $P$ where $V = \I_{\X} \cup \I_{\Y}, E = \{(I_{\X}, I_{\Y}) | I_{\X} \in \I_{\X}, I_{\Y} \in \I_{\Y}, I_{\Y} = c(I_{\X})\}$. 
\end{definition}

Let $P: \X \rightarrow \Y$ be a function and $\rvx \in \X, \rvy = P(\rvx)$ be random variables. $G_{P} = (V, E)$ of $P$ if 
\begin{enumerate}
\item $V = \{\rvx_{1}, ..., \rvx_{\emph{dim}(\X)}, \rvy_{1}, ..., \rvy_{\emph{dim}(\Y)}\}$
\item $(v_{\X}, v_{\Y}) \in E$ iff $\exists $
\end{enumerate}



and its occupancy measure is defined as $\rho_{\pi}(\rvx, \rvy) = \sum_{t = 0}^{\infty} \beta^{t} \Pr( | \pi)$ where $\beta$ is a discount factor $0 \leq \beta \leq 1$. A world model $\omega_{\theta}: \X \rightarrow \Omega(\Y)$ is stochastic function that encapsulates a property of the world. For example, $P$ is the forward dynamics kernel when $\X = \S \times \A$ and $\Y = \S$. In general, $\X, \Y \subseteq \S^{*} \times \A^{*}$ where $\S^{*}, \A^{*}$ are sets of all arbitrary length state, action sequences, i.e the Kleene closure of $\S, \A$. Further let $f: (\X \times \Y)^{*} \rightarrow \Theta$ be a learning algorithm for $\omega_{\theta}$. GAL aims to learn a policy $\pi$ to collect samples $(\rvx, \rvy)$ from the world which maximally reduce world model loss $\LL(\theta)$. 
\begin{equation}
\min_{\pi_{k+1}}{\mathop{\E}_{\substack{\rvx, \rvy \sim \\ \rho_{\pi_{k+1}}, P(\cdot | \rvx)}}[\LL(f(\cup_{i = 0}^{k} \mc{D}^{i} \cup \{(\rvx, \rvy)\})) - \LL(f(\cup_{i = 0}^{k} \mc{D}^{i}))] }
\label{eq:active_obj}
\end{equation}


\X \rightarrow \Omega(\Y)$, where $\Omega(\Y)$ is the set of probability measures on $\Y$, is a stochastic function that encapsulates a property of the world. For example, $P$ is the forward dynamics kernel when $\X = \S \times \A$ and $\Y = \S$. In general, $\X, \Y \subseteq \S^{*} \times \A^{*}$ where $\S^{*}, \A^{*}$ are sets of all arbitrary length state, action sequences, i.e the Kleene closure of $\S, \A$. The embodied agent agent interacts with the world according to a policy $\pi: \S \rightarrow \Omega(\A)$, in the process collecting samples $(\rvx, \rvy) \in \X \times \Y$ which are used to update its world model $P_{\theta}: \X \rightarrow \Omega(\Y)$ by minimizing a loss $\LL(\theta)$. Intuitively, $\pi$ distills the agent's strategy for querying useful data from the world, e.g directed attention towards animate external agents. For a policy $\pi$, we also define its occupancy measure $\rho_{\pi}: \S \times \A \rightarrow \RR$ as $\rho_{\pi}(s, a) = \sum_{t = 0}^{\infty} \beta^{t} \Pr(s_{t} = s, a_{t} = a | \pi)$ where $\beta$ is a discount factor $0 \leq \beta \leq 1$. Let $f: (\X \times \Y)^{*} \rightarrow \Theta$ be a learning algorithm. \kh{define input/output space explicitly} In traditional active learning, a single round of optimization comprises a data collection strategy update step (choosing which $\rvx$ to query a label for) and model update step. By analogy we can similarly formalize Learning with Intrinsic Motivation. In round $k + 1$, the data collection strategy update step solve the following policy optimization problem: \kh{end state distribution is the initial state distribution}:


\subsection{Active World Model Learning}
\label{sec:active_learning}
\kh{Add general definition with $z$ instead of specifying the forward problem. No access to querying prior distribution}


\kh{Define the generalization of active learning first.}



Informally, Active World Model Learning (AWML) is the process of learning how to efficiently collect information from the world to minimize world model loss. Concretely, we represent an embodied agent in a generic world (or "environment") as a tuple $(\S, \A, P)$ where $\S, \A$ are state, action spaces of the agent and $P: \X \rightarrow \Omega(\Y)$, where $\Omega(\Y)$ is the set of probability measures on $\Y$, is a stochastic function that encapsulates a property of the world. For example, $P$ is the forward dynamics kernel when $\X = \S \times \A$ and $\Y = \S$. In general, $\X, \Y \subseteq \S^{*} \times \A^{*}$ where $\S^{*}, \A^{*}$ are sets of all arbitrary length state, action sequences, i.e the Kleene closure of $\S, \A$. The embodied agent agent interacts with the world according to a policy $\pi: \S \rightarrow \Omega(\A)$, in the process collecting samples $(\rvx, \rvy) \in \X \times \Y$ which are used to update its world model $P_{\theta}: \X \rightarrow \Omega(\Y)$ by minimizing a loss $\LL(\theta)$. Intuitively, $\pi$ distills the agent's strategy for querying useful data from the world, e.g directed attention towards animate external agents. For a policy $\pi$, we also define its occupancy measure $\rho_{\pi}: \S \times \A \rightarrow \RR$ as $\rho_{\pi}(s, a) = \sum_{t = 0}^{\infty} \beta^{t} \Pr(s_{t} = s, a_{t} = a | \pi)$ where $\beta$ is a discount factor $0 \leq \beta \leq 1$. Let $f: (\X \times \Y)^{*} \rightarrow \Theta$ be a learning algorithm. \kh{define input/output space explicitly} In traditional active learning, a single round of optimization comprises a data collection strategy update step (choosing which $\rvx$ to query a label for) and model update step. By analogy we can similarly formalize Learning with Intrinsic Motivation. In round $k + 1$, the data collection strategy update step solve the following policy optimization problem: \kh{end state distribution is the initial state distribution}:


In this work we choose the forward dynamics problem as the world model problem. Specifically, we aim to learn a forward model $P_{\theta}: \X \rightarrow \Omega(\Y)$ over an input space $\X = \S \times \A$ of state-action pairs and a label space $\Y = \S$ of next states. Collectively, $(\rvx, \rvy)$ forms a transition. 


where $\mu(\rvx)$ is a prior distribution over the importance of correctly predicting the transition for $\rvx$. $\mu$ may also be interpreted as the validation data distribution. \kh{Is there something we can say about how active learning will bring $\rho_{\pi}$ closer to $\mu$?} For instance, if $\mu$ is the uniform distribution then an optimal world model must perfectly match the true environment dynamics for all $|\S|^{2}|A|$ possible transitions. Let $f: (\X \times \Y)^{*} \rightarrow \Theta$ be a learning algorithm. \kh{define input/output space explicitly} In traditional active learning, a single round of optimization comprises a data collection strategy update step (choosing which $\rvx$ to query a label for) and model update step. By analogy we can similarly formalize Learning with Intrinsic Motivation. In round $k + 1$, the data collection strategy update step solve the following policy optimization problem: \kh{end state distribution is the initial state distribution}:
\begin{equation}
\min_{\pi_{k+1}}{\mathop{\E}_{\substack{\rvx, \rvy \sim \\ \rho_{\pi_{k+1}}, P(\cdot | \rvx)}}[\LL(f(\cup_{i = 0}^{k} \mc{D}^{i} \cup \{(\rvx, \rvy)\})) - \LL(f(\cup_{i = 0}^{k} \mc{D}^{i}))] }
\label{eq:active_obj}
\end{equation}
where $\mc{D}_{i} = \{(\rvx, \rvy)_{j}\} \sim \pi_{i}$. In words, we seek a policy $\pi_{k + 1}$ which samples transitions that maximally reduce world model loss in expectation. At each iteration of the active learning loop, we perform two steps. First, optimize $\pi_{k}$ by solving Eq. \ref{eq:active_obj}. Second, update the world model parameters on the aggregate dataset $\cup_{i = 0}^{k} \mc{D}_{i}$. \Inlike the classic active learning with a pool setting, in which the data collection policy chooses $\rvx$ from a given pool of unlabeled data, we don't have access to a pool of unlabeled state-action pairs and label queries for $\rvx$ can only be made by learning a policy that can reach $\rvx$ in the environment. \kh{why can't you use a rollout of all possible trajectories as the unlabeled dataset }




\subsection{Connections between Curiosity Signals}
\label{sec:curiosity_signal}



\begin{comment}
We now formalize our the learning problem of our intrinsically motivated active learner as a batch active learning problem. At a high level, the curious agent seeks to minimize world model loss with as few interactions with the world as possible by adaptively collecting  batches of training samples. Concretely, our aim is to solve the forward dynamics world model problem defined over an input space $\X = \S \times \A$ and a label space $\Y = \S$, where $\S, \A$ are (countable) state, action spaces. Let

% While in the context of RL, world models have been leveraged to derive exploration bonuses that aid learning of a different task, our primary objective is to learn world models themselves.
Our intrinsically motivated agent engages in an active learning loop of collecting maximally informative data for the current world model, performing a world model update, and repeating the cycle. This problem corresponds to interlacing reinforcement learning over $\mc{M}(\theta_{i})$ and world model updates via supervised learning. Each MDP $\mc{M}_{i}$ seeks to learn an optimal data collection policy to maximize learning progress of the current world model. Let $\mc{M}(\theta) = (\S, \A, P, R_{\theta}, T)$ be a finite horizon MDP where $\S, \A$ are (countable) state, action spaces, $P: \S \times \A \rightarrow \mc{P}(\S)$ is the dynamics where $\mc{P}(\S)$ is the set of probability measures on $\S$, $R$ is the reward function, and $T$ is the episode length. A (stationary) policy $\pi: \S \rightarrow \mc{P}(\A)$ maps states to distributions over actions. Our objective is to learn a world model $P_{\theta}$ that matches $P$ with more emphasis on state, action pairs specified by a prior distribution $q(s, a)$.
\begin{equation}
J(\theta) = -\E_{(s, a) \sim q}[D_{KL}(P(\cdot | s, a) || P_{\theta}(\cdot | s, a))] \leq 0
\label{eq:model_performance}
\end{equation}
Intuitively, $q$ has concentrated probability mass on state-action pairs for which predicting the next state distribution correctly is more important. For example, the prior $q$ may capture the inherent inclination of humans to attend more to animate agent like features.
% where $u_{\S \times \A}$ is a uniform distribution over $\S \times \A$. A uniform distribution was chosen for simplicity, but it may be replaced with any distribution fully supported on $\S \times \A$.
Let $f: \Theta \times \mc{D} \rightarrow \Theta$ be the optimizer which updates our world model parameters $\theta$ given data $\mc{D} = \{(s, a, s')_{i}\}$ in the form of transition triplets.


\begin{equation}
\pi^*(\theta) = \argmax_{\pi} \E_{\mc{D} \sim \pi} [J(f(\theta, \mc{D})) - J(\theta)] \quad \text{where} \quad |\mc{D}| \leq K
\label{eq:pi_objective}
\end{equation}
In words, a policy behaves optimally with respect to the current world model $\theta$ and an optimizer $f$ if it samples a trajectories that maximally improve the performance of the model. $K$ captures the memory constraint of an active learning agent. We see that Eq. \ref{eq:pi_objective} cannot be directly optimzied since we cannot predict the value of $J(P_{\theta'})$ before performing an optimization step. Let us assume that the optimizer $f$ satisfies the following additive property:
\begin{align*}
J(f(\theta, \{(s, a, s')_{i}\})) - J(\theta) \approx \sum_{i} J(f(\theta, (s, a, s')_{i}) - J(\theta)
\end{align*}
Then, the policy performance objective can be written as:
\begin{align*}
    \argmax_{\pi} \E_{\mc{D} \sim \pi} [\sum_{(s, a) \in \mc{D}} J(f(\theta, (s, a, s'))) - J(\theta)] \quad \text{where} \quad |\mc{D}| \leq K
\end{align*}
Taking the policy gradient we obtain:
\begin{align*}
    \E_{\pi} [\nabla\log{\pi} \sum_{t} J(f(\theta, (s_{t}, a_{t}, s_{t+1}))) - J(\theta)] \quad \text{where} \quad |\mc{D}| \leq K
\end{align*}

The reward quantity of interest is the future progress on the objective that can be made by having the sample $(s_{t}, a_{t}, s_{t+1})$. However this quantity cannot be calculated without evaluating the our objective $J$ and taking an optimization step $f$. The former is intractable and the later is expensive. Instead we seek to make an approximation to $J(P_{\theta'}) - J(P_{\theta})$ based on information we have obtained about $f$ and $J$ in the past.

\subsubsection{adversarial}
uncertainty sampling
For example, we might assume that future progress is proportional to the current world model loss:
\begin{align*}
    J(\theta') - J(\theta) \approx -\beta J(\theta)
\end{align*}

\subsubsection{Progress}
Active learning sampling technique: estimated error reduction \\
We may instead make the assumption that future progress is proportional to our previous experience updating on the data:
\begin{align*}
    J(\theta'') - J(\theta') \approx -\beta (J(\theta') - J(\theta))
\end{align*}

\subsubsection{disagreement}
Active learning sampling technique: query by committee.
In practice we need a prior over the

Notice that we cannot directly perform RL with the objective in Eq. (2) since we do not have access to the ground truth world model $P$. Hence, we formulate a surrogate objective to (2) based on learning progress:

Note that this is equivalent to optimizing over an MDP with a non-stationary reward function. Your behavior not only changes the distribution of states you encounter, but also the reward function.
\end{comment}

